Connecting the X-ray/UV variability of Fairall 9 with NICER: A Possible Warm Corona

The Seyfert 1 AGN Fairall 9 was targeted by NICER, Swift, and ground-based observatories for a $\sim$1000-day long reverberation mapping campaign. The following analysis of NICER spectra taken at a two-day cadence provides new insights into the structure and heating mechanisms of the central black hole environment. Observations of Fairall 9 with NICER and Swift revealed a strong relationship between the flux of the UV continuum and the X-ray soft excess, indicating the presence of a "warm" Comptonized corona which likely lies in the upper layers of the innermost accretion flow, serving as a second reprocessor between the "hot" X-ray corona and the accretion disk. The X-ray emission from the hot corona lacks sufficient energy and variability to power slow changes in the UV light curve on timescales of 30 days or longer, suggesting an intrinsic disk-driven variability process in the UV and soft X-rays. Fast variability in the UV on timescales shorter than 30 days can be explained through X-ray reprocessing, and the observed weak X-ray/UV correlation suggests that the corona changes dynamically throughout the campaign.

==> Table2.tex <==
58256.95 & $31.91\pm0.17$ & $-0.650\pm0.006$ & $-10.242\substack{+0.005\\ -0.005}$ & $-10.250\substack{+0.003\\ -0.003}$ & $-12.07\substack{+0.09\\ -0.14}$ & $131.87$ & $126$ \\ 
58257.00 & $31.19\pm0.22$ & $-0.654\pm0.009$ & $-10.249\substack{+0.006\\ -0.008}$ & $-10.260\substack{+0.004\\ -0.006}$ & $-11.91\substack{+0.10\\ -0.12}$ & $110.87$ & $116$ \\ 
58272.38 & $37.26\pm0.20$ & $-0.660\pm0.006$ & $-10.202\substack{+0.004\\ -0.004}$ & $-10.223\substack{+0.003\\ -0.003}$ & $-11.57\substack{+0.03\\ -0.04}$ & $392.05$ & $158$ \\ 
58293.62 & $31.51\pm0.20$ & $-0.659\pm0.008$ & $-10.275\substack{+0.006\\ -0.007}$ & $-10.295\substack{+0.005\\ -0.005}$ & $-11.65\substack{+0.05\\ -0.05}$ & $167.40$ & $157$ \\ 
58294.65 & $31.53\pm0.18$ & $-0.652\pm0.007$ & $-10.270\substack{+0.005\\ -0.005}$ & $-10.284\substack{+0.004\\ -0.003}$ & $-11.83\substack{+0.06\\ -0.07}$ & $134.53$ & $98$ \\ 
58302.65 & $31.48\pm0.23$ & $-0.653\pm0.009$ & $-10.272\substack{+0.007\\ -0.008}$ & $-10.287\substack{+0.005\\ -0.005}$ & $-11.80\substack{+0.07\\ -0.10}$ & $156.65$ & $151$ \\ 
58304.43 & $39.51\pm0.25$ & $-0.650\pm0.008$ & $-10.174\substack{+0.006\\ -0.006}$ & $-10.186\substack{+0.004\\ -0.004}$ & $-11.79\substack{+0.07\\ -0.09}$ & $147.65$ & $154$ \\ 
58310.32 & $18.55\pm0.16$ & $-0.617\pm0.010$ & $-10.482\substack{+0.004\\ -0.004}$ & $-10.485\substack{+0.004\\ -0.004}$ & $-16.00\substack{+2.32\\ -0.00}$ & $166.95$ & $76$ \\ 
58311.22 & $17.75\pm0.12$ & $-0.637\pm0.008$ & $-10.507\substack{+0.003\\ -0.003}$ & $-10.510\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.17\\ -0.00}$ & $185.09$ & $94$ \\ 
58312.21 & $21.56\pm0.16$ & $-0.638\pm0.009$ & $-10.422\substack{+0.003\\ -0.003}$ & $-10.425\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.37\\ -0.00}$ & $132.11$ & $85$ \\ 
58313.57 & $26.55\pm0.16$ & $-0.638\pm0.007$ & $-10.333\substack{+0.003\\ -0.002}$ & $-10.335\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.81\\ -0.00}$ & $134.49$ & $104$ \\ 
58314.52 & $28.22\pm0.16$ & $-0.638\pm0.007$ & $-10.314\substack{+0.002\\ -0.002}$ & $-10.316\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.60\\ -0.00}$ & $153.15$ & $111$ \\ 
58315.30 & $25.61\pm0.15$ & $-0.637\pm0.007$ & $-10.357\substack{+0.002\\ -0.002}$ & $-10.359\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.29\\ -0.00}$ & $200.05$ & $108$ \\ 
58317.30 & $28.97\pm0.15$ & $-0.641\pm0.006$ & $-10.305\substack{+0.004\\ -0.004}$ & $-10.310\substack{+0.003\\ -0.003}$ & $-12.42\substack{+0.16\\ -0.26}$ & $263.46$ & $160$ \\ 
58318.58 & $30.20\pm0.22$ & $-0.641\pm0.009$ & $-10.286\substack{+0.007\\ -0.006}$ & $-10.290\substack{+0.005\\ -0.004}$ & $-12.55\substack{+0.29\\ -0.78}$ & $99.62$ & $82$ \\ 
58325.65 & $26.00\pm0.18$ & $-0.638\pm0.008$ & $-10.349\substack{+0.003\\ -0.003}$ & $-10.351\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.61\\ -0.00}$ & $135.09$ & $83$ \\ 
58327.16 & $28.33\pm0.17$ & $-0.638\pm0.007$ & $-10.313\substack{+0.002\\ -0.002}$ & $-10.315\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.10\\ -0.00}$ & $215.76$ & $93$ \\ 
58329.19 & $26.52\pm0.21$ & $-0.638\pm0.009$ & $-10.341\substack{+0.003\\ -0.003}$ & $-10.343\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.50\\ -0.00}$ & $102.98$ & $78$ \\ 
58331.12 & $24.14\pm0.21$ & $-0.639\pm0.010$ & $-10.377\substack{+0.004\\ -0.004}$ & $-10.379\substack{+0.003\\ -0.004}$ & $-16.00\substack{+2.67\\ -0.00}$ & $90.30$ & $80$ \\ 
58333.50 & $30.64\pm0.15$ & $-0.654\pm0.006$ & $-10.284\substack{+0.004\\ -0.004}$ & $-10.300\substack{+0.003\\ -0.003}$ & $-11.79\substack{+0.04\\ -0.05}$ & $133.77$ & $106$ \\ 
58336.46 & $35.69\pm0.22$ & $-0.648\pm0.007$ & $-10.216\substack{+0.006\\ -0.006}$ & $-10.227\substack{+0.004\\ -0.004}$ & $-11.91\substack{+0.08\\ -0.10}$ & $137.24$ & $90$ \\ 
58338.59 & $30.89\pm0.20$ & $-0.646\pm0.008$ & $-10.278\substack{+0.006\\ -0.006}$ & $-10.287\substack{+0.004\\ -0.004}$ & $-12.08\substack{+0.11\\ -0.16}$ & $117.45$ & $90$ \\ 
58340.52 & $34.42\pm0.21$ & $-0.638\pm0.007$ & $-10.228\substack{+0.004\\ -0.003}$ & $-10.230\substack{+0.002\\ -0.003}$ & $-16.00\substack{+3.29\\ -0.00}$ & $157.34$ & $91$ \\ 
58342.64 & $33.53\pm0.21$ & $-0.638\pm0.007$ & $-10.239\substack{+0.002\\ -0.002}$ & $-10.241\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.36\\ -0.00}$ & $179.06$ & $97$ \\ 
58343.60 & $28.71\pm0.19$ & $-0.638\pm0.008$ & $-10.307\substack{+0.003\\ -0.003}$ & $-10.309\substack{+0.002\\ -0.003}$ & $-16.00\substack{+2.34\\ -0.00}$ & $161.16$ & $96$ \\ 
58345.21 & $29.14\pm0.21$ & $-0.643\pm0.009$ & $-10.302\substack{+0.006\\ -0.007}$ & $-10.309\substack{+0.004\\ -0.005}$ & $-12.32\substack{+0.19\\ -0.30}$ & $379.66$ & $158$ \\ 
58348.86 & $29.56\pm0.20$ & $-0.638\pm0.008$ & $-10.294\substack{+0.004\\ -0.004}$ & $-10.296\substack{+0.002\\ -0.004}$ & $-16.00\substack{+3.31\\ -0.00}$ & $80.60$ & $87$ \\ 
58350.96 & $29.07\pm0.19$ & $-0.648\pm0.008$ & $-10.305\substack{+0.006\\ -0.006}$ & $-10.316\substack{+0.004\\ -0.004}$ & $-12.00\substack{+0.09\\ -0.11}$ & $114.46$ & $93$ \\ 
58352.82 & $28.79\pm0.18$ & $-0.640\pm0.008$ & $-10.306\substack{+0.006\\ -0.005}$ & $-10.310\substack{+0.004\\ -0.004}$ & $-12.72\substack{+0.33\\ -3.28}$ & $130.06$ & $93$ \\ 
58354.82 & $29.24\pm0.18$ & $-0.638\pm0.008$ & $-10.299\substack{+0.004\\ -0.004}$ & $-10.301\substack{+0.003\\ -0.004}$ & $-14.02\substack{+1.39\\ -1.98}$ & $134.75$ & $91$ \\ 
58358.86 & $24.67\pm0.21$ & $-0.637\pm0.010$ & $-10.373\substack{+0.004\\ -0.003}$ & $-10.375\substack{+0.003\\ -0.004}$ & $-16.00\substack{+2.88\\ -0.00}$ & $209.39$ & $158$ \\ 
58360.85 & $20.96\pm0.28$ & $-0.632\pm0.016$ & $-10.457\substack{+0.007\\ -0.008}$ & $-10.460\substack{+0.006\\ -0.008}$ & $-16.00\substack{+2.77\\ -0.00}$ & $211.03$ & $149$ \\ 
58362.85 & $20.50\pm0.29$ & $-0.632\pm0.017$ & $-10.466\substack{+0.007\\ -0.007}$ & $-10.469\substack{+0.005\\ -0.007}$ & $-16.00\substack{+3.25\\ -0.00}$ & $185.12$ & $153$ \\ 
58364.71 & $26.81\pm0.18$ & $-0.638\pm0.008$ & $-10.337\substack{+0.002\\ -0.003}$ & $-10.339\substack{+0.002\\ -0.003}$ & $-16.00\substack{+2.38\\ -0.00}$ & $251.50$ & $157$ \\ 
58367.94 & $32.70\pm0.31$ & $-0.674\pm0.011$ & $-10.270\substack{+0.009\\ -0.009}$ & $-10.286\substack{+0.007\\ -0.006}$ & $-11.78\substack{+0.08\\ -0.13}$ & $80.83$ & $67$ \\ 
58369.77 & $24.38\pm0.15$ & $-0.638\pm0.007$ & $-10.378\substack{+0.005\\ -0.004}$ & $-10.381\substack{+0.003\\ -0.004}$ & $-13.56\substack{+0.89\\ -2.44}$ & $151.67$ & $96$ \\ 
58375.54 & $24.75\pm0.19$ & $-0.645\pm0.009$ & $-10.355\substack{+0.008\\ -0.007}$ & $-10.359\substack{+0.005\\ -0.005}$ & $-12.70\substack{+0.36\\ -3.30}$ & $153.11$ & $152$ \\ 
58377.89 & $19.63\pm0.14$ & $-0.637\pm0.009$ & $-10.454\substack{+0.003\\ -0.003}$ & $-10.457\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.35\\ -0.00}$ & $174.56$ & $121$ \\ 
58379.95 & $20.04\pm0.14$ & $-0.637\pm0.008$ & $-10.445\substack{+0.003\\ -0.003}$ & $-10.448\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.12\\ -0.00}$ & $243.86$ & $135$ \\ 
58382.85 & $21.02\pm0.18$ & $-0.638\pm0.011$ & $-10.419\substack{+0.004\\ -0.004}$ & $-10.422\substack{+0.003\\ -0.004}$ & $-16.00\substack{+2.36\\ -0.00}$ & $198.11$ & $108$ \\ 
58388.42 & $23.34\pm0.17$ & $-0.639\pm0.009$ & $-10.397\substack{+0.004\\ -0.003}$ & $-10.399\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.45\\ -0.00}$ & $155.93$ & $81$ \\ 
58390.48 & $26.68\pm0.19$ & $-0.637\pm0.009$ & $-10.339\substack{+0.003\\ -0.004}$ & $-10.341\substack{+0.003\\ -0.004}$ & $-16.00\substack{+2.51\\ -0.00}$ & $126.16$ & $83$ \\ 
58392.70 & $27.34\pm0.13$ & $-0.638\pm0.006$ & $-10.328\substack{+0.002\\ -0.002}$ & $-10.330\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.02\\ -0.00}$ & $300.23$ & $112$ \\ 
58394.92 & $19.31\pm0.12$ & $-0.637\pm0.008$ & $-10.479\substack{+0.002\\ -0.003}$ & $-10.481\substack{+0.002\\ -0.003}$ & $-16.00\substack{+1.82\\ -0.00}$ & $360.91$ & $107$ \\ 
58396.59 & $20.61\pm0.15$ & $-0.638\pm0.008$ & $-10.451\substack{+0.003\\ -0.003}$ & $-10.453\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.18\\ -0.00}$ & $206.63$ & $85$ \\ 
58398.59 & $26.06\pm0.18$ & $-0.638\pm0.008$ & $-10.349\substack{+0.003\\ -0.003}$ & $-10.351\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.19\\ -0.00}$ & $512.01$ & $118$ \\ 
58400.69 & $26.02\pm0.16$ & $-0.637\pm0.007$ & $-10.350\substack{+0.003\\ -0.003}$ & $-10.352\substack{+0.002\\ -0.003}$ & $-16.00\substack{+3.03\\ -0.00}$ & $167.00$ & $153$ \\ 
58402.59 & $26.18\pm0.18$ & $-0.638\pm0.008$ & $-10.347\substack{+0.005\\ -0.004}$ & $-10.349\substack{+0.002\\ -0.004}$ & $-16.00\substack{+3.33\\ -0.00}$ & $135.08$ & $91$ \\ 
58403.93 & $22.94\pm0.18$ & $-0.638\pm0.010$ & $-10.404\substack{+0.004\\ -0.003}$ & $-10.407\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.86\\ -0.00}$ & $91.07$ & $82$ \\ 
58405.89 & $25.10\pm0.27$ & $-0.649\pm0.013$ & $-10.382\substack{+0.011\\ -0.012}$ & $-10.394\substack{+0.008\\ -0.008}$ & $-12.05\substack{+0.14\\ -0.23}$ & $70.78$ & $63$ \\ 
58407.31 & $27.98\pm0.20$ & $-0.644\pm0.009$ & $-10.320\substack{+0.007\\ -0.007}$ & $-10.327\substack{+0.004\\ -0.005}$ & $-12.26\substack{+0.17\\ -0.27}$ & $119.01$ & $79$ \\ 
58409.69 & $30.34\pm0.17$ & $-0.645\pm0.007$ & $-10.285\substack{+0.004\\ -0.005}$ & $-10.292\substack{+0.003\\ -0.003}$ & $-12.19\substack{+0.07\\ -0.17}$ & $154.02$ & $91$ \\ 
58412.07 & $22.83\pm0.17$ & $-0.667\pm0.009$ & $-10.416\substack{+0.007\\ -0.007}$ & $-10.444\substack{+0.005\\ -0.005}$ & $-11.66\substack{+0.04\\ -0.05}$ & $75.77$ & $84$ \\ 
58414.51 & $27.08\pm0.15$ & $-0.671\pm0.007$ & $-10.344\substack{+0.005\\ -0.005}$ & $-10.376\substack{+0.003\\ -0.003}$ & $-11.52\substack{+0.02\\ -0.03}$ & $290.51$ & $131$ \\ 
58416.70 & $29.19\pm0.20$ & $-0.679\pm0.008$ & $-10.314\substack{+0.007\\ -0.009}$ & $-10.354\substack{+0.005\\ -0.007}$ & $-11.39\substack{+0.03\\ -0.03}$ & $126.23$ & $115$ \\ 
58418.70 & $28.31\pm0.20$ & $-0.668\pm0.009$ & $-10.324\substack{+0.007\\ -0.007}$ & $-10.354\substack{+0.005\\ -0.005}$ & $-11.54\substack{+0.04\\ -0.04}$ & $122.30$ & $115$ \\ 
58420.63 & $27.69\pm0.21$ & $-0.646\pm0.009$ & $-10.315\substack{+0.008\\ -0.008}$ & $-10.324\substack{+0.005\\ -0.005}$ & $-12.12\substack{+0.14\\ -0.21}$ & $162.95$ & $132$ \\ 
58421.24 & $30.09\pm0.22$ & $-0.642\pm0.009$ & $-10.289\substack{+0.007\\ -0.007}$ & $-10.294\substack{+0.005\\ -0.005}$ & $-12.33\substack{+0.21\\ -0.41}$ & $103.24$ & $83$ \\ 
58422.67 & $27.29\pm0.20$ & $-0.638\pm0.009$ & $-10.329\substack{+0.003\\ -0.003}$ & $-10.331\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.59\\ -0.00}$ & $175.20$ & $84$ \\ 
58423.96 & $26.11\pm0.19$ & $-0.637\pm0.009$ & $-10.348\substack{+0.003\\ -0.003}$ & $-10.350\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.34\\ -0.00}$ & $163.15$ & $80$ \\ 
58426.46 & $28.24\pm0.17$ & $-0.638\pm0.007$ & $-10.314\substack{+0.002\\ -0.002}$ & $-10.316\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.26\\ -0.00}$ & $251.31$ & $88$ \\ 
58428.20 & $34.03\pm0.18$ & $-0.645\pm0.006$ & $-10.236\substack{+0.005\\ -0.005}$ & $-10.244\substack{+0.003\\ -0.003}$ & $-12.09\substack{+0.10\\ -0.13}$ & $132.70$ & $110$ \\ 
58429.17 & $37.49\pm0.20$ & $-0.651\pm0.007$ & $-10.196\substack{+0.005\\ -0.005}$ & $-10.210\substack{+0.003\\ -0.003}$ & $-11.77\substack{+0.06\\ -0.07}$ & $147.57$ & $103$ \\ 
58430.07 & $38.39\pm0.29$ & $-0.649\pm0.009$ & $-10.185\substack{+0.007\\ -0.007}$ & $-10.195\substack{+0.005\\ -0.005}$ & $-11.87\substack{+0.10\\ -0.14}$ & $84.90$ & $75$ \\ 
58431.16 & $35.76\pm0.21$ & $-0.650\pm0.007$ & $-10.216\substack{+0.005\\ -0.005}$ & $-10.228\substack{+0.003\\ -0.003}$ & $-11.85\substack{+0.07\\ -0.08}$ & $113.35$ & $88$ \\ 
58432.97 & $41.85\pm0.33$ & $-0.644\pm0.009$ & $-10.146\substack{+0.006\\ -0.006}$ & $-10.152\substack{+0.004\\ -0.004}$ & $-12.07\substack{+0.15\\ -0.30}$ & $69.10$ & $79$ \\ 
58433.06 & $41.24\pm0.25$ & $-0.647\pm0.007$ & $-10.153\substack{+0.006\\ -0.006}$ & $-10.162\substack{+0.004\\ -0.004}$ & $-11.90\substack{+0.10\\ -0.12}$ & $109.38$ & $89$ \\ 
58437.51 & $33.73\pm0.25$ & $-0.658\pm0.009$ & $-10.226\substack{+0.007\\ -0.008}$ & $-10.241\substack{+0.005\\ -0.005}$ & $-11.73\substack{+0.07\\ -0.09}$ & $151.51$ & $154$ \\ 
58438.42 & $31.49\pm0.33$ & $-0.668\pm0.013$ & $-10.253\substack{+0.010\\ -0.011}$ & $-10.278\substack{+0.007\\ -0.008}$ & $-11.54\substack{+0.07\\ -0.07}$ & $80.13$ & $73$ \\ 
58439.64 & $34.32\pm0.36$ & $-0.664\pm0.013$ & $-10.235\substack{+0.009\\ -0.010}$ & $-10.260\substack{+0.005\\ -0.007}$ & $-11.53\substack{+0.07\\ -0.07}$ & $108.14$ & $75$ \\ 
58449.22 & $33.58\pm0.23$ & $-0.651\pm0.008$ & $-10.217\substack{+0.006\\ -0.009}$ & $-10.225\substack{+0.004\\ -0.006}$ & $-12.01\substack{+0.12\\ -0.17}$ & $127.99$ & $133$ \\ 
58453.60 & $27.77\pm0.16$ & $-0.637\pm0.007$ & $-10.322\substack{+0.002\\ -0.002}$ & $-10.324\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.44\\ -0.00}$ & $224.54$ & $92$ \\ 
58455.11 & $23.73\pm0.19$ & $-0.638\pm0.010$ & $-10.390\substack{+0.004\\ -0.003}$ & $-10.392\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.58\\ -0.00}$ & $92.23$ & $80$ \\ 
58456.98 & $21.88\pm0.16$ & $-0.638\pm0.009$ & $-10.425\substack{+0.004\\ -0.003}$ & $-10.427\substack{+0.003\\ -0.003}$ & $-15.99\substack{+3.03\\ -0.01}$ & $77.18$ & $85$ \\ 
58458.91 & $22.43\pm0.16$ & $-0.640\pm0.008$ & $-10.415\substack{+0.007\\ -0.007}$ & $-10.419\substack{+0.004\\ -0.005}$ & $-12.74\substack{+0.32\\ -3.27}$ & $112.26$ & $87$ \\ 
58460.91 & $26.18\pm0.17$ & $-0.638\pm0.008$ & $-10.347\substack{+0.003\\ -0.002}$ & $-10.349\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.56\\ -0.00}$ & $113.97$ & $100$ \\ 
58462.90 & $22.46\pm0.17$ & $-0.637\pm0.009$ & $-10.413\substack{+0.003\\ -0.003}$ & $-10.416\substack{+0.002\\ -0.003}$ & $-16.00\substack{+2.20\\ -0.00}$ & $212.56$ & $114$ \\ 
58464.58 & $21.76\pm0.15$ & $-0.638\pm0.008$ & $-10.427\substack{+0.003\\ -0.003}$ & $-10.429\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.54\\ -0.00}$ & $121.64$ & $90$ \\ 
58466.18 & $23.44\pm0.18$ & $-0.637\pm0.009$ & $-10.395\substack{+0.004\\ -0.005}$ & $-10.397\substack{+0.002\\ -0.005}$ & $-16.00\substack{+3.25\\ -0.00}$ & $238.39$ & $147$ \\ 
58469.02 & $19.61\pm0.17$ & $-0.638\pm0.010$ & $-10.458\substack{+0.004\\ -0.003}$ & $-10.461\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.69\\ -0.00}$ & $130.71$ & $98$ \\ 
58470.68 & $20.83\pm0.16$ & $-0.637\pm0.009$ & $-10.428\substack{+0.003\\ -0.003}$ & $-10.431\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.23\\ -0.00}$ & $193.95$ & $89$ \\ 
58471.77 & $27.07\pm0.24$ & $-0.622\pm0.011$ & $-10.327\substack{+0.004\\ -0.004}$ & $-10.329\substack{+0.003\\ -0.004}$ & $-16.00\substack{+3.12\\ -0.00}$ & $112.79$ & $75$ \\ 
58473.91 & $28.33\pm0.19$ & $-0.637\pm0.008$ & $-10.296\substack{+0.003\\ -0.003}$ & $-10.297\substack{+0.002\\ -0.003}$ & $-16.00\substack{+3.04\\ -0.00}$ & $113.89$ & $118$ \\ 
58476.07 & $33.46\pm0.32$ & $-0.666\pm0.012$ & $-10.259\substack{+0.010\\ -0.010}$ & $-10.272\substack{+0.007\\ -0.007}$ & $-11.85\substack{+0.12\\ -0.16}$ & $80.84$ & $75$ \\ 
58479.11 & $31.13\pm0.21$ & $-0.654\pm0.008$ & $-10.258\substack{+0.006\\ -0.006}$ & $-10.269\substack{+0.004\\ -0.004}$ & $-11.92\substack{+0.09\\ -0.11}$ & $104.93$ & $86$ \\ 
58481.24 & $25.92\pm0.22$ & $-0.665\pm0.010$ & $-10.342\substack{+0.009\\ -0.009}$ & $-10.361\substack{+0.006\\ -0.006}$ & $-11.78\substack{+0.07\\ -0.09}$ & $134.69$ & $151$ \\ 
58487.79 & $34.32\pm0.31$ & $-0.646\pm0.011$ & $-10.207\substack{+0.009\\ -0.009}$ & $-10.229\substack{+0.006\\ -0.007}$ & $-11.53\substack{+0.06\\ -0.07}$ & $71.53$ & $78$ \\ 
58489.79 & $24.19\pm0.20$ & $-0.639\pm0.010$ & $-10.359\substack{+0.008\\ -0.008}$ & $-10.372\substack{+0.005\\ -0.006}$ & $-11.95\substack{+0.10\\ -0.12}$ & $213.96$ & $114$ \\ 
58491.53 & $21.85\pm0.24$ & $-0.616\pm0.013$ & $-10.393\substack{+0.008\\ -0.006}$ & $-10.396\substack{+0.005\\ -0.006}$ & $-14.17\substack{+1.61\\ -1.83}$ & $95.45$ & $81$ \\ 
58493.71 & $22.65\pm0.27$ & $-0.666\pm0.014$ & $-10.393\substack{+0.013\\ -0.012}$ & $-10.435\substack{+0.009\\ -0.009}$ & $-11.46\substack{+0.05\\ -0.05}$ & $107.90$ & $123$ \\ 
58497.64 & $24.29\pm0.19$ & $-0.652\pm0.010$ & $-10.358\substack{+0.008\\ -0.008}$ & $-10.374\substack{+0.006\\ -0.006}$ & $-11.87\substack{+0.08\\ -0.10}$ & $72.95$ & $92$ \\ 
58499.38 & $26.92\pm0.15$ & $-0.656\pm0.007$ & $-10.329\substack{+0.005\\ -0.005}$ & $-10.362\substack{+0.004\\ -0.004}$ & $-11.50\substack{+0.03\\ -0.03}$ & $183.47$ & $151$ \\ 
58500.48 & $27.56\pm0.16$ & $-0.671\pm0.007$ & $-10.324\substack{+0.006\\ -0.006}$ & $-10.371\substack{+0.005\\ -0.004}$ & $-11.34\substack{+0.02\\ -0.02}$ & $279.44$ & $154$ \\ 
58501.89 & $28.72\pm0.17$ & $-0.670\pm0.007$ & $-10.303\substack{+0.004\\ -0.005}$ & $-10.340\substack{+0.003\\ -0.003}$ & $-11.41\substack{+0.02\\ -0.02}$ & $139.78$ & $114$ \\ 
58503.24 & $26.65\pm0.14$ & $-0.677\pm0.006$ & $-10.339\substack{+0.005\\ -0.005}$ & $-10.388\substack{+0.004\\ -0.004}$ & $-11.34\substack{+0.02\\ -0.02}$ & $211.47$ & $144$ \\ 
58504.98 & $34.96\pm0.17$ & $-0.690\pm0.006$ & $-10.230\substack{+0.004\\ -0.005}$ & $-10.277\substack{+0.003\\ -0.003}$ & $-11.24\substack{+0.02\\ -0.02}$ & $177.20$ & $135$ \\ 
58505.95 & $37.14\pm0.18$ & $-0.679\pm0.006$ & $-10.202\substack{+0.006\\ -0.005}$ & $-10.242\substack{+0.005\\ -0.003}$ & $-11.27\substack{+0.02\\ -0.03}$ & $162.07$ & $145$ \\ 
58506.33 & $35.00\pm0.17$ & $-0.677\pm0.006$ & $-10.226\substack{+0.004\\ -0.005}$ & $-10.264\substack{+0.003\\ -0.004}$ & $-11.32\substack{+0.02\\ -0.02}$ & $167.58$ & $156$ \\ 
58507.62 & $31.60\pm0.18$ & $-0.676\pm0.007$ & $-10.271\substack{+0.005\\ -0.004}$ & $-10.309\substack{+0.003\\ -0.002}$ & $-11.37\substack{+0.02\\ -0.02}$ & $168.52$ & $147$ \\ 
58511.87 & $27.31\pm0.18$ & $-0.679\pm0.008$ & $-10.329\substack{+0.006\\ -0.006}$ & $-10.378\substack{+0.004\\ -0.005}$ & $-11.31\substack{+0.02\\ -0.02}$ & $95.75$ & $80$ \\ 
58513.28 & $27.94\pm0.15$ & $-0.669\pm0.007$ & $-10.323\substack{+0.005\\ -0.005}$ & $-10.359\substack{+0.004\\ -0.004}$ & $-11.45\substack{+0.02\\ -0.02}$ & $164.88$ & $146$ \\ 
58514.73 & $28.60\pm0.16$ & $-0.685\pm0.007$ & $-10.313\substack{+0.004\\ -0.005}$ & $-10.364\substack{+0.004\\ -0.004}$ & $-11.28\substack{+0.01\\ -0.02}$ & $191.85$ & $146$ \\ 
58515.86 & $32.26\pm0.22$ & $-0.686\pm0.008$ & $-10.259\substack{+0.006\\ -0.006}$ & $-10.316\substack{+0.005\\ -0.005}$ & $-11.19\substack{+0.02\\ -0.02}$ & $144.95$ & $106$ \\ 
58517.18 & $33.15\pm0.23$ & $-0.680\pm0.008$ & $-10.237\substack{+0.006\\ -0.006}$ & $-10.288\substack{+0.005\\ -0.005}$ & $-11.21\substack{+0.02\\ -0.02}$ & $96.48$ & $81$ \\ 
58521.53 & $37.13\pm0.22$ & $-0.698\pm0.007$ & $-10.218\substack{+0.005\\ -0.005}$ & $-10.276\substack{+0.004\\ -0.004}$ & $-11.13\substack{+0.02\\ -0.02}$ & $127.52$ & $88$ \\ 
58523.50 & $35.79\pm0.20$ & $-0.685\pm0.007$ & $-10.229\substack{+0.005\\ -0.005}$ & $-10.274\substack{+0.004\\ -0.004}$ & $-11.25\substack{+0.02\\ -0.02}$ & $188.89$ & $134$ \\ 
58527.09 & $38.44\pm0.25$ & $-0.710\pm0.008$ & $-10.207\substack{+0.006\\ -0.006}$ & $-10.279\substack{+0.004\\ -0.005}$ & $-11.04\substack{+0.01\\ -0.01}$ & $117.21$ & $79$ \\ 
58528.06 & $34.36\pm0.31$ & $-0.698\pm0.011$ & $-10.226\substack{+0.009\\ -0.009}$ & $-10.289\substack{+0.006\\ -0.007}$ & $-11.11\substack{+0.02\\ -0.03}$ & $92.15$ & $61$ \\ 
58529.87 & $32.54\pm0.25$ & $-0.695\pm0.009$ & $-10.255\substack{+0.008\\ -0.007}$ & $-10.306\substack{+0.007\\ -0.005}$ & $-11.22\substack{+0.02\\ -0.03}$ & $101.49$ & $90$ \\ 
58541.28 & $33.88\pm0.19$ & $-0.670\pm0.007$ & $-10.211\substack{+0.005\\ -0.005}$ & $-10.242\substack{+0.003\\ -0.003}$ & $-11.40\substack{+0.02\\ -0.03}$ & $112.46$ & $89$ \\ 
58544.08 & $39.57\pm0.23$ & $-0.673\pm0.007$ & $-10.142\substack{+0.005\\ -0.005}$ & $-10.168\substack{+0.004\\ -0.004}$ & $-11.41\substack{+0.03\\ -0.03}$ & $133.57$ & $96$ \\ 
58545.93 & $40.44\pm0.35$ & $-0.683\pm0.011$ & $-10.148\substack{+0.007\\ -0.010}$ & $-10.192\substack{+0.004\\ -0.008}$ & $-11.17\substack{+0.03\\ -0.03}$ & $87.80$ & $82$ \\ 
58548.20 & $43.64\pm0.25$ & $-0.695\pm0.007$ & $-10.099\substack{+0.005\\ -0.005}$ & $-10.146\substack{+0.004\\ -0.004}$ & $-11.10\substack{+0.02\\ -0.02}$ & $80.18$ & $84$ \\ 
58550.32 & $39.74\pm0.22$ & $-0.676\pm0.007$ & $-10.135\substack{+0.005\\ -0.005}$ & $-10.173\substack{+0.003\\ -0.003}$ & $-11.24\substack{+0.02\\ -0.02}$ & $100.15$ & $90$ \\ 
58553.35 & $36.42\pm0.22$ & $-0.650\pm0.007$ & $-10.185\substack{+0.005\\ -0.006}$ & $-10.208\substack{+0.004\\ -0.004}$ & $-11.52\substack{+0.04\\ -0.04}$ & $102.53$ & $85$ \\ 
58556.06 & $40.46\pm0.24$ & $-0.675\pm0.007$ & $-10.142\substack{+0.005\\ -0.005}$ & $-10.169\substack{+0.004\\ -0.004}$ & $-11.38\substack{+0.03\\ -0.03}$ & $89.36$ & $88$ \\ 
58559.95 & $30.25\pm0.25$ & $-0.664\pm0.010$ & $-10.268\substack{+0.008\\ -0.008}$ & $-10.298\substack{+0.006\\ -0.006}$ & $-11.46\substack{+0.04\\ -0.05}$ & $102.36$ & $76$ \\ 
58561.50 & $29.64\pm0.16$ & $-0.661\pm0.006$ & $-10.280\substack{+0.006\\ -0.005}$ & $-10.316\substack{+0.005\\ -0.003}$ & $-11.39\substack{+0.02\\ -0.02}$ & $120.03$ & $118$ \\ 
58562.94 & $31.08\pm0.23$ & $-0.682\pm0.009$ & $-10.263\substack{+0.006\\ -0.007}$ & $-10.311\substack{+0.005\\ -0.005}$ & $-11.26\substack{+0.02\\ -0.03}$ & $91.11$ & $73$ \\ 
58564.04 & $41.61\pm0.27$ & $-0.673\pm0.008$ & $-10.137\substack{+0.006\\ -0.007}$ & $-10.185\substack{+0.004\\ -0.005}$ & $-11.13\substack{+0.02\\ -0.02}$ & $116.31$ & $93$ \\ 
58565.78 & $40.03\pm0.24$ & $-0.681\pm0.007$ & $-10.157\substack{+0.005\\ -0.006}$ & $-10.213\substack{+0.004\\ -0.004}$ & $-11.08\substack{+0.02\\ -0.02}$ & $139.84$ & $83$ \\ 
58567.20 & $32.45\pm0.24$ & $-0.698\pm0.009$ & $-10.251\substack{+0.007\\ -0.008}$ & $-10.315\substack{+0.004\\ -0.007}$ & $-11.13\substack{+0.03\\ -0.02}$ & $152.77$ & $146$ \\ 
58568.80 & $35.31\pm0.22$ & $-0.693\pm0.008$ & $-10.215\substack{+0.006\\ -0.006}$ & $-10.283\substack{+0.004\\ -0.004}$ & $-11.06\substack{+0.01\\ -0.01}$ & $102.14$ & $84$ \\ 
58570.87 & $40.34\pm0.17$ & $-0.681\pm0.005$ & $-10.148\substack{+0.003\\ -0.003}$ & $-10.189\substack{+0.002\\ -0.002}$ & $-11.21\substack{+0.01\\ -0.01}$ & $159.09$ & $127$ \\ 
58573.06 & $38.92\pm0.18$ & $-0.690\pm0.006$ & $-10.169\substack{+0.004\\ -0.005}$ & $-10.225\substack{+0.003\\ -0.004}$ & $-11.10\substack{+0.01\\ -0.01}$ & $210.53$ & $154$ \\ 
58575.51 & $41.29\pm0.23$ & $-0.682\pm0.007$ & $-10.140\substack{+0.004\\ -0.005}$ & $-10.188\substack{+0.003\\ -0.003}$ & $-11.14\substack{+0.02\\ -0.02}$ & $170.07$ & $127$ \\ 
58577.45 & $43.04\pm0.27$ & $-0.680\pm0.008$ & $-10.125\substack{+0.005\\ -0.006}$ & $-10.180\substack{+0.004\\ -0.004}$ & $-11.06\substack{+0.02\\ -0.02}$ & $112.51$ & $79$ \\ 
58579.38 & $49.83\pm0.29$ & $-0.706\pm0.007$ & $-10.065\substack{+0.005\\ -0.005}$ & $-10.127\substack{+0.004\\ -0.004}$ & $-10.94\substack{+0.01\\ -0.01}$ & $148.57$ & $84$ \\ 
58581.35 & $40.53\pm0.27$ & $-0.677\pm0.008$ & $-10.137\substack{+0.006\\ -0.006}$ & $-10.188\substack{+0.004\\ -0.005}$ & $-11.10\substack{+0.02\\ -0.02}$ & $78.93$ & $78$ \\ 
58586.70 & $40.82\pm0.30$ & $-0.681\pm0.009$ & $-10.171\substack{+0.008\\ -0.008}$ & $-10.212\substack{+0.007\\ -0.006}$ & $-11.23\substack{+0.03\\ -0.03}$ & $207.05$ & $159$ \\ 
58588.63 & $49.02\pm0.29$ & $-0.672\pm0.007$ & $-10.088\substack{+0.005\\ -0.006}$ & $-10.119\substack{+0.004\\ -0.004}$ & $-11.26\substack{+0.03\\ -0.02}$ & $213.39$ & $161$ \\ 
58591.05 & $42.39\pm0.25$ & $-0.682\pm0.007$ & $-10.154\substack{+0.006\\ -0.007}$ & $-10.196\substack{+0.004\\ -0.005}$ & $-11.21\substack{+0.02\\ -0.02}$ & $170.98$ & $159$ \\ 
58592.65 & $45.14\pm0.23$ & $-0.650\pm0.006$ & $-10.116\substack{+0.004\\ -0.004}$ & $-10.128\substack{+0.003\\ -0.003}$ & $-11.72\substack{+0.06\\ -0.06}$ & $1119.03$ & $156$ \\ 
58594.91 & $42.42\pm0.25$ & $-0.679\pm0.007$ & $-10.153\substack{+0.005\\ -0.006}$ & $-10.192\substack{+0.004\\ -0.004}$ & $-11.23\substack{+0.02\\ -0.02}$ & $250.46$ & $158$ \\ 
58596.84 & $43.25\pm0.26$ & $-0.669\pm0.007$ & $-10.141\substack{+0.005\\ -0.005}$ & $-10.170\substack{+0.004\\ -0.003}$ & $-11.35\substack{+0.02\\ -0.03}$ & $1384.39$ & $170$ \\ 
58603.42 & $38.02\pm0.27$ & $-0.675\pm0.009$ & $-10.177\substack{+0.007\\ -0.007}$ & $-10.226\substack{+0.005\\ -0.005}$ & $-11.17\substack{+0.02\\ -0.02}$ & $101.05$ & $73$ \\ 
58605.35 & $45.61\pm0.25$ & $-0.698\pm0.007$ & $-10.090\substack{+0.005\\ -0.006}$ & $-10.140\substack{+0.003\\ -0.004}$ & $-11.06\substack{+0.02\\ -0.02}$ & $101.22$ & $90$ \\ 
58607.22 & $35.12\pm0.20$ & $-0.692\pm0.007$ & $-10.202\substack{+0.005\\ -0.005}$ & $-10.251\substack{+0.004\\ -0.004}$ & $-11.19\substack{+0.02\\ -0.02}$ & $93.18$ & $94$ \\ 
58609.28 & $38.37\pm0.20$ & $-0.677\pm0.006$ & $-10.168\substack{+0.004\\ -0.004}$ & $-10.202\substack{+0.003\\ -0.003}$ & $-11.32\substack{+0.02\\ -0.02}$ & $126.69$ & $99$ \\ 
58611.34 & $36.44\pm0.20$ & $-0.657\pm0.007$ & $-10.176\substack{+0.005\\ -0.005}$ & $-10.196\substack{+0.003\\ -0.003}$ & $-11.57\substack{+0.04\\ -0.04}$ & $116.70$ & $94$ \\ 
58612.95 & $32.28\pm0.17$ & $-0.663\pm0.006$ & $-10.239\substack{+0.005\\ -0.005}$ & $-10.264\substack{+0.003\\ -0.003}$ & $-11.52\substack{+0.03\\ -0.03}$ & $124.93$ & $98$ \\ 
58614.95 & $36.70\pm0.18$ & $-0.669\pm0.006$ & $-10.193\substack{+0.004\\ -0.005}$ & $-10.219\substack{+0.003\\ -0.004}$ & $-11.46\substack{+0.03\\ -0.03}$ & $128.62$ & $146$ \\ 
58617.01 & $33.03\pm0.21$ & $-0.669\pm0.008$ & $-10.246\substack{+0.006\\ -0.006}$ & $-10.267\substack{+0.004\\ -0.004}$ & $-11.60\substack{+0.04\\ -0.05}$ & $112.86$ & $93$ \\ 
58619.00 & $33.30\pm0.21$ & $-0.677\pm0.008$ & $-10.236\substack{+0.006\\ -0.006}$ & $-10.265\substack{+0.004\\ -0.004}$ & $-11.46\substack{+0.03\\ -0.04}$ & $106.51$ & $87$ \\ 
58621.13 & $36.85\pm0.32$ & $-0.671\pm0.011$ & $-10.198\substack{+0.008\\ -0.008}$ & $-10.239\substack{+0.005\\ -0.006}$ & $-11.26\substack{+0.03\\ -0.03}$ & $60.84$ & $67$ \\ 
58623.22 & $33.08\pm0.18$ & $-0.676\pm0.007$ & $-10.241\substack{+0.005\\ -0.005}$ & $-10.273\substack{+0.003\\ -0.003}$ & $-11.41\substack{+0.02\\ -0.03}$ & $161.74$ & $109$ \\ 
58626.73 & $32.62\pm0.22$ & $-0.662\pm0.008$ & $-10.233\substack{+0.008\\ -0.007}$ & $-10.257\substack{+0.006\\ -0.005}$ & $-11.54\substack{+0.04\\ -0.05}$ & $73.74$ & $80$ \\ 
58632.66 & $27.72\pm0.20$ & $-0.663\pm0.009$ & $-10.322\substack{+0.009\\ -0.008}$ & $-10.347\substack{+0.006\\ -0.006}$ & $-11.62\substack{+0.05\\ -0.05}$ & $89.74$ & $90$ \\ 
58635.56 & $36.47\pm0.21$ & $-0.675\pm0.007$ & $-10.217\substack{+0.005\\ -0.005}$ & $-10.252\substack{+0.004\\ -0.004}$ & $-11.34\substack{+0.02\\ -0.03}$ & $134.34$ & $100$ \\ 
58637.62 & $38.66\pm0.23$ & $-0.677\pm0.007$ & $-10.192\substack{+0.005\\ -0.006}$ & $-10.230\substack{+0.004\\ -0.004}$ & $-11.29\substack{+0.02\\ -0.02}$ & $108.10$ & $93$ \\ 
58643.87 & $47.02\pm0.30$ & $-0.674\pm0.008$ & $-10.106\substack{+0.008\\ -0.004}$ & $-10.140\substack{+0.006\\ -0.003}$ & $-11.25\substack{+0.03\\ -0.03}$ & $128.16$ & $151$ \\ 
58646.07 & $38.94\pm0.32$ & $-0.684\pm0.010$ & $-10.192\substack{+0.008\\ -0.008}$ & $-10.236\substack{+0.006\\ -0.006}$ & $-11.23\substack{+0.03\\ -0.03}$ & $213.13$ & $158$ \\ 
58651.93 & $35.49\pm0.22$ & $-0.671\pm0.007$ & $-10.228\substack{+0.005\\ -0.005}$ & $-10.259\substack{+0.004\\ -0.004}$ & $-11.40\substack{+0.03\\ -0.03}$ & $180.65$ & $153$ \\ 
58653.93 & $31.38\pm0.21$ & $-0.692\pm0.008$ & $-10.288\substack{+0.007\\ -0.006}$ & $-10.341\substack{+0.006\\ -0.004}$ & $-11.25\substack{+0.02\\ -0.02}$ & $170.56$ & $114$ \\ 
58655.93 & $35.53\pm0.21$ & $-0.696\pm0.007$ & $-10.236\substack{+0.006\\ -0.006}$ & $-10.292\substack{+0.004\\ -0.004}$ & $-11.16\substack{+0.02\\ -0.02}$ & $146.55$ & $102$ \\ 
58657.96 & $40.66\pm0.25$ & $-0.688\pm0.008$ & $-10.174\substack{+0.006\\ -0.006}$ & $-10.222\substack{+0.004\\ -0.005}$ & $-11.17\substack{+0.02\\ -0.02}$ & $133.69$ & $105$ \\ 
58660.24 & $38.57\pm0.24$ & $-0.679\pm0.008$ & $-10.194\substack{+0.006\\ -0.006}$ & $-10.234\substack{+0.005\\ -0.004}$ & $-11.28\substack{+0.02\\ -0.03}$ & $568.72$ & $165$ \\ 
58662.04 & $32.24\pm0.25$ & $-0.680\pm0.010$ & $-10.273\substack{+0.007\\ -0.008}$ & $-10.313\substack{+0.005\\ -0.006}$ & $-11.34\substack{+0.03\\ -0.03}$ & $290.08$ & $154$ \\ 
58664.24 & $37.73\pm0.24$ & $-0.682\pm0.008$ & $-10.205\substack{+0.006\\ -0.006}$ & $-10.247\substack{+0.004\\ -0.005}$ & $-11.26\substack{+0.02\\ -0.02}$ & $217.34$ & $156$ \\ 
58665.88 & $36.96\pm0.30$ & $-0.703\pm0.010$ & $-10.221\substack{+0.008\\ -0.009}$ & $-10.285\substack{+0.006\\ -0.007}$ & $-11.10\substack{+0.02\\ -0.02}$ & $197.46$ & $157$ \\ 
58673.24 & $30.31\pm0.21$ & $-0.671\pm0.008$ & $-10.220\substack{+0.006\\ -0.006}$ & $-10.247\substack{+0.004\\ -0.005}$ & $-11.47\substack{+0.04\\ -0.04}$ & $102.43$ & $82$ \\ 
58675.30 & $30.18\pm0.18$ & $-0.661\pm0.007$ & $-10.220\substack{+0.005\\ -0.006}$ & $-10.243\substack{+0.004\\ -0.004}$ & $-11.55\substack{+0.04\\ -0.04}$ & $128.32$ & $97$ \\ 
58677.17 & $26.75\pm0.15$ & $-0.671\pm0.007$ & $-10.287\substack{+0.005\\ -0.005}$ & $-10.319\substack{+0.003\\ -0.004}$ & $-11.46\substack{+0.02\\ -0.03}$ & $173.52$ & $128$ \\ 
58679.04 & $35.57\pm0.19$ & $-0.676\pm0.007$ & $-10.153\substack{+0.005\\ -0.005}$ & $-10.185\substack{+0.003\\ -0.003}$ & $-11.33\substack{+0.03\\ -0.03}$ & $140.28$ & $110$ \\ 
58680.40 & $31.77\pm0.21$ & $-0.680\pm0.008$ & $-10.205\substack{+0.007\\ -0.007}$ & $-10.245\substack{+0.005\\ -0.005}$ & $-11.28\substack{+0.03\\ -0.03}$ & $140.95$ & $139$ \\ 
58683.23 & $27.45\pm0.14$ & $-0.671\pm0.006$ & $-10.265\substack{+0.005\\ -0.005}$ & $-10.296\substack{+0.003\\ -0.004}$ & $-11.44\substack{+0.03\\ -0.02}$ & $155.60$ & $148$ \\ 
58685.11 & $30.76\pm0.19$ & $-0.663\pm0.008$ & $-10.222\substack{+0.006\\ -0.006}$ & $-10.246\substack{+0.004\\ -0.005}$ & $-11.52\substack{+0.04\\ -0.04}$ & $120.62$ & $115$ \\ 
58687.54 & $29.83\pm0.23$ & $-0.654\pm0.009$ & $-10.233\substack{+0.007\\ -0.007}$ & $-10.247\substack{+0.005\\ -0.005}$ & $-11.76\substack{+0.08\\ -0.09}$ & $139.16$ & $76$ \\ 
58690.12 & $20.16\pm0.18$ & $-0.631\pm0.011$ & $-10.458\substack{+0.009\\ -0.009}$ & $-10.467\substack{+0.006\\ -0.006}$ & $-12.24\substack{+0.15\\ -0.23}$ & $126.72$ & $76$ \\ 
58691.79 & $28.41\pm0.18$ & $-0.653\pm0.008$ & $-10.317\substack{+0.006\\ -0.006}$ & $-10.333\substack{+0.004\\ -0.004}$ & $-11.83\substack{+0.06\\ -0.07}$ & $132.02$ & $90$ \\ 
58694.70 & $32.68\pm0.19$ & $-0.688\pm0.007$ & $-10.269\substack{+0.005\\ -0.005}$ & $-10.317\substack{+0.004\\ -0.004}$ & $-11.26\substack{+0.02\\ -0.02}$ & $137.05$ & $89$ \\ 
58699.98 & $38.97\pm0.25$ & $-0.679\pm0.008$ & $-10.190\substack{+0.006\\ -0.006}$ & $-10.229\substack{+0.005\\ -0.004}$ & $-11.27\substack{+0.03\\ -0.03}$ & $87.03$ & $87$ \\ 
58702.27 & $38.31\pm0.25$ & $-0.689\pm0.008$ & $-10.200\substack{+0.006\\ -0.006}$ & $-10.249\substack{+0.004\\ -0.004}$ & $-11.18\substack{+0.02\\ -0.02}$ & $761.44$ & $159$ \\ 
58704.59 & $31.77\pm0.19$ & $-0.680\pm0.007$ & $-10.277\substack{+0.005\\ -0.006}$ & $-10.318\substack{+0.004\\ -0.004}$ & $-11.35\substack{+0.02\\ -0.02}$ & $232.95$ & $153$ \\ 
58706.46 & $35.93\pm0.21$ & $-0.664\pm0.007$ & $-10.219\substack{+0.005\\ -0.005}$ & $-10.243\substack{+0.004\\ -0.004}$ & $-11.51\substack{+0.03\\ -0.04}$ & $129.66$ & $102$ \\ 
58711.99 & $24.60\pm0.21$ & $-0.628\pm0.010$ & $-10.372\substack{+0.008\\ -0.008}$ & $-10.384\substack{+0.005\\ -0.006}$ & $-12.05\substack{+0.12\\ -0.16}$ & $100.98$ & $69$ \\ 
58712.05 & $25.68\pm0.22$ & $-0.641\pm0.010$ & $-10.356\substack{+0.008\\ -0.009}$ & $-10.374\substack{+0.006\\ -0.006}$ & $-11.81\substack{+0.07\\ -0.09}$ & $66.87$ & $69$ \\ 
58713.92 & $28.50\pm0.19$ & $-0.638\pm0.008$ & $-10.310\substack{+0.003\\ -0.002}$ & $-10.312\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.89\\ -0.00}$ & $160.89$ & $85$ \\ 
58715.57 & $31.81\pm0.19$ & $-0.645\pm0.007$ & $-10.265\substack{+0.005\\ -0.005}$ & $-10.273\substack{+0.004\\ -0.004}$ & $-12.13\substack{+0.12\\ -0.16}$ & $131.19$ & $87$ \\ 
58717.44 & $30.07\pm0.21$ & $-0.648\pm0.008$ & $-10.290\substack{+0.006\\ -0.006}$ & $-10.301\substack{+0.004\\ -0.004}$ & $-11.99\substack{+0.10\\ -0.13}$ & $150.94$ & $79$ \\ 
58719.05 & $27.58\pm0.17$ & $-0.647\pm0.007$ & $-10.328\substack{+0.005\\ -0.006}$ & $-10.338\substack{+0.004\\ -0.004}$ & $-12.06\substack{+0.09\\ -0.12}$ & $144.47$ & $86$ \\ 
58721.15 & $21.88\pm0.18$ & $-0.656\pm0.010$ & $-10.431\substack{+0.008\\ -0.008}$ & $-10.450\substack{+0.005\\ -0.005}$ & $-11.87\substack{+0.07\\ -0.08}$ & $96.57$ & $78$ \\ 
58723.06 & $28.38\pm0.23$ & $-0.683\pm0.010$ & $-10.329\substack{+0.008\\ -0.009}$ & $-10.372\substack{+0.006\\ -0.007}$ & $-11.37\substack{+0.03\\ -0.03}$ & $159.80$ & $158$ \\ 
58729.84 & $40.50\pm0.31$ & $-0.682\pm0.009$ & $-10.174\substack{+0.008\\ -0.008}$ & $-10.216\substack{+0.006\\ -0.006}$ & $-11.23\substack{+0.03\\ -0.03}$ & $84.69$ & $90$ \\ 
58737.40 & $35.87\pm0.37$ & $-0.652\pm0.012$ & $-10.191\substack{+0.009\\ -0.012}$ & $-10.223\substack{+0.006\\ -0.009}$ & $-11.36\substack{+0.05\\ -0.04}$ & $127.23$ & $133$ \\ 
58739.36 & $35.06\pm0.27$ & $-0.688\pm0.009$ & $-10.210\substack{+0.007\\ -0.007}$ & $-10.254\substack{+0.005\\ -0.005}$ & $-11.25\substack{+0.03\\ -0.03}$ & $243.35$ & $157$ \\ 
58740.65 & $34.66\pm0.28$ & $-0.694\pm0.010$ & $-10.218\substack{+0.011\\ -0.008}$ & $-10.269\substack{+0.009\\ -0.006}$ & $-11.19\substack{+0.03\\ -0.02}$ & $161.27$ & $131$ \\ 
58742.97 & $36.60\pm0.28$ & $-0.687\pm0.009$ & $-10.202\substack{+0.009\\ -0.007}$ & $-10.249\substack{+0.007\\ -0.006}$ & $-11.20\substack{+0.03\\ -0.01}$ & $129.27$ & $100$ \\ 
58743.04 & $36.83\pm0.28$ & $-0.688\pm0.009$ & $-10.200\substack{+0.007\\ -0.007}$ & $-10.248\substack{+0.005\\ -0.005}$ & $-11.19\substack{+0.02\\ -0.02}$ & $205.54$ & $154$ \\ 
58744.91 & $33.85\pm0.22$ & $-0.674\pm0.008$ & $-10.222\substack{+0.005\\ -0.006}$ & $-10.257\substack{+0.003\\ -0.006}$ & $-11.36\substack{+0.03\\ -0.02}$ & $141.71$ & $130$ \\ 
58751.71 & $27.59\pm0.19$ & $-0.665\pm0.008$ & $-10.319\substack{+0.007\\ -0.007}$ & $-10.345\substack{+0.005\\ -0.005}$ & $-11.59\substack{+0.04\\ -0.05}$ & $109.68$ & $120$ \\ 
58753.15 & $30.21\pm0.21$ & $-0.669\pm0.008$ & $-10.296\substack{+0.005\\ -0.006}$ & $-10.325\substack{+0.004\\ -0.004}$ & $-11.52\substack{+0.03\\ -0.04}$ & $85.05$ & $81$ \\ 
58755.02 & $30.85\pm0.19$ & $-0.681\pm0.008$ & $-10.291\substack{+0.007\\ -0.007}$ & $-10.332\substack{+0.006\\ -0.006}$ & $-11.36\substack{+0.02\\ -0.02}$ & $103.20$ & $98$ \\ 
58756.57 & $30.09\pm0.17$ & $-0.699\pm0.007$ & $-10.309\substack{+0.005\\ -0.005}$ & $-10.369\substack{+0.004\\ -0.003}$ & $-11.21\substack{+0.01\\ -0.02}$ & $137.82$ & $103$ \\ 
58758.38 & $29.03\pm0.18$ & $-0.699\pm0.008$ & $-10.324\substack{+0.006\\ -0.006}$ & $-10.385\substack{+0.004\\ -0.004}$ & $-11.23\substack{+0.02\\ -0.02}$ & $791.14$ & $156$ \\ 
58761.66 & $35.93\pm0.21$ & $-0.678\pm0.007$ & $-10.225\substack{+0.005\\ -0.006}$ & $-10.263\substack{+0.004\\ -0.004}$ & $-11.32\substack{+0.02\\ -0.02}$ & $148.43$ & $94$ \\ 
58765.31 & $38.24\pm0.19$ & $-0.677\pm0.006$ & $-10.197\substack{+0.005\\ -0.004}$ & $-10.234\substack{+0.003\\ -0.003}$ & $-11.31\substack{+0.02\\ -0.02}$ & $130.06$ & $113$ \\ 
58767.60 & $40.33\pm0.22$ & $-0.668\pm0.007$ & $-10.170\substack{+0.004\\ -0.005}$ & $-10.198\substack{+0.002\\ -0.004}$ & $-11.40\substack{+0.03\\ -0.03}$ & $151.45$ & $113$ \\ 
58777.69 & $36.52\pm0.19$ & $-0.661\pm0.006$ & $-10.211\substack{+0.005\\ -0.005}$ & $-10.232\substack{+0.003\\ -0.004}$ & $-11.56\substack{+0.03\\ -0.04}$ & $102.02$ & $126$ \\ 
58779.17 & $35.48\pm0.17$ & $-0.659\pm0.006$ & $-10.223\substack{+0.004\\ -0.004}$ & $-10.243\substack{+0.003\\ -0.003}$ & $-11.60\substack{+0.03\\ -0.04}$ & $145.54$ & $106$ \\ 
58781.20 & $31.93\pm0.21$ & $-0.684\pm0.008$ & $-10.277\substack{+0.006\\ -0.007}$ & $-10.321\substack{+0.005\\ -0.005}$ & $-11.31\substack{+0.01\\ -0.03}$ & $159.25$ & $145$ \\ 
58783.30 & $33.08\pm0.21$ & $-0.661\pm0.008$ & $-10.246\substack{+0.006\\ -0.007}$ & $-10.268\substack{+0.005\\ -0.005}$ & $-11.59\substack{+0.04\\ -0.05}$ & $217.45$ & $152$ \\ 
58785.09 & $35.45\pm0.25$ & $-0.682\pm0.009$ & $-10.231\substack{+0.007\\ -0.007}$ & $-10.273\substack{+0.005\\ -0.005}$ & $-11.28\substack{+0.03\\ -0.03}$ & $96.27$ & $82$ \\ 
58786.96 & $36.65\pm0.23$ & $-0.662\pm0.008$ & $-10.210\substack{+0.006\\ -0.006}$ & $-10.233\substack{+0.004\\ -0.004}$ & $-11.53\substack{+0.04\\ -0.04}$ & $142.54$ & $100$ \\ 
58789.28 & $26.50\pm0.15$ & $-0.650\pm0.007$ & $-10.346\substack{+0.005\\ -0.005}$ & $-10.359\substack{+0.004\\ -0.004}$ & $-11.96\substack{+0.07\\ -0.08}$ & $111.64$ & $99$ \\ 
58791.61 & $30.29\pm0.20$ & $-0.646\pm0.008$ & $-10.286\substack{+0.006\\ -0.006}$ & $-10.295\substack{+0.004\\ -0.004}$ & $-12.08\substack{+0.11\\ -0.15}$ & $91.76$ & $87$ \\ 
58793.60 & $29.81\pm0.21$ & $-0.658\pm0.008$ & $-10.297\substack{+0.007\\ -0.007}$ & $-10.316\substack{+0.005\\ -0.005}$ & $-11.71\substack{+0.06\\ -0.06}$ & $113.78$ & $83$ \\ 
58794.80 & $33.84\pm0.25$ & $-0.672\pm0.009$ & $-10.247\substack{+0.007\\ -0.007}$ & $-10.280\substack{+0.004\\ -0.006}$ & $-11.42\substack{+0.04\\ -0.03}$ & $87.03$ & $75$ \\ 
58800.52 & $35.17\pm0.24$ & $-0.670\pm0.008$ & $-10.205\substack{+0.006\\ -0.006}$ & $-10.228\substack{+0.004\\ -0.004}$ & $-11.54\substack{+0.04\\ -0.05}$ & $177.22$ & $156$ \\ 
58801.97 & $37.95\pm0.23$ & $-0.660\pm0.007$ & $-10.175\substack{+0.006\\ -0.006}$ & $-10.192\substack{+0.004\\ -0.004}$ & $-11.64\substack{+0.05\\ -0.06}$ & $120.63$ & $114$ \\ 
58805.13 & $33.70\pm0.19$ & $-0.667\pm0.007$ & $-10.229\substack{+0.005\\ -0.006}$ & $-10.252\substack{+0.004\\ -0.004}$ & $-11.54\substack{+0.04\\ -0.04}$ & $163.50$ & $143$ \\ 
58807.45 & $39.54\pm0.23$ & $-0.676\pm0.007$ & $-10.163\substack{+0.007\\ -0.006}$ & $-10.195\substack{+0.005\\ -0.004}$ & $-11.33\substack{+0.03\\ -0.03}$ & $223.53$ & $156$ \\ 
58808.87 & $31.72\pm0.22$ & $-0.684\pm0.008$ & $-10.261\substack{+0.008\\ -0.007}$ & $-10.301\substack{+0.006\\ -0.006}$ & $-11.34\substack{+0.03\\ -0.03}$ & $151.72$ & $147$ \\ 
58810.94 & $30.14\pm0.25$ & $-0.682\pm0.010$ & $-10.281\substack{+0.008\\ -0.008}$ & $-10.316\substack{+0.006\\ -0.006}$ & $-11.43\substack{+0.04\\ -0.03}$ & $113.09$ & $85$ \\ 
58811.00 & $30.43\pm0.26$ & $-0.648\pm0.010$ & $-10.274\substack{+0.008\\ -0.008}$ & $-10.299\substack{+0.006\\ -0.006}$ & $-11.56\substack{+0.05\\ -0.06}$ & $86.19$ & $80$ \\ 
58812.59 & $30.23\pm0.23$ & $-0.671\pm0.009$ & $-10.296\substack{+0.007\\ -0.007}$ & $-10.327\substack{+0.004\\ -0.005}$ & $-11.49\substack{+0.04\\ -0.04}$ & $86.42$ & $76$ \\ 
58815.65 & $26.05\pm0.17$ & $-0.643\pm0.008$ & $-10.351\substack{+0.006\\ -0.006}$ & $-10.358\substack{+0.004\\ -0.004}$ & $-12.34\substack{+0.16\\ -0.27}$ & $110.54$ & $90$ \\ 
58817.45 & $30.79\pm0.18$ & $-0.649\pm0.007$ & $-10.281\substack{+0.005\\ -0.005}$ & $-10.293\substack{+0.004\\ -0.004}$ & $-11.94\substack{+0.07\\ -0.09}$ & $136.83$ & $94$ \\ 
58819.36 & $33.96\pm0.21$ & $-0.681\pm0.008$ & $-10.250\substack{+0.006\\ -0.006}$ & $-10.290\substack{+0.004\\ -0.004}$ & $-11.32\substack{+0.02\\ -0.02}$ & $117.09$ & $84$ \\ 
58821.49 & $31.08\pm0.18$ & $-0.668\pm0.007$ & $-10.283\substack{+0.004\\ -0.005}$ & $-10.312\substack{+0.002\\ -0.004}$ & $-11.51\substack{+0.03\\ -0.03}$ & $115.89$ & $104$ \\ 
58823.49 & $35.41\pm0.20$ & $-0.660\pm0.007$ & $-10.224\substack{+0.005\\ -0.005}$ & $-10.246\substack{+0.004\\ -0.004}$ & $-11.58\substack{+0.04\\ -0.04}$ & $88.10$ & $93$ \\ 
58825.62 & $30.66\pm0.19$ & $-0.658\pm0.007$ & $-10.286\substack{+0.005\\ -0.005}$ & $-10.306\substack{+0.004\\ -0.004}$ & $-11.69\substack{+0.04\\ -0.06}$ & $103.79$ & $92$ \\ 
58827.62 & $28.77\pm0.18$ & $-0.659\pm0.007$ & $-10.314\substack{+0.006\\ -0.006}$ & $-10.335\substack{+0.004\\ -0.004}$ & $-11.69\substack{+0.04\\ -0.05}$ & $128.16$ & $100$ \\ 
58829.88 & $29.36\pm0.20$ & $-0.662\pm0.008$ & $-10.297\substack{+0.007\\ -0.006}$ & $-10.321\substack{+0.005\\ -0.004}$ & $-11.61\substack{+0.04\\ -0.04}$ & $92.53$ & $98$ \\ 
58832.01 & $31.05\pm0.25$ & $-0.662\pm0.010$ & $-10.255\substack{+0.005\\ -0.011}$ & $-10.278\substack{+0.003\\ -0.008}$ & $-11.58\substack{+0.05\\ -0.07}$ & $82.93$ & $101$ \\ 
58833.86 & $37.91\pm0.35$ & $-0.646\pm0.011$ & $-10.168\substack{+0.009\\ -0.006}$ & $-10.179\substack{+0.006\\ -0.003}$ & $-11.80\substack{+0.11\\ -0.17}$ & $58.83$ & $65$ \\ 
58835.88 & $36.85\pm0.28$ & $-0.665\pm0.009$ & $-10.172\substack{+0.007\\ -0.006}$ & $-10.193\substack{+0.004\\ -0.003}$ & $-11.52\substack{+0.05\\ -0.06}$ & $93.96$ & $106$ \\ 
58836.01 & $37.04\pm0.29$ & $-0.661\pm0.009$ & $-10.177\substack{+0.007\\ -0.008}$ & $-10.195\substack{+0.004\\ -0.006}$ & $-11.61\substack{+0.07\\ -0.08}$ & $114.70$ & $99$ \\ 
58844.21 & $37.83\pm0.24$ & $-0.696\pm0.008$ & $-10.180\substack{+0.005\\ -0.006}$ & $-10.232\substack{+0.004\\ -0.005}$ & $-11.14\substack{+0.02\\ -0.02}$ & $112.55$ & $79$ \\ 
58847.69 & $37.79\pm0.21$ & $-0.667\pm0.007$ & $-10.170\substack{+0.005\\ -0.005}$ & $-10.194\substack{+0.003\\ -0.004}$ & $-11.48\substack{+0.03\\ -0.03}$ & $120.02$ & $96$ \\ 
58849.83 & $31.74\pm0.20$ & $-0.661\pm0.008$ & $-10.234\substack{+0.006\\ -0.006}$ & $-10.247\substack{+0.004\\ -0.004}$ & $-11.79\substack{+0.07\\ -0.09}$ & $115.88$ & $94$ \\ 
58851.80 & $31.04\pm0.24$ & $-0.646\pm0.009$ & $-10.245\substack{+0.007\\ -0.007}$ & $-10.263\substack{+0.005\\ -0.005}$ & $-11.66\substack{+0.06\\ -0.07}$ & $322.98$ & $138$ \\ 
58853.64 & $30.83\pm0.28$ & $-0.638\pm0.011$ & $-10.242\substack{+0.010\\ -0.009}$ & $-10.258\substack{+0.007\\ -0.006}$ & $-11.74\substack{+0.09\\ -0.11}$ & $81.11$ & $91$ \\ 
58855.80 & $34.45\pm0.22$ & $-0.650\pm0.008$ & $-10.200\substack{+0.006\\ -0.006}$ & $-10.218\substack{+0.004\\ -0.004}$ & $-11.63\substack{+0.06\\ -0.06}$ & $94.73$ & $111$ \\ 
58857.80 & $32.53\pm0.21$ & $-0.645\pm0.008$ & $-10.223\substack{+0.006\\ -0.007}$ & $-10.236\substack{+0.004\\ -0.004}$ & $-11.81\substack{+0.08\\ -0.09}$ & $114.12$ & $106$ \\ 
58859.80 & $30.25\pm0.26$ & $-0.616\pm0.010$ & $-10.253\substack{+0.004\\ -0.003}$ & $-10.254\substack{+0.003\\ -0.003}$ & $-16.00\substack{+3.06\\ -0.00}$ & $94.35$ & $73$ \\ 
58861.80 & $30.19\pm0.20$ & $-0.626\pm0.008$ & $-10.259\substack{+0.003\\ -0.003}$ & $-10.260\substack{+0.002\\ -0.003}$ & $-16.00\substack{+2.49\\ -0.00}$ & $108.12$ & $93$ \\ 
58863.61 & $25.11\pm0.16$ & $-0.631\pm0.007$ & $-10.341\substack{+0.005\\ -0.005}$ & $-10.351\substack{+0.004\\ -0.004}$ & $-12.04\substack{+0.09\\ -0.08}$ & $120.57$ & $106$ \\ 
58865.22 & $29.88\pm0.18$ & $-0.653\pm0.007$ & $-10.280\substack{+0.006\\ -0.006}$ & $-10.301\substack{+0.004\\ -0.004}$ & $-11.65\substack{+0.04\\ -0.05}$ & $84.90$ & $107$ \\ 
58866.71 & $34.00\pm0.19$ & $-0.652\pm0.007$ & $-10.216\substack{+0.005\\ -0.005}$ & $-10.241\substack{+0.003\\ -0.003}$ & $-11.51\substack{+0.03\\ -0.03}$ & $239.04$ & $144$ \\ 
58868.85 & $32.21\pm0.25$ & $-0.687\pm0.009$ & $-10.253\substack{+0.007\\ -0.007}$ & $-10.293\substack{+0.005\\ -0.005}$ & $-11.33\substack{+0.03\\ -0.03}$ & $68.93$ & $71$ \\ 
58870.84 & $36.52\pm0.17$ & $-0.655\pm0.006$ & $-10.183\substack{+0.004\\ -0.004}$ & $-10.200\substack{+0.003\\ -0.003}$ & $-11.64\substack{+0.04\\ -0.04}$ & $169.63$ & $114$ \\ 
58871.67 & $33.61\pm0.31$ & $-0.667\pm0.011$ & $-10.216\substack{+0.009\\ -0.009}$ & $-10.239\substack{+0.007\\ -0.006}$ & $-11.52\substack{+0.06\\ -0.07}$ & $65.08$ & $79$ \\ 
58873.22 & $34.76\pm0.17$ & $-0.668\pm0.006$ & $-10.216\substack{+0.004\\ -0.004}$ & $-10.242\substack{+0.003\\ -0.003}$ & $-11.48\substack{+0.03\\ -0.03}$ & $133.75$ & $130$ \\ 
58875.16 & $30.35\pm0.16$ & $-0.643\pm0.006$ & $-10.271\substack{+0.005\\ -0.005}$ & $-10.288\substack{+0.003\\ -0.003}$ & $-11.75\substack{+0.05\\ -0.05}$ & $116.25$ & $101$ \\ 
58876.97 & $27.07\pm0.16$ & $-0.657\pm0.007$ & $-10.322\substack{+0.005\\ -0.005}$ & $-10.342\substack{+0.004\\ -0.004}$ & $-11.72\substack{+0.04\\ -0.05}$ & $130.48$ & $122$ \\ 
58877.68 & $30.98\pm0.23$ & $-0.666\pm0.009$ & $-10.267\substack{+0.007\\ -0.007}$ & $-10.295\substack{+0.005\\ -0.005}$ & $-11.49\substack{+0.04\\ -0.04}$ & $105.87$ & $101$ \\ 
58879.49 & $27.59\pm0.28$ & $-0.635\pm0.012$ & $-10.295\substack{+0.010\\ -0.010}$ & $-10.304\substack{+0.007\\ -0.007}$ & $-12.10\substack{+0.18\\ -0.30}$ & $72.92$ & $60$ \\ 
58884.72 & $27.47\pm0.19$ & $-0.639\pm0.008$ & $-10.327\substack{+0.007\\ -0.006}$ & $-10.330\substack{+0.004\\ -0.005}$ & $-12.85\substack{+0.45\\ -3.15}$ & $97.16$ & $102$ \\ 
58887.53 & $35.06\pm0.23$ & $-0.657\pm0.008$ & $-10.227\substack{+0.006\\ -0.006}$ & $-10.246\substack{+0.004\\ -0.004}$ & $-11.65\substack{+0.05\\ -0.06}$ & $130.67$ & $100$ \\ 
58889.57 & $32.17\pm0.18$ & $-0.673\pm0.007$ & $-10.233\substack{+0.005\\ -0.005}$ & $-10.259\substack{+0.004\\ -0.004}$ & $-11.51\substack{+0.03\\ -0.03}$ & $172.75$ & $151$ \\ 
58891.63 & $40.44\pm0.22$ & $-0.673\pm0.007$ & $-10.171\substack{+0.005\\ -0.006}$ & $-10.204\substack{+0.003\\ -0.004}$ & $-11.33\substack{+0.03\\ -0.02}$ & $138.94$ & $109$ \\ 
58893.40 & $36.25\pm0.23$ & $-0.686\pm0.008$ & $-10.197\substack{+0.006\\ -0.006}$ & $-10.243\substack{+0.004\\ -0.004}$ & $-11.21\substack{+0.02\\ -0.02}$ & $105.56$ & $81$ \\ 
58902.65 & $31.50\pm0.23$ & $-0.719\pm0.009$ & $-10.268\substack{+0.007\\ -0.007}$ & $-10.346\substack{+0.005\\ -0.005}$ & $-11.06\substack{+0.02\\ -0.02}$ & $89.08$ & $66$ \\ 
58903.97 & $34.05\pm0.24$ & $-0.699\pm0.009$ & $-10.227\substack{+0.006\\ -0.007}$ & $-10.284\substack{+0.005\\ -0.005}$ & $-11.15\substack{+0.02\\ -0.02}$ & $100.79$ & $69$ \\ 
58905.59 & $43.07\pm0.28$ & $-0.697\pm0.008$ & $-10.117\substack{+0.006\\ -0.006}$ & $-10.175\substack{+0.004\\ -0.004}$ & $-11.03\substack{+0.02\\ -0.02}$ & $104.81$ & $71$ \\ 
58909.60 & $32.46\pm0.21$ & $-0.647\pm0.008$ & $-10.236\substack{+0.007\\ -0.007}$ & $-10.260\substack{+0.005\\ -0.005}$ & $-11.53\substack{+0.04\\ -0.04}$ & $163.00$ & $141$ \\ 
58910.86 & $34.40\pm0.28$ & $-0.635\pm0.010$ & $-10.198\substack{+0.008\\ -0.008}$ & $-10.211\substack{+0.006\\ -0.006}$ & $-11.75\substack{+0.09\\ -0.11}$ & $117.94$ & $78$ \\ 
58911.31 & $34.44\pm0.26$ & $-0.650\pm0.009$ & $-10.195\substack{+0.007\\ -0.008}$ & $-10.204\substack{+0.005\\ -0.005}$ & $-11.97\substack{+0.12\\ -0.18}$ & $78.58$ & $77$ \\ 
58915.75 & $25.96\pm0.20$ & $-0.638\pm0.009$ & $-10.329\substack{+0.008\\ -0.007}$ & $-10.346\substack{+0.005\\ -0.005}$ & $-11.81\substack{+0.07\\ -0.08}$ & $117.02$ & $83$ \\ 
58917.39 & $25.47\pm0.27$ & $-0.651\pm0.013$ & $-10.343\substack{+0.005\\ -0.006}$ & $-10.345\substack{+0.004\\ -0.006}$ & $-16.00\substack{+3.15\\ -0.00}$ & $73.85$ & $59$ \\ 
58919.20 & $32.67\pm0.21$ & $-0.632\pm0.008$ & $-10.224\substack{+0.005\\ -0.005}$ & $-10.226\substack{+0.003\\ -0.004}$ & $-13.13\substack{+0.67\\ -2.88}$ & $124.11$ & $82$ \\ 
58921.27 & $34.01\pm0.22$ & $-0.657\pm0.008$ & $-10.197\substack{+0.007\\ -0.005}$ & $-10.221\substack{+0.005\\ -0.003}$ & $-11.50\substack{+0.04\\ -0.05}$ & $119.00$ & $96$ \\ 
58923.07 & $33.86\pm0.22$ & $-0.649\pm0.008$ & $-10.223\substack{+0.006\\ -0.006}$ & $-10.241\substack{+0.004\\ -0.004}$ & $-11.67\substack{+0.05\\ -0.06}$ & $83.78$ & $84$ \\ 
58929.79 & $34.59\pm0.22$ & $-0.647\pm0.008$ & $-10.197\substack{+0.006\\ -0.006}$ & $-10.216\substack{+0.004\\ -0.004}$ & $-11.59\substack{+0.05\\ -0.05}$ & $91.96$ & $86$ \\ 
58931.55 & $35.20\pm0.25$ & $-0.651\pm0.008$ & $-10.197\substack{+0.006\\ -0.007}$ & $-10.211\substack{+0.004\\ -0.004}$ & $-11.72\substack{+0.07\\ -0.08}$ & $100.32$ & $78$ \\ 
58933.41 & $33.79\pm0.21$ & $-0.634\pm0.007$ & $-10.203\substack{+0.005\\ -0.006}$ & $-10.212\substack{+0.004\\ -0.004}$ & $-12.00\substack{+0.10\\ -0.14}$ & $104.22$ & $81$ \\ 
58935.42 & $33.05\pm0.21$ & $-0.630\pm0.007$ & $-10.211\substack{+0.006\\ -0.006}$ & $-10.216\substack{+0.004\\ -0.004}$ & $-12.31\substack{+0.19\\ -0.35}$ & $138.16$ & $80$ \\ 
58937.60 & $28.42\pm0.22$ & $-0.637\pm0.009$ & $-10.280\substack{+0.008\\ -0.007}$ & $-10.288\substack{+0.005\\ -0.005}$ & $-12.17\substack{+0.16\\ -0.28}$ & $91.27$ & $82$ \\ 
58939.87 & $32.30\pm0.17$ & $-0.630\pm0.006$ & $-10.233\substack{+0.004\\ -0.004}$ & $-10.243\substack{+0.003\\ -0.003}$ & $-11.95\substack{+0.07\\ -0.08}$ & $153.40$ & $146$ \\ 
58941.71 & $30.96\pm0.24$ & $-0.631\pm0.009$ & $-10.248\substack{+0.003\\ -0.003}$ & $-10.249\substack{+0.003\\ -0.003}$ & $-16.00\substack{+2.91\\ -0.00}$ & $118.62$ & $71$ \\ 
58943.49 & $33.33\pm0.24$ & $-0.640\pm0.009$ & $-10.219\substack{+0.007\\ -0.007}$ & $-10.228\substack{+0.005\\ -0.005}$ & $-12.00\substack{+0.12\\ -0.17}$ & $98.96$ & $75$ \\ 
58945.04 & $37.72\pm0.37$ & $-0.631\pm0.012$ & $-10.151\substack{+0.009\\ -0.010}$ & $-10.160\substack{+0.006\\ -0.007}$ & $-11.92\substack{+0.16\\ -0.24}$ & $63.63$ & $57$ \\ 
58953.41 & $40.70\pm0.26$ & $-0.680\pm0.008$ & $-10.171\substack{+0.006\\ -0.006}$ & $-10.211\substack{+0.004\\ -0.004}$ & $-11.24\substack{+0.02\\ -0.02}$ & $214.71$ & $154$ \\ 
58955.66 & $49.73\pm0.30$ & $-0.690\pm0.007$ & $-10.088\substack{+0.006\\ -0.005}$ & $-10.138\substack{+0.005\\ -0.003}$ & $-11.07\substack{+0.01\\ -0.02}$ & $124.02$ & $91$ \\ 
58957.37 & $50.37\pm0.26$ & $-0.691\pm0.006$ & $-10.083\substack{+0.005\\ -0.005}$ & $-10.133\substack{+0.003\\ -0.004}$ & $-11.05\substack{+0.01\\ -0.02}$ & $182.38$ & $156$ \\ 
58963.86 & $44.86\pm0.28$ & $-0.678\pm0.008$ & $-10.111\substack{+0.006\\ -0.006}$ & $-10.148\substack{+0.004\\ -0.005}$ & $-11.21\substack{+0.03\\ -0.03}$ & $173.15$ & $160$ \\ 
58969.26 & $47.15\pm0.29$ & $-0.673\pm0.008$ & $-10.065\substack{+0.006\\ -0.005}$ & $-10.113\substack{+0.004\\ -0.004}$ & $-11.06\substack{+0.02\\ -0.02}$ & $91.77$ & $79$ \\ 
58971.20 & $41.62\pm0.27$ & $-0.660\pm0.008$ & $-10.122\substack{+0.006\\ -0.005}$ & $-10.153\substack{+0.004\\ -0.003}$ & $-11.30\substack{+0.03\\ -0.04}$ & $87.61$ & $81$ \\ 
58973.33 & $41.04\pm0.21$ & $-0.678\pm0.006$ & $-10.131\substack{+0.004\\ -0.004}$ & $-10.169\substack{+0.003\\ -0.003}$ & $-11.22\substack{+0.02\\ -0.02}$ & $133.93$ & $96$ \\ 
58975.26 & $41.89\pm0.22$ & $-0.695\pm0.006$ & $-10.133\substack{+0.004\\ -0.004}$ & $-10.203\substack{+0.003\\ -0.003}$ & $-10.97\substack{+0.01\\ -0.01}$ & $297.15$ & $156$ \\ 
58977.26 & $44.17\pm0.21$ & $-0.666\pm0.006$ & $-10.106\substack{+0.004\\ -0.004}$ & $-10.137\substack{+0.003\\ -0.003}$ & $-11.29\substack{+0.02\\ -0.02}$ & $92.29$ & $108$ \\ 
58979.50 & $49.18\pm0.33$ & $-0.680\pm0.008$ & $-10.062\substack{+0.006\\ -0.006}$ & $-10.102\substack{+0.004\\ -0.004}$ & $-11.13\substack{+0.02\\ -0.03}$ & $123.48$ & $78$ \\ 
58981.42 & $37.67\pm0.21$ & $-0.709\pm0.007$ & $-10.188\substack{+0.005\\ -0.005}$ & $-10.259\substack{+0.003\\ -0.004}$ & $-11.02\substack{+0.01\\ -0.01}$ & $142.08$ & $88$ \\ 
58983.35 & $37.98\pm0.22$ & $-0.722\pm0.007$ & $-10.187\substack{+0.005\\ -0.005}$ & $-10.264\substack{+0.004\\ -0.004}$ & $-10.98\substack{+0.01\\ -0.01}$ & $185.40$ & $86$ \\ 
58985.26 & $41.40\pm0.24$ & $-0.699\pm0.007$ & $-10.150\substack{+0.005\\ -0.006}$ & $-10.201\substack{+0.004\\ -0.005}$ & $-11.12\substack{+0.02\\ -0.02}$ & $117.59$ & $103$ \\ 
58987.26 & $38.05\pm0.36$ & $-0.669\pm0.012$ & $-10.169\substack{+0.009\\ -0.011}$ & $-10.212\substack{+0.006\\ -0.009}$ & $-11.21\substack{+0.04\\ -0.03}$ & $106.50$ & $65$ \\ 
58994.55 & $42.34\pm0.23$ & $-0.695\pm0.007$ & $-10.151\substack{+0.005\\ -0.005}$ & $-10.206\substack{+0.004\\ -0.004}$ & $-11.09\substack{+0.01\\ -0.02}$ & $154.18$ & $117$ \\ 
59008.58 & $37.23\pm0.20$ & $-0.652\pm0.006$ & $-10.199\substack{+0.005\\ -0.005}$ & $-10.213\substack{+0.003\\ -0.004}$ & $-11.77\substack{+0.06\\ -0.07}$ & $103.43$ & $120$ \\ 
59014.56 & $37.82\pm0.23$ & $-0.694\pm0.008$ & $-10.208\substack{+0.005\\ -0.006}$ & $-10.262\substack{+0.004\\ -0.005}$ & $-11.15\substack{+0.02\\ -0.02}$ & $201.26$ & $118$ \\ 
59022.87 & $34.61\pm0.33$ & $-0.718\pm0.012$ & $-10.254\substack{+0.010\\ -0.010}$ & $-10.331\substack{+0.008\\ -0.008}$ & $-11.05\substack{+0.02\\ -0.02}$ & $485.02$ & $156$ \\ 
59025.00 & $40.23\pm0.37$ & $-0.702\pm0.011$ & $-10.188\substack{+0.009\\ -0.009}$ & $-10.260\substack{+0.007\\ -0.007}$ & $-11.01\substack{+0.02\\ -0.02}$ & $216.31$ & $135$ \\ 
59027.00 & $48.45\pm0.39$ & $-0.687\pm0.010$ & $-10.098\substack{+0.008\\ -0.008}$ & $-10.145\substack{+0.006\\ -0.006}$ & $-11.10\substack{+0.03\\ -0.03}$ & $264.31$ & $151$ \\ 
59028.72 & $44.27\pm0.23$ & $-0.669\pm0.006$ & $-10.131\substack{+0.006\\ -0.004}$ & $-10.160\substack{+0.005\\ -0.003}$ & $-11.34\substack{+0.02\\ -0.03}$ & $143.32$ & $137$ \\ 
59029.88 & $37.93\pm0.32$ & $-0.677\pm0.010$ & $-10.198\substack{+0.009\\ -0.009}$ & $-10.227\substack{+0.006\\ -0.006}$ & $-11.41\substack{+0.05\\ -0.05}$ & $66.12$ & $72$ \\ 
59034.31 & $37.54\pm0.27$ & $-0.684\pm0.009$ & $-10.179\substack{+0.007\\ -0.007}$ & $-10.218\substack{+0.005\\ -0.005}$ & $-11.26\substack{+0.03\\ -0.03}$ & $95.52$ & $74$ \\ 
59036.63 & $37.86\pm0.31$ & $-0.694\pm0.010$ & $-10.178\substack{+0.008\\ -0.008}$ & $-10.224\substack{+0.005\\ -0.006}$ & $-11.19\substack{+0.03\\ -0.03}$ & $62.66$ & $67$ \\ 
59038.89 & $43.30\pm0.23$ & $-0.706\pm0.007$ & $-10.136\substack{+0.004\\ -0.004}$ & $-10.203\substack{+0.003\\ -0.003}$ & $-10.99\substack{+0.01\\ -0.01}$ & $254.26$ & $115$ \\ 
59042.55 & $43.13\pm0.30$ & $-0.696\pm0.008$ & $-10.152\substack{+0.007\\ -0.006}$ & $-10.208\substack{+0.005\\ -0.004}$ & $-11.08\substack{+0.02\\ -0.02}$ & $138.46$ & $120$ \\ 
59043.95 & $36.26\pm0.28$ & $-0.705\pm0.009$ & $-10.221\substack{+0.007\\ -0.007}$ & $-10.286\substack{+0.005\\ -0.005}$ & $-11.09\substack{+0.02\\ -0.02}$ & $118.70$ & $70$ \\ 
59044.01 & $35.41\pm0.25$ & $-0.703\pm0.009$ & $-10.231\substack{+0.007\\ -0.007}$ & $-10.294\substack{+0.005\\ -0.005}$ & $-11.11\substack{+0.02\\ -0.02}$ & $112.84$ & $76$ \\ 
59053.90 & $41.14\pm0.22$ & $-0.691\pm0.006$ & $-10.143\substack{+0.005\\ -0.005}$ & $-10.195\substack{+0.003\\ -0.003}$ & $-11.11\substack{+0.01\\ -0.02}$ & $105.45$ & $105$ \\ 
59056.47 & $36.52\pm0.22$ & $-0.710\pm0.007$ & $-10.220\substack{+0.005\\ -0.005}$ & $-10.292\substack{+0.004\\ -0.004}$ & $-11.05\substack{+0.01\\ -0.01}$ & $219.85$ & $110$ \\ 
59060.66 & $42.01\pm0.23$ & $-0.691\pm0.007$ & $-10.153\substack{+0.005\\ -0.005}$ & $-10.204\substack{+0.003\\ -0.004}$ & $-11.12\substack{+0.02\\ -0.02}$ & $130.20$ & $94$ \\ 
59062.59 & $46.54\pm0.27$ & $-0.683\pm0.007$ & $-10.106\substack{+0.005\\ -0.006}$ & $-10.149\substack{+0.003\\ -0.004}$ & $-11.15\substack{+0.02\\ -0.02}$ & $130.45$ & $86$ \\ 
59064.59 & $42.68\pm0.24$ & $-0.676\pm0.007$ & $-10.141\substack{+0.005\\ -0.005}$ & $-10.177\substack{+0.004\\ -0.004}$ & $-11.26\substack{+0.02\\ -0.02}$ & $104.26$ & $102$ \\ 
59066.56 & $44.45\pm0.25$ & $-0.682\pm0.007$ & $-10.125\substack{+0.005\\ -0.005}$ & $-10.167\substack{+0.004\\ -0.004}$ & $-11.18\substack{+0.02\\ -0.02}$ & $123.82$ & $89$ \\ 
59070.92 & $43.07\pm0.27$ & $-0.680\pm0.008$ & $-10.137\substack{+0.008\\ -0.006}$ & $-10.178\substack{+0.007\\ -0.004}$ & $-11.21\substack{+0.02\\ -0.02}$ & $119.38$ & $108$ \\ 
59072.73 & $45.33\pm0.29$ & $-0.672\pm0.008$ & $-10.112\substack{+0.006\\ -0.008}$ & $-10.144\substack{+0.004\\ -0.006}$ & $-11.28\substack{+0.03\\ -0.03}$ & $88.49$ & $124$ \\ 
59074.96 & $45.85\pm0.27$ & $-0.691\pm0.007$ & $-10.115\substack{+0.005\\ -0.005}$ & $-10.166\substack{+0.004\\ -0.004}$ & $-11.08\substack{+0.02\\ -0.02}$ & $185.78$ & $153$ \\ 
59076.91 & $40.47\pm0.21$ & $-0.693\pm0.006$ & $-10.170\substack{+0.005\\ -0.004}$ & $-10.222\substack{+0.003\\ -0.004}$ & $-11.13\substack{+0.02\\ -0.01}$ & $140.29$ & $99$ \\ 
59077.97 & $38.39\pm0.22$ & $-0.679\pm0.007$ & $-10.187\substack{+0.005\\ -0.005}$ & $-10.226\substack{+0.004\\ -0.004}$ & $-11.27\substack{+0.02\\ -0.02}$ & $125.54$ & $89$ \\ 
59080.91 & $37.66\pm0.22$ & $-0.673\pm0.007$ & $-10.193\substack{+0.005\\ -0.005}$ & $-10.226\substack{+0.004\\ -0.004}$ & $-11.35\substack{+0.03\\ -0.03}$ & $109.95$ & $90$ \\ 
59082.88 & $40.06\pm0.31$ & $-0.680\pm0.010$ & $-10.170\substack{+0.008\\ -0.007}$ & $-10.210\substack{+0.006\\ -0.005}$ & $-11.24\substack{+0.03\\ -0.03}$ & $70.67$ & $72$ \\ 
59083.01 & $41.38\pm0.26$ & $-0.679\pm0.008$ & $-10.155\substack{+0.006\\ -0.006}$ & $-10.193\substack{+0.004\\ -0.004}$ & $-11.25\substack{+0.02\\ -0.03}$ & $124.64$ & $80$ \\ 
59084.93 & $30.54\pm0.24$ & $-0.673\pm0.010$ & $-10.285\substack{+0.009\\ -0.008}$ & $-10.319\substack{+0.006\\ -0.006}$ & $-11.44\substack{+0.04\\ -0.04}$ & $153.90$ & $152$ \\ 
59088.99 & $33.98\pm0.27$ & $-0.677\pm0.010$ & $-10.241\substack{+0.007\\ -0.008}$ & $-10.278\substack{+0.004\\ -0.006}$ & $-11.34\substack{+0.04\\ -0.03}$ & $196.15$ & $154$ \\ 
59093.97 & $23.69\pm0.30$ & $-0.668\pm0.015$ & $-10.408\substack{+0.012\\ -0.019}$ & $-10.419\substack{+0.008\\ -0.014}$ & $-12.09\substack{+0.17\\ -0.29}$ & $81.64$ & $62$ \\ 
59095.94 & $36.97\pm0.24$ & $-0.675\pm0.008$ & $-10.202\substack{+0.006\\ -0.006}$ & $-10.237\substack{+0.005\\ -0.004}$ & $-11.33\substack{+0.03\\ -0.03}$ & $87.67$ & $81$ \\ 
59101.27 & $42.81\pm0.26$ & $-0.689\pm0.007$ & $-10.105\substack{+0.005\\ -0.006}$ & $-10.146\substack{+0.004\\ -0.004}$ & $-11.17\substack{+0.02\\ -0.02}$ & $102.33$ & $114$ \\ 
59103.86 & $48.66\pm0.27$ & $-0.681\pm0.007$ & $-10.048\substack{+0.005\\ -0.005}$ & $-10.084\substack{+0.003\\ -0.004}$ & $-11.17\substack{+0.02\\ -0.02}$ & $205.75$ & $145$ \\ 
59105.31 & $41.84\pm0.29$ & $-0.672\pm0.009$ & $-10.111\substack{+0.008\\ -0.008}$ & $-10.138\substack{+0.006\\ -0.006}$ & $-11.34\substack{+0.04\\ -0.04}$ & $221.88$ & $151$ \\ 
59107.95 & $39.23\pm0.26$ & $-0.647\pm0.008$ & $-10.139\substack{+0.007\\ -0.007}$ & $-10.148\substack{+0.004\\ -0.004}$ & $-11.88\substack{+0.11\\ -0.14}$ & $104.15$ & $104$ \\ 
59109.31 & $31.13\pm0.25$ & $-0.658\pm0.010$ & $-10.232\substack{+0.007\\ -0.011}$ & $-10.247\substack{+0.004\\ -0.010}$ & $-11.76\substack{+0.09\\ -0.06}$ & $127.00$ & $111$ \\ 
59116.29 & $26.43\pm0.18$ & $-0.648\pm0.008$ & $-10.338\substack{+0.007\\ -0.007}$ & $-10.349\substack{+0.004\\ -0.005}$ & $-12.01\substack{+0.09\\ -0.12}$ & $164.96$ & $93$ \\ 
59118.43 & $26.51\pm0.14$ & $-0.637\pm0.006$ & $-10.333\substack{+0.002\\ -0.002}$ & $-10.335\substack{+0.002\\ -0.002}$ & $-16.00\substack{+2.15\\ -0.00}$ & $265.76$ & $120$ \\ 
59120.59 & $27.56\pm0.18$ & $-0.638\pm0.008$ & $-10.317\substack{+0.004\\ -0.004}$ & $-10.319\substack{+0.003\\ -0.004}$ & $-16.00\substack{+3.00\\ -0.00}$ & $148.19$ & $106$ \\ 
59122.53 & $34.79\pm0.18$ & $-0.642\pm0.006$ & $-10.217\substack{+0.005\\ -0.005}$ & $-10.223\substack{+0.003\\ -0.003}$ & $-12.29\substack{+0.15\\ -0.24}$ & $120.80$ & $106$ \\ 
59124.47 & $27.13\pm0.17$ & $-0.651\pm0.008$ & $-10.328\substack{+0.006\\ -0.006}$ & $-10.342\substack{+0.004\\ -0.004}$ & $-11.91\substack{+0.07\\ -0.09}$ & $99.69$ & $111$ \\ 
59126.20 & $31.12\pm0.29$ & $-0.668\pm0.011$ & $-10.283\substack{+0.009\\ -0.010}$ & $-10.298\substack{+0.006\\ -0.007}$ & $-11.80\substack{+0.10\\ -0.12}$ & $75.68$ & $64$ \\ 
59128.12 & $29.66\pm0.21$ & $-0.651\pm0.008$ & $-10.281\substack{+0.006\\ -0.008}$ & $-10.294\substack{+0.004\\ -0.006}$ & $-11.85\substack{+0.08\\ -0.10}$ & $122.70$ & $115$ \\ 
59129.56 & $32.38\pm0.22$ & $-0.650\pm0.008$ & $-10.251\substack{+0.006\\ -0.006}$ & $-10.263\substack{+0.004\\ -0.004}$ & $-11.87\substack{+0.08\\ -0.10}$ & $103.22$ & $84$ \\ 
59130.75 & $35.28\pm0.25$ & $-0.647\pm0.008$ & $-10.213\substack{+0.007\\ -0.007}$ & $-10.222\substack{+0.004\\ -0.004}$ & $-11.98\substack{+0.11\\ -0.16}$ & $120.51$ & $86$ \\ 
59136.81 & $34.83\pm0.29$ & $-0.652\pm0.010$ & $-10.218\substack{+0.008\\ -0.008}$ & $-10.229\substack{+0.005\\ -0.005}$ & $-11.92\substack{+0.12\\ -0.16}$ & $100.57$ & $71$ \\ 
59138.33 & $35.39\pm0.22$ & $-0.657\pm0.008$ & $-10.214\substack{+0.006\\ -0.006}$ & $-10.232\substack{+0.004\\ -0.004}$ & $-11.65\substack{+0.05\\ -0.06}$ & $113.46$ & $89$ \\ 
59141.04 & $32.09\pm0.22$ & $-0.666\pm0.008$ & $-10.260\substack{+0.007\\ -0.007}$ & $-10.287\substack{+0.005\\ -0.005}$ & $-11.51\substack{+0.04\\ -0.04}$ & $180.49$ & $142$ \\ 
59142.79 & $30.94\pm0.34$ & $-0.666\pm0.013$ & $-10.290\substack{+0.012\\ -0.007}$ & $-10.316\substack{+0.009\\ -0.004}$ & $-11.56\substack{+0.05\\ -0.06}$ & $60.23$ & $69$ \\ 
59144.40 & $31.22\pm0.21$ & $-0.671\pm0.008$ & $-10.274\substack{+0.006\\ -0.006}$ & $-10.305\substack{+0.004\\ -0.004}$ & $-11.45\substack{+0.03\\ -0.03}$ & $124.82$ & $91$ \\ 
59148.93 & $32.93\pm0.23$ & $-0.665\pm0.008$ & $-10.248\substack{+0.007\\ -0.007}$ & $-10.273\substack{+0.005\\ -0.005}$ & $-11.52\substack{+0.04\\ -0.05}$ & $80.05$ & $85$ \\ 
59150.52 & $28.10\pm0.19$ & $-0.669\pm0.008$ & $-10.318\substack{+0.006\\ -0.006}$ & $-10.347\substack{+0.004\\ -0.005}$ & $-11.53\substack{+0.04\\ -0.04}$ & $100.08$ & $82$ \\ 
59151.84 & $31.66\pm0.19$ & $-0.677\pm0.007$ & $-10.270\substack{+0.006\\ -0.007}$ & $-10.307\substack{+0.004\\ -0.006}$ & $-11.38\substack{+0.03\\ -0.02}$ & $93.15$ & $93$ \\ 
59153.87 & $27.93\pm0.18$ & $-0.684\pm0.008$ & $-10.326\substack{+0.006\\ -0.006}$ & $-10.371\substack{+0.004\\ -0.004}$ & $-11.36\substack{+0.02\\ -0.02}$ & $133.09$ & $84$ \\ 
59155.71 & $27.66\pm0.24$ & $-0.688\pm0.010$ & $-10.329\substack{+0.008\\ -0.008}$ & $-10.370\substack{+0.006\\ -0.006}$ & $-11.40\substack{+0.03\\ -0.04}$ & $110.27$ & $67$ \\ 
59157.68 & $30.20\pm0.20$ & $-0.703\pm0.008$ & $-10.299\substack{+0.006\\ -0.006}$ & $-10.363\substack{+0.004\\ -0.005}$ & $-11.18\substack{+0.02\\ -0.02}$ & $182.81$ & $77$ \\ 
59165.69 & $38.01\pm0.33$ & $-0.674\pm0.011$ & $-10.165\substack{+0.009\\ -0.009}$ & $-10.204\substack{+0.006\\ -0.007}$ & $-11.25\substack{+0.04\\ -0.04}$ & $48.40$ & $72$ \\ 
59166.40 & $33.83\pm0.23$ & $-0.692\pm0.008$ & $-10.219\substack{+0.008\\ -0.008}$ & $-10.268\substack{+0.007\\ -0.006}$ & $-11.21\substack{+0.02\\ -0.02}$ & $157.78$ & $149$ \\ 
59170.40 & $32.57\pm0.20$ & $-0.701\pm0.008$ & $-10.238\substack{+0.005\\ -0.006}$ & $-10.296\substack{+0.003\\ -0.005}$ & $-11.16\substack{+0.02\\ -0.01}$ & $191.23$ & $155$ \\ 
59172.72 & $38.56\pm0.31$ & $-0.680\pm0.010$ & $-10.155\substack{+0.008\\ -0.008}$ & $-10.187\substack{+0.006\\ -0.006}$ & $-11.33\substack{+0.04\\ -0.04}$ & $70.89$ & $79$ \\ 
59179.54 & $37.59\pm0.22$ & $-0.664\pm0.007$ & $-10.190\substack{+0.005\\ -0.005}$ & $-10.215\substack{+0.003\\ -0.004}$ & $-11.48\substack{+0.04\\ -0.04}$ & $131.13$ & $88$ \\ 
59181.25 & $31.99\pm0.23$ & $-0.663\pm0.009$ & $-10.260\substack{+0.006\\ -0.006}$ & $-10.283\substack{+0.004\\ -0.004}$ & $-11.57\substack{+0.04\\ -0.05}$ & $108.23$ & $78$ \\ 
59183.48 & $26.97\pm0.19$ & $-0.659\pm0.009$ & $-10.333\substack{+0.007\\ -0.007}$ & $-10.353\substack{+0.005\\ -0.005}$ & $-11.72\substack{+0.05\\ -0.06}$ & $132.23$ & $78$ \\ 
59185.35 & $28.42\pm0.18$ & $-0.658\pm0.008$ & $-10.310\substack{+0.006\\ -0.006}$ & $-10.329\substack{+0.004\\ -0.004}$ & $-11.72\substack{+0.05\\ -0.06}$ & $172.56$ & $81$ \\ 
59187.36 & $29.35\pm0.29$ & $-0.673\pm0.012$ & $-10.309\substack{+0.010\\ -0.010}$ & $-10.328\substack{+0.007\\ -0.007}$ & $-11.74\substack{+0.08\\ -0.10}$ & $70.02$ & $61$ \\ 
59189.60 & $25.62\pm0.26$ & $-0.672\pm0.012$ & $-10.352\substack{+0.009\\ -0.010}$ & $-10.382\substack{+0.007\\ -0.007}$ & $-11.55\substack{+0.05\\ -0.06}$ & $78.63$ & $58$ \\ 
59191.30 & $26.59\pm0.23$ & $-0.678\pm0.010$ & $-10.328\substack{+0.008\\ -0.008}$ & $-10.367\substack{+0.006\\ -0.006}$ & $-11.42\substack{+0.03\\ -0.04}$ & $526.48$ & $150$ \\ 
59192.98 & $33.13\pm0.27$ & $-0.661\pm0.010$ & $-10.236\substack{+0.008\\ -0.010}$ & $-10.259\substack{+0.006\\ -0.007}$ & $-11.57\substack{+0.06\\ -0.07}$ & $119.94$ & $121$ \\ 
59193.11 & $33.44\pm0.29$ & $-0.671\pm0.010$ & $-10.226\substack{+0.008\\ -0.008}$ & $-10.257\substack{+0.006\\ -0.006}$ & $-11.41\substack{+0.04\\ -0.05}$ & $179.34$ & $149$ \\ 
59195.20 & $35.53\pm0.38$ & $-0.677\pm0.013$ & $-10.190\substack{+0.010\\ -0.011}$ & $-10.237\substack{+0.008\\ -0.008}$ & $-11.20\substack{+0.04\\ -0.04}$ & $207.72$ & $131$ \\ 
59213.22 & $28.80\pm0.18$ & $-0.628\pm0.008$ & $-10.259\substack{+0.006\\ -0.006}$ & $-10.266\substack{+0.004\\ -0.004}$ & $-12.13\substack{+0.13\\ -0.19}$ & $112.00$ & $98$ \\ 
59215.07 & $37.59\pm0.18$ & $-0.667\pm0.006$ & $-10.172\substack{+0.004\\ -0.004}$ & $-10.196\substack{+0.003\\ -0.003}$ & $-11.47\substack{+0.03\\ -0.03}$ & $97.51$ & $99$ \\ 
59217.36 & $38.93\pm0.21$ & $-0.670\pm0.007$ & $-10.148\substack{+0.005\\ -0.005}$ & $-10.170\substack{+0.004\\ -0.004}$ & $-11.48\substack{+0.03\\ -0.04}$ & $184.61$ & $138$ \\ 
59219.49 & $28.86\pm0.16$ & $-0.673\pm0.007$ & $-10.278\substack{+0.005\\ -0.005}$ & $-10.305\substack{+0.004\\ -0.004}$ & $-11.54\substack{+0.03\\ -0.03}$ & $161.66$ & $148$ \\ 
59223.62 & $24.67\pm0.28$ & $-0.644\pm0.013$ & $-10.330\substack{+0.011\\ -0.008}$ & $-10.351\substack{+0.008\\ -0.005}$ & $-11.70\substack{+0.07\\ -0.08}$ & $84.93$ & $74$ \\ 
59225.17 & $21.49\pm0.17$ & $-0.648\pm0.010$ & $-10.391\substack{+0.008\\ -0.008}$ & $-10.402\substack{+0.005\\ -0.005}$ & $-12.06\substack{+0.11\\ -0.14}$ & $112.48$ & $73$ \\ 
59226.98 & $19.22\pm0.18$ & $-0.635\pm0.011$ & $-10.436\substack{+0.009\\ -0.009}$ & $-10.454\substack{+0.006\\ -0.006}$ & $-11.87\substack{+0.08\\ -0.10}$ & $83.56$ & $68$ \\ 
59227.05 & $19.73\pm0.24$ & $-0.655\pm0.015$ & $-10.423\substack{+0.012\\ -0.013}$ & $-10.437\substack{+0.008\\ -0.008}$ & $-12.01\substack{+0.14\\ -0.21}$ & $49.65$ & $53$ \\ 
59228.97 & $24.02\pm0.16$ & $-0.666\pm0.008$ & $-10.350\substack{+0.007\\ -0.005}$ & $-10.378\substack{+0.005\\ -0.004}$ & $-11.58\substack{+0.04\\ -0.04}$ & $83.04$ & $95$ \\ 
59230.99 & $24.40\pm0.17$ & $-0.678\pm0.009$ & $-10.347\substack{+0.006\\ -0.007}$ & $-10.392\substack{+0.005\\ -0.005}$ & $-11.38\substack{+0.02\\ -0.03}$ & $124.68$ & $71$ \\ 
59231.63 & $24.09\pm0.20$ & $-0.688\pm0.010$ & $-10.356\substack{+0.008\\ -0.008}$ & $-10.409\substack{+0.006\\ -0.006}$ & $-11.31\substack{+0.02\\ -0.03}$ & $100.12$ & $63$ \\ 
59232.50 & $19.67\pm0.12$ & $-0.663\pm0.008$ & $-10.370\substack{+0.006\\ -0.006}$ & $-10.404\substack{+0.004\\ -0.004}$ & $-11.52\substack{+0.03\\ -0.03}$ & $196.69$ & $79$ \\ 
59233.39 & $19.67\pm0.15$ & $-0.669\pm0.009$ & $-10.384\substack{+0.008\\ -0.007}$ & $-10.415\substack{+0.005\\ -0.004}$ & $-11.57\substack{+0.04\\ -0.04}$ & $84.59$ & $89$ \\ 
59234.98 & $14.00\pm0.11$ & $-0.661\pm0.009$ & $-10.523\substack{+0.007\\ -0.007}$ & $-10.553\substack{+0.005\\ -0.005}$ & $-11.75\substack{+0.04\\ -0.04}$ & $177.09$ & $72$ \\ 
59236.98 & $20.00\pm0.12$ & $-0.690\pm0.008$ & $-10.448\substack{+0.005\\ -0.006}$ & $-10.492\substack{+0.003\\ -0.005}$ & $-11.48\substack{+0.03\\ -0.02}$ & $111.38$ & $89$ \\ 
59239.46 & $19.82\pm0.11$ & $-0.709\pm0.007$ & $-10.381\substack{+0.005\\ -0.005}$ & $-10.440\substack{+0.004\\ -0.004}$ & $-11.29\substack{+0.01\\ -0.01}$ & $706.54$ & $161$ \\ 
59240.26 & $23.70\pm0.22$ & $-0.699\pm0.012$ & $-10.359\substack{+0.009\\ -0.010}$ & $-10.425\substack{+0.006\\ -0.008}$ & $-11.23\substack{+0.02\\ -0.02}$ & $331.02$ & $148$ \\ 
59241.17 & $21.73\pm0.18$ & $-0.680\pm0.010$ & $-10.401\substack{+0.007\\ -0.010}$ & $-10.452\substack{+0.005\\ -0.009}$ & $-11.37\substack{+0.02\\ -0.03}$ & $207.00$ & $156$ \\ 
59243.24 & $19.53\pm0.18$ & $-0.708\pm0.011$ & $-10.444\substack{+0.009\\ -0.009}$ & $-10.516\substack{+0.007\\ -0.007}$ & $-11.28\substack{+0.02\\ -0.02}$ & $104.32$ & $69$ \\ 
59245.18 & $24.21\pm0.26$ & $-0.708\pm0.013$ & $-10.348\substack{+0.010\\ -0.011}$ & $-10.426\substack{+0.008\\ -0.008}$ & $-11.14\substack{+0.02\\ -0.03}$ & $42.90$ & $51$ \\ 
59248.93 & $35.18\pm0.22$ & $-0.684\pm0.008$ & $-10.236\substack{+0.007\\ -0.006}$ & $-10.280\substack{+0.005\\ -0.004}$ & $-11.27\substack{+0.02\\ -0.02}$ & $123.05$ & $111$ \\ 
59253.49 & $33.30\pm0.21$ & $-0.719\pm0.008$ & $-10.216\substack{+0.006\\ -0.007}$ & $-10.290\substack{+0.005\\ -0.006}$ & $-11.03\substack{+0.01\\ -0.01}$ & $131.37$ & $137$ \\ 
59255.41 & $33.61\pm0.24$ & $-0.714\pm0.009$ & $-10.221\substack{+0.007\\ -0.007}$ & $-10.297\substack{+0.005\\ -0.005}$ & $-11.02\substack{+0.02\\ -0.02}$ & $137.37$ & $69$ \\ 
59257.23 & $39.31\pm0.27$ & $-0.705\pm0.008$ & $-10.168\substack{+0.007\\ -0.007}$ & $-10.234\substack{+0.005\\ -0.005}$ & $-11.03\substack{+0.02\\ -0.02}$ & $251.60$ & $149$ \\ 
59258.56 & $37.43\pm0.29$ & $-0.691\pm0.009$ & $-10.211\substack{+0.008\\ -0.007}$ & $-10.262\substack{+0.006\\ -0.005}$ & $-11.18\substack{+0.02\\ -0.03}$ & $150.02$ & $137$ \\ 


==> Table4.tex <==
58256.95 & $32.10\pm0.17$ & $-0.641\pm0.006$ & $-10.233\substack{+0.003\\ -0.003}$ & $-10.248\substack{+0.003\\ -0.003}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.739\substack{+0.008\\ -0.008}$ & $115.28$ & $126$ \\ 
58257.00 & $31.14\pm0.22$ & $-0.652\pm0.009$ & $-10.247\substack{+0.006\\ -0.004}$ & $-10.263\substack{+0.006\\ -0.004}$ & $2.13\substack{+0.01\\ -0.02}$ & $-11.739\substack{+0.008\\ -0.008}$ & $111.59$ & $116$ \\ 
58272.38 & $37.25\pm0.20$ & $-0.660\pm0.006$ & $-10.203\substack{+0.002\\ -0.003}$ & $-10.222\substack{+0.002\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.619\substack{+0.008\\ -0.008}$ & $392.01$ & $158$ \\ 
58293.62 & $31.44\pm0.20$ & $-0.663\pm0.008$ & $-10.278\substack{+0.004\\ -0.004}$ & $-10.296\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.738\substack{+0.008\\ -0.008}$ & $166.26$ & $157$ \\ 
58294.65 & $31.56\pm0.18$ & $-0.649\pm0.007$ & $-10.267\substack{+0.003\\ -0.003}$ & $-10.283\substack{+0.003\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.760\substack{+0.008\\ -0.008}$ & $132.15$ & $98$ \\ 
58302.65 & $31.54\pm0.23$ & $-0.650\pm0.009$ & $-10.270\substack{+0.005\\ -0.005}$ & $-10.285\substack{+0.006\\ -0.006}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.798\substack{+0.008\\ -0.008}$ & $155.91$ & $151$ \\ 
58304.43 & $39.52\pm0.25$ & $-0.650\pm0.008$ & $-10.173\substack{+0.004\\ -0.004}$ & $-10.186\substack{+0.004\\ -0.004}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.781\substack{+0.008\\ -0.008}$ & $147.63$ & $154$ \\ 
58310.32 & $18.86\pm0.16$ & $-0.575\pm0.010$ & $-10.448\substack{+0.004\\ -0.005}$ & $-10.463\substack{+0.004\\ -0.005}$ & $1.99\substack{+0.01\\ -0.01}$ & $-11.999\substack{+0.008\\ -0.008}$ & $87.59$ & $76$ \\ 
58311.22 & $18.04\pm0.12$ & $-0.601\pm0.008$ & $-10.475\substack{+0.004\\ -0.004}$ & $-10.490\substack{+0.004\\ -0.004}$ & $2.01\substack{+0.01\\ -0.01}$ & $-12.049\substack{+0.008\\ -0.008}$ & $103.18$ & $94$ \\ 
58312.21 & $21.85\pm0.16$ & $-0.607\pm0.009$ & $-10.396\substack{+0.004\\ -0.004}$ & $-10.408\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-12.095\substack{+0.008\\ -0.008}$ & $80.29$ & $85$ \\ 
58313.57 & $26.69\pm0.16$ & $-0.626\pm0.007$ & $-10.323\substack{+0.003\\ -0.003}$ & $-10.333\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-12.052\substack{+0.008\\ -0.008}$ & $120.84$ & $104$ \\ 
58314.52 & $28.52\pm0.16$ & $-0.621\pm0.007$ & $-10.298\substack{+0.004\\ -0.003}$ & $-10.308\substack{+0.004\\ -0.003}$ & $2.08\substack{+0.01\\ -0.01}$ & $-12.082\substack{+0.008\\ -0.008}$ & $129.26$ & $111$ \\ 
58315.30 & $25.77\pm0.15$ & $-0.614\pm0.007$ & $-10.339\substack{+0.004\\ -0.003}$ & $-10.348\substack{+0.004\\ -0.003}$ & $2.06\substack{+0.01\\ -0.01}$ & $-12.098\substack{+0.008\\ -0.008}$ & $149.04$ & $108$ \\ 
58317.30 & $29.02\pm0.15$ & $-0.638\pm0.006$ & $-10.301\substack{+0.003\\ -0.002}$ & $-10.310\substack{+0.003\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.096\substack{+0.008\\ -0.008}$ & $259.14$ & $160$ \\ 
58318.58 & $30.28\pm0.22$ & $-0.633\pm0.009$ & $-10.280\substack{+0.004\\ -0.004}$ & $-10.288\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-12.114\substack{+0.008\\ -0.008}$ & $93.63$ & $82$ \\ 
58325.65 & $26.17\pm0.18$ & $-0.618\pm0.008$ & $-10.334\substack{+0.004\\ -0.004}$ & $-10.341\substack{+0.004\\ -0.004}$ & $2.08\substack{+0.01\\ -0.01}$ & $-12.281\substack{+0.008\\ -0.008}$ & $98.33$ & $83$ \\ 
58327.16 & $28.68\pm0.17$ & $-0.601\pm0.007$ & $-10.285\substack{+0.003\\ -0.003}$ & $-10.292\substack{+0.003\\ -0.003}$ & $2.03\substack{+0.01\\ -0.01}$ & $-12.213\substack{+0.008\\ -0.008}$ & $96.32$ & $93$ \\ 
58329.19 & $26.79\pm0.21$ & $-0.613\pm0.009$ & $-10.322\substack{+0.004\\ -0.004}$ & $-10.330\substack{+0.005\\ -0.005}$ & $2.06\substack{+0.01\\ -0.01}$ & $-12.166\substack{+0.008\\ -0.008}$ & $76.42$ & $78$ \\ 
58331.12 & $24.33\pm0.21$ & $-0.617\pm0.010$ & $-10.360\substack{+0.005\\ -0.006}$ & $-10.369\substack{+0.005\\ -0.006}$ & $2.06\substack{+0.02\\ -0.01}$ & $-12.128\substack{+0.008\\ -0.008}$ & $77.22$ & $80$ \\ 
58333.50 & $30.62\pm0.15$ & $-0.652\pm0.006$ & $-10.285\substack{+0.002\\ -0.002}$ & $-10.294\substack{+0.002\\ -0.002}$ & $2.17\substack{+0.01\\ -0.01}$ & $-12.076\substack{+0.008\\ -0.008}$ & $148.89$ & $106$ \\ 
58336.46 & $35.74\pm0.22$ & $-0.642\pm0.007$ & $-10.213\substack{+0.003\\ -0.003}$ & $-10.221\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-12.048\substack{+0.008\\ -0.008}$ & $137.96$ & $90$ \\ 
58338.59 & $30.92\pm0.20$ & $-0.642\pm0.008$ & $-10.275\substack{+0.003\\ -0.004}$ & $-10.285\substack{+0.003\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.027\substack{+0.008\\ -0.008}$ & $115.16$ & $90$ \\ 
58340.52 & $34.58\pm0.21$ & $-0.626\pm0.007$ & $-10.218\substack{+0.003\\ -0.003}$ & $-10.225\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-12.083\substack{+0.008\\ -0.008}$ & $128.81$ & $91$ \\ 
58342.64 & $33.97\pm0.21$ & $-0.609\pm0.007$ & $-10.215\substack{+0.003\\ -0.003}$ & $-10.223\substack{+0.003\\ -0.003}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.109\substack{+0.008\\ -0.008}$ & $102.10$ & $97$ \\ 
58343.60 & $29.04\pm0.19$ & $-0.611\pm0.008$ & $-10.285\substack{+0.004\\ -0.004}$ & $-10.293\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.122\substack{+0.008\\ -0.008}$ & $112.02$ & $96$ \\ 
58345.21 & $29.22\pm0.21$ & $-0.635\pm0.008$ & $-10.297\substack{+0.004\\ -0.004}$ & $-10.305\substack{+0.004\\ -0.004}$ & $2.12\substack{+0.01\\ -0.01}$ & $-12.130\substack{+0.008\\ -0.008}$ & $373.38$ & $158$ \\ 
58348.86 & $29.65\pm0.20$ & $-0.628\pm0.008$ & $-10.286\substack{+0.004\\ -0.004}$ & $-10.294\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-12.168\substack{+0.008\\ -0.008}$ & $69.20$ & $87$ \\ 
58350.96 & $29.08\pm0.19$ & $-0.645\pm0.008$ & $-10.304\substack{+0.004\\ -0.003}$ & $-10.311\substack{+0.004\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-12.220\substack{+0.008\\ -0.008}$ & $117.30$ & $93$ \\ 
58352.82 & $28.88\pm0.18$ & $-0.633\pm0.008$ & $-10.300\substack{+0.004\\ -0.003}$ & $-10.307\substack{+0.004\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-12.257\substack{+0.008\\ -0.008}$ & $121.40$ & $93$ \\ 
58354.82 & $29.34\pm0.18$ & $-0.630\pm0.008$ & $-10.292\substack{+0.003\\ -0.003}$ & $-10.299\substack{+0.003\\ -0.003}$ & $2.11\substack{+0.01\\ -0.01}$ & $-12.230\substack{+0.008\\ -0.008}$ & $122.88$ & $91$ \\ 
58358.86 & $25.05\pm0.21$ & $-0.619\pm0.010$ & $-10.355\substack{+0.006\\ -0.006}$ & $-10.361\substack{+0.006\\ -0.006}$ & $2.09\substack{+0.02\\ -0.02}$ & $-12.399\substack{+0.008\\ -0.008}$ & $198.66$ & $158$ \\ 
58360.85 & $21.40\pm0.28$ & $-0.597\pm0.015$ & $-10.427\substack{+0.010\\ -0.010}$ & $-10.433\substack{+0.010\\ -0.010}$ & $2.04\substack{+0.02\\ -0.03}$ & $-12.495\substack{+0.008\\ -0.008}$ & $198.82$ & $149$ \\ 
58362.85 & $20.66\pm0.29$ & $-0.618\pm0.017$ & $-10.454\substack{+0.010\\ -0.010}$ & $-10.461\substack{+0.010\\ -0.010}$ & $2.10\substack{+0.02\\ -0.02}$ & $-12.449\substack{+0.008\\ -0.008}$ & $182.82$ & $153$ \\ 
58364.71 & $27.40\pm0.18$ & $-0.610\pm0.008$ & $-10.311\substack{+0.005\\ -0.004}$ & $-10.317\substack{+0.005\\ -0.004}$ & $2.06\substack{+0.01\\ -0.01}$ & $-12.365\substack{+0.008\\ -0.008}$ & $207.45$ & $157$ \\ 
58367.94 & $32.67\pm0.31$ & $-0.672\pm0.011$ & $-10.271\substack{+0.005\\ -0.005}$ & $-10.277\substack{+0.005\\ -0.005}$ & $2.18\substack{+0.02\\ -0.01}$ & $-12.337\substack{+0.008\\ -0.008}$ & $86.64$ & $67$ \\ 
58369.77 & $24.50\pm0.15$ & $-0.626\pm0.007$ & $-10.368\substack{+0.003\\ -0.003}$ & $-10.376\substack{+0.003\\ -0.003}$ & $2.10\substack{+0.01\\ -0.01}$ & $-12.212\substack{+0.008\\ -0.008}$ & $127.88$ & $96$ \\ 
58375.54 & $24.81\pm0.19$ & $-0.641\pm0.009$ & $-10.351\substack{+0.006\\ -0.004}$ & $-10.356\substack{+0.006\\ -0.004}$ & $2.14\substack{+0.01\\ -0.02}$ & $-12.586\substack{+0.008\\ -0.008}$ & $151.95$ & $152$ \\ 
58377.89 & $19.90\pm0.14$ & $-0.610\pm0.009$ & $-10.432\substack{+0.005\\ -0.003}$ & $-10.437\substack{+0.005\\ -0.003}$ & $2.06\substack{+0.01\\ -0.01}$ & $-12.632\substack{+0.008\\ -0.008}$ & $140.16$ & $121$ \\ 
58379.95 & $20.58\pm0.14$ & $-0.598\pm0.008$ & $-10.411\substack{+0.005\\ -0.005}$ & $-10.416\substack{+0.005\\ -0.005}$ & $2.03\substack{+0.01\\ -0.01}$ & $-12.689\substack{+0.008\\ -0.008}$ & $162.04$ & $135$ \\ 
58382.85 & $21.62\pm0.18$ & $-0.599\pm0.010$ & $-10.385\substack{+0.006\\ -0.006}$ & $-10.388\substack{+0.006\\ -0.006}$ & $2.04\substack{+0.01\\ -0.01}$ & $-13.385\substack{+0.008\\ -0.008}$ & $145.02$ & $108$ \\ 
58388.42 & $23.58\pm0.17$ & $-0.614\pm0.009$ & $-10.378\substack{+0.003\\ -0.005}$ & $-10.382\substack{+0.003\\ -0.005}$ & $2.08\substack{+0.01\\ -0.01}$ & $-12.812\substack{+0.008\\ -0.008}$ & $115.88$ & $81$ \\ 
58390.48 & $26.85\pm0.19$ & $-0.615\pm0.008$ & $-10.324\substack{+0.004\\ -0.004}$ & $-10.326\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-14.106\substack{+0.008\\ -0.008}$ & $90.44$ & $83$ \\ 
58392.70 & $27.64\pm0.13$ & $-0.611\pm0.006$ & $-10.308\substack{+0.002\\ -0.002}$ & $-10.312\substack{+0.002\\ -0.002}$ & $2.07\substack{+0.01\\ -0.01}$ & $-12.801\substack{+0.008\\ -0.008}$ & $175.79$ & $112$ \\ 
58394.92 & $19.79\pm0.12$ & $-0.585\pm0.007$ & $-10.438\substack{+0.004\\ -0.004}$ & $-10.442\substack{+0.004\\ -0.004}$ & $2.00\substack{+0.01\\ -0.01}$ & $-12.860\substack{+0.008\\ -0.008}$ & $136.82$ & $107$ \\ 
58396.59 & $20.82\pm0.15$ & $-0.605\pm0.008$ & $-10.427\substack{+0.004\\ -0.004}$ & $-10.432\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.651\substack{+0.008\\ -0.008}$ & $127.19$ & $85$ \\ 
58398.59 & $26.75\pm0.18$ & $-0.585\pm0.008$ & $-10.308\substack{+0.004\\ -0.004}$ & $-10.312\substack{+0.004\\ -0.004}$ & $2.00\substack{+0.01\\ -0.01}$ & $-12.573\substack{+0.008\\ -0.008}$ & $356.48$ & $118$ \\ 
58400.69 & $26.23\pm0.16$ & $-0.628\pm0.007$ & $-10.340\substack{+0.004\\ -0.004}$ & $-10.347\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-12.364\substack{+0.008\\ -0.008}$ & $161.18$ & $153$ \\ 
58402.59 & $26.26\pm0.18$ & $-0.629\pm0.008$ & $-10.340\substack{+0.004\\ -0.004}$ & $-10.345\substack{+0.004\\ -0.004}$ & $2.12\substack{+0.01\\ -0.01}$ & $-12.485\substack{+0.008\\ -0.008}$ & $126.89$ & $91$ \\ 
58403.93 & $23.10\pm0.18$ & $-0.621\pm0.009$ & $-10.391\substack{+0.005\\ -0.005}$ & $-10.397\substack{+0.005\\ -0.005}$ & $2.09\substack{+0.01\\ -0.01}$ & $-12.546\substack{+0.008\\ -0.008}$ & $75.13$ & $82$ \\ 
58405.89 & $25.09\pm0.27$ & $-0.646\pm0.013$ & $-10.382\substack{+0.007\\ -0.007}$ & $-10.387\substack{+0.008\\ -0.007}$ & $2.16\substack{+0.02\\ -0.02}$ & $-12.565\substack{+0.008\\ -0.008}$ & $73.28$ & $63$ \\ 
58407.31 & $28.02\pm0.20$ & $-0.637\pm0.009$ & $-10.316\substack{+0.004\\ -0.004}$ & $-10.322\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.406\substack{+0.008\\ -0.008}$ & $117.31$ & $79$ \\ 
58409.69 & $30.36\pm0.17$ & $-0.641\pm0.007$ & $-10.283\substack{+0.003\\ -0.003}$ & $-10.289\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-12.360\substack{+0.008\\ -0.008}$ & $154.76$ & $91$ \\ 
58412.07 & $22.70\pm0.17$ & $-0.673\pm0.009$ & $-10.426\substack{+0.004\\ -0.004}$ & $-10.435\substack{+0.004\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-12.256\substack{+0.008\\ -0.008}$ & $82.79$ & $84$ \\ 
58414.51 & $26.96\pm0.15$ & $-0.675\pm0.007$ & $-10.353\substack{+0.003\\ -0.003}$ & $-10.362\substack{+0.003\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-12.174\substack{+0.008\\ -0.008}$ & $350.18$ & $131$ \\ 
58416.70 & $28.74\pm0.20$ & $-0.694\pm0.008$ & $-10.335\substack{+0.004\\ -0.004}$ & $-10.344\substack{+0.004\\ -0.004}$ & $2.30\substack{+0.01\\ -0.01}$ & $-12.138\substack{+0.008\\ -0.008}$ & $137.22$ & $115$ \\ 
58418.70 & $28.08\pm0.20$ & $-0.674\pm0.009$ & $-10.335\substack{+0.004\\ -0.004}$ & $-10.344\substack{+0.004\\ -0.004}$ & $2.24\substack{+0.01\\ -0.01}$ & $-12.174\substack{+0.008\\ -0.008}$ & $140.48$ & $115$ \\ 
58420.63 & $27.69\pm0.21$ & $-0.645\pm0.009$ & $-10.314\substack{+0.005\\ -0.005}$ & $-10.322\substack{+0.005\\ -0.005}$ & $2.15\substack{+0.01\\ -0.01}$ & $-12.209\substack{+0.008\\ -0.008}$ & $163.20$ & $132$ \\ 
58421.24 & $30.14\pm0.22$ & $-0.638\pm0.009$ & $-10.285\substack{+0.004\\ -0.004}$ & $-10.292\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.209\substack{+0.008\\ -0.008}$ & $101.21$ & $83$ \\ 
58422.67 & $27.57\pm0.20$ & $-0.612\pm0.009$ & $-10.308\substack{+0.004\\ -0.004}$ & $-10.315\substack{+0.004\\ -0.004}$ & $2.06\substack{+0.01\\ -0.01}$ & $-12.258\substack{+0.008\\ -0.008}$ & $132.34$ & $84$ \\ 
58423.96 & $26.38\pm0.19$ & $-0.605\pm0.009$ & $-10.324\substack{+0.004\\ -0.004}$ & $-10.331\substack{+0.004\\ -0.004}$ & $2.04\substack{+0.01\\ -0.01}$ & $-12.252\substack{+0.008\\ -0.008}$ & $90.49$ & $80$ \\ 
58426.46 & $28.43\pm0.17$ & $-0.615\pm0.007$ & $-10.297\substack{+0.003\\ -0.003}$ & $-10.304\substack{+0.003\\ -0.003}$ & $2.07\substack{+0.01\\ -0.01}$ & $-12.187\substack{+0.008\\ -0.008}$ & $195.81$ & $88$ \\ 
58428.20 & $34.08\pm0.18$ & $-0.641\pm0.006$ & $-10.233\substack{+0.003\\ -0.003}$ & $-10.240\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-12.128\substack{+0.008\\ -0.008}$ & $130.87$ & $110$ \\ 
58429.17 & $37.47\pm0.20$ & $-0.649\pm0.007$ & $-10.197\substack{+0.003\\ -0.003}$ & $-10.204\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-12.080\substack{+0.008\\ -0.008}$ & $157.08$ & $103$ \\ 
58430.07 & $38.37\pm0.29$ & $-0.648\pm0.009$ & $-10.186\substack{+0.004\\ -0.004}$ & $-10.193\substack{+0.004\\ -0.004}$ & $2.16\substack{+0.01\\ -0.01}$ & $-12.020\substack{+0.008\\ -0.008}$ & $85.57$ & $75$ \\ 
58431.16 & $35.76\pm0.21$ & $-0.648\pm0.007$ & $-10.216\substack{+0.003\\ -0.003}$ & $-10.225\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.994\substack{+0.008\\ -0.008}$ & $115.56$ & $88$ \\ 
58432.97 & $41.85\pm0.33$ & $-0.641\pm0.009$ & $-10.144\substack{+0.003\\ -0.004}$ & $-10.152\substack{+0.003\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.969\substack{+0.008\\ -0.008}$ & $68.26$ & $79$ \\ 
58433.06 & $41.29\pm0.25$ & $-0.642\pm0.007$ & $-10.150\substack{+0.003\\ -0.003}$ & $-10.158\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.966\substack{+0.008\\ -0.008}$ & $108.19$ & $89$ \\ 
58437.51 & $33.67\pm0.25$ & $-0.660\pm0.009$ & $-10.228\substack{+0.004\\ -0.004}$ & $-10.239\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.902\substack{+0.008\\ -0.008}$ & $152.04$ & $154$ \\ 
58438.42 & $31.41\pm0.33$ & $-0.672\pm0.013$ & $-10.259\substack{+0.005\\ -0.006}$ & $-10.271\substack{+0.005\\ -0.006}$ & $2.20\substack{+0.02\\ -0.02}$ & $-11.880\substack{+0.008\\ -0.008}$ & $80.77$ & $73$ \\ 
58439.64 & $34.27\pm0.36$ & $-0.666\pm0.013$ & $-10.240\substack{+0.006\\ -0.006}$ & $-10.252\substack{+0.006\\ -0.006}$ & $2.20\substack{+0.02\\ -0.02}$ & $-11.907\substack{+0.008\\ -0.008}$ & $112.76$ & $75$ \\ 
58449.22 & $33.64\pm0.23$ & $-0.648\pm0.008$ & $-10.214\substack{+0.003\\ -0.006}$ & $-10.224\substack{+0.003\\ -0.006}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.911\substack{+0.008\\ -0.008}$ & $126.86$ & $133$ \\ 
58453.60 & $27.94\pm0.16$ & $-0.618\pm0.007$ & $-10.306\substack{+0.003\\ -0.003}$ & $-10.317\substack{+0.003\\ -0.003}$ & $2.06\substack{+0.01\\ -0.01}$ & $-11.956\substack{+0.008\\ -0.008}$ & $171.88$ & $92$ \\ 
58455.11 & $23.92\pm0.19$ & $-0.615\pm0.009$ & $-10.371\substack{+0.005\\ -0.005}$ & $-10.382\substack{+0.005\\ -0.005}$ & $2.06\substack{+0.01\\ -0.01}$ & $-12.083\substack{+0.008\\ -0.008}$ & $72.09$ & $80$ \\ 
58456.98 & $21.99\pm0.16$ & $-0.626\pm0.009$ & $-10.413\substack{+0.004\\ -0.005}$ & $-10.426\substack{+0.004\\ -0.005}$ & $2.08\substack{+0.01\\ -0.02}$ & $-12.075\substack{+0.008\\ -0.008}$ & $66.63$ & $85$ \\ 
58458.91 & $22.51\pm0.16$ & $-0.632\pm0.008$ & $-10.407\substack{+0.004\\ -0.004}$ & $-10.418\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-12.140\substack{+0.008\\ -0.008}$ & $103.11$ & $87$ \\ 
58460.91 & $26.35\pm0.17$ & $-0.622\pm0.008$ & $-10.333\substack{+0.003\\ -0.003}$ & $-10.343\substack{+0.003\\ -0.003}$ & $2.08\substack{+0.01\\ -0.01}$ & $-12.074\substack{+0.008\\ -0.008}$ & $96.31$ & $100$ \\ 
58462.90 & $22.98\pm0.17$ & $-0.594\pm0.009$ & $-10.377\substack{+0.004\\ -0.004}$ & $-10.387\substack{+0.005\\ -0.005}$ & $2.00\substack{+0.01\\ -0.01}$ & $-12.106\substack{+0.008\\ -0.008}$ & $116.72$ & $114$ \\ 
58464.58 & $22.00\pm0.15$ & $-0.613\pm0.008$ & $-10.406\substack{+0.004\\ -0.004}$ & $-10.417\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.115\substack{+0.008\\ -0.008}$ & $77.95$ & $90$ \\ 
58466.18 & $23.48\pm0.18$ & $-0.631\pm0.009$ & $-10.389\substack{+0.004\\ -0.004}$ & $-10.399\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-12.147\substack{+0.008\\ -0.008}$ & $235.39$ & $147$ \\ 
58469.02 & $19.93\pm0.17$ & $-0.615\pm0.010$ & $-10.435\substack{+0.006\\ -0.006}$ & $-10.447\substack{+0.006\\ -0.006}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.130\substack{+0.008\\ -0.008}$ & $112.18$ & $98$ \\ 
58470.68 & $21.22\pm0.16$ & $-0.596\pm0.009$ & $-10.394\substack{+0.004\\ -0.004}$ & $-10.406\substack{+0.005\\ -0.005}$ & $2.00\substack{+0.01\\ -0.01}$ & $-12.067\substack{+0.008\\ -0.008}$ & $113.98$ & $89$ \\ 
58471.77 & $27.22\pm0.24$ & $-0.607\pm0.010$ & $-10.315\substack{+0.005\\ -0.005}$ & $-10.325\substack{+0.005\\ -0.005}$ & $2.08\substack{+0.01\\ -0.01}$ & $-12.032\substack{+0.008\\ -0.008}$ & $102.51$ & $75$ \\ 
58473.91 & $28.53\pm0.19$ & $-0.624\pm0.008$ & $-10.283\substack{+0.004\\ -0.005}$ & $-10.293\substack{+0.004\\ -0.005}$ & $2.08\substack{+0.01\\ -0.01}$ & $-12.015\substack{+0.008\\ -0.008}$ & $99.03$ & $118$ \\ 
58476.07 & $33.52\pm0.32$ & $-0.661\pm0.011$ & $-10.255\substack{+0.006\\ -0.006}$ & $-10.267\substack{+0.006\\ -0.006}$ & $2.14\substack{+0.02\\ -0.02}$ & $-11.900\substack{+0.008\\ -0.008}$ & $80.50$ & $75$ \\ 
58479.11 & $31.16\pm0.21$ & $-0.651\pm0.008$ & $-10.255\substack{+0.004\\ -0.004}$ & $-10.268\substack{+0.004\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.847\substack{+0.008\\ -0.008}$ & $103.62$ & $86$ \\ 
58481.24 & $25.92\pm0.22$ & $-0.665\pm0.010$ & $-10.343\substack{+0.006\\ -0.006}$ & $-10.358\substack{+0.006\\ -0.006}$ & $2.16\substack{+0.02\\ -0.02}$ & $-11.859\substack{+0.008\\ -0.008}$ & $135.28$ & $151$ \\ 
58487.79 & $34.24\pm0.31$ & $-0.652\pm0.011$ & $-10.213\substack{+0.005\\ -0.006}$ & $-10.227\substack{+0.005\\ -0.006}$ & $2.20\substack{+0.02\\ -0.02}$ & $-11.771\substack{+0.008\\ -0.008}$ & $70.31$ & $78$ \\ 
58489.79 & $24.24\pm0.20$ & $-0.636\pm0.010$ & $-10.355\substack{+0.005\\ -0.004}$ & $-10.375\substack{+0.005\\ -0.005}$ & $2.12\substack{+0.01\\ -0.02}$ & $-11.747\substack{+0.008\\ -0.008}$ & $213.74$ & $114$ \\ 
58491.53 & $22.10\pm0.24$ & $-0.603\pm0.013$ & $-10.376\substack{+0.006\\ -0.007}$ & $-10.397\substack{+0.007\\ -0.007}$ & $2.05\substack{+0.02\\ -0.02}$ & $-11.755\substack{+0.008\\ -0.008}$ & $97.27$ & $81$ \\ 
58493.71 & $22.41\pm0.27$ & $-0.679\pm0.015$ & $-10.408\substack{+0.008\\ -0.008}$ & $-10.431\substack{+0.008\\ -0.009}$ & $2.26\substack{+0.03\\ -0.02}$ & $-11.758\substack{+0.008\\ -0.008}$ & $107.53$ & $123$ \\ 
58497.64 & $24.35\pm0.19$ & $-0.647\pm0.009$ & $-10.353\substack{+0.005\\ -0.005}$ & $-10.376\substack{+0.006\\ -0.005}$ & $2.11\substack{+0.02\\ -0.02}$ & $-11.692\substack{+0.008\\ -0.008}$ & $73.62$ & $92$ \\ 
58499.38 & $26.86\pm0.15$ & $-0.662\pm0.007$ & $-10.335\substack{+0.003\\ -0.004}$ & $-10.360\substack{+0.003\\ -0.005}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.638\substack{+0.008\\ -0.008}$ & $183.98$ & $151$ \\ 
58500.48 & $27.29\pm0.16$ & $-0.692\pm0.007$ & $-10.344\substack{+0.004\\ -0.003}$ & $-10.370\substack{+0.004\\ -0.004}$ & $2.29\substack{+0.01\\ -0.01}$ & $-11.610\substack{+0.008\\ -0.008}$ & $240.32$ & $154$ \\ 
58501.89 & $28.58\pm0.17$ & $-0.680\pm0.007$ & $-10.313\substack{+0.004\\ -0.004}$ & $-10.339\substack{+0.004\\ -0.004}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.592\substack{+0.008\\ -0.008}$ & $130.64$ & $114$ \\ 
58503.24 & $26.48\pm0.14$ & $-0.694\pm0.007$ & $-10.356\substack{+0.003\\ -0.003}$ & $-10.384\substack{+0.003\\ -0.003}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.588\substack{+0.008\\ -0.008}$ & $184.86$ & $144$ \\ 
58504.98 & $34.75\pm0.17$ & $-0.705\pm0.006$ & $-10.246\substack{+0.002\\ -0.002}$ & $-10.269\substack{+0.003\\ -0.003}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.561\substack{+0.008\\ -0.008}$ & $177.62$ & $135$ \\ 
58505.95 & $36.92\pm0.18$ & $-0.692\pm0.006$ & $-10.215\substack{+0.002\\ -0.002}$ & $-10.237\substack{+0.002\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.560\substack{+0.008\\ -0.008}$ & $161.51$ & $145$ \\ 
58506.33 & $34.73\pm0.17$ & $-0.690\pm0.006$ & $-10.240\substack{+0.003\\ -0.003}$ & $-10.262\substack{+0.003\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.570\substack{+0.008\\ -0.008}$ & $156.06$ & $156$ \\ 
58507.62 & $31.46\pm0.18$ & $-0.686\pm0.007$ & $-10.281\substack{+0.002\\ -0.002}$ & $-10.306\substack{+0.003\\ -0.003}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.565\substack{+0.008\\ -0.008}$ & $161.93$ & $147$ \\ 
58511.87 & $27.25\pm0.18$ & $-0.688\pm0.008$ & $-10.339\substack{+0.003\\ -0.003}$ & $-10.370\substack{+0.004\\ -0.004}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.534\substack{+0.008\\ -0.008}$ & $93.94$ & $80$ \\ 
58513.28 & $27.87\pm0.15$ & $-0.674\pm0.007$ & $-10.327\substack{+0.003\\ -0.003}$ & $-10.359\substack{+0.003\\ -0.003}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.509\substack{+0.008\\ -0.008}$ & $162.33$ & $146$ \\ 
58514.73 & $28.34\pm0.16$ & $-0.701\pm0.007$ & $-10.330\substack{+0.003\\ -0.002}$ & $-10.361\substack{+0.003\\ -0.003}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.520\substack{+0.008\\ -0.008}$ & $180.14$ & $146$ \\ 
58515.86 & $32.10\pm0.22$ & $-0.703\pm0.008$ & $-10.276\substack{+0.003\\ -0.003}$ & $-10.306\substack{+0.004\\ -0.004}$ & $2.30\substack{+0.01\\ -0.01}$ & $-11.479\substack{+0.008\\ -0.008}$ & $119.00$ & $106$ \\ 
58517.18 & $33.04\pm0.23$ & $-0.693\pm0.008$ & $-10.250\substack{+0.004\\ -0.003}$ & $-10.280\substack{+0.004\\ -0.003}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $81.58$ & $81$ \\ 
58521.53 & $37.00\pm0.22$ & $-0.710\pm0.007$ & $-10.231\substack{+0.002\\ -0.004}$ & $-10.263\substack{+0.002\\ -0.004}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.400\substack{+0.008\\ -0.008}$ & $111.48$ & $88$ \\ 
58523.50 & $35.71\pm0.20$ & $-0.689\pm0.007$ & $-10.234\substack{+0.003\\ -0.003}$ & $-10.270\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.349\substack{+0.008\\ -0.008}$ & $191.72$ & $134$ \\ 
58527.09 & $38.24\pm0.25$ & $-0.726\pm0.008$ & $-10.225\substack{+0.004\\ -0.003}$ & $-10.261\substack{+0.004\\ -0.004}$ & $2.32\substack{+0.01\\ -0.01}$ & $-11.340\substack{+0.008\\ -0.008}$ & $92.50$ & $79$ \\ 
58528.06 & $34.22\pm0.31$ & $-0.711\pm0.011$ & $-10.240\substack{+0.005\\ -0.005}$ & $-10.276\substack{+0.005\\ -0.006}$ & $2.29\substack{+0.02\\ -0.02}$ & $-11.357\substack{+0.008\\ -0.008}$ & $86.28$ & $61$ \\ 
58529.87 & $32.38\pm0.25$ & $-0.705\pm0.010$ & $-10.265\substack{+0.006\\ -0.005}$ & $-10.306\substack{+0.006\\ -0.005}$ & $2.22\substack{+0.02\\ -0.02}$ & $-11.327\substack{+0.008\\ -0.008}$ & $94.08$ & $90$ \\ 
58541.28 & $33.89\pm0.19$ & $-0.665\pm0.007$ & $-10.209\substack{+0.002\\ -0.003}$ & $-10.241\substack{+0.002\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.378\substack{+0.008\\ -0.008}$ & $108.78$ & $89$ \\ 
58544.08 & $39.58\pm0.23$ & $-0.671\pm0.007$ & $-10.140\substack{+0.003\\ -0.003}$ & $-10.167\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.375\substack{+0.008\\ -0.008}$ & $132.34$ & $96$ \\ 
58545.93 & $40.31\pm0.35$ & $-0.691\pm0.011$ & $-10.157\substack{+0.004\\ -0.005}$ & $-10.186\substack{+0.005\\ -0.005}$ & $2.23\substack{+0.02\\ -0.02}$ & $-11.373\substack{+0.008\\ -0.008}$ & $86.66$ & $82$ \\ 
58548.20 & $43.58\pm0.25$ & $-0.706\pm0.007$ & $-10.110\substack{+0.003\\ -0.003}$ & $-10.137\substack{+0.003\\ -0.003}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.362\substack{+0.008\\ -0.008}$ & $69.13$ & $84$ \\ 
58550.32 & $39.70\pm0.22$ & $-0.678\pm0.007$ & $-10.139\substack{+0.003\\ -0.003}$ & $-10.167\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.361\substack{+0.008\\ -0.008}$ & $107.41$ & $90$ \\ 
58553.35 & $36.42\pm0.22$ & $-0.643\pm0.007$ & $-10.180\substack{+0.004\\ -0.003}$ & $-10.209\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.390\substack{+0.008\\ -0.008}$ & $96.88$ & $85$ \\ 
58556.06 & $40.45\pm0.24$ & $-0.676\pm0.007$ & $-10.143\substack{+0.003\\ -0.003}$ & $-10.169\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.393\substack{+0.008\\ -0.008}$ & $89.15$ & $88$ \\ 
58559.95 & $30.29\pm0.25$ & $-0.660\pm0.010$ & $-10.264\substack{+0.005\\ -0.005}$ & $-10.300\substack{+0.005\\ -0.005}$ & $2.12\substack{+0.02\\ -0.02}$ & $-11.387\substack{+0.008\\ -0.008}$ & $101.75$ & $76$ \\ 
58561.50 & $29.64\pm0.16$ & $-0.662\pm0.006$ & $-10.280\substack{+0.003\\ -0.003}$ & $-10.318\substack{+0.004\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.386\substack{+0.008\\ -0.008}$ & $120.06$ & $118$ \\ 
58562.94 & $31.06\pm0.23$ & $-0.690\pm0.009$ & $-10.270\substack{+0.004\\ -0.005}$ & $-10.308\substack{+0.004\\ -0.005}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.368\substack{+0.008\\ -0.008}$ & $84.55$ & $73$ \\ 
58564.04 & $41.33\pm0.27$ & $-0.683\pm0.008$ & $-10.149\substack{+0.004\\ -0.003}$ & $-10.178\substack{+0.005\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.359\substack{+0.008\\ -0.008}$ & $115.35$ & $93$ \\ 
58565.78 & $40.02\pm0.24$ & $-0.697\pm0.007$ & $-10.170\substack{+0.003\\ -0.003}$ & $-10.202\substack{+0.003\\ -0.003}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.345\substack{+0.008\\ -0.008}$ & $113.58$ & $83$ \\ 
58567.20 & $32.03\pm0.24$ & $-0.718\pm0.009$ & $-10.272\substack{+0.008\\ -0.003}$ & $-10.313\substack{+0.008\\ -0.004}$ & $2.30\substack{+0.01\\ -0.01}$ & $-11.334\substack{+0.008\\ -0.008}$ & $131.26$ & $146$ \\ 
58568.80 & $35.18\pm0.22$ & $-0.706\pm0.008$ & $-10.230\substack{+0.003\\ -0.003}$ & $-10.268\substack{+0.003\\ -0.003}$ & $2.30\substack{+0.01\\ -0.01}$ & $-11.322\substack{+0.008\\ -0.008}$ & $101.55$ & $84$ \\ 
58570.87 & $40.31\pm0.17$ & $-0.685\pm0.005$ & $-10.153\substack{+0.002\\ -0.002}$ & $-10.186\substack{+0.002\\ -0.002}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.306\substack{+0.008\\ -0.008}$ & $158.49$ & $127$ \\ 
58573.06 & $38.48\pm0.18$ & $-0.708\pm0.006$ & $-10.188\substack{+0.004\\ -0.002}$ & $-10.224\substack{+0.004\\ -0.002}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.300\substack{+0.008\\ -0.008}$ & $168.50$ & $154$ \\ 
58575.51 & $41.28\pm0.23$ & $-0.690\pm0.007$ & $-10.148\substack{+0.003\\ -0.003}$ & $-10.182\substack{+0.003\\ -0.003}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.290\substack{+0.008\\ -0.008}$ & $163.54$ & $127$ \\ 
58577.45 & $43.06\pm0.27$ & $-0.693\pm0.008$ & $-10.136\substack{+0.003\\ -0.003}$ & $-10.171\substack{+0.003\\ -0.003}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.269\substack{+0.008\\ -0.008}$ & $96.60$ & $79$ \\ 
58579.38 & $49.60\pm0.29$ & $-0.721\pm0.007$ & $-10.081\substack{+0.003\\ -0.003}$ & $-10.112\substack{+0.003\\ -0.003}$ & $2.31\substack{+0.01\\ -0.01}$ & $-11.259\substack{+0.008\\ -0.008}$ & $120.10$ & $84$ \\ 
58581.35 & $40.49\pm0.27$ & $-0.684\pm0.008$ & $-10.145\substack{+0.003\\ -0.003}$ & $-10.180\substack{+0.004\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.275\substack{+0.008\\ -0.008}$ & $81.44$ & $78$ \\ 
58586.70 & $40.70\pm0.30$ & $-0.687\pm0.009$ & $-10.176\substack{+0.005\\ -0.005}$ & $-10.214\substack{+0.006\\ -0.006}$ & $2.18\substack{+0.01\\ -0.02}$ & $-11.277\substack{+0.008\\ -0.008}$ & $204.66$ & $159$ \\ 
58588.63 & $48.96\pm0.29$ & $-0.675\pm0.007$ & $-10.091\substack{+0.004\\ -0.004}$ & $-10.120\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.289\substack{+0.008\\ -0.008}$ & $213.39$ & $161$ \\ 
58591.05 & $42.26\pm0.25$ & $-0.691\pm0.007$ & $-10.162\substack{+0.002\\ -0.003}$ & $-10.197\substack{+0.002\\ -0.004}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.294\substack{+0.008\\ -0.008}$ & $165.03$ & $159$ \\ 
58592.65 & $45.66\pm0.23$ & $-0.620\pm0.006$ & $-10.089\substack{+0.003\\ -0.003}$ & $-10.118\substack{+0.003\\ -0.003}$ & $2.00\substack{+0.01\\ -0.01}$ & $-11.297\substack{+0.008\\ -0.008}$ & $923.56$ & $156$ \\ 
58594.91 & $42.32\pm0.25$ & $-0.684\pm0.007$ & $-10.158\substack{+0.003\\ -0.004}$ & $-10.191\substack{+0.003\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.323\substack{+0.008\\ -0.008}$ & $244.99$ & $158$ \\ 
58596.84 & $43.54\pm0.26$ & $-0.649\pm0.007$ & $-10.126\substack{+0.003\\ -0.003}$ & $-10.157\substack{+0.003\\ -0.003}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.311\substack{+0.008\\ -0.008}$ & $1340.93$ & $170$ \\ 
58603.42 & $37.96\pm0.27$ & $-0.681\pm0.009$ & $-10.184\substack{+0.003\\ -0.004}$ & $-10.221\substack{+0.003\\ -0.005}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.294\substack{+0.008\\ -0.008}$ & $94.98$ & $73$ \\ 
58605.35 & $45.46\pm0.25$ & $-0.709\pm0.007$ & $-10.101\substack{+0.003\\ -0.003}$ & $-10.130\substack{+0.003\\ -0.003}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.311\substack{+0.008\\ -0.008}$ & $86.26$ & $90$ \\ 
58607.22 & $35.03\pm0.20$ & $-0.698\pm0.007$ & $-10.210\substack{+0.003\\ -0.003}$ & $-10.245\substack{+0.004\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.334\substack{+0.008\\ -0.008}$ & $93.55$ & $94$ \\ 
58609.28 & $38.35\pm0.20$ & $-0.677\pm0.006$ & $-10.169\substack{+0.002\\ -0.003}$ & $-10.199\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.357\substack{+0.008\\ -0.008}$ & $128.49$ & $99$ \\ 
58611.34 & $36.53\pm0.20$ & $-0.649\pm0.007$ & $-10.168\substack{+0.002\\ -0.003}$ & $-10.197\substack{+0.002\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.384\substack{+0.008\\ -0.008}$ & $97.32$ & $94$ \\ 
58612.95 & $32.34\pm0.17$ & $-0.657\pm0.006$ & $-10.234\substack{+0.003\\ -0.003}$ & $-10.266\substack{+0.003\\ -0.003}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.407\substack{+0.008\\ -0.008}$ & $117.25$ & $98$ \\ 
58614.95 & $36.71\pm0.18$ & $-0.669\pm0.006$ & $-10.193\substack{+0.003\\ -0.003}$ & $-10.221\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.419\substack{+0.008\\ -0.008}$ & $130.11$ & $146$ \\ 
58617.01 & $33.10\pm0.21$ & $-0.663\pm0.008$ & $-10.239\substack{+0.004\\ -0.003}$ & $-10.271\substack{+0.004\\ -0.003}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.415\substack{+0.008\\ -0.008}$ & $110.64$ & $93$ \\ 
58619.00 & $33.31\pm0.21$ & $-0.676\pm0.008$ & $-10.235\substack{+0.003\\ -0.003}$ & $-10.266\substack{+0.004\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.419\substack{+0.008\\ -0.008}$ & $107.12$ & $87$ \\ 
58621.13 & $36.86\pm0.32$ & $-0.681\pm0.011$ & $-10.205\substack{+0.004\\ -0.006}$ & $-10.234\substack{+0.005\\ -0.007}$ & $2.22\substack{+0.02\\ -0.02}$ & $-11.423\substack{+0.008\\ -0.008}$ & $53.73$ & $67$ \\ 
58623.22 & $33.07\pm0.18$ & $-0.676\pm0.007$ & $-10.241\substack{+0.003\\ -0.003}$ & $-10.271\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.431\substack{+0.008\\ -0.008}$ & $162.43$ & $109$ \\ 
58626.73 & $32.67\pm0.22$ & $-0.663\pm0.008$ & $-10.232\substack{+0.004\\ -0.004}$ & $-10.261\substack{+0.005\\ -0.005}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $76.84$ & $80$ \\ 
58632.66 & $27.86\pm0.20$ & $-0.660\pm0.009$ & $-10.317\substack{+0.004\\ -0.006}$ & $-10.350\substack{+0.005\\ -0.007}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.476\substack{+0.008\\ -0.008}$ & $94.11$ & $90$ \\ 
58635.56 & $36.35\pm0.21$ & $-0.680\pm0.007$ & $-10.222\substack{+0.003\\ -0.003}$ & $-10.251\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.452\substack{+0.008\\ -0.008}$ & $124.87$ & $100$ \\ 
58637.62 & $38.56\pm0.23$ & $-0.682\pm0.007$ & $-10.198\substack{+0.003\\ -0.003}$ & $-10.224\substack{+0.003\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.469\substack{+0.008\\ -0.008}$ & $111.25$ & $93$ \\ 
58643.87 & $46.92\pm0.30$ & $-0.682\pm0.008$ & $-10.113\substack{+0.004\\ -0.005}$ & $-10.139\substack{+0.005\\ -0.005}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.376\substack{+0.008\\ -0.008}$ & $123.79$ & $151$ \\ 
58646.07 & $38.67\pm0.32$ & $-0.697\pm0.010$ & $-10.205\substack{+0.005\\ -0.005}$ & $-10.237\substack{+0.005\\ -0.005}$ & $2.23\substack{+0.01\\ -0.02}$ & $-11.376\substack{+0.008\\ -0.008}$ & $202.96$ & $158$ \\ 
58651.93 & $35.50\pm0.22$ & $-0.673\pm0.007$ & $-10.228\substack{+0.003\\ -0.003}$ & $-10.262\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.370\substack{+0.008\\ -0.008}$ & $181.97$ & $153$ \\ 
58653.93 & $31.28\pm0.21$ & $-0.701\pm0.008$ & $-10.296\substack{+0.004\\ -0.003}$ & $-10.340\substack{+0.004\\ -0.004}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.332\substack{+0.008\\ -0.008}$ & $151.44$ & $114$ \\ 
58655.93 & $35.31\pm0.21$ & $-0.708\pm0.007$ & $-10.248\substack{+0.003\\ -0.003}$ & $-10.289\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.320\substack{+0.008\\ -0.008}$ & $127.21$ & $102$ \\ 
58657.96 & $40.59\pm0.25$ & $-0.697\pm0.008$ & $-10.183\substack{+0.003\\ -0.003}$ & $-10.218\substack{+0.003\\ -0.004}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.317\substack{+0.008\\ -0.008}$ & $117.54$ & $105$ \\ 
58660.24 & $38.45\pm0.24$ & $-0.685\pm0.008$ & $-10.200\substack{+0.004\\ -0.004}$ & $-10.235\substack{+0.004\\ -0.004}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.329\substack{+0.008\\ -0.008}$ & $564.69$ & $165$ \\ 
58662.04 & $32.16\pm0.25$ & $-0.691\pm0.010$ & $-10.279\substack{+0.004\\ -0.004}$ & $-10.323\substack{+0.005\\ -0.005}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.310\substack{+0.008\\ -0.008}$ & $287.89$ & $154$ \\ 
58664.24 & $37.66\pm0.24$ & $-0.690\pm0.008$ & $-10.211\substack{+0.003\\ -0.003}$ & $-10.250\substack{+0.004\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.296\substack{+0.008\\ -0.008}$ & $208.57$ & $156$ \\ 
58665.88 & $36.40\pm0.30$ & $-0.724\pm0.010$ & $-10.244\substack{+0.005\\ -0.005}$ & $-10.284\substack{+0.005\\ -0.006}$ & $2.31\substack{+0.02\\ -0.02}$ & $-11.316\substack{+0.008\\ -0.008}$ & $175.83$ & $157$ \\ 
58673.24 & $30.38\pm0.21$ & $-0.667\pm0.008$ & $-10.215\substack{+0.004\\ -0.004}$ & $-10.249\substack{+0.005\\ -0.005}$ & $2.11\substack{+0.01\\ -0.02}$ & $-11.368\substack{+0.008\\ -0.008}$ & $101.42$ & $82$ \\ 
58675.30 & $30.24\pm0.18$ & $-0.657\pm0.007$ & $-10.214\substack{+0.003\\ -0.004}$ & $-10.247\substack{+0.003\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.375\substack{+0.008\\ -0.008}$ & $130.78$ & $97$ \\ 
58677.17 & $26.79\pm0.15$ & $-0.670\pm0.007$ & $-10.284\substack{+0.003\\ -0.003}$ & $-10.322\substack{+0.003\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.391\substack{+0.008\\ -0.008}$ & $177.28$ & $128$ \\ 
58679.04 & $35.54\pm0.19$ & $-0.675\pm0.007$ & $-10.154\substack{+0.003\\ -0.003}$ & $-10.180\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.403\substack{+0.008\\ -0.008}$ & $145.99$ & $110$ \\ 
58680.40 & $31.60\pm0.21$ & $-0.688\pm0.008$ & $-10.214\substack{+0.005\\ -0.004}$ & $-10.243\substack{+0.005\\ -0.004}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.440\substack{+0.008\\ -0.008}$ & $138.47$ & $139$ \\ 
58683.23 & $27.42\pm0.14$ & $-0.673\pm0.006$ & $-10.267\substack{+0.003\\ -0.003}$ & $-10.297\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.462\substack{+0.008\\ -0.008}$ & $154.52$ & $148$ \\ 
58685.11 & $30.80\pm0.19$ & $-0.661\pm0.008$ & $-10.220\substack{+0.004\\ -0.004}$ & $-10.246\substack{+0.004\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.482\substack{+0.008\\ -0.008}$ & $120.40$ & $115$ \\ 
58687.54 & $29.88\pm0.23$ & $-0.644\pm0.009$ & $-10.224\substack{+0.004\\ -0.004}$ & $-10.249\substack{+0.004\\ -0.004}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.507\substack{+0.008\\ -0.008}$ & $127.76$ & $76$ \\ 
58690.12 & $20.31\pm0.18$ & $-0.617\pm0.010$ & $-10.439\substack{+0.005\\ -0.005}$ & $-10.476\substack{+0.006\\ -0.006}$ & $2.01\substack{+0.02\\ -0.02}$ & $-11.566\substack{+0.008\\ -0.008}$ & $130.87$ & $76$ \\ 
58691.79 & $28.48\pm0.18$ & $-0.649\pm0.008$ & $-10.310\substack{+0.003\\ -0.003}$ & $-10.339\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.522\substack{+0.008\\ -0.008}$ & $134.94$ & $90$ \\ 
58694.70 & $32.57\pm0.19$ & $-0.694\pm0.007$ & $-10.278\substack{+0.003\\ -0.003}$ & $-10.306\substack{+0.003\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.501\substack{+0.008\\ -0.008}$ & $141.93$ & $89$ \\ 
58699.98 & $38.80\pm0.25$ & $-0.688\pm0.008$ & $-10.200\substack{+0.004\\ -0.004}$ & $-10.223\substack{+0.004\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.502\substack{+0.008\\ -0.008}$ & $87.74$ & $87$ \\ 
58702.27 & $38.00\pm0.25$ & $-0.710\pm0.008$ & $-10.220\substack{+0.003\\ -0.003}$ & $-10.244\substack{+0.003\\ -0.003}$ & $2.31\substack{+0.01\\ -0.01}$ & $-11.521\substack{+0.008\\ -0.008}$ & $676.00$ & $159$ \\ 
58704.59 & $31.62\pm0.19$ & $-0.692\pm0.008$ & $-10.289\substack{+0.003\\ -0.003}$ & $-10.316\substack{+0.003\\ -0.003}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.528\substack{+0.008\\ -0.008}$ & $200.51$ & $153$ \\ 
58706.46 & $35.92\pm0.21$ & $-0.663\pm0.007$ & $-10.220\substack{+0.003\\ -0.003}$ & $-10.241\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.564\substack{+0.008\\ -0.008}$ & $130.72$ & $102$ \\ 
58711.99 & $24.65\pm0.21$ & $-0.625\pm0.010$ & $-10.367\substack{+0.004\\ -0.004}$ & $-10.391\substack{+0.005\\ -0.005}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.678\substack{+0.008\\ -0.008}$ & $104.24$ & $69$ \\ 
58712.05 & $25.71\pm0.22$ & $-0.638\pm0.010$ & $-10.353\substack{+0.005\\ -0.005}$ & $-10.376\substack{+0.005\\ -0.005}$ & $2.12\substack{+0.01\\ -0.02}$ & $-11.678\substack{+0.008\\ -0.008}$ & $65.75$ & $69$ \\ 
58713.92 & $28.70\pm0.19$ & $-0.618\pm0.008$ & $-10.290\substack{+0.004\\ -0.003}$ & $-10.311\substack{+0.004\\ -0.003}$ & $2.03\substack{+0.01\\ -0.01}$ & $-11.671\substack{+0.008\\ -0.008}$ & $108.49$ & $85$ \\ 
58715.57 & $31.88\pm0.19$ & $-0.639\pm0.007$ & $-10.258\substack{+0.003\\ -0.003}$ & $-10.277\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.669\substack{+0.008\\ -0.008}$ & $121.93$ & $87$ \\ 
58717.44 & $30.15\pm0.21$ & $-0.640\pm0.008$ & $-10.282\substack{+0.004\\ -0.004}$ & $-10.302\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.665\substack{+0.008\\ -0.008}$ & $137.74$ & $79$ \\ 
58719.05 & $27.66\pm0.17$ & $-0.641\pm0.007$ & $-10.320\substack{+0.003\\ -0.003}$ & $-10.342\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.659\substack{+0.008\\ -0.008}$ & $134.74$ & $86$ \\ 
58721.15 & $21.95\pm0.18$ & $-0.650\pm0.010$ & $-10.423\substack{+0.004\\ -0.005}$ & $-10.453\substack{+0.005\\ -0.005}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.635\substack{+0.008\\ -0.008}$ & $95.10$ & $78$ \\ 
58723.06 & $28.06\pm0.23$ & $-0.694\pm0.010$ & $-10.343\substack{+0.005\\ -0.005}$ & $-10.370\substack{+0.006\\ -0.006}$ & $2.25\substack{+0.02\\ -0.02}$ & $-11.613\substack{+0.008\\ -0.008}$ & $156.40$ & $158$ \\ 
58729.84 & $40.23\pm0.31$ & $-0.694\pm0.010$ & $-10.188\substack{+0.004\\ -0.005}$ & $-10.210\substack{+0.004\\ -0.005}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.518\substack{+0.008\\ -0.008}$ & $83.73$ & $90$ \\ 
58737.40 & $35.72\pm0.37$ & $-0.659\pm0.012$ & $-10.198\substack{+0.005\\ -0.007}$ & $-10.221\substack{+0.005\\ -0.008}$ & $2.20\substack{+0.01\\ -0.02}$ & $-11.525\substack{+0.008\\ -0.008}$ & $124.40$ & $133$ \\ 
58739.36 & $34.78\pm0.27$ & $-0.702\pm0.010$ & $-10.226\substack{+0.004\\ -0.004}$ & $-10.250\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.508\substack{+0.008\\ -0.008}$ & $218.03$ & $157$ \\ 
58740.65 & $34.32\pm0.28$ & $-0.708\pm0.010$ & $-10.234\substack{+0.005\\ -0.003}$ & $-10.261\substack{+0.005\\ -0.003}$ & $2.28\substack{+0.02\\ -0.01}$ & $-11.479\substack{+0.008\\ -0.008}$ & $149.45$ & $131$ \\ 
58742.97 & $36.31\pm0.28$ & $-0.699\pm0.010$ & $-10.216\substack{+0.006\\ -0.004}$ & $-10.243\substack{+0.006\\ -0.005}$ & $2.26\substack{+0.02\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $128.10$ & $100$ \\ 
58743.04 & $36.63\pm0.28$ & $-0.701\pm0.009$ & $-10.213\substack{+0.004\\ -0.004}$ & $-10.241\substack{+0.004\\ -0.004}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $190.57$ & $154$ \\ 
58744.91 & $33.75\pm0.22$ & $-0.680\pm0.008$ & $-10.228\substack{+0.004\\ -0.004}$ & $-10.257\substack{+0.004\\ -0.005}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $139.98$ & $130$ \\ 
58751.71 & $27.65\pm0.19$ & $-0.661\pm0.008$ & $-10.315\substack{+0.004\\ -0.005}$ & $-10.348\substack{+0.004\\ -0.005}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.472\substack{+0.008\\ -0.008}$ & $112.67$ & $120$ \\ 
58753.15 & $30.25\pm0.21$ & $-0.671\pm0.008$ & $-10.296\substack{+0.004\\ -0.002}$ & $-10.329\substack{+0.004\\ -0.002}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.460\substack{+0.008\\ -0.008}$ & $87.11$ & $81$ \\ 
58755.02 & $30.84\pm0.19$ & $-0.684\pm0.008$ & $-10.295\substack{+0.003\\ -0.004}$ & $-10.330\substack{+0.003\\ -0.004}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.425\substack{+0.008\\ -0.008}$ & $102.19$ & $98$ \\ 
58756.57 & $29.96\pm0.17$ & $-0.710\pm0.007$ & $-10.322\substack{+0.003\\ -0.003}$ & $-10.359\substack{+0.003\\ -0.003}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.435\substack{+0.008\\ -0.008}$ & $123.88$ & $103$ \\ 
58758.38 & $28.87\pm0.18$ & $-0.719\pm0.008$ & $-10.342\substack{+0.003\\ -0.003}$ & $-10.380\substack{+0.003\\ -0.003}$ & $2.30\substack{+0.01\\ -0.01}$ & $-11.444\substack{+0.008\\ -0.008}$ & $702.19$ & $156$ \\ 
58761.66 & $35.86\pm0.21$ & $-0.681\pm0.007$ & $-10.229\substack{+0.003\\ -0.003}$ & $-10.259\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.423\substack{+0.008\\ -0.008}$ & $149.40$ & $94$ \\ 
58765.31 & $38.11\pm0.19$ & $-0.683\pm0.006$ & $-10.204\substack{+0.003\\ -0.002}$ & $-10.232\substack{+0.004\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.443\substack{+0.008\\ -0.008}$ & $125.24$ & $113$ \\ 
58767.60 & $40.29\pm0.22$ & $-0.669\pm0.007$ & $-10.173\substack{+0.003\\ -0.003}$ & $-10.196\substack{+0.003\\ -0.003}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.488\substack{+0.008\\ -0.008}$ & $152.90$ & $113$ \\ 
58777.69 & $36.56\pm0.19$ & $-0.659\pm0.006$ & $-10.209\substack{+0.003\\ -0.004}$ & $-10.233\substack{+0.003\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.510\substack{+0.008\\ -0.008}$ & $102.06$ & $126$ \\ 
58779.17 & $35.53\pm0.17$ & $-0.655\pm0.006$ & $-10.219\substack{+0.002\\ -0.002}$ & $-10.245\substack{+0.002\\ -0.002}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.493\substack{+0.008\\ -0.008}$ & $142.22$ & $106$ \\ 
58781.20 & $31.67\pm0.21$ & $-0.697\pm0.008$ & $-10.291\substack{+0.006\\ -0.004}$ & $-10.322\substack{+0.007\\ -0.004}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.481\substack{+0.008\\ -0.008}$ & $144.23$ & $145$ \\ 
58783.30 & $33.12\pm0.21$ & $-0.659\pm0.008$ & $-10.243\substack{+0.004\\ -0.004}$ & $-10.270\substack{+0.004\\ -0.005}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.499\substack{+0.008\\ -0.008}$ & $219.18$ & $152$ \\ 
58785.09 & $35.36\pm0.25$ & $-0.691\pm0.009$ & $-10.241\substack{+0.003\\ -0.004}$ & $-10.267\substack{+0.004\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.506\substack{+0.008\\ -0.008}$ & $88.44$ & $82$ \\ 
58786.96 & $36.65\pm0.23$ & $-0.661\pm0.008$ & $-10.210\substack{+0.003\\ -0.003}$ & $-10.231\substack{+0.004\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.552\substack{+0.008\\ -0.008}$ & $142.93$ & $100$ \\ 
58789.28 & $26.58\pm0.15$ & $-0.640\pm0.007$ & $-10.335\substack{+0.003\\ -0.004}$ & $-10.363\substack{+0.003\\ -0.004}$ & $2.06\substack{+0.01\\ -0.01}$ & $-11.564\substack{+0.008\\ -0.008}$ & $107.39$ & $99$ \\ 
58791.61 & $30.42\pm0.20$ & $-0.635\pm0.008$ & $-10.274\substack{+0.003\\ -0.004}$ & $-10.299\substack{+0.004\\ -0.004}$ & $2.06\substack{+0.01\\ -0.01}$ & $-11.570\substack{+0.008\\ -0.008}$ & $81.56$ & $87$ \\ 
58793.60 & $29.84\pm0.21$ & $-0.649\pm0.008$ & $-10.290\substack{+0.004\\ -0.004}$ & $-10.316\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.566\substack{+0.008\\ -0.008}$ & $104.42$ & $83$ \\ 
58794.80 & $33.81\pm0.25$ & $-0.674\pm0.009$ & $-10.251\substack{+0.003\\ -0.004}$ & $-10.274\substack{+0.003\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.582\substack{+0.008\\ -0.008}$ & $90.65$ & $75$ \\ 
58800.52 & $35.15\pm0.24$ & $-0.673\pm0.008$ & $-10.208\substack{+0.003\\ -0.004}$ & $-10.228\substack{+0.003\\ -0.004}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.573\substack{+0.008\\ -0.008}$ & $175.79$ & $156$ \\ 
58801.97 & $38.00\pm0.23$ & $-0.658\pm0.007$ & $-10.173\substack{+0.003\\ -0.003}$ & $-10.192\substack{+0.003\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.565\substack{+0.008\\ -0.008}$ & $120.04$ & $114$ \\ 
58805.13 & $33.69\pm0.19$ & $-0.668\pm0.007$ & $-10.230\substack{+0.003\\ -0.005}$ & $-10.253\substack{+0.003\\ -0.005}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.561\substack{+0.008\\ -0.008}$ & $163.02$ & $143$ \\ 
58807.45 & $39.37\pm0.23$ & $-0.686\pm0.007$ & $-10.173\substack{+0.004\\ -0.004}$ & $-10.194\substack{+0.004\\ -0.004}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.524\substack{+0.008\\ -0.008}$ & $214.79$ & $156$ \\ 
58808.87 & $31.48\pm0.22$ & $-0.695\pm0.009$ & $-10.273\substack{+0.005\\ -0.004}$ & $-10.300\substack{+0.006\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.535\substack{+0.008\\ -0.008}$ & $148.74$ & $147$ \\ 
58810.94 & $30.17\pm0.25$ & $-0.686\pm0.010$ & $-10.285\substack{+0.004\\ -0.006}$ & $-10.311\substack{+0.004\\ -0.006}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.548\substack{+0.008\\ -0.008}$ & $113.17$ & $85$ \\ 
58811.00 & $30.44\pm0.26$ & $-0.644\pm0.010$ & $-10.271\substack{+0.005\\ -0.004}$ & $-10.297\substack{+0.006\\ -0.005}$ & $2.14\substack{+0.01\\ -0.02}$ & $-11.548\substack{+0.008\\ -0.008}$ & $85.14$ & $80$ \\ 
58812.59 & $30.29\pm0.23$ & $-0.675\pm0.009$ & $-10.299\substack{+0.004\\ -0.004}$ & $-10.325\substack{+0.004\\ -0.004}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.555\substack{+0.008\\ -0.008}$ & $91.59$ & $76$ \\ 
58815.65 & $26.20\pm0.17$ & $-0.628\pm0.008$ & $-10.334\substack{+0.004\\ -0.004}$ & $-10.363\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-11.556\substack{+0.008\\ -0.008}$ & $99.81$ & $90$ \\ 
58817.45 & $30.89\pm0.18$ & $-0.638\pm0.007$ & $-10.270\substack{+0.003\\ -0.003}$ & $-10.296\substack{+0.003\\ -0.003}$ & $2.07\substack{+0.01\\ -0.01}$ & $-11.531\substack{+0.008\\ -0.008}$ & $122.97$ & $94$ \\ 
58819.36 & $33.86\pm0.21$ & $-0.688\pm0.008$ & $-10.259\substack{+0.003\\ -0.003}$ & $-10.284\substack{+0.003\\ -0.003}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.535\substack{+0.008\\ -0.008}$ & $112.10$ & $84$ \\ 
58821.49 & $31.06\pm0.18$ & $-0.672\pm0.007$ & $-10.287\substack{+0.003\\ -0.004}$ & $-10.314\substack{+0.004\\ -0.005}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.537\substack{+0.008\\ -0.008}$ & $113.10$ & $104$ \\ 
58823.49 & $35.42\pm0.20$ & $-0.661\pm0.007$ & $-10.225\substack{+0.003\\ -0.003}$ & $-10.247\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.561\substack{+0.008\\ -0.008}$ & $88.31$ & $93$ \\ 
58825.62 & $30.69\pm0.19$ & $-0.655\pm0.007$ & $-10.283\substack{+0.003\\ -0.003}$ & $-10.308\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.567\substack{+0.008\\ -0.008}$ & $104.31$ & $92$ \\ 
58827.62 & $28.80\pm0.18$ & $-0.656\pm0.007$ & $-10.310\substack{+0.005\\ -0.003}$ & $-10.336\substack{+0.006\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.582\substack{+0.008\\ -0.008}$ & $125.84$ & $100$ \\ 
58829.88 & $29.41\pm0.20$ & $-0.658\pm0.008$ & $-10.293\substack{+0.006\\ -0.003}$ & $-10.321\substack{+0.006\\ -0.004}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.526\substack{+0.008\\ -0.008}$ & $88.57$ & $98$ \\ 
58832.01 & $31.03\pm0.25$ & $-0.660\pm0.010$ & $-10.253\substack{+0.004\\ -0.006}$ & $-10.279\substack{+0.004\\ -0.006}$ & $2.13\substack{+0.01\\ -0.02}$ & $-11.521\substack{+0.008\\ -0.008}$ & $82.93$ & $101$ \\ 
58833.86 & $37.97\pm0.35$ & $-0.639\pm0.011$ & $-10.161\substack{+0.005\\ -0.006}$ & $-10.181\substack{+0.005\\ -0.006}$ & $2.10\substack{+0.02\\ -0.01}$ & $-11.525\substack{+0.008\\ -0.008}$ & $57.28$ & $65$ \\ 
58835.88 & $36.90\pm0.28$ & $-0.659\pm0.009$ & $-10.168\substack{+0.004\\ -0.005}$ & $-10.190\substack{+0.005\\ -0.005}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.499\substack{+0.008\\ -0.008}$ & $91.39$ & $106$ \\ 
58836.01 & $37.06\pm0.29$ & $-0.658\pm0.009$ & $-10.174\substack{+0.005\\ -0.005}$ & $-10.197\substack{+0.005\\ -0.005}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.496\substack{+0.008\\ -0.008}$ & $115.03$ & $99$ \\ 
58844.21 & $37.74\pm0.24$ & $-0.705\pm0.008$ & $-10.191\substack{+0.003\\ -0.004}$ & $-10.218\substack{+0.003\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.439\substack{+0.008\\ -0.008}$ & $110.43$ & $79$ \\ 
58847.69 & $37.80\pm0.21$ & $-0.666\pm0.007$ & $-10.169\substack{+0.002\\ -0.003}$ & $-10.192\substack{+0.002\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.479\substack{+0.008\\ -0.008}$ & $119.53$ & $96$ \\ 
58849.83 & $31.86\pm0.20$ & $-0.650\pm0.007$ & $-10.223\substack{+0.004\\ -0.004}$ & $-10.248\substack{+0.004\\ -0.004}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.493\substack{+0.008\\ -0.008}$ & $111.75$ & $94$ \\ 
58851.80 & $31.06\pm0.24$ & $-0.647\pm0.009$ & $-10.243\substack{+0.004\\ -0.004}$ & $-10.269\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.02}$ & $-11.513\substack{+0.008\\ -0.008}$ & $327.59$ & $138$ \\ 
58853.64 & $31.07\pm0.28$ & $-0.627\pm0.011$ & $-10.230\substack{+0.005\\ -0.005}$ & $-10.255\substack{+0.006\\ -0.005}$ & $2.08\substack{+0.02\\ -0.02}$ & $-11.510\substack{+0.008\\ -0.008}$ & $76.26$ & $91$ \\ 
58855.80 & $34.52\pm0.22$ & $-0.646\pm0.008$ & $-10.195\substack{+0.004\\ -0.003}$ & $-10.218\substack{+0.004\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.521\substack{+0.008\\ -0.008}$ & $94.00$ & $111$ \\ 
58857.80 & $32.66\pm0.21$ & $-0.637\pm0.008$ & $-10.214\substack{+0.004\\ -0.004}$ & $-10.237\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.540\substack{+0.008\\ -0.008}$ & $113.35$ & $106$ \\ 
58859.80 & $30.51\pm0.26$ & $-0.590\pm0.010$ & $-10.228\substack{+0.005\\ -0.005}$ & $-10.251\substack{+0.005\\ -0.006}$ & $2.00\substack{+0.01\\ -0.01}$ & $-11.547\substack{+0.008\\ -0.008}$ & $75.49$ & $73$ \\ 
58861.80 & $30.66\pm0.20$ & $-0.596\pm0.008$ & $-10.228\substack{+0.004\\ -0.005}$ & $-10.252\substack{+0.004\\ -0.005}$ & $1.99\substack{+0.01\\ -0.01}$ & $-11.530\substack{+0.008\\ -0.008}$ & $93.25$ & $93$ \\ 
58863.61 & $25.28\pm0.16$ & $-0.619\pm0.007$ & $-10.325\substack{+0.003\\ -0.004}$ & $-10.357\substack{+0.004\\ -0.004}$ & $2.04\substack{+0.01\\ -0.01}$ & $-11.514\substack{+0.008\\ -0.008}$ & $137.98$ & $106$ \\ 
58865.22 & $29.97\pm0.18$ & $-0.649\pm0.007$ & $-10.274\substack{+0.004\\ -0.004}$ & $-10.303\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.501\substack{+0.008\\ -0.008}$ & $85.54$ & $107$ \\ 
58866.71 & $34.00\pm0.19$ & $-0.653\pm0.007$ & $-10.216\substack{+0.003\\ -0.003}$ & $-10.242\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.489\substack{+0.008\\ -0.008}$ & $239.41$ & $144$ \\ 
58868.85 & $32.17\pm0.25$ & $-0.691\pm0.009$ & $-10.259\substack{+0.004\\ -0.004}$ & $-10.288\substack{+0.004\\ -0.004}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.475\substack{+0.008\\ -0.008}$ & $70.57$ & $71$ \\ 
58870.84 & $36.59\pm0.17$ & $-0.650\pm0.006$ & $-10.177\substack{+0.002\\ -0.003}$ & $-10.201\substack{+0.002\\ -0.003}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.478\substack{+0.008\\ -0.008}$ & $165.25$ & $114$ \\ 
58871.67 & $33.62\pm0.31$ & $-0.667\pm0.011$ & $-10.215\substack{+0.006\\ -0.005}$ & $-10.241\substack{+0.006\\ -0.005}$ & $2.14\substack{+0.02\\ -0.02}$ & $-11.484\substack{+0.008\\ -0.008}$ & $65.20$ & $79$ \\ 
58873.22 & $34.76\pm0.17$ & $-0.669\pm0.006$ & $-10.217\substack{+0.003\\ -0.003}$ & $-10.242\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.495\substack{+0.008\\ -0.008}$ & $133.66$ & $130$ \\ 
58875.16 & $30.42\pm0.16$ & $-0.636\pm0.006$ & $-10.264\substack{+0.003\\ -0.003}$ & $-10.291\substack{+0.003\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.509\substack{+0.008\\ -0.008}$ & $113.46$ & $101$ \\ 
58876.97 & $27.16\pm0.16$ & $-0.649\pm0.007$ & $-10.314\substack{+0.003\\ -0.004}$ & $-10.344\substack{+0.003\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.522\substack{+0.008\\ -0.008}$ & $126.34$ & $122$ \\ 
58877.68 & $30.97\pm0.23$ & $-0.668\pm0.009$ & $-10.268\substack{+0.004\\ -0.004}$ & $-10.295\substack{+0.004\\ -0.004}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.527\substack{+0.008\\ -0.008}$ & $105.54$ & $101$ \\ 
58879.49 & $27.75\pm0.28$ & $-0.619\pm0.012$ & $-10.279\substack{+0.006\\ -0.006}$ & $-10.306\substack{+0.006\\ -0.006}$ & $2.04\substack{+0.02\\ -0.02}$ & $-11.527\substack{+0.008\\ -0.008}$ & $65.89$ & $60$ \\ 
58884.72 & $27.77\pm0.19$ & $-0.622\pm0.008$ & $-10.306\substack{+0.003\\ -0.004}$ & $-10.333\substack{+0.004\\ -0.004}$ & $2.02\substack{+0.01\\ -0.01}$ & $-11.554\substack{+0.008\\ -0.008}$ & $83.66$ & $102$ \\ 
58887.53 & $35.15\pm0.23$ & $-0.652\pm0.008$ & $-10.222\substack{+0.003\\ -0.003}$ & $-10.246\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.510\substack{+0.008\\ -0.008}$ & $126.86$ & $100$ \\ 
58889.57 & $32.17\pm0.18$ & $-0.673\pm0.007$ & $-10.233\substack{+0.003\\ -0.003}$ & $-10.258\substack{+0.004\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.505\substack{+0.008\\ -0.008}$ & $172.74$ & $151$ \\ 
58891.63 & $40.32\pm0.22$ & $-0.676\pm0.007$ & $-10.176\substack{+0.003\\ -0.003}$ & $-10.200\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.461\substack{+0.008\\ -0.008}$ & $140.43$ & $109$ \\ 
58893.40 & $36.16\pm0.23$ & $-0.693\pm0.008$ & $-10.206\substack{+0.003\\ -0.003}$ & $-10.233\substack{+0.004\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.442\substack{+0.008\\ -0.008}$ & $117.07$ & $81$ \\ 
58902.65 & $31.41\pm0.23$ & $-0.733\pm0.009$ & $-10.285\substack{+0.004\\ -0.004}$ & $-10.319\substack{+0.004\\ -0.004}$ & $2.35\substack{+0.01\\ -0.01}$ & $-11.430\substack{+0.008\\ -0.008}$ & $92.77$ & $66$ \\ 
58903.97 & $33.90\pm0.24$ & $-0.709\pm0.009$ & $-10.240\substack{+0.004\\ -0.003}$ & $-10.270\substack{+0.004\\ -0.003}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.432\substack{+0.008\\ -0.008}$ & $108.81$ & $69$ \\ 
58905.59 & $43.00\pm0.28$ & $-0.709\pm0.008$ & $-10.131\substack{+0.003\\ -0.003}$ & $-10.155\substack{+0.003\\ -0.003}$ & $2.31\substack{+0.01\\ -0.01}$ & $-11.435\substack{+0.008\\ -0.008}$ & $101.46$ & $71$ \\ 
58909.60 & $32.46\pm0.21$ & $-0.648\pm0.008$ & $-10.236\substack{+0.004\\ -0.005}$ & $-10.261\substack{+0.004\\ -0.005}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.510\substack{+0.008\\ -0.008}$ & $163.24$ & $141$ \\ 
58910.86 & $34.51\pm0.28$ & $-0.629\pm0.010$ & $-10.191\substack{+0.005\\ -0.005}$ & $-10.213\substack{+0.006\\ -0.005}$ & $2.10\substack{+0.02\\ -0.02}$ & $-11.531\substack{+0.008\\ -0.008}$ & $117.68$ & $78$ \\ 
58911.31 & $34.37\pm0.26$ & $-0.637\pm0.009$ & $-10.185\substack{+0.006\\ -0.005}$ & $-10.207\substack{+0.007\\ -0.005}$ & $2.07\substack{+0.02\\ -0.02}$ & $-11.531\substack{+0.008\\ -0.008}$ & $67.09$ & $77$ \\ 
58915.75 & $26.00\pm0.20$ & $-0.638\pm0.009$ & $-10.326\substack{+0.005\\ -0.004}$ & $-10.354\substack{+0.005\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.552\substack{+0.008\\ -0.008}$ & $126.47$ & $83$ \\ 
58917.39 & $25.67\pm0.27$ & $-0.623\pm0.013$ & $-10.315\substack{+0.007\\ -0.008}$ & $-10.342\substack{+0.007\\ -0.008}$ & $1.98\substack{+0.02\\ -0.02}$ & $-11.568\substack{+0.008\\ -0.008}$ & $66.39$ & $59$ \\ 
58919.20 & $32.75\pm0.21$ & $-0.620\pm0.008$ & $-10.211\substack{+0.004\\ -0.004}$ & $-10.232\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-11.586\substack{+0.008\\ -0.008}$ & $118.65$ & $82$ \\ 
58921.27 & $33.86\pm0.22$ & $-0.664\pm0.008$ & $-10.204\substack{+0.004\\ -0.004}$ & $-10.223\substack{+0.005\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.594\substack{+0.008\\ -0.008}$ & $115.00$ & $96$ \\ 
58923.07 & $33.89\pm0.22$ & $-0.646\pm0.008$ & $-10.221\substack{+0.003\\ -0.004}$ & $-10.241\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.601\substack{+0.008\\ -0.008}$ & $82.12$ & $84$ \\ 
58929.79 & $34.58\pm0.22$ & $-0.647\pm0.008$ & $-10.198\substack{+0.003\\ -0.004}$ & $-10.215\substack{+0.003\\ -0.004}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.629\substack{+0.008\\ -0.008}$ & $92.01$ & $86$ \\ 
58931.55 & $35.24\pm0.25$ & $-0.647\pm0.008$ & $-10.193\substack{+0.004\\ -0.004}$ & $-10.210\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.637\substack{+0.008\\ -0.008}$ & $97.95$ & $78$ \\ 
58933.41 & $33.83\pm0.21$ & $-0.627\pm0.007$ & $-10.196\substack{+0.003\\ -0.003}$ & $-10.214\substack{+0.003\\ -0.003}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.646\substack{+0.008\\ -0.008}$ & $94.79$ & $81$ \\ 
58935.42 & $33.10\pm0.21$ & $-0.621\pm0.007$ & $-10.202\substack{+0.003\\ -0.003}$ & $-10.219\substack{+0.003\\ -0.003}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.657\substack{+0.008\\ -0.008}$ & $123.43$ & $80$ \\ 
58937.60 & $28.60\pm0.22$ & $-0.626\pm0.009$ & $-10.268\substack{+0.005\\ -0.005}$ & $-10.288\substack{+0.005\\ -0.005}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.670\substack{+0.008\\ -0.008}$ & $86.02$ & $82$ \\ 
58939.87 & $32.34\pm0.17$ & $-0.627\pm0.006$ & $-10.229\substack{+0.003\\ -0.002}$ & $-10.246\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.674\substack{+0.008\\ -0.008}$ & $155.94$ & $146$ \\ 
58941.71 & $31.12\pm0.24$ & $-0.612\pm0.009$ & $-10.230\substack{+0.004\\ -0.004}$ & $-10.248\substack{+0.004\\ -0.004}$ & $2.04\substack{+0.01\\ -0.02}$ & $-11.671\substack{+0.008\\ -0.008}$ & $96.92$ & $71$ \\ 
58943.49 & $33.45\pm0.24$ & $-0.629\pm0.009$ & $-10.209\substack{+0.003\\ -0.005}$ & $-10.227\substack{+0.003\\ -0.005}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.655\substack{+0.008\\ -0.008}$ & $85.54$ & $75$ \\ 
58945.04 & $37.78\pm0.37$ & $-0.628\pm0.012$ & $-10.147\substack{+0.004\\ -0.006}$ & $-10.163\substack{+0.005\\ -0.006}$ & $2.12\substack{+0.02\\ -0.01}$ & $-11.639\substack{+0.008\\ -0.008}$ & $64.07$ & $57$ \\ 
58953.41 & $40.52\pm0.26$ & $-0.687\pm0.008$ & $-10.180\substack{+0.002\\ -0.004}$ & $-10.203\substack{+0.003\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.511\substack{+0.008\\ -0.008}$ & $212.71$ & $154$ \\ 
58955.66 & $49.36\pm0.30$ & $-0.703\pm0.007$ & $-10.105\substack{+0.003\\ -0.003}$ & $-10.124\substack{+0.003\\ -0.003}$ & $2.29\substack{+0.01\\ -0.01}$ & $-11.490\substack{+0.008\\ -0.008}$ & $130.62$ & $91$ \\ 
58957.37 & $49.75\pm0.26$ & $-0.713\pm0.006$ & $-10.106\substack{+0.003\\ -0.003}$ & $-10.126\substack{+0.003\\ -0.003}$ & $2.32\substack{+0.01\\ -0.01}$ & $-11.477\substack{+0.008\\ -0.008}$ & $142.12$ & $156$ \\ 
58963.86 & $44.47\pm0.28$ & $-0.689\pm0.008$ & $-10.124\substack{+0.004\\ -0.004}$ & $-10.146\substack{+0.004\\ -0.004}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.460\substack{+0.008\\ -0.008}$ & $170.24$ & $160$ \\ 
58969.26 & $47.01\pm0.29$ & $-0.684\pm0.008$ & $-10.077\substack{+0.002\\ -0.003}$ & $-10.099\substack{+0.003\\ -0.004}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.407\substack{+0.008\\ -0.008}$ & $88.30$ & $79$ \\ 
58971.20 & $41.61\pm0.27$ & $-0.663\pm0.008$ & $-10.125\substack{+0.003\\ -0.004}$ & $-10.151\substack{+0.003\\ -0.004}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.392\substack{+0.008\\ -0.008}$ & $88.63$ & $81$ \\ 
58973.33 & $40.99\pm0.21$ & $-0.681\pm0.006$ & $-10.136\substack{+0.002\\ -0.002}$ & $-10.163\substack{+0.002\\ -0.002}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.376\substack{+0.008\\ -0.008}$ & $140.42$ & $96$ \\ 
58975.26 & $41.59\pm0.22$ & $-0.716\pm0.007$ & $-10.155\substack{+0.002\\ -0.002}$ & $-10.184\substack{+0.002\\ -0.002}$ & $2.36\substack{+0.01\\ -0.01}$ & $-11.359\substack{+0.008\\ -0.008}$ & $200.23$ & $156$ \\ 
58977.26 & $44.15\pm0.21$ & $-0.666\pm0.006$ & $-10.107\substack{+0.002\\ -0.003}$ & $-10.135\substack{+0.002\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.341\substack{+0.008\\ -0.008}$ & $95.17$ & $108$ \\ 
58979.50 & $49.13\pm0.33$ & $-0.688\pm0.008$ & $-10.071\substack{+0.003\\ -0.003}$ & $-10.097\substack{+0.003\\ -0.003}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.321\substack{+0.008\\ -0.008}$ & $108.99$ & $78$ \\ 
58981.42 & $37.50\pm0.21$ & $-0.723\pm0.007$ & $-10.204\substack{+0.002\\ -0.003}$ & $-10.241\substack{+0.002\\ -0.004}$ & $2.31\substack{+0.01\\ -0.01}$ & $-11.305\substack{+0.008\\ -0.008}$ & $119.13$ & $88$ \\ 
58983.35 & $37.82\pm0.22$ & $-0.741\pm0.007$ & $-10.206\substack{+0.002\\ -0.003}$ & $-10.245\substack{+0.003\\ -0.003}$ & $2.35\substack{+0.01\\ -0.01}$ & $-11.290\substack{+0.008\\ -0.008}$ & $121.25$ & $86$ \\ 
58985.26 & $41.16\pm0.24$ & $-0.710\pm0.007$ & $-10.162\substack{+0.003\\ -0.004}$ & $-10.198\substack{+0.003\\ -0.004}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.276\substack{+0.008\\ -0.008}$ & $103.31$ & $103$ \\ 
58987.26 & $38.12\pm0.36$ & $-0.681\pm0.012$ & $-10.176\substack{+0.005\\ -0.006}$ & $-10.213\substack{+0.005\\ -0.006}$ & $2.21\substack{+0.02\\ -0.02}$ & $-11.275\substack{+0.008\\ -0.008}$ & $106.08$ & $65$ \\ 
58994.55 & $42.04\pm0.23$ & $-0.708\pm0.007$ & $-10.165\substack{+0.003\\ -0.003}$ & $-10.201\substack{+0.003\\ -0.003}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.276\substack{+0.008\\ -0.008}$ & $138.12$ & $117$ \\ 
59008.58 & $37.57\pm0.20$ & $-0.634\pm0.006$ & $-10.178\substack{+0.004\\ -0.002}$ & $-10.216\substack{+0.004\\ -0.003}$ & $2.00\substack{+0.01\\ -0.01}$ & $-11.264\substack{+0.008\\ -0.008}$ & $112.65$ & $120$ \\ 
59014.56 & $37.76\pm0.23$ & $-0.705\pm0.008$ & $-10.217\substack{+0.003\\ -0.005}$ & $-10.260\substack{+0.003\\ -0.005}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.262\substack{+0.008\\ -0.008}$ & $172.84$ & $118$ \\ 
59022.87 & $33.94\pm0.33$ & $-0.749\pm0.012$ & $-10.284\substack{+0.006\\ -0.006}$ & $-10.338\substack{+0.006\\ -0.006}$ & $2.35\substack{+0.02\\ -0.02}$ & $-11.234\substack{+0.008\\ -0.008}$ & $424.99$ & $156$ \\ 
59025.00 & $39.97\pm0.37$ & $-0.723\pm0.012$ & $-10.208\substack{+0.006\\ -0.004}$ & $-10.251\substack{+0.006\\ -0.005}$ & $2.33\substack{+0.01\\ -0.02}$ & $-11.252\substack{+0.008\\ -0.008}$ & $182.10$ & $135$ \\ 
59027.00 & $48.37\pm0.39$ & $-0.704\pm0.010$ & $-10.111\substack{+0.004\\ -0.004}$ & $-10.144\substack{+0.005\\ -0.005}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.269\substack{+0.008\\ -0.008}$ & $253.43$ & $151$ \\ 
59028.72 & $44.39\pm0.23$ & $-0.667\pm0.006$ & $-10.127\substack{+0.003\\ -0.003}$ & $-10.161\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.276\substack{+0.008\\ -0.008}$ & $144.60$ & $137$ \\ 
59029.88 & $38.04\pm0.32$ & $-0.675\pm0.010$ & $-10.193\substack{+0.005\\ -0.005}$ & $-10.231\substack{+0.006\\ -0.006}$ & $2.11\substack{+0.02\\ -0.02}$ & $-11.280\substack{+0.008\\ -0.008}$ & $69.72$ & $72$ \\ 
59034.31 & $37.51\pm0.27$ & $-0.688\pm0.009$ & $-10.182\substack{+0.004\\ -0.004}$ & $-10.218\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.298\substack{+0.008\\ -0.008}$ & $93.33$ & $74$ \\ 
59036.63 & $37.81\pm0.31$ & $-0.701\pm0.010$ & $-10.184\substack{+0.004\\ -0.005}$ & $-10.221\substack{+0.004\\ -0.005}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.295\substack{+0.008\\ -0.008}$ & $57.48$ & $67$ \\ 
59038.89 & $43.17\pm0.23$ & $-0.722\pm0.007$ & $-10.152\substack{+0.002\\ -0.002}$ & $-10.186\substack{+0.002\\ -0.003}$ & $2.32\substack{+0.01\\ -0.01}$ & $-11.290\substack{+0.008\\ -0.008}$ & $166.04$ & $115$ \\ 
59042.55 & $42.75\pm0.30$ & $-0.712\pm0.009$ & $-10.168\substack{+0.004\\ -0.004}$ & $-10.205\substack{+0.004\\ -0.004}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.282\substack{+0.008\\ -0.008}$ & $111.75$ & $120$ \\ 
59043.95 & $36.16\pm0.28$ & $-0.717\pm0.009$ & $-10.234\substack{+0.004\\ -0.004}$ & $-10.276\substack{+0.004\\ -0.004}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.281\substack{+0.008\\ -0.008}$ & $92.19$ & $70$ \\ 
59044.01 & $35.31\pm0.25$ & $-0.716\pm0.009$ & $-10.243\substack{+0.004\\ -0.004}$ & $-10.287\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.280\substack{+0.008\\ -0.008}$ & $91.81$ & $76$ \\ 
59053.90 & $41.03\pm0.22$ & $-0.698\pm0.006$ & $-10.151\substack{+0.003\\ -0.003}$ & $-10.188\substack{+0.003\\ -0.003}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.254\substack{+0.008\\ -0.008}$ & $101.90$ & $105$ \\ 
59056.47 & $36.38\pm0.22$ & $-0.725\pm0.008$ & $-10.235\substack{+0.003\\ -0.003}$ & $-10.281\substack{+0.003\\ -0.004}$ & $2.29\substack{+0.01\\ -0.01}$ & $-11.246\substack{+0.008\\ -0.008}$ & $168.20$ & $110$ \\ 
59060.66 & $41.92\pm0.23$ & $-0.701\pm0.007$ & $-10.163\substack{+0.002\\ -0.003}$ & $-10.200\substack{+0.003\\ -0.003}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.260\substack{+0.008\\ -0.008}$ & $98.26$ & $94$ \\ 
59062.59 & $46.46\pm0.27$ & $-0.691\pm0.007$ & $-10.113\substack{+0.003\\ -0.003}$ & $-10.145\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.278\substack{+0.008\\ -0.008}$ & $117.31$ & $86$ \\ 
59064.59 & $42.66\pm0.24$ & $-0.678\pm0.007$ & $-10.143\substack{+0.003\\ -0.003}$ & $-10.176\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.285\substack{+0.008\\ -0.008}$ & $103.78$ & $102$ \\ 
59066.56 & $44.38\pm0.25$ & $-0.688\pm0.007$ & $-10.131\substack{+0.003\\ -0.003}$ & $-10.164\substack{+0.003\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.292\substack{+0.008\\ -0.008}$ & $118.82$ & $89$ \\ 
59070.92 & $42.99\pm0.27$ & $-0.687\pm0.008$ & $-10.144\substack{+0.005\\ -0.005}$ & $-10.174\substack{+0.005\\ -0.006}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.334\substack{+0.008\\ -0.008}$ & $116.68$ & $108$ \\ 
59072.73 & $45.25\pm0.29$ & $-0.675\pm0.008$ & $-10.116\substack{+0.004\\ -0.005}$ & $-10.143\substack{+0.004\\ -0.006}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.343\substack{+0.008\\ -0.008}$ & $87.90$ & $124$ \\ 
59074.96 & $45.70\pm0.27$ & $-0.704\pm0.007$ & $-10.128\substack{+0.003\\ -0.004}$ & $-10.156\substack{+0.003\\ -0.004}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.356\substack{+0.008\\ -0.008}$ & $161.31$ & $153$ \\ 
59076.91 & $40.26\pm0.21$ & $-0.705\pm0.006$ & $-10.183\substack{+0.003\\ -0.002}$ & $-10.214\substack{+0.003\\ -0.003}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.366\substack{+0.008\\ -0.008}$ & $117.69$ & $99$ \\ 
59077.97 & $38.34\pm0.22$ & $-0.683\pm0.007$ & $-10.192\substack{+0.003\\ -0.003}$ & $-10.223\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.373\substack{+0.008\\ -0.008}$ & $123.83$ & $89$ \\ 
59080.91 & $37.63\pm0.22$ & $-0.675\pm0.007$ & $-10.195\substack{+0.003\\ -0.003}$ & $-10.226\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.390\substack{+0.008\\ -0.008}$ & $109.42$ & $90$ \\ 
59082.88 & $39.99\pm0.31$ & $-0.688\pm0.010$ & $-10.178\substack{+0.004\\ -0.004}$ & $-10.206\substack{+0.005\\ -0.004}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.402\substack{+0.008\\ -0.008}$ & $65.40$ & $72$ \\ 
59083.01 & $41.34\pm0.26$ & $-0.685\pm0.008$ & $-10.161\substack{+0.003\\ -0.003}$ & $-10.189\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.402\substack{+0.008\\ -0.008}$ & $117.30$ & $80$ \\ 
59084.93 & $30.51\pm0.24$ & $-0.670\pm0.010$ & $-10.284\substack{+0.005\\ -0.006}$ & $-10.319\substack{+0.006\\ -0.007}$ & $2.14\substack{+0.02\\ -0.01}$ & $-11.413\substack{+0.008\\ -0.008}$ & $151.78$ & $152$ \\ 
59088.99 & $33.91\pm0.27$ & $-0.687\pm0.010$ & $-10.249\substack{+0.004\\ -0.004}$ & $-10.279\substack{+0.005\\ -0.005}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.438\substack{+0.008\\ -0.008}$ & $189.64$ & $154$ \\ 
59093.97 & $24.00\pm0.30$ & $-0.646\pm0.015$ & $-10.380\substack{+0.009\\ -0.009}$ & $-10.421\substack{+0.009\\ -0.010}$ & $1.98\substack{+0.03\\ -0.03}$ & $-11.451\substack{+0.008\\ -0.008}$ & $83.43$ & $62$ \\ 
59095.94 & $36.93\pm0.24$ & $-0.679\pm0.008$ & $-10.206\substack{+0.003\\ -0.003}$ & $-10.234\substack{+0.004\\ -0.004}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.439\substack{+0.008\\ -0.008}$ & $87.49$ & $81$ \\ 
59101.27 & $42.51\pm0.26$ & $-0.701\pm0.007$ & $-10.119\substack{+0.003\\ -0.003}$ & $-10.141\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.449\substack{+0.008\\ -0.008}$ & $92.78$ & $114$ \\ 
59103.86 & $48.54\pm0.27$ & $-0.690\pm0.007$ & $-10.058\substack{+0.002\\ -0.004}$ & $-10.076\substack{+0.003\\ -0.004}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.468\substack{+0.008\\ -0.008}$ & $187.95$ & $145$ \\ 
59105.31 & $41.64\pm0.29$ & $-0.677\pm0.009$ & $-10.117\substack{+0.006\\ -0.005}$ & $-10.137\substack{+0.006\\ -0.005}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.479\substack{+0.008\\ -0.008}$ & $222.76$ & $151$ \\ 
59107.95 & $39.50\pm0.26$ & $-0.638\pm0.008$ & $-10.128\substack{+0.003\\ -0.005}$ & $-10.148\substack{+0.003\\ -0.005}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.506\substack{+0.008\\ -0.008}$ & $96.83$ & $104$ \\ 
59109.31 & $31.13\pm0.25$ & $-0.656\pm0.010$ & $-10.229\substack{+0.004\\ -0.006}$ & $-10.252\substack{+0.004\\ -0.006}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.539\substack{+0.008\\ -0.008}$ & $130.07$ & $111$ \\ 
59116.29 & $26.62\pm0.18$ & $-0.633\pm0.008$ & $-10.322\substack{+0.004\\ -0.004}$ & $-10.348\substack{+0.004\\ -0.004}$ & $2.06\substack{+0.01\\ -0.01}$ & $-11.608\substack{+0.008\\ -0.008}$ & $136.98$ & $93$ \\ 
59118.43 & $26.94\pm0.14$ & $-0.603\pm0.006$ & $-10.300\substack{+0.003\\ -0.003}$ & $-10.323\substack{+0.003\\ -0.003}$ & $1.98\substack{+0.01\\ -0.01}$ & $-11.628\substack{+0.008\\ -0.008}$ & $153.73$ & $120$ \\ 
59120.59 & $27.84\pm0.18$ & $-0.618\pm0.008$ & $-10.295\substack{+0.004\\ -0.004}$ & $-10.318\substack{+0.004\\ -0.004}$ & $2.02\substack{+0.01\\ -0.01}$ & $-11.623\substack{+0.008\\ -0.008}$ & $120.52$ & $106$ \\ 
59122.53 & $34.92\pm0.18$ & $-0.634\pm0.006$ & $-10.208\substack{+0.003\\ -0.003}$ & $-10.226\substack{+0.003\\ -0.003}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.618\substack{+0.008\\ -0.008}$ & $110.53$ & $106$ \\ 
59124.47 & $27.24\pm0.17$ & $-0.644\pm0.008$ & $-10.319\substack{+0.005\\ -0.004}$ & $-10.344\substack{+0.005\\ -0.005}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.614\substack{+0.008\\ -0.008}$ & $99.30$ & $111$ \\ 
59126.20 & $31.16\pm0.29$ & $-0.668\pm0.011$ & $-10.281\substack{+0.006\\ -0.005}$ & $-10.304\substack{+0.006\\ -0.006}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.610\substack{+0.008\\ -0.008}$ & $78.12$ & $64$ \\ 
59128.12 & $29.63\pm0.21$ & $-0.647\pm0.008$ & $-10.276\substack{+0.006\\ -0.003}$ & $-10.299\substack{+0.006\\ -0.003}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.605\substack{+0.008\\ -0.008}$ & $125.11$ & $115$ \\ 
59129.56 & $32.44\pm0.22$ & $-0.648\pm0.008$ & $-10.247\substack{+0.004\\ -0.004}$ & $-10.268\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.602\substack{+0.008\\ -0.008}$ & $108.16$ & $84$ \\ 
59130.75 & $35.43\pm0.25$ & $-0.637\pm0.008$ & $-10.203\substack{+0.004\\ -0.004}$ & $-10.222\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.599\substack{+0.008\\ -0.008}$ & $108.58$ & $86$ \\ 
59136.81 & $34.91\pm0.29$ & $-0.645\pm0.010$ & $-10.211\substack{+0.004\\ -0.004}$ & $-10.231\substack{+0.005\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.586\substack{+0.008\\ -0.008}$ & $95.18$ & $71$ \\ 
59138.33 & $35.45\pm0.22$ & $-0.656\pm0.008$ & $-10.212\substack{+0.003\\ -0.004}$ & $-10.233\substack{+0.003\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.583\substack{+0.008\\ -0.008}$ & $115.58$ & $89$ \\ 
59141.04 & $31.99\pm0.22$ & $-0.671\pm0.008$ & $-10.265\substack{+0.004\\ -0.004}$ & $-10.290\substack{+0.004\\ -0.005}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.553\substack{+0.008\\ -0.008}$ & $177.99$ & $142$ \\ 
59142.79 & $30.97\pm0.34$ & $-0.665\pm0.013$ & $-10.289\substack{+0.008\\ -0.007}$ & $-10.316\substack{+0.008\\ -0.007}$ & $2.14\substack{+0.02\\ -0.02}$ & $-11.534\substack{+0.008\\ -0.008}$ & $60.22$ & $69$ \\ 
59144.40 & $31.20\pm0.21$ & $-0.673\pm0.008$ & $-10.276\substack{+0.003\\ -0.004}$ & $-10.303\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.518\substack{+0.008\\ -0.008}$ & $125.67$ & $91$ \\ 
59148.93 & $32.97\pm0.23$ & $-0.661\pm0.008$ & $-10.245\substack{+0.004\\ -0.004}$ & $-10.272\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.493\substack{+0.008\\ -0.008}$ & $78.58$ & $85$ \\ 
59150.52 & $28.11\pm0.19$ & $-0.668\pm0.008$ & $-10.316\substack{+0.004\\ -0.003}$ & $-10.348\substack{+0.004\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.487\substack{+0.008\\ -0.008}$ & $99.89$ & $82$ \\ 
59151.84 & $31.53\pm0.19$ & $-0.683\pm0.007$ & $-10.277\substack{+0.004\\ -0.004}$ & $-10.307\substack{+0.004\\ -0.004}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.480\substack{+0.008\\ -0.008}$ & $88.99$ & $93$ \\ 
59153.87 & $27.91\pm0.18$ & $-0.688\pm0.008$ & $-10.331\substack{+0.003\\ -0.003}$ & $-10.366\substack{+0.003\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.461\substack{+0.008\\ -0.008}$ & $129.49$ & $84$ \\ 
59155.71 & $27.64\pm0.24$ & $-0.690\pm0.010$ & $-10.331\substack{+0.004\\ -0.004}$ & $-10.368\substack{+0.005\\ -0.005}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.443\substack{+0.008\\ -0.008}$ & $109.72$ & $67$ \\ 
59157.68 & $30.14\pm0.20$ & $-0.714\pm0.008$ & $-10.312\substack{+0.003\\ -0.003}$ & $-10.348\substack{+0.003\\ -0.003}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.426\substack{+0.008\\ -0.008}$ & $167.53$ & $77$ \\ 
59165.69 & $37.82\pm0.33$ & $-0.683\pm0.011$ & $-10.175\substack{+0.005\\ -0.005}$ & $-10.202\substack{+0.006\\ -0.006}$ & $2.22\substack{+0.02\\ -0.02}$ & $-11.429\substack{+0.008\\ -0.008}$ & $46.32$ & $72$ \\ 
59166.40 & $33.61\pm0.23$ & $-0.703\pm0.008$ & $-10.231\substack{+0.005\\ -0.005}$ & $-10.262\substack{+0.006\\ -0.005}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.427\substack{+0.008\\ -0.008}$ & $148.01$ & $149$ \\ 
59170.40 & $32.35\pm0.20$ & $-0.717\pm0.008$ & $-10.255\substack{+0.003\\ -0.004}$ & $-10.287\substack{+0.003\\ -0.004}$ & $2.29\substack{+0.01\\ -0.01}$ & $-11.424\substack{+0.008\\ -0.008}$ & $159.29$ & $155$ \\ 
59172.72 & $38.48\pm0.31$ & $-0.686\pm0.010$ & $-10.161\substack{+0.006\\ -0.005}$ & $-10.187\substack{+0.006\\ -0.005}$ & $2.19\substack{+0.02\\ -0.01}$ & $-11.430\substack{+0.008\\ -0.008}$ & $67.78$ & $79$ \\ 
59179.54 & $37.67\pm0.22$ & $-0.664\pm0.007$ & $-10.189\substack{+0.003\\ -0.003}$ & $-10.215\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.454\substack{+0.008\\ -0.008}$ & $134.11$ & $88$ \\ 
59181.25 & $32.02\pm0.23$ & $-0.662\pm0.009$ & $-10.258\substack{+0.003\\ -0.003}$ & $-10.287\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.475\substack{+0.008\\ -0.008}$ & $109.25$ & $78$ \\ 
59183.48 & $27.04\pm0.19$ & $-0.654\pm0.009$ & $-10.326\substack{+0.004\\ -0.004}$ & $-10.359\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.489\substack{+0.008\\ -0.008}$ & $130.06$ & $78$ \\ 
59185.35 & $28.47\pm0.18$ & $-0.657\pm0.008$ & $-10.306\substack{+0.003\\ -0.003}$ & $-10.337\substack{+0.003\\ -0.003}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.492\substack{+0.008\\ -0.008}$ & $182.12$ & $81$ \\ 
59187.36 & $29.42\pm0.29$ & $-0.670\pm0.012$ & $-10.303\substack{+0.006\\ -0.006}$ & $-10.334\substack{+0.006\\ -0.006}$ & $2.10\substack{+0.02\\ -0.02}$ & $-11.495\substack{+0.008\\ -0.008}$ & $73.38$ & $61$ \\ 
59189.60 & $25.62\pm0.26$ & $-0.676\pm0.012$ & $-10.353\substack{+0.005\\ -0.005}$ & $-10.389\substack{+0.006\\ -0.006}$ & $2.15\substack{+0.02\\ -0.02}$ & $-11.479\substack{+0.008\\ -0.008}$ & $80.86$ & $58$ \\ 
59191.30 & $26.49\pm0.23$ & $-0.689\pm0.010$ & $-10.336\substack{+0.005\\ -0.005}$ & $-10.371\substack{+0.005\\ -0.005}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.472\substack{+0.008\\ -0.008}$ & $517.81$ & $150$ \\ 
59192.98 & $33.15\pm0.27$ & $-0.661\pm0.010$ & $-10.234\substack{+0.005\\ -0.006}$ & $-10.262\substack{+0.006\\ -0.007}$ & $2.13\substack{+0.02\\ -0.02}$ & $-11.465\substack{+0.008\\ -0.008}$ & $121.70$ & $121$ \\ 
59193.11 & $33.30\pm0.29$ & $-0.672\pm0.010$ & $-10.229\substack{+0.006\\ -0.004}$ & $-10.257\substack{+0.006\\ -0.005}$ & $2.17\substack{+0.02\\ -0.02}$ & $-11.465\substack{+0.008\\ -0.008}$ & $174.56$ & $149$ \\ 
59195.20 & $35.22\pm0.38$ & $-0.693\pm0.013$ & $-10.207\substack{+0.006\\ -0.006}$ & $-10.232\substack{+0.006\\ -0.006}$ & $2.28\substack{+0.02\\ -0.02}$ & $-11.483\substack{+0.008\\ -0.008}$ & $189.56$ & $131$ \\ 
59213.22 & $28.92\pm0.18$ & $-0.615\pm0.008$ & $-10.245\substack{+0.004\\ -0.004}$ & $-10.271\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-11.507\substack{+0.008\\ -0.008}$ & $108.13$ & $98$ \\ 
59215.07 & $37.59\pm0.18$ & $-0.666\pm0.006$ & $-10.172\substack{+0.002\\ -0.002}$ & $-10.194\substack{+0.002\\ -0.002}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.499\substack{+0.008\\ -0.008}$ & $98.26$ & $99$ \\ 
59217.36 & $38.86\pm0.21$ & $-0.673\pm0.007$ & $-10.150\substack{+0.003\\ -0.003}$ & $-10.172\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.483\substack{+0.008\\ -0.008}$ & $183.44$ & $138$ \\ 
59219.49 & $28.87\pm0.16$ & $-0.673\pm0.007$ & $-10.277\substack{+0.004\\ -0.003}$ & $-10.307\substack{+0.004\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.484\substack{+0.008\\ -0.008}$ & $163.51$ & $148$ \\ 
59223.62 & $24.76\pm0.28$ & $-0.640\pm0.013$ & $-10.324\substack{+0.008\\ -0.008}$ & $-10.354\substack{+0.009\\ -0.008}$ & $2.10\substack{+0.02\\ -0.02}$ & $-11.525\substack{+0.008\\ -0.008}$ & $85.76$ & $74$ \\ 
59225.17 & $21.59\pm0.17$ & $-0.637\pm0.010$ & $-10.377\substack{+0.004\\ -0.004}$ & $-10.410\substack{+0.005\\ -0.005}$ & $2.04\substack{+0.01\\ -0.01}$ & $-11.539\substack{+0.008\\ -0.008}$ & $105.59$ & $73$ \\ 
59226.98 & $19.33\pm0.18$ & $-0.622\pm0.011$ & $-10.421\substack{+0.005\\ -0.005}$ & $-10.459\substack{+0.006\\ -0.006}$ & $2.04\substack{+0.02\\ -0.02}$ & $-11.527\substack{+0.008\\ -0.008}$ & $80.47$ & $68$ \\ 
59227.05 & $19.84\pm0.24$ & $-0.639\pm0.015$ & $-10.405\substack{+0.007\\ -0.006}$ & $-10.442\substack{+0.008\\ -0.007}$ & $2.02\substack{+0.02\\ -0.02}$ & $-11.525\substack{+0.008\\ -0.008}$ & $46.72$ & $53$ \\ 
59228.97 & $24.07\pm0.16$ & $-0.661\pm0.008$ & $-10.344\substack{+0.005\\ -0.003}$ & $-10.379\substack{+0.005\\ -0.003}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.483\substack{+0.008\\ -0.008}$ & $82.40$ & $95$ \\ 
59230.99 & $24.38\pm0.17$ & $-0.683\pm0.009$ & $-10.352\substack{+0.004\\ -0.004}$ & $-10.389\substack{+0.004\\ -0.005}$ & $2.19\substack{+0.02\\ -0.01}$ & $-11.471\substack{+0.008\\ -0.008}$ & $119.56$ & $71$ \\ 
59231.63 & $24.04\pm0.20$ & $-0.693\pm0.010$ & $-10.363\substack{+0.005\\ -0.005}$ & $-10.400\substack{+0.005\\ -0.006}$ & $2.22\substack{+0.02\\ -0.01}$ & $-11.474\substack{+0.008\\ -0.008}$ & $97.72$ & $63$ \\ 
59232.50 & $19.68\pm0.12$ & $-0.665\pm0.008$ & $-10.370\substack{+0.003\\ -0.003}$ & $-10.407\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.478\substack{+0.008\\ -0.008}$ & $198.56$ & $79$ \\ 
59233.39 & $19.70\pm0.15$ & $-0.668\pm0.009$ & $-10.381\substack{+0.005\\ -0.004}$ & $-10.419\substack{+0.005\\ -0.004}$ & $2.12\substack{+0.02\\ -0.02}$ & $-11.482\substack{+0.008\\ -0.008}$ & $87.31$ & $89$ \\ 
59234.98 & $14.04\pm0.11$ & $-0.654\pm0.009$ & $-10.512\substack{+0.004\\ -0.004}$ & $-10.564\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-11.481\substack{+0.008\\ -0.008}$ & $189.05$ & $72$ \\ 
59236.98 & $19.99\pm0.12$ & $-0.694\pm0.008$ & $-10.449\substack{+0.003\\ -0.003}$ & $-10.498\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.450\substack{+0.008\\ -0.008}$ & $113.49$ & $89$ \\ 
59239.46 & $19.57\pm0.11$ & $-0.729\pm0.007$ & $-10.401\substack{+0.003\\ -0.003}$ & $-10.449\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.407\substack{+0.008\\ -0.008}$ & $641.54$ & $161$ \\ 
59240.26 & $23.54\pm0.22$ & $-0.718\pm0.012$ & $-10.376\substack{+0.005\\ -0.005}$ & $-10.423\substack{+0.005\\ -0.006}$ & $2.29\substack{+0.02\\ -0.02}$ & $-11.391\substack{+0.008\\ -0.008}$ & $306.15$ & $148$ \\ 
59241.17 & $21.69\pm0.18$ & $-0.687\pm0.010$ & $-10.406\substack{+0.004\\ -0.009}$ & $-10.458\substack{+0.004\\ -0.010}$ & $2.17\substack{+0.02\\ -0.01}$ & $-11.374\substack{+0.008\\ -0.008}$ & $204.39$ & $156$ \\ 
59243.24 & $19.49\pm0.18$ & $-0.719\pm0.011$ & $-10.453\substack{+0.005\\ -0.005}$ & $-10.515\substack{+0.006\\ -0.006}$ & $2.22\substack{+0.02\\ -0.02}$ & $-11.350\substack{+0.008\\ -0.008}$ & $97.18$ & $69$ \\ 
59245.18 & $24.21\pm0.26$ & $-0.721\pm0.013$ & $-10.360\substack{+0.005\\ -0.006}$ & $-10.410\substack{+0.006\\ -0.006}$ & $2.29\substack{+0.02\\ -0.02}$ & $-11.340\substack{+0.008\\ -0.008}$ & $39.61$ & $51$ \\ 
59248.93 & $35.17\pm0.22$ & $-0.689\pm0.008$ & $-10.240\substack{+0.003\\ -0.004}$ & $-10.278\substack{+0.003\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.332\substack{+0.008\\ -0.008}$ & $118.58$ & $111$ \\ 
59253.49 & $32.87\pm0.21$ & $-0.740\pm0.008$ & $-10.239\substack{+0.003\\ -0.004}$ & $-10.280\substack{+0.004\\ -0.004}$ & $2.34\substack{+0.01\\ -0.01}$ & $-11.304\substack{+0.008\\ -0.008}$ & $102.88$ & $137$ \\ 
59255.41 & $33.54\pm0.24$ & $-0.729\pm0.009$ & $-10.237\substack{+0.003\\ -0.003}$ & $-10.277\substack{+0.004\\ -0.004}$ & $2.32\substack{+0.01\\ -0.01}$ & $-11.308\substack{+0.008\\ -0.008}$ & $109.49$ & $69$ \\ 
59257.23 & $39.19\pm0.27$ & $-0.727\pm0.009$ & $-10.187\substack{+0.003\\ -0.003}$ & $-10.222\substack{+0.004\\ -0.004}$ & $2.33\substack{+0.01\\ -0.01}$ & $-11.321\substack{+0.008\\ -0.008}$ & $190.72$ & $149$ \\ 
59258.56 & $37.23\pm0.29$ & $-0.704\pm0.009$ & $-10.224\substack{+0.005\\ -0.004}$ & $-10.261\substack{+0.005\\ -0.005}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.326\substack{+0.008\\ -0.008}$ & $136.19$ & $137$ \\ 


==> Table5.tex <==
58256.95 & $32.10\pm0.17$ & $1.10$ & $1652.00$ & $2.10\substack{+0.01\\ -0.01}$ & $115.28$ & $126$ \\ 
58257.00 & $31.14\pm0.22$ & $2.14$ & $809.00$ & $2.13\substack{+0.01\\ -0.02}$ & $111.59$ & $116$ \\ 
58272.38 & $37.25\pm0.20$ & $3.34$ & $1515.00$ & $2.16\substack{+0.01\\ -0.01}$ & $392.01$ & $158$ \\ 
58293.62 & $31.44\pm0.20$ & $4.24$ & $1103.00$ & $2.17\substack{+0.01\\ -0.01}$ & $166.26$ & $157$ \\ 
58294.65 & $31.56\pm0.18$ & $0.71$ & $1290.00$ & $2.13\substack{+0.01\\ -0.01}$ & $132.15$ & $98$ \\ 
58302.65 & $31.54\pm0.23$ & $5.81$ & $877.00$ & $2.14\substack{+0.01\\ -0.01}$ & $155.91$ & $151$ \\ 
58304.43 & $39.52\pm0.25$ & $7.31$ & $983.00$ & $2.15\substack{+0.01\\ -0.01}$ & $147.63$ & $154$ \\ 
58310.32 & $18.86\pm0.16$ & $0.54$ & $839.24$ & $1.99\substack{+0.01\\ -0.01}$ & $87.59$ & $76$ \\ 
58311.22 & $18.04\pm0.12$ & $0.69$ & $1450.00$ & $2.01\substack{+0.01\\ -0.01}$ & $103.18$ & $94$ \\ 
58312.21 & $21.85\pm0.16$ & $0.76$ & $977.00$ & $2.03\substack{+0.01\\ -0.01}$ & $80.29$ & $85$ \\ 
58313.57 & $26.69\pm0.16$ & $0.97$ & $1485.00$ & $2.09\substack{+0.01\\ -0.01}$ & $120.84$ & $104$ \\ 
58314.52 & $28.52\pm0.16$ & $1.10$ & $1555.00$ & $2.08\substack{+0.01\\ -0.01}$ & $129.26$ & $111$ \\ 
58315.30 & $25.77\pm0.15$ & $1.22$ & $1555.00$ & $2.06\substack{+0.01\\ -0.01}$ & $149.04$ & $108$ \\ 
58317.30 & $29.02\pm0.15$ & $4.33$ & $2125.00$ & $2.13\substack{+0.01\\ -0.01}$ & $259.14$ & $160$ \\ 
58318.58 & $30.28\pm0.22$ & $0.79$ & $771.68$ & $2.11\substack{+0.01\\ -0.01}$ & $93.63$ & $82$ \\ 
58325.65 & $26.17\pm0.18$ & $0.66$ & $930.00$ & $2.08\substack{+0.01\\ -0.01}$ & $98.33$ & $83$ \\ 
58327.16 & $28.68\pm0.17$ & $0.61$ & $1239.00$ & $2.03\substack{+0.01\\ -0.01}$ & $96.32$ & $93$ \\ 
58329.19 & $26.79\pm0.21$ & $0.72$ & $710.00$ & $2.06\substack{+0.01\\ -0.01}$ & $76.42$ & $78$ \\ 
58331.12 & $24.33\pm0.21$ & $0.99$ & $663.00$ & $2.06\substack{+0.02\\ -0.01}$ & $77.22$ & $80$ \\ 
58333.50 & $30.62\pm0.15$ & $0.72$ & $2112.00$ & $2.17\substack{+0.01\\ -0.01}$ & $148.89$ & $106$ \\ 
58336.46 & $35.74\pm0.22$ & $0.74$ & $992.00$ & $2.14\substack{+0.01\\ -0.01}$ & $137.96$ & $90$ \\ 
58338.59 & $30.92\pm0.20$ & $0.94$ & $1013.00$ & $2.13\substack{+0.01\\ -0.01}$ & $115.16$ & $90$ \\ 
58340.52 & $34.58\pm0.21$ & $0.85$ & $1011.00$ & $2.09\substack{+0.01\\ -0.01}$ & $128.81$ & $91$ \\ 
58342.64 & $33.97\pm0.21$ & $1.33$ & $1006.00$ & $2.05\substack{+0.01\\ -0.01}$ & $102.10$ & $97$ \\ 
58343.60 & $29.04\pm0.19$ & $1.31$ & $1012.00$ & $2.05\substack{+0.01\\ -0.01}$ & $112.02$ & $96$ \\ 
58345.21 & $29.22\pm0.21$ & $4.95$ & $952.00$ & $2.12\substack{+0.01\\ -0.01}$ & $373.38$ & $158$ \\ 
58348.86 & $29.65\pm0.20$ & $0.97$ & $900.00$ & $2.10\substack{+0.01\\ -0.01}$ & $69.20$ & $87$ \\ 
58350.96 & $29.08\pm0.19$ & $1.00$ & $1079.00$ & $2.15\substack{+0.01\\ -0.01}$ & $117.30$ & $93$ \\ 
58352.82 & $28.88\pm0.18$ & $0.88$ & $1120.00$ & $2.12\substack{+0.01\\ -0.01}$ & $121.40$ & $93$ \\ 
58354.82 & $29.34\pm0.18$ & $0.79$ & $1095.00$ & $2.11\substack{+0.01\\ -0.01}$ & $122.88$ & $91$ \\ 
58358.86 & $25.05\pm0.21$ & $7.41$ & $804.00$ & $2.09\substack{+0.02\\ -0.02}$ & $198.66$ & $158$ \\ 
58360.85 & $21.40\pm0.28$ & $9.00$ & $420.00$ & $2.04\substack{+0.02\\ -0.03}$ & $198.82$ & $149$ \\ 
58362.85 & $20.66\pm0.29$ & $12.40$ & $424.00$ & $2.10\substack{+0.02\\ -0.02}$ & $182.82$ & $153$ \\ 
58364.71 & $27.40\pm0.18$ & $5.81$ & $1236.00$ & $2.06\substack{+0.01\\ -0.01}$ & $207.45$ & $157$ \\ 
58367.94 & $32.67\pm0.31$ & $1.06$ & $401.00$ & $2.18\substack{+0.02\\ -0.01}$ & $86.64$ & $67$ \\ 
58369.77 & $24.50\pm0.15$ & $0.80$ & $1354.00$ & $2.10\substack{+0.01\\ -0.01}$ & $127.88$ & $96$ \\ 
58375.54 & $24.81\pm0.19$ & $4.41$ & $932.00$ & $2.14\substack{+0.01\\ -0.02}$ & $151.95$ & $152$ \\ 
58377.89 & $19.90\pm0.14$ & $1.59$ & $1202.00$ & $2.06\substack{+0.01\\ -0.01}$ & $140.16$ & $121$ \\ 
58379.95 & $20.58\pm0.14$ & $1.79$ & $1370.00$ & $2.03\substack{+0.01\\ -0.01}$ & $162.04$ & $135$ \\ 
58382.85 & $21.62\pm0.18$ & $1.89$ & $769.00$ & $2.04\substack{+0.01\\ -0.01}$ & $145.02$ & $108$ \\ 
58388.42 & $23.58\pm0.17$ & $0.65$ & $920.00$ & $2.08\substack{+0.01\\ -0.01}$ & $115.88$ & $81$ \\ 
58390.48 & $26.85\pm0.19$ & $0.70$ & $887.00$ & $2.09\substack{+0.01\\ -0.01}$ & $90.44$ & $83$ \\ 
58392.70 & $27.64\pm0.13$ & $0.81$ & $2306.00$ & $2.07\substack{+0.01\\ -0.01}$ & $175.79$ & $112$ \\ 
58394.92 & $19.79\pm0.12$ & $1.20$ & $1686.00$ & $2.00\substack{+0.01\\ -0.01}$ & $136.82$ & $107$ \\ 
58396.59 & $20.82\pm0.15$ & $0.63$ & $1193.00$ & $2.05\substack{+0.01\\ -0.01}$ & $127.19$ & $85$ \\ 
58398.59 & $26.75\pm0.18$ & $2.47$ & $1014.00$ & $2.00\substack{+0.01\\ -0.01}$ & $356.48$ & $118$ \\ 
58400.69 & $26.23\pm0.16$ & $3.60$ & $1481.00$ & $2.11\substack{+0.01\\ -0.01}$ & $161.18$ & $153$ \\ 
58402.59 & $26.26\pm0.18$ & $1.39$ & $1002.00$ & $2.12\substack{+0.01\\ -0.01}$ & $126.89$ & $91$ \\ 
58403.93 & $23.10\pm0.18$ & $0.92$ & $810.00$ & $2.09\substack{+0.01\\ -0.01}$ & $75.13$ & $82$ \\ 
58405.89 & $25.09\pm0.27$ & $1.14$ & $396.00$ & $2.16\substack{+0.02\\ -0.02}$ & $73.28$ & $63$ \\ 
58407.31 & $28.02\pm0.20$ & $0.77$ & $808.00$ & $2.13\substack{+0.01\\ -0.01}$ & $117.31$ & $79$ \\ 
58409.69 & $30.36\pm0.17$ & $0.80$ & $1358.00$ & $2.15\substack{+0.01\\ -0.01}$ & $154.76$ & $91$ \\ 
58412.07 & $22.70\pm0.17$ & $0.89$ & $994.00$ & $2.23\substack{+0.01\\ -0.01}$ & $82.79$ & $84$ \\ 
58414.51 & $26.96\pm0.15$ & $1.68$ & $1744.00$ & $2.24\substack{+0.01\\ -0.01}$ & $350.18$ & $131$ \\ 
58416.70 & $28.74\pm0.20$ & $2.40$ & $975.00$ & $2.30\substack{+0.01\\ -0.01}$ & $137.22$ & $115$ \\ 
58418.70 & $28.08\pm0.20$ & $2.14$ & $894.00$ & $2.24\substack{+0.01\\ -0.01}$ & $140.48$ & $115$ \\ 
58420.63 & $27.69\pm0.21$ & $2.75$ & $808.00$ & $2.15\substack{+0.01\\ -0.01}$ & $163.20$ & $132$ \\ 
58421.24 & $30.14\pm0.22$ & $1.27$ & $742.00$ & $2.13\substack{+0.01\\ -0.01}$ & $101.21$ & $83$ \\ 
58422.67 & $27.57\pm0.20$ & $0.82$ & $803.00$ & $2.06\substack{+0.01\\ -0.01}$ & $132.34$ & $84$ \\ 
58423.96 & $26.38\pm0.19$ & $0.65$ & $862.00$ & $2.04\substack{+0.01\\ -0.01}$ & $90.49$ & $80$ \\ 
58426.46 & $28.43\pm0.17$ & $0.63$ & $1215.00$ & $2.07\substack{+0.01\\ -0.01}$ & $195.81$ & $88$ \\ 
58428.20 & $34.08\pm0.18$ & $1.14$ & $1493.00$ & $2.14\substack{+0.01\\ -0.01}$ & $130.87$ & $110$ \\ 
58429.17 & $37.47\pm0.20$ & $1.00$ & $1273.00$ & $2.16\substack{+0.01\\ -0.01}$ & $157.08$ & $103$ \\ 
58430.07 & $38.37\pm0.29$ & $0.74$ & $538.00$ & $2.16\substack{+0.01\\ -0.01}$ & $85.57$ & $75$ \\ 
58431.16 & $35.76\pm0.21$ & $0.68$ & $1074.00$ & $2.15\substack{+0.01\\ -0.01}$ & $115.56$ & $88$ \\ 
58432.97 & $41.85\pm0.33$ & $1.25$ & $455.00$ & $2.14\substack{+0.01\\ -0.01}$ & $68.26$ & $79$ \\ 
58433.06 & $41.29\pm0.25$ & $0.79$ & $830.00$ & $2.14\substack{+0.01\\ -0.01}$ & $108.19$ & $89$ \\ 
58437.51 & $33.67\pm0.25$ & $5.88$ & $731.00$ & $2.17\substack{+0.01\\ -0.01}$ & $152.04$ & $154$ \\ 
58438.42 & $31.41\pm0.33$ & $2.01$ & $336.00$ & $2.20\substack{+0.02\\ -0.02}$ & $80.77$ & $73$ \\ 
58449.22 & $33.64\pm0.23$ & $2.41$ & $814.00$ & $2.14\substack{+0.01\\ -0.01}$ & $126.86$ & $133$ \\ 
58453.60 & $27.94\pm0.16$ & $0.58$ & $1408.00$ & $2.06\substack{+0.01\\ -0.01}$ & $171.88$ & $92$ \\ 
58455.11 & $23.92\pm0.19$ & $0.75$ & $785.00$ & $2.06\substack{+0.01\\ -0.01}$ & $72.09$ & $80$ \\ 
58456.98 & $21.99\pm0.16$ & $0.78$ & $991.00$ & $2.08\substack{+0.01\\ -0.02}$ & $66.63$ & $85$ \\ 
58458.91 & $22.51\pm0.16$ & $0.85$ & $1115.00$ & $2.11\substack{+0.01\\ -0.01}$ & $103.11$ & $87$ \\ 
58460.91 & $26.35\pm0.17$ & $1.18$ & $1193.00$ & $2.08\substack{+0.01\\ -0.01}$ & $96.31$ & $100$ \\ 
58462.90 & $22.98\pm0.17$ & $2.18$ & $1060.00$ & $2.00\substack{+0.01\\ -0.01}$ & $116.72$ & $114$ \\ 
58464.58 & $22.00\pm0.15$ & $1.07$ & $1146.00$ & $2.05\substack{+0.01\\ -0.01}$ & $77.95$ & $90$ \\ 
58466.18 & $23.48\pm0.18$ & $2.49$ & $904.00$ & $2.11\substack{+0.01\\ -0.01}$ & $235.39$ & $147$ \\ 
58469.02 & $19.93\pm0.17$ & $1.87$ & $873.00$ & $2.05\substack{+0.01\\ -0.01}$ & $112.18$ & $98$ \\ 
58470.68 & $21.22\pm0.16$ & $0.86$ & $973.00$ & $2.00\substack{+0.01\\ -0.01}$ & $113.98$ & $89$ \\ 
58471.77 & $27.22\pm0.24$ & $1.16$ & $548.00$ & $2.08\substack{+0.01\\ -0.01}$ & $102.51$ & $75$ \\ 
58473.91 & $28.53\pm0.19$ & $2.33$ & $1054.00$ & $2.08\substack{+0.01\\ -0.01}$ & $99.03$ & $118$ \\ 
58476.07 & $33.52\pm0.32$ & $1.33$ & $379.00$ & $2.14\substack{+0.02\\ -0.02}$ & $80.50$ & $75$ \\ 
58479.11 & $31.16\pm0.21$ & $0.74$ & $919.00$ & $2.14\substack{+0.01\\ -0.01}$ & $103.62$ & $86$ \\ 
58481.24 & $25.92\pm0.22$ & $4.95$ & $718.00$ & $2.16\substack{+0.02\\ -0.02}$ & $135.28$ & $151$ \\ 
58487.79 & $34.24\pm0.31$ & $1.89$ & $422.00$ & $2.20\substack{+0.02\\ -0.02}$ & $70.31$ & $78$ \\ 
58489.79 & $24.24\pm0.20$ & $1.62$ & $711.00$ & $2.12\substack{+0.01\\ -0.02}$ & $213.74$ & $114$ \\ 
58491.53 & $22.10\pm0.24$ & $1.87$ & $435.00$ & $2.05\substack{+0.02\\ -0.02}$ & $97.27$ & $81$ \\ 
58493.71 & $22.41\pm0.27$ & $4.30$ & $401.00$ & $2.26\substack{+0.03\\ -0.02}$ & $107.53$ & $123$ \\ 
58497.64 & $24.35\pm0.19$ & $1.45$ & $814.00$ & $2.11\substack{+0.02\\ -0.02}$ & $73.62$ & $92$ \\ 
58499.38 & $26.86\pm0.15$ & $3.30$ & $1772.00$ & $2.20\substack{+0.01\\ -0.01}$ & $183.98$ & $151$ \\ 
58500.48 & $27.29\pm0.16$ & $4.74$ & $1669.00$ & $2.29\substack{+0.01\\ -0.01}$ & $240.32$ & $154$ \\ 
58501.89 & $28.58\pm0.17$ & $1.43$ & $1534.00$ & $2.22\substack{+0.01\\ -0.01}$ & $130.64$ & $114$ \\ 
58503.24 & $26.48\pm0.14$ & $2.60$ & $2194.00$ & $2.27\substack{+0.01\\ -0.01}$ & $184.86$ & $144$ \\ 
58504.98 & $34.75\pm0.17$ & $1.65$ & $1887.00$ & $2.28\substack{+0.01\\ -0.01}$ & $177.62$ & $135$ \\ 
58506.33 & $34.73\pm0.17$ & $3.37$ & $2117.00$ & $2.24\substack{+0.01\\ -0.01}$ & $156.06$ & $156$ \\ 
58507.62 & $31.46\pm0.18$ & $2.76$ & $1516.00$ & $2.23\substack{+0.01\\ -0.01}$ & $161.93$ & $147$ \\ 
58511.87 & $27.25\pm0.18$ & $0.67$ & $1063.00$ & $2.25\substack{+0.01\\ -0.01}$ & $93.94$ & $80$ \\ 
58513.28 & $27.87\pm0.15$ & $2.11$ & $1828.00$ & $2.18\substack{+0.01\\ -0.01}$ & $162.33$ & $146$ \\ 
58514.73 & $28.34\pm0.16$ & $2.65$ & $1856.00$ & $2.27\substack{+0.01\\ -0.01}$ & $180.14$ & $146$ \\ 
58515.86 & $32.10\pm0.22$ & $1.98$ & $956.00$ & $2.30\substack{+0.01\\ -0.01}$ & $119.00$ & $106$ \\ 
58517.18 & $33.04\pm0.23$ & $0.97$ & $855.00$ & $2.26\substack{+0.01\\ -0.01}$ & $81.58$ & $81$ \\ 
58521.53 & $37.00\pm0.22$ & $0.64$ & $1053.00$ & $2.28\substack{+0.01\\ -0.01}$ & $111.48$ & $88$ \\ 
58523.50 & $35.71\pm0.20$ & $2.71$ & $1434.00$ & $2.19\substack{+0.01\\ -0.01}$ & $191.72$ & $134$ \\ 
58527.09 & $38.24\pm0.25$ & $0.71$ & $769.00$ & $2.32\substack{+0.01\\ -0.01}$ & $92.50$ & $79$ \\ 
58528.06 & $34.22\pm0.31$ & $0.87$ & $421.00$ & $2.29\substack{+0.02\\ -0.02}$ & $86.28$ & $61$ \\ 
58529.87 & $32.38\pm0.25$ & $1.74$ & $655.00$ & $2.22\substack{+0.02\\ -0.02}$ & $94.08$ & $90$ \\ 
58541.28 & $33.89\pm0.19$ & $0.58$ & $1394.00$ & $2.13\substack{+0.01\\ -0.01}$ & $108.78$ & $89$ \\ 
58544.08 & $39.58\pm0.23$ & $1.12$ & $1071.00$ & $2.14\substack{+0.01\\ -0.01}$ & $132.34$ & $96$ \\ 
58550.32 & $39.70\pm0.22$ & $0.64$ & $1228.00$ & $2.19\substack{+0.01\\ -0.01}$ & $107.41$ & $90$ \\ 
58553.35 & $36.42\pm0.22$ & $0.83$ & $972.00$ & $2.10\substack{+0.01\\ -0.01}$ & $96.88$ & $85$ \\ 
58556.06 & $40.45\pm0.24$ & $1.05$ & $971.00$ & $2.16\substack{+0.01\\ -0.01}$ & $89.15$ & $88$ \\ 
58561.50 & $29.64\pm0.16$ & $1.59$ & $1928.00$ & $2.15\substack{+0.01\\ -0.01}$ & $120.06$ & $118$ \\ 
58562.94 & $31.06\pm0.23$ & $1.02$ & $734.00$ & $2.21\substack{+0.01\\ -0.01}$ & $84.55$ & $73$ \\ 
58570.87 & $40.31\pm0.17$ & $1.23$ & $2567.00$ & $2.19\substack{+0.01\\ -0.01}$ & $158.49$ & $127$ \\ 
58581.35 & $40.49\pm0.27$ & $0.85$ & $711.00$ & $2.23\substack{+0.01\\ -0.01}$ & $81.44$ & $78$ \\ 
58586.70 & $40.70\pm0.30$ & $11.09$ & $718.00$ & $2.18\substack{+0.01\\ -0.02}$ & $204.66$ & $159$ \\ 
58588.63 & $48.96\pm0.29$ & $10.41$ & $991.00$ & $2.17\substack{+0.01\\ -0.01}$ & $213.39$ & $161$ \\ 
58591.05 & $42.26\pm0.25$ & $5.28$ & $1039.00$ & $2.20\substack{+0.01\\ -0.01}$ & $165.03$ & $159$ \\ 
58592.65 & $45.66\pm0.23$ & $3.92$ & $1311.00$ & $2.00\substack{+0.01\\ -0.01}$ & $923.56$ & $156$ \\ 
58594.91 & $42.32\pm0.25$ & $5.64$ & $984.00$ & $2.19\substack{+0.01\\ -0.01}$ & $244.99$ & $158$ \\ 
58603.42 & $37.96\pm0.27$ & $0.63$ & $660.00$ & $2.21\substack{+0.01\\ -0.01}$ & $94.98$ & $73$ \\ 
58611.34 & $36.53\pm0.20$ & $0.62$ & $1337.00$ & $2.09\substack{+0.01\\ -0.01}$ & $97.32$ & $94$ \\ 
58612.95 & $32.34\pm0.17$ & $0.68$ & $1620.00$ & $2.11\substack{+0.01\\ -0.01}$ & $117.25$ & $98$ \\ 
58617.01 & $33.10\pm0.21$ & $0.98$ & $1028.00$ & $2.10\substack{+0.01\\ -0.01}$ & $110.64$ & $93$ \\ 
58619.00 & $33.31\pm0.21$ & $0.82$ & $945.00$ & $2.14\substack{+0.01\\ -0.01}$ & $107.12$ & $87$ \\ 
58621.13 & $36.86\pm0.32$ & $0.82$ & $416.00$ & $2.22\substack{+0.02\\ -0.02}$ & $53.73$ & $67$ \\ 
58623.22 & $33.07\pm0.18$ & $1.31$ & $1419.00$ & $2.15\substack{+0.01\\ -0.01}$ & $162.43$ & $109$ \\ 
58626.73 & $32.67\pm0.22$ & $0.60$ & $818.00$ & $2.14\substack{+0.01\\ -0.01}$ & $76.84$ & $80$ \\ 
58632.66 & $27.86\pm0.20$ & $1.17$ & $832.00$ & $2.11\substack{+0.01\\ -0.01}$ & $94.11$ & $90$ \\ 
58635.56 & $36.35\pm0.21$ & $1.15$ & $1132.00$ & $2.19\substack{+0.01\\ -0.01}$ & $124.87$ & $100$ \\ 
58637.62 & $38.56\pm0.23$ & $1.16$ & $1027.00$ & $2.20\substack{+0.01\\ -0.01}$ & $111.25$ & $93$ \\ 
58643.87 & $46.92\pm0.30$ & $3.97$ & $746.00$ & $2.20\substack{+0.01\\ -0.01}$ & $123.79$ & $151$ \\ 
58646.07 & $38.67\pm0.32$ & $10.58$ & $571.00$ & $2.23\substack{+0.01\\ -0.02}$ & $202.96$ & $158$ \\ 
58651.93 & $35.50\pm0.22$ & $3.33$ & $1078.00$ & $2.15\substack{+0.01\\ -0.01}$ & $181.97$ & $153$ \\ 
58653.93 & $31.28\pm0.21$ & $1.33$ & $972.00$ & $2.21\substack{+0.01\\ -0.01}$ & $151.44$ & $114$ \\ 
58655.93 & $35.31\pm0.21$ & $1.21$ & $1123.00$ & $2.25\substack{+0.01\\ -0.01}$ & $127.21$ & $102$ \\ 
58657.96 & $40.59\pm0.25$ & $1.12$ & $832.00$ & $2.22\substack{+0.01\\ -0.01}$ & $117.54$ & $105$ \\ 
58660.24 & $38.45\pm0.24$ & $8.91$ & $1043.00$ & $2.18\substack{+0.01\\ -0.01}$ & $564.69$ & $165$ \\ 
58662.04 & $32.16\pm0.25$ & $4.92$ & $675.00$ & $2.17\substack{+0.01\\ -0.01}$ & $287.89$ & $154$ \\ 
58664.24 & $37.66\pm0.24$ & $4.20$ & $894.00$ & $2.19\substack{+0.01\\ -0.01}$ & $208.57$ & $156$ \\ 
58665.88 & $36.40\pm0.30$ & $8.55$ & $606.00$ & $2.31\substack{+0.02\\ -0.02}$ & $175.83$ & $157$ \\ 
58673.24 & $30.38\pm0.21$ & $0.64$ & $875.00$ & $2.11\substack{+0.01\\ -0.02}$ & $101.42$ & $82$ \\ 
58675.30 & $30.24\pm0.18$ & $0.75$ & $1244.00$ & $2.10\substack{+0.01\\ -0.01}$ & $130.78$ & $97$ \\ 
58677.17 & $26.79\pm0.15$ & $1.51$ & $1874.00$ & $2.13\substack{+0.01\\ -0.01}$ & $177.28$ & $128$ \\ 
58679.04 & $35.54\pm0.19$ & $1.13$ & $1353.00$ & $2.16\substack{+0.01\\ -0.01}$ & $145.99$ & $110$ \\ 
58680.40 & $31.60\pm0.21$ & $2.85$ & $988.00$ & $2.22\substack{+0.01\\ -0.01}$ & $138.47$ & $139$ \\ 
58683.23 & $27.42\pm0.14$ & $1.74$ & $2094.00$ & $2.16\substack{+0.01\\ -0.01}$ & $154.52$ & $148$ \\ 
58685.11 & $30.80\pm0.19$ & $1.87$ & $1135.00$ & $2.14\substack{+0.01\\ -0.01}$ & $120.40$ & $115$ \\ 
58687.54 & $29.88\pm0.23$ & $0.51$ & $674.00$ & $2.08\substack{+0.01\\ -0.01}$ & $127.76$ & $76$ \\ 
58690.12 & $20.31\pm0.18$ & $0.77$ & $733.00$ & $2.01\substack{+0.02\\ -0.02}$ & $130.87$ & $76$ \\ 
58691.79 & $28.48\pm0.18$ & $0.71$ & $1115.00$ & $2.09\substack{+0.01\\ -0.01}$ & $134.94$ & $90$ \\ 
58694.70 & $32.57\pm0.19$ & $0.71$ & $1194.00$ & $2.24\substack{+0.01\\ -0.01}$ & $141.93$ & $89$ \\ 
58699.98 & $38.80\pm0.25$ & $1.12$ & $769.00$ & $2.23\substack{+0.01\\ -0.01}$ & $87.74$ & $87$ \\ 
58702.27 & $38.00\pm0.25$ & $5.97$ & $911.00$ & $2.31\substack{+0.01\\ -0.01}$ & $676.00$ & $159$ \\ 
58704.59 & $31.62\pm0.19$ & $2.67$ & $1193.00$ & $2.23\substack{+0.01\\ -0.01}$ & $200.51$ & $153$ \\ 
58706.46 & $35.92\pm0.21$ & $1.47$ & $1102.00$ & $2.16\substack{+0.01\\ -0.01}$ & $130.72$ & $102$ \\ 
58711.99 & $24.65\pm0.21$ & $0.67$ & $628.00$ & $2.10\substack{+0.01\\ -0.01}$ & $104.24$ & $69$ \\ 
58712.05 & $25.71\pm0.22$ & $0.65$ & $610.00$ & $2.12\substack{+0.01\\ -0.02}$ & $65.75$ & $69$ \\ 
58713.92 & $28.70\pm0.19$ & $0.60$ & $1028.00$ & $2.03\substack{+0.01\\ -0.01}$ & $108.49$ & $85$ \\ 
58715.57 & $31.88\pm0.19$ & $0.59$ & $1152.00$ & $2.09\substack{+0.01\\ -0.01}$ & $121.93$ & $87$ \\ 
58717.44 & $30.15\pm0.21$ & $0.74$ & $834.00$ & $2.09\substack{+0.01\\ -0.01}$ & $137.74$ & $79$ \\ 
58719.05 & $27.66\pm0.17$ & $0.57$ & $1231.00$ & $2.09\substack{+0.01\\ -0.01}$ & $134.74$ & $86$ \\ 
58721.15 & $21.95\pm0.18$ & $0.57$ & $834.00$ & $2.09\substack{+0.01\\ -0.01}$ & $95.10$ & $78$ \\ 
58723.06 & $28.06\pm0.23$ & $7.51$ & $771.00$ & $2.25\substack{+0.02\\ -0.02}$ & $156.40$ & $158$ \\ 
58729.84 & $40.23\pm0.31$ & $1.96$ & $498.00$ & $2.26\substack{+0.01\\ -0.01}$ & $83.73$ & $90$ \\ 
58742.97 & $36.31\pm0.28$ & $2.53$ & $574.00$ & $2.26\substack{+0.02\\ -0.01}$ & $128.10$ & $100$ \\ 
58743.04 & $36.63\pm0.28$ & $6.74$ & $655.00$ & $2.27\substack{+0.01\\ -0.01}$ & $190.57$ & $154$ \\ 
58751.71 & $27.65\pm0.19$ & $1.37$ & $1006.00$ & $2.11\substack{+0.01\\ -0.01}$ & $112.67$ & $120$ \\ 
58753.15 & $30.25\pm0.21$ & $0.57$ & $824.00$ & $2.14\substack{+0.01\\ -0.01}$ & $87.11$ & $81$ \\ 
58755.02 & $30.84\pm0.19$ & $1.02$ & $1139.00$ & $2.18\substack{+0.01\\ -0.01}$ & $102.19$ & $98$ \\ 
58756.57 & $29.96\pm0.17$ & $1.11$ & $1396.00$ & $2.27\substack{+0.01\\ -0.01}$ & $123.88$ & $103$ \\ 
58758.38 & $28.87\pm0.18$ & $2.95$ & $1268.00$ & $2.30\substack{+0.01\\ -0.01}$ & $702.19$ & $156$ \\ 
58761.66 & $35.86\pm0.21$ & $0.89$ & $1065.00$ & $2.19\substack{+0.01\\ -0.01}$ & $149.40$ & $94$ \\ 
58765.31 & $38.11\pm0.19$ & $0.93$ & $1700.00$ & $2.20\substack{+0.01\\ -0.01}$ & $125.24$ & $113$ \\ 
58767.60 & $40.29\pm0.22$ & $1.58$ & $1227.00$ & $2.17\substack{+0.01\\ -0.01}$ & $152.90$ & $113$ \\ 
58777.69 & $36.56\pm0.19$ & $1.63$ & $1600.54$ & $2.14\substack{+0.01\\ -0.01}$ & $102.06$ & $126$ \\ 
58779.17 & $35.53\pm0.17$ & $0.74$ & $1835.00$ & $2.12\substack{+0.01\\ -0.01}$ & $142.22$ & $106$ \\ 
58781.20 & $31.67\pm0.21$ & $4.56$ & $984.00$ & $2.24\substack{+0.01\\ -0.01}$ & $144.23$ & $145$ \\ 
58783.30 & $33.12\pm0.21$ & $3.92$ & $1026.00$ & $2.13\substack{+0.01\\ -0.01}$ & $219.18$ & $152$ \\ 
58785.09 & $35.36\pm0.25$ & $0.94$ & $703.00$ & $2.23\substack{+0.01\\ -0.01}$ & $88.44$ & $82$ \\ 
58786.96 & $36.65\pm0.23$ & $1.51$ & $881.00$ & $2.15\substack{+0.01\\ -0.01}$ & $142.93$ & $100$ \\ 
58789.28 & $26.58\pm0.15$ & $0.65$ & $1506.00$ & $2.06\substack{+0.01\\ -0.01}$ & $107.39$ & $99$ \\ 
58791.61 & $30.42\pm0.20$ & $0.63$ & $996.00$ & $2.06\substack{+0.01\\ -0.01}$ & $81.56$ & $87$ \\ 
58793.60 & $29.84\pm0.21$ & $0.80$ & $832.00$ & $2.10\substack{+0.01\\ -0.01}$ & $104.42$ & $83$ \\ 
58794.80 & $33.81\pm0.25$ & $0.62$ & $663.00$ & $2.19\substack{+0.01\\ -0.01}$ & $90.65$ & $75$ \\ 
58801.97 & $38.00\pm0.23$ & $1.62$ & $933.00$ & $2.13\substack{+0.01\\ -0.01}$ & $120.04$ & $114$ \\ 
58805.13 & $33.69\pm0.19$ & $3.32$ & $1375.00$ & $2.16\substack{+0.01\\ -0.01}$ & $163.02$ & $143$ \\ 
58808.87 & $31.48\pm0.22$ & $3.60$ & $897.00$ & $2.23\substack{+0.01\\ -0.01}$ & $148.74$ & $147$ \\ 
58810.94 & $30.17\pm0.25$ & $1.63$ & $594.00$ & $2.19\substack{+0.01\\ -0.01}$ & $113.17$ & $85$ \\ 
58811.00 & $30.44\pm0.26$ & $1.61$ & $540.00$ & $2.14\substack{+0.01\\ -0.02}$ & $85.14$ & $80$ \\ 
58812.59 & $30.29\pm0.23$ & $0.66$ & $699.00$ & $2.18\substack{+0.01\\ -0.01}$ & $91.59$ & $76$ \\ 
58815.65 & $26.20\pm0.17$ & $0.63$ & $1147.00$ & $2.03\substack{+0.01\\ -0.01}$ & $99.81$ & $90$ \\ 
58817.45 & $30.89\pm0.18$ & $0.60$ & $1294.00$ & $2.07\substack{+0.01\\ -0.01}$ & $122.97$ & $94$ \\ 
58819.36 & $33.86\pm0.21$ & $0.68$ & $971.00$ & $2.23\substack{+0.01\\ -0.01}$ & $112.10$ & $84$ \\ 
58821.49 & $31.06\pm0.18$ & $1.01$ & $1263.00$ & $2.17\substack{+0.01\\ -0.01}$ & $113.10$ & $104$ \\ 
58823.49 & $35.42\pm0.20$ & $0.65$ & $1174.00$ & $2.15\substack{+0.01\\ -0.01}$ & $88.31$ & $93$ \\ 
58825.62 & $30.69\pm0.19$ & $0.82$ & $1142.00$ & $2.12\substack{+0.01\\ -0.01}$ & $104.31$ & $92$ \\ 
58827.62 & $28.80\pm0.18$ & $1.22$ & $1222.00$ & $2.12\substack{+0.01\\ -0.01}$ & $125.84$ & $100$ \\ 
58829.88 & $29.41\pm0.20$ & $1.88$ & $976.00$ & $2.12\substack{+0.01\\ -0.01}$ & $88.57$ & $98$ \\ 
58832.01 & $31.03\pm0.25$ & $2.67$ & $611.00$ & $2.13\substack{+0.01\\ -0.02}$ & $82.93$ & $101$ \\ 
58833.86 & $37.97\pm0.35$ & $0.70$ & $357.00$ & $2.10\substack{+0.02\\ -0.01}$ & $57.28$ & $65$ \\ 
58844.21 & $37.74\pm0.24$ & $0.61$ & $834.00$ & $2.26\substack{+0.01\\ -0.01}$ & $110.43$ & $79$ \\ 
58847.69 & $37.80\pm0.21$ & $0.92$ & $1266.00$ & $2.14\substack{+0.01\\ -0.01}$ & $119.53$ & $96$ \\ 
58849.83 & $31.86\pm0.20$ & $0.86$ & $1067.00$ & $2.08\substack{+0.01\\ -0.01}$ & $111.75$ & $94$ \\ 
58851.80 & $31.06\pm0.24$ & $2.58$ & $705.00$ & $2.13\substack{+0.01\\ -0.02}$ & $327.59$ & $138$ \\ 
58853.64 & $31.07\pm0.28$ & $2.47$ & $499.00$ & $2.08\substack{+0.02\\ -0.02}$ & $76.26$ & $91$ \\ 
58855.80 & $34.52\pm0.22$ & $1.32$ & $896.00$ & $2.12\substack{+0.01\\ -0.01}$ & $94.00$ & $111$ \\ 
58857.80 & $32.66\pm0.21$ & $1.57$ & $927.00$ & $2.09\substack{+0.01\\ -0.01}$ & $113.35$ & $106$ \\ 
58859.80 & $30.51\pm0.26$ & $0.86$ & $542.00$ & $2.00\substack{+0.01\\ -0.01}$ & $75.49$ & $73$ \\ 
58861.80 & $30.66\pm0.20$ & $0.77$ & $1013.54$ & $1.99\substack{+0.01\\ -0.01}$ & $93.25$ & $93$ \\ 
58863.61 & $25.28\pm0.16$ & $0.85$ & $1383.00$ & $2.04\substack{+0.01\\ -0.01}$ & $137.98$ & $106$ \\ 
58865.22 & $29.97\pm0.18$ & $1.71$ & $1280.00$ & $2.11\substack{+0.01\\ -0.01}$ & $85.54$ & $107$ \\ 
58866.71 & $34.00\pm0.19$ & $1.70$ & $1446.00$ & $2.15\substack{+0.01\\ -0.01}$ & $239.41$ & $144$ \\ 
58870.84 & $36.59\pm0.17$ & $0.99$ & $2072.00$ & $2.11\substack{+0.01\\ -0.01}$ & $165.25$ & $114$ \\ 
58871.67 & $33.62\pm0.31$ & $1.81$ & $422.00$ & $2.14\substack{+0.02\\ -0.02}$ & $65.20$ & $79$ \\ 
58873.22 & $34.76\pm0.17$ & $1.56$ & $1895.00$ & $2.15\substack{+0.01\\ -0.01}$ & $133.66$ & $130$ \\ 
58875.16 & $30.42\pm0.16$ & $1.00$ & $1752.00$ & $2.09\substack{+0.01\\ -0.01}$ & $113.46$ & $101$ \\ 
58876.97 & $27.16\pm0.16$ & $1.91$ & $1684.00$ & $2.09\substack{+0.01\\ -0.01}$ & $126.34$ & $122$ \\ 
58877.68 & $30.97\pm0.23$ & $1.27$ & $747.00$ & $2.16\substack{+0.01\\ -0.01}$ & $105.54$ & $101$ \\ 
58879.49 & $27.75\pm0.28$ & $0.75$ & $396.00$ & $2.04\substack{+0.02\\ -0.02}$ & $65.89$ & $60$ \\ 
58884.72 & $27.77\pm0.19$ & $1.00$ & $900.00$ & $2.02\substack{+0.01\\ -0.01}$ & $83.66$ & $102$ \\ 
58887.53 & $35.15\pm0.23$ & $1.59$ & $898.00$ & $2.11\substack{+0.01\\ -0.01}$ & $126.86$ & $100$ \\ 
58889.57 & $32.17\pm0.18$ & $3.41$ & $1671.00$ & $2.15\substack{+0.01\\ -0.01}$ & $172.74$ & $151$ \\ 
58891.63 & $40.32\pm0.22$ & $1.21$ & $1152.00$ & $2.19\substack{+0.01\\ -0.01}$ & $140.43$ & $109$ \\ 
58893.40 & $36.16\pm0.23$ & $0.86$ & $916.00$ & $2.24\substack{+0.01\\ -0.01}$ & $117.07$ & $81$ \\ 
58902.65 & $31.41\pm0.23$ & $0.60$ & $743.00$ & $2.35\substack{+0.01\\ -0.01}$ & $92.77$ & $66$ \\ 
58905.59 & $43.00\pm0.28$ & $0.61$ & $709.00$ & $2.31\substack{+0.01\\ -0.01}$ & $101.46$ & $71$ \\ 
58909.60 & $32.46\pm0.21$ & $3.17$ & $1098.00$ & $2.15\substack{+0.01\\ -0.01}$ & $163.24$ & $141$ \\ 
58915.75 & $26.00\pm0.20$ & $1.19$ & $781.00$ & $2.11\substack{+0.01\\ -0.01}$ & $126.47$ & $83$ \\ 
58917.39 & $25.67\pm0.27$ & $0.85$ & $392.00$ & $1.98\substack{+0.02\\ -0.02}$ & $66.39$ & $59$ \\ 
58919.20 & $32.75\pm0.21$ & $0.91$ & $931.00$ & $2.05\substack{+0.01\\ -0.01}$ & $118.65$ & $82$ \\ 
58923.07 & $33.89\pm0.22$ & $1.18$ & $938.00$ & $2.13\substack{+0.01\\ -0.01}$ & $82.12$ & $84$ \\ 
58933.41 & $33.83\pm0.21$ & $0.60$ & $1013.00$ & $2.10\substack{+0.01\\ -0.01}$ & $94.79$ & $81$ \\ 
58935.42 & $33.10\pm0.21$ & $0.55$ & $1005.00$ & $2.08\substack{+0.01\\ -0.01}$ & $123.43$ & $80$ \\ 
58937.60 & $28.60\pm0.22$ & $1.18$ & $720.00$ & $2.08\substack{+0.01\\ -0.01}$ & $86.02$ & $82$ \\ 
58939.87 & $32.34\pm0.17$ & $2.06$ & $1736.00$ & $2.12\substack{+0.01\\ -0.01}$ & $155.94$ & $146$ \\ 
58941.71 & $31.12\pm0.24$ & $0.61$ & $675.00$ & $2.04\substack{+0.01\\ -0.02}$ & $96.92$ & $71$ \\ 
58943.49 & $33.45\pm0.24$ & $0.54$ & $706.00$ & $2.09\substack{+0.01\\ -0.01}$ & $85.54$ & $75$ \\ 
58945.04 & $37.78\pm0.37$ & $0.57$ & $316.00$ & $2.12\substack{+0.02\\ -0.01}$ & $64.07$ & $57$ \\ 
58953.41 & $40.52\pm0.26$ & $4.09$ & $867.00$ & $2.23\substack{+0.01\\ -0.01}$ & $212.71$ & $154$ \\ 
58955.66 & $49.36\pm0.30$ & $1.25$ & $751.00$ & $2.29\substack{+0.01\\ -0.01}$ & $130.62$ & $91$ \\ 
58957.37 & $49.75\pm0.26$ & $6.08$ & $1270.00$ & $2.32\substack{+0.01\\ -0.01}$ & $142.12$ & $156$ \\ 
58963.86 & $44.47\pm0.28$ & $8.48$ & $869.00$ & $2.24\substack{+0.01\\ -0.01}$ & $170.24$ & $160$ \\ 
58994.55 & $42.04\pm0.23$ & $1.28$ & $1181.00$ & $2.26\substack{+0.01\\ -0.01}$ & $138.12$ & $117$ \\ 
59008.58 & $37.57\pm0.20$ & $1.42$ & $1437.00$ & $2.00\substack{+0.01\\ -0.01}$ & $112.65$ & $120$ \\ 
59014.56 & $37.76\pm0.23$ & $1.45$ & $938.00$ & $2.23\substack{+0.01\\ -0.01}$ & $172.84$ & $118$ \\ 
59022.87 & $33.94\pm0.33$ & $11.24$ & $455.00$ & $2.35\substack{+0.02\\ -0.02}$ & $424.99$ & $156$ \\ 
59025.00 & $39.97\pm0.37$ & $4.44$ & $363.00$ & $2.33\substack{+0.01\\ -0.02}$ & $182.10$ & $135$ \\ 
59028.72 & $44.39\pm0.23$ & $1.73$ & $1242.00$ & $2.13\substack{+0.01\\ -0.01}$ & $144.60$ & $137$ \\ 
59029.88 & $38.04\pm0.32$ & $0.96$ & $430.00$ & $2.11\substack{+0.02\\ -0.02}$ & $69.72$ & $72$ \\ 
59044.01 & $35.31\pm0.25$ & $0.61$ & $689.00$ & $2.26\substack{+0.01\\ -0.01}$ & $91.81$ & $76$ \\ 
59053.90 & $41.03\pm0.22$ & $1.59$ & $1347.00$ & $2.22\substack{+0.01\\ -0.01}$ & $101.90$ & $105$ \\ 
59056.47 & $36.38\pm0.22$ & $1.05$ & $1024.00$ & $2.29\substack{+0.01\\ -0.01}$ & $168.20$ & $110$ \\ 
59060.66 & $41.92\pm0.23$ & $0.64$ & $1194.00$ & $2.23\substack{+0.01\\ -0.01}$ & $98.26$ & $94$ \\ 
59062.59 & $46.46\pm0.27$ & $0.56$ & $886.00$ & $2.21\substack{+0.01\\ -0.01}$ & $117.31$ & $86$ \\ 
59064.59 & $42.66\pm0.24$ & $1.16$ & $1053.00$ & $2.16\substack{+0.01\\ -0.01}$ & $103.78$ & $102$ \\ 
59066.56 & $44.38\pm0.25$ & $0.66$ & $994.00$ & $2.20\substack{+0.01\\ -0.01}$ & $118.82$ & $89$ \\ 
59070.92 & $42.99\pm0.27$ & $2.05$ & $778.00$ & $2.20\substack{+0.01\\ -0.01}$ & $116.68$ & $108$ \\ 
59072.73 & $45.25\pm0.29$ & $3.35$ & $722.00$ & $2.17\substack{+0.01\\ -0.01}$ & $87.90$ & $124$ \\ 
59074.96 & $45.70\pm0.27$ & $4.03$ & $952.00$ & $2.27\substack{+0.01\\ -0.01}$ & $161.31$ & $153$ \\ 
59076.91 & $40.26\pm0.21$ & $0.74$ & $1420.00$ & $2.26\substack{+0.01\\ -0.01}$ & $117.69$ & $99$ \\ 
59077.97 & $38.34\pm0.22$ & $0.62$ & $1064.00$ & $2.19\substack{+0.01\\ -0.01}$ & $123.83$ & $89$ \\ 
59080.91 & $37.63\pm0.22$ & $0.56$ & $1078.00$ & $2.16\substack{+0.01\\ -0.01}$ & $109.42$ & $90$ \\ 
59082.88 & $39.99\pm0.31$ & $0.88$ & $486.00$ & $2.21\substack{+0.01\\ -0.01}$ & $65.40$ & $72$ \\ 
59083.01 & $41.34\pm0.26$ & $0.56$ & $775.00$ & $2.21\substack{+0.01\\ -0.01}$ & $117.30$ & $80$ \\ 
59084.93 & $30.51\pm0.24$ & $5.27$ & $707.00$ & $2.14\substack{+0.02\\ -0.01}$ & $151.78$ & $152$ \\ 
59093.97 & $24.00\pm0.30$ & $1.28$ & $309.00$ & $1.98\substack{+0.03\\ -0.03}$ & $83.43$ & $62$ \\ 
59109.31 & $31.13\pm0.25$ & $2.42$ & $627.00$ & $2.11\substack{+0.01\\ -0.01}$ & $130.07$ & $111$ \\ 
59116.29 & $26.62\pm0.18$ & $1.14$ & $978.00$ & $2.06\substack{+0.01\\ -0.01}$ & $136.98$ & $93$ \\ 
59118.43 & $26.94\pm0.14$ & $1.04$ & $1998.00$ & $1.98\substack{+0.01\\ -0.01}$ & $153.73$ & $120$ \\ 
59120.59 & $27.84\pm0.18$ & $1.39$ & $1091.00$ & $2.02\substack{+0.01\\ -0.01}$ & $120.52$ & $106$ \\ 
59122.53 & $34.92\pm0.18$ & $0.98$ & $1498.00$ & $2.08\substack{+0.01\\ -0.01}$ & $110.53$ & $106$ \\ 
59124.47 & $27.24\pm0.17$ & $1.18$ & $1196.00$ & $2.09\substack{+0.01\\ -0.01}$ & $99.30$ & $111$ \\ 
59126.20 & $31.16\pm0.29$ & $0.73$ & $412.00$ & $2.13\substack{+0.01\\ -0.01}$ & $78.12$ & $64$ \\ 
59128.12 & $29.63\pm0.21$ & $2.64$ & $918.00$ & $2.10\substack{+0.01\\ -0.01}$ & $125.11$ & $115$ \\ 
59129.56 & $32.44\pm0.22$ & $0.77$ & $875.00$ & $2.11\substack{+0.01\\ -0.01}$ & $108.16$ & $84$ \\ 
59130.75 & $35.43\pm0.25$ & $1.12$ & $717.00$ & $2.09\substack{+0.01\\ -0.01}$ & $108.58$ & $86$ \\ 
59136.81 & $34.91\pm0.29$ & $0.64$ & $486.00$ & $2.10\substack{+0.01\\ -0.01}$ & $95.18$ & $71$ \\ 
59138.33 & $35.45\pm0.22$ & $0.87$ & $922.00$ & $2.14\substack{+0.01\\ -0.01}$ & $115.58$ & $89$ \\ 
59141.04 & $31.99\pm0.22$ & $2.08$ & $887.00$ & $2.17\substack{+0.01\\ -0.01}$ & $177.99$ & $142$ \\ 
59142.79 & $30.97\pm0.34$ & $2.09$ & $320.00$ & $2.14\substack{+0.02\\ -0.02}$ & $60.22$ & $69$ \\ 
59144.40 & $31.20\pm0.21$ & $1.40$ & $948.00$ & $2.17\substack{+0.01\\ -0.01}$ & $125.67$ & $91$ \\ 
59148.93 & $32.97\pm0.23$ & $0.94$ & $762.00$ & $2.13\substack{+0.01\\ -0.01}$ & $78.58$ & $85$ \\ 
59150.52 & $28.11\pm0.19$ & $0.50$ & $950.00$ & $2.14\substack{+0.01\\ -0.01}$ & $99.89$ & $82$ \\ 
59151.84 & $31.53\pm0.19$ & $0.79$ & $1126.00$ & $2.20\substack{+0.01\\ -0.01}$ & $88.99$ & $93$ \\ 
59153.87 & $27.91\pm0.18$ & $0.54$ & $1090.00$ & $2.19\substack{+0.01\\ -0.01}$ & $129.49$ & $84$ \\ 
59155.71 & $27.64\pm0.24$ & $0.63$ & $574.00$ & $2.17\substack{+0.01\\ -0.01}$ & $109.72$ & $67$ \\ 
59157.68 & $30.14\pm0.20$ & $0.57$ & $944.00$ & $2.28\substack{+0.01\\ -0.01}$ & $167.53$ & $77$ \\ 
59179.54 & $37.67\pm0.22$ & $0.50$ & $1020.00$ & $2.15\substack{+0.01\\ -0.01}$ & $134.11$ & $88$ \\ 
59181.25 & $32.02\pm0.23$ & $0.64$ & $769.00$ & $2.13\substack{+0.01\\ -0.01}$ & $109.25$ & $78$ \\ 
59183.48 & $27.04\pm0.19$ & $0.53$ & $860.00$ & $2.09\substack{+0.01\\ -0.01}$ & $130.06$ & $78$ \\ 
59185.35 & $28.47\pm0.18$ & $0.55$ & $1050.00$ & $2.10\substack{+0.01\\ -0.01}$ & $182.12$ & $81$ \\ 
59187.36 & $29.42\pm0.29$ & $0.68$ & $384.00$ & $2.10\substack{+0.02\\ -0.02}$ & $73.38$ & $61$ \\ 
59189.60 & $25.62\pm0.26$ & $0.48$ & $436.00$ & $2.15\substack{+0.02\\ -0.02}$ & $80.86$ & $58$ \\ 
59192.98 & $33.15\pm0.27$ & $4.68$ & $581.00$ & $2.13\substack{+0.02\\ -0.02}$ & $121.70$ & $121$ \\ 
59213.22 & $28.92\pm0.18$ & $1.13$ & $1122.00$ & $2.05\substack{+0.01\\ -0.01}$ & $108.13$ & $98$ \\ 
59215.07 & $37.59\pm0.18$ & $0.75$ & $1828.00$ & $2.15\substack{+0.01\\ -0.01}$ & $98.26$ & $99$ \\ 
59217.36 & $38.86\pm0.21$ & $2.60$ & $1363.00$ & $2.16\substack{+0.01\\ -0.01}$ & $183.44$ & $138$ \\ 
59219.49 & $28.87\pm0.16$ & $3.37$ & $1731.00$ & $2.14\substack{+0.01\\ -0.01}$ & $163.51$ & $148$ \\ 
59223.62 & $24.76\pm0.28$ & $1.88$ & $375.00$ & $2.10\substack{+0.02\\ -0.02}$ & $85.76$ & $74$ \\ 
59225.17 & $21.59\pm0.17$ & $0.82$ & $862.00$ & $2.04\substack{+0.01\\ -0.01}$ & $105.59$ & $73$ \\ 
59226.98 & $19.33\pm0.18$ & $0.64$ & $684.13$ & $2.04\substack{+0.02\\ -0.02}$ & $80.47$ & $68$ \\ 
59227.05 & $19.84\pm0.24$ & $0.60$ & $363.00$ & $2.02\substack{+0.02\\ -0.02}$ & $46.72$ & $53$ \\ 
59228.97 & $24.07\pm0.16$ & $1.22$ & $1280.00$ & $2.11\substack{+0.01\\ -0.01}$ & $82.40$ & $95$ \\ 
59231.63 & $24.04\pm0.20$ & $0.56$ & $725.00$ & $2.22\substack{+0.02\\ -0.01}$ & $97.72$ & $63$ \\ 
59232.50 & $19.68\pm0.12$ & $0.38$ & $1715.00$ & $2.15\substack{+0.01\\ -0.01}$ & $198.56$ & $79$ \\ 
59233.39 & $19.70\pm0.15$ & $0.75$ & $1063.54$ & $2.12\substack{+0.02\\ -0.02}$ & $87.31$ & $89$ \\ 
59234.98 & $14.04\pm0.11$ & $0.48$ & $1497.00$ & $2.05\substack{+0.01\\ -0.01}$ & $189.05$ & $72$ \\ 
59239.46 & $19.57\pm0.11$ & $4.31$ & $3182.00$ & $2.26\substack{+0.01\\ -0.01}$ & $641.54$ & $161$ \\ 
59240.26 & $23.54\pm0.22$ & $6.29$ & $690.00$ & $2.29\substack{+0.02\\ -0.02}$ & $306.15$ & $148$ \\ 
59241.17 & $21.69\pm0.18$ & $9.47$ & $1192.00$ & $2.17\substack{+0.02\\ -0.01}$ & $204.39$ & $156$ \\ 
59243.24 & $19.49\pm0.18$ & $0.94$ & $748.00$ & $2.22\substack{+0.02\\ -0.02}$ & $97.18$ & $69$ \\ 
59245.18 & $24.21\pm0.26$ & $0.46$ & $412.00$ & $2.29\substack{+0.02\\ -0.02}$ & $39.61$ & $51$ \\ 
59248.93 & $35.17\pm0.22$ & $1.84$ & $988.00$ & $2.19\substack{+0.01\\ -0.01}$ & $118.58$ & $111$ \\ 
59253.49 & $32.87\pm0.21$ & $2.30$ & $1016.00$ & $2.34\substack{+0.01\\ -0.01}$ & $102.88$ & $137$ \\ 
59255.41 & $33.54\pm0.24$ & $0.63$ & $709.00$ & $2.32\substack{+0.01\\ -0.01}$ & $109.49$ & $69$ \\ 
59257.23 & $39.19\pm0.27$ & $3.13$ & $723.00$ & $2.33\substack{+0.01\\ -0.01}$ & $190.72$ & $149$ \\ 
59258.56 & $37.23\pm0.29$ & $6.27$ & $632.00$ & $2.24\substack{+0.01\\ -0.01}$ & $136.19$ & $137$ \\ 


==> Table6.tex <==
58256.96 & $33.70\pm0.18$ & $0.78$ & $1057.00$ & $2.08\substack{+0.01\\ -0.01}$ & $106.14$ & $141$ \\ 
58257.00 & $32.33\pm0.23$ & $1.73$ & $647.00$ & $2.12\substack{+0.01\\ -0.01}$ & $134.74$ & $136$ \\ 
58272.38 & $38.43\pm0.20$ & $1.83$ & $960.00$ & $2.17\substack{+0.01\\ -0.01}$ & $179.00$ & $137$ \\ 
58293.63 & $32.98\pm0.19$ & $0.73$ & $902.00$ & $2.15\substack{+0.01\\ -0.01}$ & $101.90$ & $141$ \\ 
58294.65 & $32.76\pm0.16$ & $0.58$ & $1266.00$ & $2.13\substack{+0.01\\ -0.01}$ & $171.03$ & $193$ \\ 
58302.65 & $34.10\pm0.36$ & $2.25$ & $277.00$ & $2.09\substack{+0.02\\ -0.02}$ & $136.15$ & $108$ \\ 
58304.20 & $41.43\pm0.59$ & $0.35$ & $120.00$ & $2.14\substack{+0.02\\ -0.02}$ & $31.81$ & $78$ \\ 
58310.32 & $19.76\pm0.16$ & $0.42$ & $839.24$ & $1.98\substack{+0.01\\ -0.01}$ & $96.01$ & $144$ \\ 
58311.22 & $18.80\pm0.12$ & $0.53$ & $1333.00$ & $2.00\substack{+0.01\\ -0.01}$ & $120.07$ & $121$ \\ 
58312.21 & $22.56\pm0.16$ & $0.67$ & $960.00$ & $2.03\substack{+0.01\\ -0.01}$ & $122.07$ & $199$ \\ 
58313.57 & $27.43\pm0.16$ & $1.02$ & $1119.00$ & $2.10\substack{+0.01\\ -0.01}$ & $198.08$ & $180$ \\ 
58314.52 & $29.44\pm0.15$ & $1.06$ & $1435.00$ & $2.08\substack{+0.01\\ -0.01}$ & $140.87$ & $130$ \\ 
58315.30 & $26.79\pm0.14$ & $0.89$ & $1435.00$ & $2.08\substack{+0.01\\ -0.01}$ & $148.24$ & $130$ \\ 
58317.30 & $30.14\pm0.14$ & $1.81$ & $1690.00$ & $2.12\substack{+0.01\\ -0.01}$ & $185.74$ & $162$ \\ 
58318.58 & $31.43\pm0.21$ & $0.58$ & $756.97$ & $2.11\substack{+0.01\\ -0.01}$ & $210.73$ & $262$ \\ 
58325.65 & $26.99\pm0.17$ & $0.60$ & $930.00$ & $2.08\substack{+0.01\\ -0.01}$ & $105.72$ & $145$ \\ 
58327.16 & $29.60\pm0.16$ & $0.54$ & $1217.00$ & $2.04\substack{+0.01\\ -0.01}$ & $166.83$ & $207$ \\ 
58329.19 & $27.66\pm0.20$ & $0.66$ & $710.00$ & $2.07\substack{+0.01\\ -0.01}$ & $176.44$ & $252$ \\ 
58331.12 & $25.65\pm0.23$ & $0.74$ & $480.00$ & $2.05\substack{+0.01\\ -0.01}$ & $110.87$ & $213$ \\ 
58333.50 & $31.67\pm0.12$ & $0.66$ & $2112.00$ & $2.18\substack{+0.01\\ -0.01}$ & $171.00$ & $170$ \\ 
58336.46 & $37.08\pm0.20$ & $0.50$ & $977.00$ & $2.14\substack{+0.01\\ -0.01}$ & $143.35$ & $188$ \\ 
58338.59 & $32.18\pm0.18$ & $0.66$ & $1013.00$ & $2.13\substack{+0.01\\ -0.01}$ & $165.02$ & $192$ \\ 
58340.52 & $35.91\pm0.19$ & $0.63$ & $1011.00$ & $2.10\substack{+0.01\\ -0.01}$ & $207.76$ & $220$ \\ 
58342.64 & $35.34\pm0.20$ & $0.99$ & $873.00$ & $2.04\substack{+0.01\\ -0.01}$ & $102.96$ & $105$ \\ 
58343.60 & $30.11\pm0.18$ & $1.03$ & $977.00$ & $2.05\substack{+0.01\\ -0.01}$ & $190.61$ & $187$ \\ 
58345.21 & $30.48\pm0.37$ & $1.41$ & $232.00$ & $2.16\substack{+0.02\\ -0.02}$ & $76.97$ & $124$ \\ 
58348.86 & $30.82\pm0.19$ & $0.70$ & $900.00$ & $2.09\substack{+0.01\\ -0.01}$ & $164.38$ & $251$ \\ 
58350.96 & $30.32\pm0.17$ & $0.72$ & $1079.00$ & $2.14\substack{+0.01\\ -0.01}$ & $198.79$ & $189$ \\ 
58352.82 & $29.97\pm0.18$ & $0.81$ & $1000.00$ & $2.12\substack{+0.01\\ -0.01}$ & $140.21$ & $147$ \\ 
58354.82 & $30.37\pm0.17$ & $0.64$ & $1095.00$ & $2.11\substack{+0.01\\ -0.01}$ & $130.03$ & $136$ \\ 
58358.86 & $26.03\pm0.29$ & $1.88$ & $324.00$ & $2.08\substack{+0.02\\ -0.02}$ & $62.89$ & $113$ \\ 
58360.85 & $21.80\pm0.30$ & $4.31$ & $300.00$ & $2.06\substack{+0.02\\ -0.02}$ & $130.82$ & $130$ \\ 
58362.85 & $22.52\pm0.60$ & $20.41$ & $120.00$ & $1.97\substack{+0.04\\ -0.04}$ & $162.95$ & $148$ \\ 
58364.72 & $29.69\pm0.20$ & $2.03$ & $756.00$ & $1.97\substack{+0.01\\ -0.01}$ & $264.49$ & $133$ \\ 
58367.94 & $33.27\pm0.35$ & $0.55$ & $281.00$ & $2.17\substack{+0.02\\ -0.02}$ & $91.30$ & $123$ \\ 
58369.77 & $25.38\pm0.14$ & $0.65$ & $1354.00$ & $2.09\substack{+0.01\\ -0.01}$ & $133.83$ & $104$ \\ 
58375.76 & $25.79\pm0.22$ & $0.97$ & $539.00$ & $2.12\substack{+0.01\\ -0.01}$ & $81.70$ & $99$ \\ 
58377.89 & $20.85\pm0.16$ & $1.23$ & $894.00$ & $2.07\substack{+0.01\\ -0.01}$ & $128.38$ & $134$ \\ 
58379.95 & $21.37\pm0.15$ & $1.31$ & $960.00$ & $2.04\substack{+0.01\\ -0.01}$ & $131.01$ & $135$ \\ 
58382.85 & $22.39\pm0.26$ & $1.78$ & $360.00$ & $2.10\substack{+0.02\\ -0.02}$ & $122.49$ & $85$ \\ 
58388.42 & $24.38\pm0.16$ & $0.55$ & $920.00$ & $2.08\substack{+0.01\\ -0.01}$ & $132.60$ & $169$ \\ 
58390.48 & $27.66\pm0.18$ & $0.61$ & $872.00$ & $2.09\substack{+0.01\\ -0.01}$ & $195.00$ & $247$ \\ 
58392.70 & $28.56\pm0.11$ & $0.70$ & $2306.00$ & $2.07\substack{+0.01\\ -0.01}$ & $219.79$ & $179$ \\ 
58394.92 & $20.46\pm0.12$ & $0.86$ & $1510.00$ & $2.01\substack{+0.01\\ -0.01}$ & $156.60$ & $145$ \\ 
58396.59 & $21.66\pm0.14$ & $0.40$ & $1193.00$ & $2.04\substack{+0.01\\ -0.01}$ & $101.27$ & $148$ \\ 
58398.59 & $29.26\pm0.18$ & $0.79$ & $960.00$ & $1.91\substack{+0.01\\ -0.01}$ & $834.42$ & $145$ \\ 
58400.69 & $28.19\pm0.18$ & $1.95$ & $951.00$ & $2.03\substack{+0.01\\ -0.01}$ & $254.61$ & $157$ \\ 
58402.59 & $27.46\pm0.17$ & $0.99$ & $1002.00$ & $2.11\substack{+0.01\\ -0.01}$ & $138.84$ & $131$ \\ 
58403.93 & $23.97\pm0.18$ & $0.67$ & $735.00$ & $2.08\substack{+0.01\\ -0.01}$ & $88.09$ & $89$ \\ 
58405.89 & $25.66\pm0.28$ & $0.57$ & $338.00$ & $2.13\substack{+0.02\\ -0.02}$ & $89.86$ & $87$ \\ 
58407.31 & $28.93\pm0.19$ & $0.72$ & $808.00$ & $2.15\substack{+0.01\\ -0.01}$ & $290.39$ & $297$ \\ 
58409.68 & $31.44\pm0.16$ & $0.53$ & $1247.00$ & $2.15\substack{+0.01\\ -0.01}$ & $173.33$ & $266$ \\ 
58412.07 & $23.59\pm0.18$ & $0.66$ & $747.00$ & $2.23\substack{+0.01\\ -0.01}$ & $104.98$ & $92$ \\ 
58414.51 & $28.22\pm0.14$ & $1.14$ & $1474.00$ & $2.24\substack{+0.01\\ -0.01}$ & $341.46$ & $133$ \\ 
58416.70 & $30.10\pm0.26$ & $1.73$ & $484.00$ & $2.29\substack{+0.01\\ -0.01}$ & $149.47$ & $131$ \\ 
58418.70 & $29.18\pm0.22$ & $1.76$ & $649.00$ & $2.25\substack{+0.01\\ -0.01}$ & $146.34$ & $124$ \\ 
58420.63 & $29.07\pm0.21$ & $2.30$ & $688.00$ & $2.14\substack{+0.01\\ -0.01}$ & $164.41$ & $142$ \\ 
58421.24 & $31.32\pm0.21$ & $1.03$ & $727.00$ & $2.13\substack{+0.01\\ -0.01}$ & $156.66$ & $235$ \\ 
58422.67 & $28.71\pm0.19$ & $0.47$ & $803.00$ & $2.05\substack{+0.01\\ -0.01}$ & $162.78$ & $205$ \\ 
58423.96 & $27.35\pm0.18$ & $0.45$ & $862.00$ & $2.04\substack{+0.01\\ -0.01}$ & $211.18$ & $343$ \\ 
58426.46 & $29.55\pm0.16$ & $0.37$ & $1215.00$ & $2.06\substack{+0.01\\ -0.01}$ & $122.56$ & $164$ \\ 
58428.20 & $35.54\pm0.16$ & $0.80$ & $1373.00$ & $2.13\substack{+0.01\\ -0.01}$ & $196.96$ & $178$ \\ 
58429.17 & $39.01\pm0.18$ & $0.67$ & $1273.00$ & $2.15\substack{+0.01\\ -0.01}$ & $256.53$ & $206$ \\ 
58430.07 & $39.85\pm0.27$ & $0.48$ & $538.00$ & $2.15\substack{+0.01\\ -0.01}$ & $92.48$ & $98$ \\ 
58431.16 & $37.14\pm0.19$ & $0.44$ & $1074.00$ & $2.15\substack{+0.01\\ -0.01}$ & $236.58$ & $287$ \\ 
58432.97 & $44.10\pm0.37$ & $0.60$ & $335.00$ & $2.11\substack{+0.01\\ -0.01}$ & $172.23$ & $281$ \\ 
58433.06 & $42.81\pm0.23$ & $0.61$ & $830.00$ & $2.14\substack{+0.01\\ -0.01}$ & $124.48$ & $160$ \\ 
58437.51 & $34.56\pm0.40$ & $3.15$ & $236.00$ & $2.16\substack{+0.02\\ -0.02}$ & $83.91$ & $102$ \\ 
58438.42 & $31.32\pm0.54$ & $3.97$ & $120.00$ & $2.32\substack{+0.03\\ -0.03}$ & $166.63$ & $134$ \\ 
58449.22 & $34.37\pm0.39$ & $1.82$ & $240.00$ & $2.14\substack{+0.02\\ -0.02}$ & $69.46$ & $92$ \\ 
58453.60 & $28.98\pm0.14$ & $0.37$ & $1408.00$ & $2.06\substack{+0.01\\ -0.01}$ & $134.04$ & $253$ \\ 
58455.11 & $24.93\pm0.19$ & $0.50$ & $720.00$ & $2.04\substack{+0.01\\ -0.01}$ & $132.79$ & $247$ \\ 
58456.98 & $22.56\pm0.15$ & $0.85$ & $991.00$ & $2.10\substack{+0.01\\ -0.01}$ & $98.66$ & $142$ \\ 
58458.91 & $23.30\pm0.15$ & $0.74$ & $1115.00$ & $2.11\substack{+0.01\\ -0.01}$ & $129.89$ & $184$ \\ 
58460.91 & $27.38\pm0.16$ & $0.84$ & $1080.00$ & $2.07\substack{+0.01\\ -0.01}$ & $98.23$ & $118$ \\ 
58462.90 & $24.59\pm0.20$ & $1.20$ & $668.00$ & $1.93\substack{+0.01\\ -0.01}$ & $209.19$ & $152$ \\ 
58464.58 & $22.87\pm0.14$ & $0.91$ & $1146.00$ & $2.05\substack{+0.01\\ -0.01}$ & $156.87$ & $209$ \\ 
58466.18 & $23.92\pm0.27$ & $2.45$ & $360.00$ & $2.13\substack{+0.02\\ -0.02}$ & $141.54$ & $102$ \\ 
58469.03 & $20.45\pm0.29$ & $2.12$ & $273.00$ & $2.09\substack{+0.02\\ -0.02}$ & $191.95$ & $153$ \\ 
58470.68 & $22.04\pm0.16$ & $0.66$ & $840.00$ & $2.00\substack{+0.01\\ -0.01}$ & $212.61$ & $234$ \\ 
58471.77 & $28.83\pm0.23$ & $0.67$ & $548.00$ & $2.06\substack{+0.01\\ -0.01}$ & $225.77$ & $300$ \\ 
58473.91 & $30.42\pm0.20$ & $1.40$ & $814.00$ & $2.04\substack{+0.01\\ -0.01}$ & $189.85$ & $121$ \\ 
58476.07 & $33.55\pm0.30$ & $1.39$ & $378.00$ & $2.15\substack{+0.01\\ -0.01}$ & $91.50$ & $118$ \\ 
58479.11 & $32.26\pm0.19$ & $0.68$ & $906.00$ & $2.14\substack{+0.01\\ -0.01}$ & $110.00$ & $94$ \\ 
58481.24 & $27.68\pm0.26$ & $2.22$ & $451.00$ & $2.10\substack{+0.02\\ -0.02}$ & $194.64$ & $121$ \\ 
58487.79 & $36.21\pm0.56$ & $1.10$ & $120.00$ & $2.22\substack{+0.03\\ -0.03}$ & $52.17$ & $104$ \\ 
58489.78 & $25.83\pm0.33$ & $0.78$ & $240.00$ & $2.08\substack{+0.02\\ -0.02}$ & $116.49$ & $299$ \\ 
58491.53 & $23.35\pm0.29$ & $1.87$ & $290.00$ & $2.05\substack{+0.02\\ -0.02}$ & $148.69$ & $172$ \\ 
58493.71 & $24.65\pm0.33$ & $1.18$ & $240.00$ & $2.20\substack{+0.02\\ -0.02}$ & $71.82$ & $134$ \\ 
58497.64 & $25.48\pm0.21$ & $1.38$ & $600.00$ & $2.12\substack{+0.01\\ -0.01}$ & $110.07$ & $139$ \\ 
58499.38 & $28.59\pm0.19$ & $1.92$ & $840.00$ & $2.18\substack{+0.01\\ -0.01}$ & $175.78$ & $134$ \\ 
58500.48 & $30.26\pm0.36$ & $1.14$ & $240.00$ & $2.23\substack{+0.02\\ -0.02}$ & $106.00$ & $173$ \\ 
58501.89 & $30.23\pm0.21$ & $1.38$ & $693.00$ & $2.22\substack{+0.01\\ -0.01}$ & $124.17$ & $104$ \\ 
58503.24 & $28.60\pm0.20$ & $1.23$ & $720.00$ & $2.23\substack{+0.01\\ -0.01}$ & $158.05$ & $165$ \\ 
58504.99 & $36.93\pm0.43$ & $0.80$ & $207.00$ & $2.26\substack{+0.02\\ -0.02}$ & $71.53$ & $240$ \\ 
58506.34 & $36.90\pm0.32$ & $0.82$ & $360.00$ & $2.19\substack{+0.02\\ -0.02}$ & $194.92$ & $451$ \\ 
58507.62 & $33.87\pm0.24$ & $1.21$ & $600.00$ & $2.22\substack{+0.01\\ -0.01}$ & $104.20$ & $143$ \\ 
58511.87 & $28.92\pm0.17$ & $0.72$ & $1063.00$ & $2.22\substack{+0.01\\ -0.01}$ & $138.11$ & $122$ \\ 
58513.28 & $29.92\pm0.19$ & $1.20$ & $868.00$ & $2.15\substack{+0.01\\ -0.01}$ & $132.34$ & $99$ \\ 
58514.73 & $30.55\pm0.15$ & $1.97$ & $1537.00$ & $2.23\substack{+0.01\\ -0.01}$ & $247.97$ & $153$ \\ 
58515.86 & $34.74\pm0.25$ & $1.13$ & $596.00$ & $2.22\substack{+0.01\\ -0.01}$ & $275.22$ & $156$ \\ 
58517.18 & $35.23\pm0.26$ & $1.03$ & $532.00$ & $2.25\substack{+0.01\\ -0.01}$ & $292.77$ & $291$ \\ 
58521.53 & $38.51\pm0.19$ & $0.57$ & $1053.00$ & $2.29\substack{+0.01\\ -0.01}$ & $130.89$ & $121$ \\ 
58523.50 & $38.56\pm0.20$ & $1.22$ & $973.00$ & $2.13\substack{+0.01\\ -0.01}$ & $552.83$ & $131$ \\ 
58527.09 & $39.89\pm0.23$ & $0.63$ & $769.00$ & $2.34\substack{+0.01\\ -0.01}$ & $139.96$ & $181$ \\ 
58528.06 & $36.48\pm0.78$ & $0.70$ & $61.00$ & $2.35\substack{+0.04\\ -0.04}$ & $55.80$ & $220$ \\ 
58529.87 & $33.66\pm0.32$ & $2.05$ & $350.00$ & $2.25\substack{+0.02\\ -0.02}$ & $98.50$ & $109$ \\ 
58541.28 & $35.88\pm0.16$ & $0.79$ & $1394.00$ & $2.13\substack{+0.01\\ -0.01}$ & $176.53$ & $184$ \\ 
58544.08 & $41.94\pm0.23$ & $1.16$ & $835.00$ & $2.11\substack{+0.01\\ -0.01}$ & $166.91$ & $126$ \\ 
58550.29 & $42.48\pm0.35$ & $0.90$ & $355.00$ & $2.17\substack{+0.01\\ -0.01}$ & $178.50$ & $338$ \\ 
58553.35 & $38.29\pm0.41$ & $1.08$ & $240.00$ & $2.12\substack{+0.02\\ -0.02}$ & $52.11$ & $77$ \\ 
58556.05 & $42.83\pm0.61$ & $1.21$ & $120.00$ & $2.17\substack{+0.03\\ -0.02}$ & $34.18$ & $75$ \\ 
58561.49 & $30.82\pm0.23$ & $2.02$ & $600.00$ & $2.17\substack{+0.01\\ -0.01}$ & $100.16$ & $91$ \\ 
58562.94 & $32.67\pm0.38$ & $1.26$ & $240.00$ & $2.25\substack{+0.02\\ -0.02}$ & $72.32$ & $206$ \\ 
58570.86 & $42.97\pm1.10$ & $1.44$ & $37.00$ & $2.22\substack{+0.05\\ -0.05}$ & $231.58$ & $796$ \\ 
58581.31 & $43.86\pm0.61$ & $0.53$ & $120.00$ & $2.20\substack{+0.03\\ -0.02}$ & $65.11$ & $144$ \\ 
58586.70 & $43.52\pm0.37$ & $4.60$ & $358.00$ & $2.12\substack{+0.02\\ -0.02}$ & $192.17$ & $147$ \\ 
58588.63 & $52.36\pm0.39$ & $6.87$ & $391.00$ & $2.12\substack{+0.01\\ -0.01}$ & $208.28$ & $157$ \\ 
58591.06 & $44.48\pm0.34$ & $1.14$ & $389.00$ & $2.20\substack{+0.01\\ -0.01}$ & $89.23$ & $134$ \\ 
58592.65 & $44.62\pm0.29$ & $1.84$ & $536.00$ & $2.12\substack{+0.01\\ -0.01}$ & $199.30$ & $142$ \\ 
58594.91 & $43.56\pm0.40$ & $6.66$ & $311.00$ & $2.23\substack{+0.02\\ -0.02}$ & $180.92$ & $147$ \\ 
58603.42 & $40.30\pm1.84$ & $0.36$ & $12.00$ & $2.24\substack{+0.08\\ -0.08}$ & $63.67$ & $1026$ \\ 
58611.34 & $37.66\pm0.40$ & $0.66$ & $240.00$ & $2.11\substack{+0.02\\ -0.02}$ & $80.13$ & $209$ \\ 
58612.95 & $33.18\pm0.27$ & $0.85$ & $476.00$ & $2.12\substack{+0.01\\ -0.01}$ & $133.95$ & $207$ \\ 
58617.01 & $34.66\pm0.43$ & $0.87$ & $188.00$ & $2.12\substack{+0.02\\ -0.02}$ & $68.06$ & $223$ \\ 
58619.00 & $35.23\pm1.31$ & $0.58$ & $21.00$ & $2.10\substack{+0.06\\ -0.06}$ & $160.29$ & $1132$ \\ 
58621.13 & $37.14\pm1.48$ & $0.33$ & $17.00$ & $2.32\substack{+0.07\\ -0.07}$ & $140.40$ & $968$ \\ 
58623.19 & $34.72\pm0.55$ & $1.08$ & $120.00$ & $2.08\substack{+0.03\\ -0.03}$ & $57.23$ & $137$ \\ 
58626.73 & $35.24\pm0.29$ & $0.49$ & $420.00$ & $2.16\substack{+0.01\\ -0.01}$ & $114.59$ & $255$ \\ 
58632.66 & $28.86\pm0.19$ & $1.16$ & $832.00$ & $2.12\substack{+0.01\\ -0.01}$ & $145.82$ & $176$ \\ 
58635.56 & $37.90\pm0.20$ & $1.00$ & $960.00$ & $2.19\substack{+0.01\\ -0.01}$ & $170.79$ & $100$ \\ 
58637.62 & $40.05\pm0.22$ & $0.89$ & $840.00$ & $2.21\substack{+0.01\\ -0.01}$ & $144.89$ & $172$ \\ 
58643.87 & $48.43\pm0.31$ & $3.62$ & $529.00$ & $2.21\substack{+0.01\\ -0.01}$ & $110.51$ & $144$ \\ 
58646.07 & $40.43\pm0.38$ & $5.07$ & $318.00$ & $2.26\substack{+0.02\\ -0.02}$ & $164.92$ & $126$ \\ 
58651.93 & $36.87\pm0.25$ & $1.65$ & $598.00$ & $2.15\substack{+0.01\\ -0.01}$ & $109.19$ & $97$ \\ 
58653.93 & $32.61\pm0.23$ & $0.65$ & $625.00$ & $2.21\substack{+0.01\\ -0.01}$ & $156.40$ & $214$ \\ 
58655.93 & $36.78\pm0.22$ & $0.69$ & $763.00$ & $2.24\substack{+0.01\\ -0.01}$ & $155.86$ & $198$ \\ 
58657.93 & $42.15\pm0.23$ & $0.59$ & $817.00$ & $2.24\substack{+0.01\\ -0.01}$ & $192.95$ & $226$ \\ 
58660.23 & $42.93\pm0.35$ & $1.93$ & $360.00$ & $2.04\substack{+0.02\\ -0.02}$ & $406.61$ & $116$ \\ 
58662.04 & $32.86\pm0.39$ & $3.41$ & $240.00$ & $2.20\substack{+0.02\\ -0.02}$ & $183.68$ & $93$ \\ 
58664.23 & $39.25\pm0.42$ & $3.04$ & $240.00$ & $2.18\substack{+0.02\\ -0.02}$ & $90.70$ & $117$ \\ 
58665.85 & $39.06\pm0.41$ & $1.09$ & $235.00$ & $2.23\substack{+0.02\\ -0.02}$ & $125.87$ & $147$ \\ 
58673.24 & $31.66\pm0.25$ & $0.41$ & $515.00$ & $2.12\substack{+0.01\\ -0.01}$ & $313.49$ & $445$ \\ 
58675.30 & $31.43\pm0.17$ & $0.65$ & $1104.00$ & $2.10\substack{+0.01\\ -0.01}$ & $150.08$ & $150$ \\ 
58677.17 & $27.94\pm0.14$ & $0.70$ & $1394.00$ & $2.13\substack{+0.01\\ -0.01}$ & $224.26$ & $197$ \\ 
58679.04 & $36.90\pm0.28$ & $0.83$ & $480.00$ & $2.20\substack{+0.01\\ -0.01}$ & $142.77$ & $237$ \\ 
58680.40 & $32.78\pm0.27$ & $1.94$ & $480.00$ & $2.21\substack{+0.01\\ -0.01}$ & $99.78$ & $109$ \\ 
58683.23 & $28.36\pm0.14$ & $1.51$ & $1450.00$ & $2.18\substack{+0.01\\ -0.01}$ & $160.74$ & $154$ \\ 
58685.11 & $32.07\pm0.18$ & $1.51$ & $984.00$ & $2.15\substack{+0.01\\ -0.01}$ & $136.05$ & $149$ \\ 
58687.54 & $30.85\pm0.22$ & $0.52$ & $674.00$ & $2.11\substack{+0.01\\ -0.01}$ & $158.34$ & $91$ \\ 
58690.12 & $21.43\pm0.19$ & $0.51$ & $613.00$ & $2.02\substack{+0.02\\ -0.01}$ & $130.57$ & $150$ \\ 
58691.79 & $29.25\pm0.17$ & $0.88$ & $995.00$ & $2.11\substack{+0.01\\ -0.01}$ & $231.27$ & $116$ \\ 
58694.70 & $33.86\pm0.18$ & $0.60$ & $1074.00$ & $2.25\substack{+0.01\\ -0.01}$ & $241.07$ & $289$ \\ 
58699.98 & $40.47\pm0.24$ & $0.95$ & $697.00$ & $2.23\substack{+0.01\\ -0.01}$ & $94.29$ & $139$ \\ 
58702.27 & $39.40\pm0.38$ & $3.21$ & $294.00$ & $2.29\substack{+0.02\\ -0.02}$ & $130.17$ & $116$ \\ 
58704.49 & $32.21\pm0.27$ & $0.69$ & $466.00$ & $2.21\substack{+0.01\\ -0.01}$ & $209.19$ & $339$ \\ 
58706.46 & $37.54\pm0.19$ & $1.06$ & $1102.00$ & $2.15\substack{+0.01\\ -0.01}$ & $167.65$ & $118$ \\ 
58711.99 & $25.96\pm0.21$ & $0.54$ & $628.00$ & $2.10\substack{+0.01\\ -0.01}$ & $192.35$ & $345$ \\ 
58712.05 & $27.07\pm0.21$ & $0.48$ & $610.00$ & $2.12\substack{+0.01\\ -0.01}$ & $157.32$ & $333$ \\ 
58713.92 & $29.66\pm0.17$ & $0.52$ & $1028.00$ & $2.03\substack{+0.01\\ -0.01}$ & $148.06$ & $304$ \\ 
58715.57 & $33.09\pm0.17$ & $0.38$ & $1152.00$ & $2.09\substack{+0.01\\ -0.01}$ & $140.68$ & $319$ \\ 
58717.44 & $31.38\pm0.20$ & $0.39$ & $834.00$ & $2.09\substack{+0.01\\ -0.01}$ & $205.43$ & $384$ \\ 
58719.05 & $28.75\pm0.15$ & $0.38$ & $1231.00$ & $2.08\substack{+0.01\\ -0.01}$ & $108.49$ & $195$ \\ 
58721.15 & $22.62\pm0.18$ & $0.63$ & $714.00$ & $2.11\substack{+0.01\\ -0.01}$ & $221.85$ & $309$ \\ 
58723.06 & $30.72\pm0.36$ & $1.22$ & $240.00$ & $2.19\substack{+0.02\\ -0.02}$ & $115.23$ & $172$ \\ 
58729.84 & $42.43\pm0.35$ & $0.83$ & $360.00$ & $2.22\substack{+0.01\\ -0.01}$ & $93.42$ & $120$ \\ 
58742.97 & $37.47\pm0.57$ & $1.01$ & $120.00$ & $2.28\substack{+0.03\\ -0.03}$ & $273.40$ & $432$ \\ 
58743.04 & $37.77\pm0.57$ & $1.23$ & $120.00$ & $2.29\substack{+0.02\\ -0.02}$ & $102.38$ & $223$ \\ 
58751.71 & $28.70\pm0.20$ & $1.41$ & $766.00$ & $2.13\substack{+0.01\\ -0.01}$ & $117.18$ & $116$ \\ 
58753.15 & $31.31\pm0.20$ & $0.61$ & $824.00$ & $2.15\substack{+0.01\\ -0.01}$ & $231.60$ & $263$ \\ 
58755.02 & $32.13\pm0.19$ & $0.99$ & $878.00$ & $2.19\substack{+0.01\\ -0.01}$ & $113.02$ & $129$ \\ 
58756.57 & $31.40\pm0.15$ & $0.80$ & $1396.00$ & $2.26\substack{+0.01\\ -0.01}$ & $205.70$ & $140$ \\ 
58758.38 & $30.67\pm0.26$ & $1.26$ & $455.00$ & $2.29\substack{+0.02\\ -0.02}$ & $89.01$ & $98$ \\ 
58761.66 & $37.35\pm0.19$ & $0.72$ & $1065.00$ & $2.18\substack{+0.01\\ -0.01}$ & $190.48$ & $139$ \\ 
58765.31 & $39.37\pm0.18$ & $0.76$ & $1233.00$ & $2.21\substack{+0.01\\ -0.01}$ & $133.64$ & $147$ \\ 
58767.60 & $42.19\pm0.21$ & $1.14$ & $987.00$ & $2.15\substack{+0.01\\ -0.01}$ & $222.38$ & $156$ \\ 
58777.69 & $38.01\pm0.17$ & $1.53$ & $1339.54$ & $2.13\substack{+0.01\\ -0.01}$ & $134.76$ & $146$ \\ 
58779.17 & $36.59\pm0.16$ & $0.84$ & $1475.00$ & $2.13\substack{+0.01\\ -0.01}$ & $146.09$ & $133$ \\ 
58781.21 & $35.24\pm0.39$ & $1.26$ & $240.00$ & $2.12\substack{+0.02\\ -0.02}$ & $222.18$ & $190$ \\ 
58783.30 & $34.85\pm0.29$ & $1.95$ & $427.00$ & $2.12\substack{+0.01\\ -0.01}$ & $118.54$ & $98$ \\ 
58785.09 & $36.96\pm0.23$ & $0.75$ & $703.00$ & $2.22\substack{+0.01\\ -0.01}$ & $150.98$ & $234$ \\ 
58786.96 & $38.77\pm0.22$ & $0.70$ & $802.00$ & $2.11\substack{+0.01\\ -0.01}$ & $271.22$ & $180$ \\ 
58789.28 & $27.42\pm0.14$ & $0.71$ & $1506.00$ & $2.08\substack{+0.01\\ -0.01}$ & $128.99$ & $154$ \\ 
58791.61 & $31.33\pm0.18$ & $0.67$ & $996.00$ & $2.07\substack{+0.01\\ -0.01}$ & $118.22$ & $205$ \\ 
58793.60 & $31.03\pm0.20$ & $0.57$ & $818.00$ & $2.11\substack{+0.01\\ -0.01}$ & $122.22$ & $89$ \\ 
58794.80 & $35.16\pm0.24$ & $0.47$ & $623.00$ & $2.19\substack{+0.01\\ -0.01}$ & $95.93$ & $159$ \\ 
58801.97 & $37.88\pm0.43$ & $1.93$ & $213.00$ & $2.15\substack{+0.02\\ -0.02}$ & $117.57$ & $167$ \\ 
58805.13 & $34.94\pm0.32$ & $1.28$ & $360.00$ & $2.12\substack{+0.02\\ -0.02}$ & $61.93$ & $102$ \\ 
58808.88 & $33.18\pm0.66$ & $0.63$ & $78.00$ & $2.19\substack{+0.04\\ -0.04}$ & $230.09$ & $759$ \\ 
58810.94 & $31.86\pm0.53$ & $0.50$ & $114.00$ & $2.16\substack{+0.03\\ -0.03}$ & $135.74$ & $407$ \\ 
58811.00 & $31.96\pm0.33$ & $1.23$ & $300.00$ & $2.13\substack{+0.02\\ -0.02}$ & $129.04$ & $251$ \\ 
58812.59 & $31.44\pm0.21$ & $0.57$ & $699.00$ & $2.18\substack{+0.01\\ -0.01}$ & $127.48$ & $152$ \\ 
58815.65 & $27.01\pm0.16$ & $0.67$ & $1147.00$ & $2.04\substack{+0.01\\ -0.01}$ & $219.90$ & $242$ \\ 
58817.45 & $31.86\pm0.16$ & $0.62$ & $1277.00$ & $2.08\substack{+0.01\\ -0.01}$ & $131.85$ & $154$ \\ 
58819.36 & $35.07\pm0.19$ & $0.63$ & $960.00$ & $2.23\substack{+0.01\\ -0.01}$ & $122.87$ & $142$ \\ 
58821.52 & $32.20\pm0.18$ & $0.83$ & $986.00$ & $2.18\substack{+0.01\\ -0.01}$ & $158.88$ & $167$ \\ 
58823.49 & $36.61\pm0.18$ & $0.66$ & $1174.00$ & $2.16\substack{+0.01\\ -0.01}$ & $96.17$ & $103$ \\ 
58825.62 & $31.73\pm0.17$ & $0.86$ & $1142.00$ & $2.13\substack{+0.01\\ -0.01}$ & $123.22$ & $137$ \\ 
58827.62 & $30.05\pm0.18$ & $0.92$ & $975.00$ & $2.14\substack{+0.01\\ -0.01}$ & $109.87$ & $104$ \\ 
58829.88 & $31.07\pm0.21$ & $1.18$ & $720.00$ & $2.14\substack{+0.01\\ -0.01}$ & $139.08$ & $185$ \\ 
58832.01 & $32.95\pm0.37$ & $1.74$ & $251.00$ & $2.10\substack{+0.02\\ -0.02}$ & $108.12$ & $155$ \\ 
58833.86 & $40.20\pm0.58$ & $0.71$ & $120.00$ & $2.12\substack{+0.02\\ -0.02}$ & $239.62$ & $759$ \\ 
58844.19 & $39.31\pm0.38$ & $0.73$ & $275.00$ & $2.29\substack{+0.02\\ -0.02}$ & $146.70$ & $428$ \\ 
58847.69 & $39.27\pm0.23$ & $0.56$ & $786.00$ & $2.16\substack{+0.01\\ -0.01}$ & $131.77$ & $190$ \\ 
58849.83 & $33.52\pm0.24$ & $0.59$ & $600.00$ & $2.08\substack{+0.01\\ -0.01}$ & $90.01$ & $158$ \\ 
58851.80 & $32.84\pm0.35$ & $0.69$ & $278.00$ & $2.08\substack{+0.02\\ -0.02}$ & $99.07$ & $266$ \\ 
58853.64 & $33.42\pm0.33$ & $2.07$ & $318.00$ & $2.06\substack{+0.02\\ -0.02}$ & $87.69$ & $135$ \\ 
58855.80 & $35.78\pm0.34$ & $1.45$ & $326.00$ & $2.15\substack{+0.02\\ -0.02}$ & $102.81$ & $160$ \\ 
58857.80 & $34.68\pm0.27$ & $0.99$ & $492.00$ & $2.05\substack{+0.01\\ -0.01}$ & $109.84$ & $110$ \\ 
58859.80 & $32.57\pm0.35$ & $0.97$ & $279.00$ & $2.00\substack{+0.02\\ -0.02}$ & $99.57$ & $251$ \\ 
58861.80 & $31.80\pm0.21$ & $1.07$ & $773.54$ & $1.99\substack{+0.01\\ -0.01}$ & $157.17$ & $186$ \\ 
58863.62 & $26.76\pm0.17$ & $0.62$ & $983.00$ & $2.05\substack{+0.01\\ -0.01}$ & $139.24$ & $198$ \\ 
58865.22 & $31.48\pm0.26$ & $1.71$ & $480.00$ & $2.12\substack{+0.01\\ -0.01}$ & $96.65$ & $150$ \\ 
58866.72 & $36.06\pm0.39$ & $0.87$ & $240.00$ & $2.14\substack{+0.02\\ -0.02}$ & $274.85$ & $468$ \\ 
58870.84 & $37.91\pm0.39$ & $1.26$ & $259.00$ & $2.11\substack{+0.02\\ -0.02}$ & $213.66$ & $275$ \\ 
58871.73 & $35.73\pm0.56$ & $1.52$ & $120.00$ & $2.18\substack{+0.03\\ -0.03}$ & $70.24$ & $57$ \\ 
58873.24 & $38.37\pm1.82$ & $1.30$ & $12.00$ & $2.12\substack{+0.09\\ -0.09}$ & $257.28$ & $1172$ \\ 
58875.16 & $31.85\pm0.30$ & $0.75$ & $360.00$ & $2.09\substack{+0.02\\ -0.02}$ & $114.56$ & $328$ \\ 
58876.97 & $29.04\pm0.18$ & $1.08$ & $960.00$ & $2.06\substack{+0.01\\ -0.01}$ & $116.23$ & $171$ \\ 
58877.69 & $31.86\pm0.76$ & $1.13$ & $57.00$ & $2.19\substack{+0.05\\ -0.04}$ & $35.54$ & $49$ \\ 
58879.49 & $29.57\pm0.28$ & $1.01$ & $396.00$ & $2.04\substack{+0.02\\ -0.02}$ & $105.02$ & $181$ \\ 
58884.72 & $28.63\pm0.20$ & $0.83$ & $720.00$ & $2.03\substack{+0.01\\ -0.01}$ & $79.28$ & $131$ \\ 
58887.53 & $36.66\pm0.21$ & $1.25$ & $840.00$ & $2.11\substack{+0.01\\ -0.01}$ & $199.40$ & $171$ \\ 
58889.57 & $34.76\pm0.25$ & $2.44$ & $600.00$ & $2.09\substack{+0.01\\ -0.01}$ & $154.70$ & $122$ \\ 
58891.63 & $41.22\pm0.20$ & $1.62$ & $1103.00$ & $2.22\substack{+0.01\\ -0.01}$ & $216.80$ & $141$ \\ 
58893.40 & $37.70\pm0.30$ & $0.83$ & $436.00$ & $2.25\substack{+0.01\\ -0.01}$ & $135.88$ & $304$ \\ 
58902.62 & $34.06\pm1.48$ & $0.94$ & $16.00$ & $2.48\substack{+0.09\\ -0.09}$ & $141.30$ & $1147$ \\ 
58905.59 & $46.47\pm0.66$ & $1.10$ & $109.00$ & $2.32\substack{+0.03\\ -0.03}$ & $70.47$ & $292$ \\ 
58909.60 & $34.59\pm0.28$ & $4.66$ & $491.00$ & $2.17\substack{+0.02\\ -0.02}$ & $164.50$ & $142$ \\ 
58915.75 & $27.71\pm0.21$ & $1.31$ & $638.00$ & $2.10\substack{+0.01\\ -0.01}$ & $138.50$ & $145$ \\ 
58917.39 & $26.78\pm0.32$ & $0.94$ & $273.00$ & $1.98\substack{+0.02\\ -0.02}$ & $336.57$ & $545$ \\ 
58919.20 & $35.15\pm0.55$ & $0.94$ & $120.00$ & $2.07\substack{+0.03\\ -0.03}$ & $180.12$ & $778$ \\ 
58923.07 & $34.35\pm1.06$ & $0.36$ & $31.00$ & $2.14\substack{+0.05\\ -0.05}$ & $152.87$ & $979$ \\ 
58933.41 & $35.73\pm0.28$ & $0.77$ & $480.00$ & $2.10\substack{+0.01\\ -0.01}$ & $347.81$ & $489$ \\ 
58935.42 & $34.94\pm0.24$ & $0.69$ & $600.00$ & $2.08\substack{+0.01\\ -0.01}$ & $154.17$ & $331$ \\ 
58937.59 & $33.25\pm0.80$ & $0.38$ & $52.00$ & $2.00\substack{+0.04\\ -0.04}$ & $210.06$ & $886$ \\ 
58939.87 & $34.60\pm0.29$ & $0.99$ & $412.00$ & $2.07\substack{+0.01\\ -0.01}$ & $278.38$ & $415$ \\ 
58941.71 & $32.73\pm0.22$ & $0.82$ & $675.00$ & $2.02\substack{+0.01\\ -0.01}$ & $169.93$ & $316$ \\ 
58943.49 & $35.15\pm0.25$ & $0.75$ & $586.00$ & $2.09\substack{+0.01\\ -0.01}$ & $386.51$ & $456$ \\ 
58945.04 & $41.40\pm0.46$ & $0.69$ & $196.00$ & $2.12\substack{+0.02\\ -0.02}$ & $297.55$ & $832$ \\ 
58953.41 & $41.78\pm0.36$ & $4.38$ & $355.00$ & $2.25\substack{+0.02\\ -0.01}$ & $152.72$ & $136$ \\ 
58955.66 & $51.52\pm0.29$ & $1.05$ & $615.00$ & $2.29\substack{+0.01\\ -0.01}$ & $131.70$ & $188$ \\ 
58957.37 & $56.38\pm0.50$ & $3.03$ & $240.00$ & $2.21\substack{+0.02\\ -0.02}$ & $317.01$ & $166$ \\ 
58963.87 & $46.47\pm0.74$ & $1.53$ & $87.00$ & $2.23\substack{+0.03\\ -0.03}$ & $353.89$ & $491$ \\ 
58994.55 & $43.71\pm0.31$ & $0.65$ & $469.00$ & $2.24\substack{+0.01\\ -0.01}$ & $180.37$ & $222$ \\ 
59008.58 & $38.70\pm0.17$ & $1.50$ & $1405.00$ & $2.02\substack{+0.01\\ -0.01}$ & $155.70$ & $151$ \\ 
59014.56 & $39.66\pm0.26$ & $1.08$ & $600.00$ & $2.23\substack{+0.01\\ -0.01}$ & $95.27$ & $90$ \\ 
59022.88 & $34.41\pm0.46$ & $7.48$ & $201.00$ & $2.38\substack{+0.02\\ -0.02}$ & $214.89$ & $117$ \\ 
59025.00 & $42.79\pm0.62$ & $2.71$ & $120.00$ & $2.31\substack{+0.03\\ -0.03}$ & $96.01$ & $77$ \\ 
59028.72 & $45.44\pm0.21$ & $2.29$ & $1117.00$ & $2.16\substack{+0.01\\ -0.01}$ & $167.29$ & $144$ \\ 
59029.88 & $39.38\pm0.31$ & $0.96$ & $417.00$ & $2.12\substack{+0.01\\ -0.01}$ & $93.80$ & $124$ \\ 
59044.02 & $35.60\pm1.55$ & $0.40$ & $15.00$ & $2.29\substack{+0.09\\ -0.09}$ & $396.00$ & $1241$ \\ 
59053.89 & $42.79\pm0.35$ & $1.27$ & $360.00$ & $2.24\substack{+0.01\\ -0.01}$ & $79.08$ & $78$ \\ 
59056.46 & $38.18\pm0.25$ & $0.78$ & $600.00$ & $2.30\substack{+0.01\\ -0.01}$ & $221.06$ & $227$ \\ 
59060.66 & $43.47\pm0.19$ & $0.71$ & $1194.00$ & $2.24\substack{+0.01\\ -0.01}$ & $122.81$ & $134$ \\ 
59062.59 & $48.19\pm0.24$ & $0.58$ & $883.00$ & $2.22\substack{+0.01\\ -0.01}$ & $122.62$ & $107$ \\ 
59064.59 & $44.03\pm0.23$ & $1.05$ & $858.00$ & $2.18\substack{+0.01\\ -0.01}$ & $119.86$ & $116$ \\ 
59066.56 & $46.13\pm0.22$ & $0.57$ & $972.00$ & $2.21\substack{+0.01\\ -0.01}$ & $133.01$ & $114$ \\ 
59070.86 & $44.83\pm0.44$ & $1.86$ & $240.00$ & $2.21\substack{+0.02\\ -0.02}$ & $85.04$ & $137$ \\ 
59072.73 & $47.78\pm0.32$ & $1.93$ & $473.00$ & $2.14\substack{+0.01\\ -0.01}$ & $141.14$ & $135$ \\ 
59074.96 & $47.47\pm0.29$ & $3.65$ & $592.00$ & $2.30\substack{+0.01\\ -0.01}$ & $175.11$ & $157$ \\ 
59076.91 & $42.10\pm0.21$ & $0.51$ & $960.00$ & $2.27\substack{+0.01\\ -0.01}$ & $157.81$ & $241$ \\ 
59077.97 & $39.80\pm0.21$ & $0.67$ & $960.00$ & $2.20\substack{+0.01\\ -0.01}$ & $244.41$ & $277$ \\ 
59080.91 & $39.00\pm0.20$ & $0.54$ & $1018.00$ & $2.17\substack{+0.01\\ -0.01}$ & $125.93$ & $142$ \\ 
59082.88 & $41.74\pm0.30$ & $0.54$ & $480.00$ & $2.22\substack{+0.01\\ -0.01}$ & $149.71$ & $286$ \\ 
59083.01 & $42.88\pm0.24$ & $0.61$ & $775.00$ & $2.23\substack{+0.01\\ -0.01}$ & $193.81$ & $267$ \\ 
59084.93 & $32.28\pm0.27$ & $2.56$ & $467.00$ & $2.13\substack{+0.02\\ -0.02}$ & $133.50$ & $126$ \\ 
59093.97 & $24.53\pm0.33$ & $0.87$ & $240.00$ & $1.96\substack{+0.02\\ -0.02}$ & $95.85$ & $141$ \\ 
59109.31 & $32.50\pm0.54$ & $2.08$ & $120.00$ & $2.11\substack{+0.03\\ -0.03}$ & $71.42$ & $181$ \\ 
59116.29 & $27.64\pm0.20$ & $0.82$ & $684.00$ & $2.04\substack{+0.01\\ -0.01}$ & $145.70$ & $202$ \\ 
59118.43 & $27.81\pm0.14$ & $0.84$ & $1461.00$ & $1.97\substack{+0.01\\ -0.01}$ & $168.16$ & $158$ \\ 
59120.59 & $28.97\pm0.18$ & $1.04$ & $956.00$ & $2.00\substack{+0.01\\ -0.01}$ & $192.99$ & $200$ \\ 
59122.53 & $36.07\pm0.16$ & $0.86$ & $1378.00$ & $2.09\substack{+0.01\\ -0.01}$ & $119.11$ & $114$ \\ 
59124.47 & $28.49\pm0.19$ & $0.85$ & $805.00$ & $2.09\substack{+0.01\\ -0.01}$ & $124.23$ & $199$ \\ 
59126.20 & $31.36\pm0.28$ & $0.54$ & $412.00$ & $2.12\substack{+0.01\\ -0.01}$ & $219.43$ & $444$ \\ 
59128.12 & $31.05\pm0.24$ & $2.07$ & $558.00$ & $2.10\substack{+0.01\\ -0.01}$ & $123.10$ & $141$ \\ 
59129.56 & $33.57\pm0.20$ & $0.65$ & $875.00$ & $2.11\substack{+0.01\\ -0.01}$ & $161.42$ & $252$ \\ 
59130.75 & $36.70\pm0.23$ & $0.96$ & $695.00$ & $2.09\substack{+0.01\\ -0.01}$ & $188.60$ & $212$ \\ 
59136.85 & $36.28\pm0.64$ & $0.47$ & $91.00$ & $2.09\substack{+0.03\\ -0.03}$ & $35.30$ & $160$ \\ 
59138.33 & $36.94\pm0.28$ & $0.80$ & $480.00$ & $2.15\substack{+0.01\\ -0.01}$ & $135.26$ & $295$ \\ 
59141.04 & $33.66\pm0.38$ & $0.70$ & $240.00$ & $2.16\substack{+0.02\\ -0.02}$ & $103.80$ & $224$ \\ 
59142.79 & $31.51\pm0.46$ & $1.92$ & $161.00$ & $2.13\substack{+0.02\\ -0.02}$ & $64.12$ & $67$ \\ 
59144.40 & $32.70\pm0.27$ & $1.23$ & $469.00$ & $2.16\substack{+0.01\\ -0.01}$ & $84.20$ & $88$ \\ 
59148.93 & $34.40\pm0.22$ & $0.72$ & $744.00$ & $2.13\substack{+0.01\\ -0.01}$ & $101.61$ & $142$ \\ 
59150.52 & $29.16\pm0.18$ & $0.40$ & $928.00$ & $2.13\substack{+0.01\\ -0.01}$ & $135.18$ & $294$ \\ 
59151.84 & $32.58\pm0.19$ & $0.81$ & $886.00$ & $2.20\substack{+0.01\\ -0.01}$ & $103.30$ & $152$ \\ 
59153.87 & $29.01\pm0.16$ & $0.51$ & $1090.00$ & $2.21\substack{+0.01\\ -0.01}$ & $144.36$ & $108$ \\ 
59155.71 & $28.86\pm0.23$ & $0.44$ & $574.00$ & $2.18\substack{+0.01\\ -0.01}$ & $179.05$ & $418$ \\ 
59157.68 & $31.44\pm0.18$ & $0.50$ & $944.00$ & $2.30\substack{+0.01\\ -0.01}$ & $205.32$ & $292$ \\ 
59179.54 & $39.16\pm0.24$ & $0.43$ & $669.00$ & $2.14\substack{+0.01\\ -0.01}$ & $133.57$ & $238$ \\ 
59181.25 & $33.11\pm0.27$ & $0.59$ & $470.00$ & $2.15\substack{+0.01\\ -0.01}$ & $196.72$ & $467$ \\ 
59183.48 & $28.12\pm0.18$ & $0.35$ & $860.00$ & $2.08\substack{+0.01\\ -0.01}$ & $104.72$ & $140$ \\ 
59185.35 & $29.64\pm0.17$ & $0.34$ & $1050.00$ & $2.10\substack{+0.01\\ -0.01}$ & $281.48$ & $312$ \\ 
59187.36 & $29.50\pm0.28$ & $0.66$ & $384.00$ & $2.12\substack{+0.02\\ -0.02}$ & $125.50$ & $142$ \\ 
59189.60 & $26.96\pm0.25$ & $0.42$ & $436.00$ & $2.15\substack{+0.02\\ -0.02}$ & $259.58$ & $681$ \\ 
59192.98 & $35.67\pm0.56$ & $1.31$ & $120.00$ & $2.06\substack{+0.03\\ -0.03}$ & $104.28$ & $217$ \\ 
59213.22 & $30.43\pm0.17$ & $0.90$ & $1106.00$ & $2.03\substack{+0.01\\ -0.01}$ & $147.22$ & $143$ \\ 
59215.07 & $39.34\pm0.25$ & $0.85$ & $628.00$ & $2.15\substack{+0.01\\ -0.01}$ & $168.70$ & $254$ \\ 
59217.23 & $41.51\pm0.43$ & $1.41$ & $231.00$ & $2.12\substack{+0.02\\ -0.02}$ & $98.84$ & $180$ \\ 
59219.45 & $30.67\pm0.23$ & $1.45$ & $586.00$ & $2.09\substack{+0.01\\ -0.01}$ & $85.28$ & $106$ \\ 
59223.62 & $26.52\pm0.33$ & $1.73$ & $255.00$ & $2.10\substack{+0.02\\ -0.02}$ & $61.03$ & $75$ \\ 
59225.17 & $22.74\pm0.22$ & $0.75$ & $508.00$ & $2.05\substack{+0.02\\ -0.02}$ & $89.33$ & $144$ \\ 
59226.98 & $20.35\pm0.19$ & $0.99$ & $615.13$ & $2.08\substack{+0.02\\ -0.02}$ & $182.15$ & $202$ \\ 
59227.05 & $21.18\pm0.30$ & $0.73$ & $240.00$ & $2.05\substack{+0.03\\ -0.03}$ & $53.33$ & $82$ \\ 
59228.97 & $25.27\pm0.15$ & $1.28$ & $1160.00$ & $2.13\substack{+0.01\\ -0.01}$ & $107.42$ & $106$ \\ 
59231.63 & $26.41\pm0.47$ & $0.54$ & $120.00$ & $2.23\substack{+0.03\\ -0.03}$ & $365.55$ & $964$ \\ 
59232.02 & $21.46\pm0.25$ & $0.43$ & $360.00$ & $2.20\substack{+0.02\\ -0.02}$ & $105.79$ & $459$ \\ 
59233.24 & $20.41\pm0.42$ & $0.42$ & $120.00$ & $2.14\substack{+0.04\\ -0.04}$ & $171.59$ & $723$ \\ 
59234.98 & $14.09\pm0.30$ & $0.88$ & $165.00$ & $2.03\substack{+0.04\\ -0.04}$ & $215.57$ & $655$ \\ 
59239.47 & $21.17\pm0.09$ & $0.86$ & $2692.00$ & $2.17\substack{+0.01\\ -0.01}$ & $302.59$ & $157$ \\ 
59240.26 & $22.71\pm0.50$ & $7.59$ & $120.00$ & $2.37\substack{+0.04\\ -0.04}$ & $326.74$ & $79$ \\ 
59241.17 & $22.43\pm0.29$ & $5.02$ & $326.00$ & $2.31\substack{+0.03\\ -0.03}$ & $135.30$ & $115$ \\ 
59243.24 & $21.08\pm0.17$ & $0.96$ & $720.00$ & $2.19\substack{+0.02\\ -0.02}$ & $161.36$ & $180$ \\ 
59245.18 & $26.35\pm0.26$ & $0.80$ & $412.00$ & $2.31\substack{+0.02\\ -0.02}$ & $142.50$ & $370$ \\ 
59248.92 & $37.25\pm0.25$ & $0.81$ & $615.00$ & $2.15\substack{+0.01\\ -0.01}$ & $244.12$ & $148$ \\ 
59253.48 & $35.81\pm0.56$ & $1.18$ & $120.00$ & $2.25\substack{+0.03\\ -0.03}$ & $124.90$ & $337$ \\ 
59255.41 & $35.10\pm0.28$ & $0.51$ & $469.00$ & $2.35\substack{+0.01\\ -0.01}$ & $157.10$ & $326$ \\ 
59257.22 & $40.71\pm0.43$ & $2.73$ & $240.00$ & $2.36\substack{+0.02\\ -0.02}$ & $111.88$ & $104$ \\ 
59258.56 & $41.16\pm0.34$ & $1.52$ & $373.00$ & $2.12\substack{+0.02\\ -0.02}$ & $335.86$ & $164$ \\ 


==> Table7.tex <==
58251.66 & $1.71\pm0.11$ & $-10.23\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.781\substack{+0.008\\ -0.008}$ & $40.36$ & $39$ \\ 
58252.46 & $1.69\pm0.10$ & $-10.24\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.775\substack{+0.008\\ -0.008}$ & $32.81$ & $92$ \\ 
58253.86 & $1.71\pm0.10$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.749\substack{+0.008\\ -0.008}$ & $37.71$ & $42$ \\ 
58254.58 & $1.76\pm0.10$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.759\substack{+0.008\\ -0.008}$ & $46.36$ & $39$ \\ 
58255.52 & $1.49\pm0.08$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.751\substack{+0.008\\ -0.008}$ & $62.90$ & $41$ \\ 
58256.11 & $1.67\pm0.11$ & $-10.23\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.738\substack{+0.008\\ -0.008}$ & $35.88$ & $37$ \\ 
58257.05 & $1.58\pm0.09$ & $-10.27\substack{+0.02\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.729\substack{+0.008\\ -0.008}$ & $44.53$ & $41$ \\ 
58263.77 & $2.17\pm0.12$ & $-10.14\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.598\substack{+0.008\\ -0.008}$ & $40.75$ & $42$ \\ 
58264.90 & $2.07\pm0.11$ & $-10.16\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.591\substack{+0.008\\ -0.008}$ & $35.63$ & $41$ \\ 
58265.75 & $2.42\pm0.12$ & $-10.10\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.592\substack{+0.008\\ -0.008}$ & $24.93$ & $41$ \\ 
58266.09 & $2.16\pm0.10$ & $-10.17\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.592\substack{+0.008\\ -0.008}$ & $64.06$ & $43$ \\ 
58267.48 & $1.83\pm0.11$ & $-10.22\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.587\substack{+0.008\\ -0.008}$ & $42.84$ & $86$ \\ 
58268.81 & $1.92\pm0.09$ & $-10.21\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.660\substack{+0.008\\ -0.008}$ & $34.90$ & $57$ \\ 
58269.74 & $1.66\pm0.09$ & $-10.23\substack{+0.02\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.634\substack{+0.008\\ -0.008}$ & $31.27$ & $42$ \\ 
58270.74 & $2.01\pm0.10$ & $-10.18\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.636\substack{+0.008\\ -0.008}$ & $28.90$ & $42$ \\ 
58271.73 & $1.74\pm0.10$ & $-10.23\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.624\substack{+0.008\\ -0.008}$ & $34.09$ & $81$ \\ 
58272.66 & $1.68\pm0.11$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.605\substack{+0.008\\ -0.008}$ & $29.74$ & $44$ \\ 
58274.91 & $1.67\pm0.09$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.562\substack{+0.008\\ -0.008}$ & $55.71$ & $49$ \\ 
58275.93 & $1.59\pm0.10$ & $-10.31\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.528\substack{+0.008\\ -0.008}$ & $36.10$ & $40$ \\ 
58276.57 & $1.47\pm0.09$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.528\substack{+0.008\\ -0.008}$ & $49.40$ & $39$ \\ 
58277.57 & $1.35\pm0.07$ & $-10.38\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.530\substack{+0.008\\ -0.008}$ & $38.81$ & $68$ \\ 
58278.57 & $1.55\pm0.08$ & $-10.34\substack{+0.02\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.547\substack{+0.008\\ -0.008}$ & $39.16$ & $243$ \\ 
58279.23 & $1.66\pm0.09$ & $-10.27\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.553\substack{+0.008\\ -0.008}$ & $36.67$ & $42$ \\ 
58280.82 & $1.57\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.571\substack{+0.008\\ -0.008}$ & $47.02$ & $43$ \\ 
58281.82 & $1.43\pm0.08$ & $-10.36\substack{+0.02\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.604\substack{+0.008\\ -0.008}$ & $47.37$ & $58$ \\ 
58282.81 & $1.57\pm0.07$ & $-10.32\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.609\substack{+0.008\\ -0.008}$ & $59.50$ & $43$ \\ 
58284.94 & $1.37\pm0.08$ & $-10.38\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.626\substack{+0.008\\ -0.008}$ & $37.28$ & $37$ \\ 
58285.74 & $1.72\pm0.15$ & $-10.25\substack{+0.05\\ -0.05}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.639\substack{+0.008\\ -0.008}$ & $38.26$ & $169$ \\ 
58286.07 & $1.53\pm0.08$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.644\substack{+0.008\\ -0.008}$ & $33.83$ & $48$ \\ 
58287.73 & $1.33\pm0.08$ & $-10.32\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.651\substack{+0.008\\ -0.008}$ & $29.02$ & $43$ \\ 
58288.93 & $1.63\pm0.10$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.671\substack{+0.008\\ -0.008}$ & $28.93$ & $39$ \\ 
58289.72 & $2.00\pm0.14$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.661\substack{+0.008\\ -0.008}$ & $40.14$ & $216$ \\ 
58290.06 & $1.95\pm0.09$ & $-10.22\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.656\substack{+0.008\\ -0.008}$ & $45.97$ & $43$ \\ 
58291.58 & $1.68\pm0.11$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.692\substack{+0.008\\ -0.008}$ & $42.68$ & $69$ \\ 
58292.51 & $1.34\pm0.10$ & $-10.31\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.707\substack{+0.008\\ -0.008}$ & $39.75$ & $158$ \\ 
58294.04 & $1.44\pm0.08$ & $-10.34\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.732\substack{+0.008\\ -0.008}$ & $48.29$ & $41$ \\ 
58295.83 & $1.36\pm0.08$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.762\substack{+0.008\\ -0.008}$ & $48.04$ & $59$ \\ 
58296.03 & $1.24\pm0.07$ & $-10.37\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.758\substack{+0.008\\ -0.008}$ & $45.81$ & $41$ \\ 
58297.09 & $1.42\pm0.11$ & $-10.35\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.752\substack{+0.008\\ -0.008}$ & $42.38$ & $69$ \\ 
58298.03 & $1.50\pm0.13$ & $-10.30\substack{+0.04\\ -0.04}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.737\substack{+0.008\\ -0.008}$ & $28.88$ & $85$ \\ 
58299.68 & $1.62\pm0.09$ & $-10.27\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.746\substack{+0.008\\ -0.008}$ & $44.81$ & $92$ \\ 
58300.69 & $1.74\pm0.13$ & $-10.24\substack{+0.03\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.745\substack{+0.008\\ -0.008}$ & $30.86$ & $36$ \\ 
58301.22 & $1.66\pm0.09$ & $-10.28\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.755\substack{+0.008\\ -0.008}$ & $43.35$ & $40$ \\ 
58302.42 & $1.63\pm0.11$ & $-10.26\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.800\substack{+0.008\\ -0.008}$ & $40.54$ & $79$ \\ 
58303.24 & $1.53\pm0.06$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.771\substack{+0.008\\ -0.008}$ & $55.54$ & $47$ \\ 
58304.34 & $1.90\pm0.09$ & $-10.22\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.760\substack{+0.008\\ -0.008}$ & $46.04$ & $40$ \\ 
58305.33 & $1.76\pm0.10$ & $-10.23\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.820\substack{+0.008\\ -0.008}$ & $33.73$ & $42$ \\ 
58306.65 & $1.90\pm0.10$ & $-10.21\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.864\substack{+0.008\\ -0.008}$ & $40.18$ & $43$ \\ 
58307.25 & $1.46\pm0.09$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.900\substack{+0.008\\ -0.008}$ & $36.88$ & $39$ \\ 
58308.25 & $1.19\pm0.08$ & $-10.38\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.957\substack{+0.008\\ -0.008}$ & $38.64$ & $161$ \\ 
58309.99 & $1.08\pm0.08$ & $-10.42\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.000\substack{+0.008\\ -0.008}$ & $51.44$ & $120$ \\ 
58310.32 & $1.00\pm0.07$ & $-10.46\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.991\substack{+0.008\\ -0.008}$ & $33.46$ & $37$ \\ 
58311.51 & $1.00\pm0.08$ & $-10.47\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.051\substack{+0.008\\ -0.008}$ & $29.95$ & $52$ \\ 
58312.31 & $1.16\pm0.08$ & $-10.43\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.085\substack{+0.008\\ -0.008}$ & $45.85$ & $39$ \\ 
58313.31 & $1.34\pm0.11$ & $-10.37\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.037\substack{+0.008\\ -0.008}$ & $34.42$ & $127$ \\ 
58314.04 & $1.32\pm0.07$ & $-10.36\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.046\substack{+0.008\\ -0.008}$ & $62.18$ & $128$ \\ 
58315.17 & $1.28\pm0.07$ & $-10.39\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.090\substack{+0.008\\ -0.008}$ & $37.90$ & $44$ \\ 
58316.16 & $1.37\pm0.08$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.079\substack{+0.008\\ -0.008}$ & $40.18$ & $42$ \\ 
58317.62 & $1.47\pm0.07$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.089\substack{+0.008\\ -0.008}$ & $30.23$ & $42$ \\ 
58318.69 & $1.43\pm0.09$ & $-10.30\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.104\substack{+0.008\\ -0.008}$ & $34.88$ & $40$ \\ 
58319.75 & $1.33\pm0.09$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.157\substack{+0.008\\ -0.008}$ & $25.00$ & $37$ \\ 
58320.54 & $1.12\pm0.07$ & $-10.40\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.201\substack{+0.008\\ -0.008}$ & $45.94$ & $39$ \\ 
58321.01 & $1.11\pm0.06$ & $-10.40\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.230\substack{+0.008\\ -0.008}$ & $51.17$ & $123$ \\ 
58322.08 & $1.11\pm0.06$ & $-10.47\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.295\substack{+0.008\\ -0.008}$ & $51.71$ & $41$ \\ 
58323.93 & $1.29\pm0.07$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.313\substack{+0.008\\ -0.008}$ & $35.07$ & $41$ \\ 
58324.19 & $1.07\pm0.07$ & $-10.45\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.296\substack{+0.008\\ -0.008}$ & $52.25$ & $42$ \\ 
58325.93 & $1.38\pm0.07$ & $-10.36\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.261\substack{+0.008\\ -0.008}$ & $37.78$ & $46$ \\ 
58326.59 & $1.81\pm0.11$ & $-10.24\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.231\substack{+0.008\\ -0.008}$ & $47.31$ & $77$ \\ 
58327.59 & $1.44\pm0.09$ & $-10.31\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.192\substack{+0.008\\ -0.008}$ & $34.06$ & $90$ \\ 
58328.57 & $1.32\pm0.08$ & $-10.38\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.170\substack{+0.008\\ -0.008}$ & $25.02$ & $84$ \\ 
58329.65 & $1.38\pm0.07$ & $-10.34\substack{+0.02\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.148\substack{+0.008\\ -0.008}$ & $51.56$ & $42$ \\ 
58331.57 & $1.38\pm0.07$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.111\substack{+0.008\\ -0.008}$ & $57.72$ & $42$ \\ 
58332.82 & $1.44\pm0.08$ & $-10.34\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.061\substack{+0.008\\ -0.008}$ & $40.02$ & $78$ \\ 
58333.95 & $1.24\pm0.06$ & $-10.42\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.068\substack{+0.008\\ -0.008}$ & $58.62$ & $44$ \\ 
58334.69 & $1.59\pm0.07$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.073\substack{+0.008\\ -0.008}$ & $40.68$ & $43$ \\ 
58335.74 & $1.52\pm0.11$ & $-10.27\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.076\substack{+0.008\\ -0.008}$ & $51.26$ & $305$ \\ 
58336.75 & $1.62\pm0.09$ & $-10.28\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.030\substack{+0.008\\ -0.008}$ & $40.61$ & $91$ \\ 
58337.95 & $1.66\pm0.14$ & $-10.23\substack{+0.04\\ -0.04}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.003\substack{+0.008\\ -0.008}$ & $38.26$ & $88$ \\ 
58338.86 & $1.48\pm0.07$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.019\substack{+0.008\\ -0.008}$ & $47.83$ & $67$ \\ 
58339.74 & $1.84\pm0.27$ & $-10.20\substack{+0.06\\ -0.06}$ & $2.2\substack{+0.2\\ -0.2}$ & $-12.057\substack{+0.008\\ -0.008}$ & $19.61$ & $322$ \\ 
58340.01 & $1.67\pm0.10$ & $-10.25\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.065\substack{+0.008\\ -0.008}$ & $38.74$ & $51$ \\ 
58341.01 & $1.67\pm0.10$ & $-10.26\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.077\substack{+0.008\\ -0.008}$ & $22.25$ & $40$ \\ 
58343.06 & $1.66\pm0.10$ & $-10.21\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.103\substack{+0.008\\ -0.008}$ & $53.39$ & $40$ \\ 
58345.86 & $1.60\pm0.10$ & $-10.27\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.110\substack{+0.008\\ -0.008}$ & $27.97$ & $38$ \\ 
58346.90 & $1.35\pm0.09$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.102\substack{+0.008\\ -0.008}$ & $50.47$ & $37$ \\ 
58347.30 & $1.25\pm0.07$ & $-10.35\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.112\substack{+0.008\\ -0.008}$ & $40.11$ & $41$ \\ 
58348.44 & $1.53\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.143\substack{+0.008\\ -0.008}$ & $41.91$ & $141$ \\ 
58349.03 & $1.53\pm0.08$ & $-10.28\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.160\substack{+0.008\\ -0.008}$ & $36.39$ & $91$ \\ 
58350.10 & $1.50\pm0.09$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.192\substack{+0.008\\ -0.008}$ & $36.16$ & $41$ \\ 
58351.23 & $1.30\pm0.06$ & $-10.39\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.213\substack{+0.008\\ -0.008}$ & $47.42$ & $45$ \\ 
58352.89 & $1.59\pm0.11$ & $-10.28\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.246\substack{+0.008\\ -0.008}$ & $26.13$ & $37$ \\ 
58353.60 & $1.26\pm0.08$ & $-10.37\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.261\substack{+0.008\\ -0.008}$ & $41.26$ & $81$ \\ 
58354.62 & $1.53\pm0.09$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.263\substack{+0.008\\ -0.008}$ & $45.32$ & $41$ \\ 
58355.61 & $1.33\pm0.11$ & $-10.33\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.157\substack{+0.008\\ -0.008}$ & $31.57$ & $35$ \\ 
58356.60 & $1.23\pm0.07$ & $-10.39\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.265\substack{+0.008\\ -0.008}$ & $36.99$ & $46$ \\ 
58357.60 & $1.35\pm0.11$ & $-10.36\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.198\substack{+0.008\\ -0.008}$ & $39.12$ & $154$ \\ 
58358.73 & $1.60\pm0.13$ & $-10.25\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.376\substack{+0.008\\ -0.008}$ & $20.73$ & $41$ \\ 
58359.13 & $1.22\pm0.07$ & $-10.39\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.397\substack{+0.008\\ -0.008}$ & $45.65$ & $127$ \\ 
58361.52 & $1.04\pm0.10$ & $-10.45\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.453\substack{+0.008\\ -0.008}$ & $27.56$ & $29$ \\ 
58361.99 & $0.89\pm0.07$ & $-10.51\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.482\substack{+0.008\\ -0.008}$ & $30.02$ & $37$ \\ 
58362.25 & $0.94\pm0.07$ & $-10.49\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.472\substack{+0.008\\ -0.008}$ & $38.85$ & $36$ \\ 
58363.12 & $1.20\pm0.07$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.431\substack{+0.008\\ -0.008}$ & $43.29$ & $75$ \\ 
58364.71 & $1.54\pm0.10$ & $-10.30\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.359\substack{+0.008\\ -0.008}$ & $34.91$ & $54$ \\ 
58365.18 & $1.38\pm0.07$ & $-10.33\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.340\substack{+0.008\\ -0.008}$ & $26.58$ & $42$ \\ 
58366.31 & $1.27\pm0.07$ & $-10.37\substack{+0.02\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.313\substack{+0.008\\ -0.008}$ & $40.80$ & $42$ \\ 
58367.04 & $1.54\pm0.08$ & $-10.26\substack{+0.02\\ -0.02}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.318\substack{+0.008\\ -0.008}$ & $46.26$ & $44$ \\ 
58368.04 & $1.65\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.326\substack{+0.008\\ -0.008}$ & $47.12$ & $45$ \\ 
58369.96 & $1.16\pm0.07$ & $-10.42\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.205\substack{+0.008\\ -0.008}$ & $55.27$ & $124$ \\ 
58370.49 & $1.24\pm0.10$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.223\substack{+0.008\\ -0.008}$ & $31.28$ & $38$ \\ 
58372.15 & $1.31\pm0.07$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.208\substack{+0.008\\ -0.008}$ & $53.76$ & $172$ \\ 
58373.02 & $1.46\pm0.08$ & $-10.30\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.299\substack{+0.008\\ -0.008}$ & $44.35$ & $105$ \\ 
58374.01 & $1.38\pm0.08$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.439\substack{+0.008\\ -0.008}$ & $29.24$ & $40$ \\ 
58375.73 & $1.17\pm0.07$ & $-10.39\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.577\substack{+0.008\\ -0.008}$ & $24.37$ & $91$ \\ 
58376.39 & $1.28\pm0.08$ & $-10.37\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.588\substack{+0.008\\ -0.008}$ & $20.29$ & $163$ \\ 
58378.52 & $1.14\pm0.12$ & $-10.38\substack{+0.05\\ -0.05}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.635\substack{+0.008\\ -0.008}$ & $19.36$ & $31$ \\ 
58379.06 & $1.29\pm0.08$ & $-10.39\substack{+0.02\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.650\substack{+0.008\\ -0.008}$ & $57.36$ & $42$ \\ 
58380.06 & $1.07\pm0.08$ & $-10.45\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.679\substack{+0.008\\ -0.008}$ & $51.18$ & $138$ \\ 
58381.13 & $0.89\pm0.06$ & $-10.52\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.712\substack{+0.008\\ -0.008}$ & $70.96$ & $43$ \\ 
58382.58 & $1.12\pm0.06$ & $-10.42\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-13.332\substack{+0.008\\ -0.008}$ & $41.83$ & $93$ \\ 
58383.37 & $0.98\pm0.07$ & $-10.45\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-13.430\substack{+0.008\\ -0.008}$ & $26.44$ & $62$ \\ 
58384.69 & $0.98\pm0.07$ & $-10.44\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-13.209\substack{+0.008\\ -0.008}$ & $37.90$ & $43$ \\ 
58385.04 & $1.06\pm0.07$ & $-10.47\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-13.152\substack{+0.008\\ -0.008}$ & $43.26$ & $88$ \\ 
58386.57 & $1.31\pm0.14$ & $-10.30\substack{+0.05\\ -0.05}$ & $1.6\substack{+0.2\\ -0.2}$ & $-12.816\substack{+0.008\\ -0.008}$ & $35.40$ & $61$ \\ 
58387.77 & $1.10\pm0.07$ & $-10.41\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.816\substack{+0.008\\ -0.008}$ & $37.13$ & $41$ \\ 
58388.21 & $1.28\pm0.06$ & $-10.36\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.807\substack{+0.008\\ -0.008}$ & $39.89$ & $42$ \\ 
58389.02 & $1.37\pm0.08$ & $-10.32\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.792\substack{+0.008\\ -0.008}$ & $51.90$ & $207$ \\ 
58390.27 & $1.28\pm0.07$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-13.565\substack{+0.008\\ -0.008}$ & $35.96$ & $39$ \\ 
58391.60 & $1.44\pm0.09$ & $-10.30\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.983\substack{+0.008\\ -0.008}$ & $35.71$ & $133$ \\ 
58392.87 & $1.35\pm0.09$ & $-10.30\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.788\substack{+0.008\\ -0.008}$ & $32.07$ & $39$ \\ 
58393.19 & $1.36\pm0.08$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.775\substack{+0.008\\ -0.008}$ & $36.63$ & $80$ \\ 
58395.25 & $1.30\pm0.09$ & $-10.37\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.885\substack{+0.008\\ -0.008}$ & $30.01$ & $39$ \\ 
58396.39 & $0.98\pm0.07$ & $-10.45\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.633\substack{+0.008\\ -0.008}$ & $34.21$ & $42$ \\ 
58397.45 & $1.20\pm0.07$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.6\substack{+0.1\\ -0.1}$ & $-12.659\substack{+0.008\\ -0.008}$ & $42.30$ & $119$ \\ 
58398.32 & $1.44\pm0.07$ & $-10.32\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.670\substack{+0.008\\ -0.008}$ & $36.19$ & $42$ \\ 
58399.37 & $1.34\pm0.08$ & $-10.33\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.450\substack{+0.008\\ -0.008}$ & $43.09$ & $105$ \\ 
58400.16 & $1.34\pm0.11$ & $-10.36\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.394\substack{+0.008\\ -0.008}$ & $28.38$ & $55$ \\ 
58401.97 & $1.16\pm0.07$ & $-10.42\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.446\substack{+0.008\\ -0.008}$ & $47.06$ & $40$ \\ 
58402.43 & $1.28\pm0.08$ & $-10.37\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.464\substack{+0.008\\ -0.008}$ & $59.08$ & $39$ \\ 
58403.03 & $1.50\pm0.10$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.490\substack{+0.008\\ -0.008}$ & $46.38$ & $135$ \\ 
58404.75 & $0.98\pm0.06$ & $-10.48\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.527\substack{+0.008\\ -0.008}$ & $30.19$ & $102$ \\ 
58405.35 & $1.05\pm0.06$ & $-10.47\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.506\substack{+0.008\\ -0.008}$ & $45.60$ & $124$ \\ 
58406.81 & $1.31\pm0.12$ & $-10.36\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.485\substack{+0.008\\ -0.008}$ & $32.80$ & $32$ \\ 
58407.33 & $1.72\pm0.13$ & $-10.23\substack{+0.04\\ -0.04}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.397\substack{+0.008\\ -0.008}$ & $33.25$ & $95$ \\ 
58408.40 & $1.48\pm0.08$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.375\substack{+0.008\\ -0.008}$ & $32.71$ & $41$ \\ 
58410.86 & $1.37\pm0.07$ & $-10.36\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.308\substack{+0.008\\ -0.008}$ & $52.74$ & $65$ \\ 
58411.79 & $1.07\pm0.06$ & $-10.46\substack{+0.02\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.229\substack{+0.008\\ -0.008}$ & $51.66$ & $45$ \\ 
58412.92 & $1.09\pm0.06$ & $-10.45\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.230\substack{+0.008\\ -0.008}$ & $26.54$ & $138$ \\ 
58413.46 & $1.25\pm0.08$ & $-10.38\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.208\substack{+0.008\\ -0.008}$ & $42.79$ & $186$ \\ 
58414.72 & $1.14\pm0.07$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.159\substack{+0.008\\ -0.008}$ & $24.72$ & $83$ \\ 
58415.85 & $1.09\pm0.07$ & $-10.43\substack{+0.02\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.164\substack{+0.008\\ -0.008}$ & $26.86$ & $195$ \\ 
58416.45 & $1.31\pm0.07$ & $-10.39\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.141\substack{+0.008\\ -0.008}$ & $27.74$ & $41$ \\ 
58417.99 & $1.28\pm0.07$ & $-10.36\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.115\substack{+0.008\\ -0.008}$ & $48.73$ & $175$ \\ 
58418.57 & $1.33\pm0.07$ & $-10.39\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.149\substack{+0.008\\ -0.008}$ & $54.86$ & $43$ \\ 
58420.49 & $1.46\pm0.08$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.209\substack{+0.008\\ -0.008}$ & $36.28$ & $39$ \\ 
58421.69 & $1.55\pm0.10$ & $-10.31\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.232\substack{+0.008\\ -0.008}$ & $30.99$ & $228$ \\ 
58422.16 & $1.28\pm0.08$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.281\substack{+0.008\\ -0.008}$ & $37.63$ & $39$ \\ 
58423.28 & $1.40\pm0.09$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.220\substack{+0.008\\ -0.008}$ & $34.32$ & $38$ \\ 
58424.34 & $1.41\pm0.12$ & $-10.31\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.250\substack{+0.008\\ -0.008}$ & $22.41$ & $35$ \\ 
58425.67 & $1.34\pm0.08$ & $-10.33\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.309\substack{+0.008\\ -0.008}$ & $50.34$ & $119$ \\ 
58426.82 & $1.27\pm0.08$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.165\substack{+0.008\\ -0.008}$ & $37.25$ & $36$ \\ 
58427.33 & $1.66\pm0.09$ & $-10.24\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.142\substack{+0.008\\ -0.008}$ & $37.83$ & $83$ \\ 
58428.59 & $1.68\pm0.08$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.111\substack{+0.008\\ -0.008}$ & $44.94$ & $55$ \\ 
58429.79 & $1.88\pm0.11$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.035\substack{+0.008\\ -0.008}$ & $32.16$ & $150$ \\ 
58430.65 & $1.64\pm0.10$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.983\substack{+0.008\\ -0.008}$ & $30.85$ & $40$ \\ 
58431.71 & $1.75\pm0.09$ & $-10.24\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.983\substack{+0.008\\ -0.008}$ & $28.41$ & $43$ \\ 
58433.32 & $1.88\pm0.11$ & $-10.18\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.951\substack{+0.008\\ -0.008}$ & $30.11$ & $63$ \\ 
58434.45 & $1.90\pm0.11$ & $-10.20\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.873\substack{+0.008\\ -0.008}$ & $50.16$ & $101$ \\ 
58435.38 & $1.74\pm0.12$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.975\substack{+0.008\\ -0.008}$ & $51.23$ & $40$ \\ 
58436.38 & $1.95\pm0.13$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.917\substack{+0.008\\ -0.008}$ & $45.36$ & $142$ \\ 
58437.35 & $1.96\pm0.12$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.898\substack{+0.008\\ -0.008}$ & $29.01$ & $42$ \\ 
58438.35 & $1.68\pm0.10$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.873\substack{+0.008\\ -0.008}$ & $59.93$ & $137$ \\ 
58439.69 & $1.43\pm0.08$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.895\substack{+0.008\\ -0.008}$ & $38.78$ & $44$ \\ 
58440.61 & $1.76\pm0.13$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.889\substack{+0.008\\ -0.008}$ & $47.96$ & $205$ \\ 
58441.47 & $2.13\pm0.12$ & $-10.13\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.823\substack{+0.008\\ -0.008}$ & $52.05$ & $42$ \\ 
58442.40 & $1.72\pm0.10$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.817\substack{+0.008\\ -0.008}$ & $35.69$ & $85$ \\ 
58443.27 & $2.17\pm0.11$ & $-10.15\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.841\substack{+0.008\\ -0.008}$ & $32.35$ & $42$ \\ 
58444.53 & $1.78\pm0.12$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.832\substack{+0.008\\ -0.008}$ & $36.16$ & $79$ \\ 
58445.54 & $1.59\pm0.10$ & $-10.30\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.810\substack{+0.008\\ -0.008}$ & $39.28$ & $41$ \\ 
58446.33 & $1.65\pm0.11$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.782\substack{+0.008\\ -0.008}$ & $53.92$ & $117$ \\ 
58447.59 & $1.86\pm0.12$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.875\substack{+0.008\\ -0.008}$ & $23.25$ & $86$ \\ 
58448.59 & $1.84\pm0.11$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.883\substack{+0.008\\ -0.008}$ & $30.89$ & $148$ \\ 
58449.04 & $1.62\pm0.12$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.894\substack{+0.008\\ -0.008}$ & $31.57$ & $91$ \\ 
58450.64 & $1.61\pm0.09$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.921\substack{+0.008\\ -0.008}$ & $33.29$ & $40$ \\ 
58451.37 & $1.34\pm0.08$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.937\substack{+0.008\\ -0.008}$ & $41.42$ & $38$ \\ 
58452.97 & $1.40\pm0.08$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.970\substack{+0.008\\ -0.008}$ & $39.50$ & $61$ \\ 
58453.90 & $1.18\pm0.07$ & $-10.37\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.945\substack{+0.008\\ -0.008}$ & $54.55$ & $40$ \\ 
58454.23 & $1.35\pm0.07$ & $-10.38\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.955\substack{+0.008\\ -0.008}$ & $43.74$ & $45$ \\ 
58455.22 & $1.43\pm0.09$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.074\substack{+0.008\\ -0.008}$ & $29.45$ & $35$ \\ 
58456.56 & $1.13\pm0.07$ & $-10.41\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.022\substack{+0.008\\ -0.008}$ & $36.23$ & $39$ \\ 
58457.34 & $1.08\pm0.08$ & $-10.40\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.087\substack{+0.008\\ -0.008}$ & $44.91$ & $38$ \\ 
58458.48 & $0.97\pm0.07$ & $-10.50\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.079\substack{+0.008\\ -0.008}$ & $30.70$ & $38$ \\ 
58459.47 & $1.02\pm0.06$ & $-10.45\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.137\substack{+0.008\\ -0.008}$ & $34.61$ & $47$ \\ 
58460.34 & $1.33\pm0.12$ & $-10.35\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.084\substack{+0.008\\ -0.008}$ & $19.37$ & $122$ \\ 
58461.87 & $1.25\pm0.07$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.070\substack{+0.008\\ -0.008}$ & $29.04$ & $145$ \\ 
58462.80 & $1.14\pm0.07$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.046\substack{+0.008\\ -0.008}$ & $29.08$ & $145$ \\ 
58463.86 & $1.13\pm0.07$ & $-10.42\substack{+0.02\\ -0.02}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.098\substack{+0.008\\ -0.008}$ & $25.21$ & $61$ \\ 
58464.12 & $1.37\pm0.12$ & $-10.33\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.097\substack{+0.008\\ -0.008}$ & $30.52$ & $31$ \\ 
58465.26 & $1.23\pm0.08$ & $-10.40\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.114\substack{+0.008\\ -0.008}$ & $27.29$ & $40$ \\ 
58466.52 & $1.29\pm0.11$ & $-10.32\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.134\substack{+0.008\\ -0.008}$ & $36.71$ & $50$ \\ 
58467.12 & $1.15\pm0.13$ & $-10.38\substack{+0.06\\ -0.06}$ & $1.6\substack{+0.2\\ -0.2}$ & $-12.127\substack{+0.008\\ -0.008}$ & $15.99$ & $67$ \\ 
58468.05 & $0.81\pm0.06$ & $-10.55\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.108\substack{+0.008\\ -0.008}$ & $33.33$ & $38$ \\ 
58469.78 & $0.95\pm0.09$ & $-10.49\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.093\substack{+0.008\\ -0.008}$ & $33.25$ & $100$ \\ 
58470.11 & $0.95\pm0.11$ & $-10.44\substack{+0.05\\ -0.05}$ & $1.8\substack{+0.2\\ -0.2}$ & $-12.081\substack{+0.008\\ -0.008}$ & $21.79$ & $28$ \\ 
58471.04 & $1.35\pm0.11$ & $-10.33\substack{+0.04\\ -0.04}$ & $1.7\substack{+0.1\\ -0.1}$ & $-12.048\substack{+0.008\\ -0.008}$ & $55.72$ & $79$ \\ 
58472.96 & $1.30\pm0.07$ & $-10.38\substack{+0.02\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.985\substack{+0.008\\ -0.008}$ & $49.12$ & $40$ \\ 
58473.56 & $1.29\pm0.10$ & $-10.36\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.931\substack{+0.008\\ -0.008}$ & $20.11$ & $34$ \\ 
58474.83 & $1.45\pm0.09$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.939\substack{+0.008\\ -0.008}$ & $47.64$ & $136$ \\ 
58475.08 & $1.67\pm0.10$ & $-10.24\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.921\substack{+0.008\\ -0.008}$ & $42.80$ & $42$ \\ 
58476.35 & $1.40\pm0.07$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.886\substack{+0.008\\ -0.008}$ & $33.91$ & $69$ \\ 
58477.62 & $1.41\pm0.07$ & $-10.34\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.868\substack{+0.008\\ -0.008}$ & $45.88$ & $43$ \\ 
58478.74 & $1.53\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.846\substack{+0.008\\ -0.008}$ & $41.08$ & $95$ \\ 
58480.46 & $1.27\pm0.07$ & $-10.40\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.843\substack{+0.008\\ -0.008}$ & $51.76$ & $119$ \\ 
58481.45 & $1.31\pm0.07$ & $-10.33\substack{+0.02\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.840\substack{+0.008\\ -0.008}$ & $42.47$ & $76$ \\ 
58482.25 & $1.63\pm0.13$ & $-10.31\substack{+0.04\\ -0.04}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.790\substack{+0.008\\ -0.008}$ & $44.55$ & $244$ \\ 
58483.18 & $1.37\pm0.08$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.761\substack{+0.008\\ -0.008}$ & $33.11$ & $41$ \\ 
58484.05 & $1.45\pm0.08$ & $-10.30\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.737\substack{+0.008\\ -0.008}$ & $41.58$ & $45$ \\ 
58485.50 & $1.31\pm0.08$ & $-10.40\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.736\substack{+0.008\\ -0.008}$ & $34.42$ & $43$ \\ 
58486.30 & $1.21\pm0.07$ & $-10.41\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.744\substack{+0.008\\ -0.008}$ & $36.98$ & $75$ \\ 
58487.18 & $1.42\pm0.13$ & $-10.35\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.755\substack{+0.008\\ -0.008}$ & $31.59$ & $279$ \\ 
58488.57 & $1.55\pm0.08$ & $-10.35\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.741\substack{+0.008\\ -0.008}$ & $36.94$ & $60$ \\ 
58489.24 & $1.46\pm0.08$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.720\substack{+0.008\\ -0.008}$ & $43.35$ & $41$ \\ 
58490.23 & $1.17\pm0.07$ & $-10.43\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.745\substack{+0.008\\ -0.008}$ & $46.76$ & $133$ \\ 
58491.69 & $1.11\pm0.07$ & $-10.46\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.744\substack{+0.008\\ -0.008}$ & $31.17$ & $41$ \\ 
58493.29 & $1.20\pm0.06$ & $-10.44\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.738\substack{+0.008\\ -0.008}$ & $43.77$ & $42$ \\ 
58494.41 & $1.23\pm0.07$ & $-10.37\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.754\substack{+0.008\\ -0.008}$ & $35.37$ & $39$ \\ 
58495.34 & $1.42\pm0.12$ & $-10.30\substack{+0.04\\ -0.04}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.747\substack{+0.008\\ -0.008}$ & $37.68$ & $86$ \\ 
58496.99 & $1.14\pm0.07$ & $-10.42\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.736\substack{+0.008\\ -0.008}$ & $39.72$ & $44$ \\ 
58497.33 & $1.24\pm0.12$ & $-10.40\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.714\substack{+0.008\\ -0.008}$ & $30.76$ & $228$ \\ 
58498.20 & $1.21\pm0.11$ & $-10.45\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.660\substack{+0.008\\ -0.008}$ & $31.90$ & $243$ \\ 
58499.05 & $1.33\pm0.08$ & $-10.39\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.642\substack{+0.008\\ -0.008}$ & $47.50$ & $40$ \\ 
58500.25 & $1.32\pm0.07$ & $-10.38\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.605\substack{+0.008\\ -0.008}$ & $32.00$ & $128$ \\ 
58501.12 & $1.33\pm0.10$ & $-10.40\substack{+0.04\\ -0.04}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.591\substack{+0.008\\ -0.008}$ & $38.23$ & $263$ \\ 
58502.38 & $1.51\pm0.09$ & $-10.33\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.580\substack{+0.008\\ -0.008}$ & $39.97$ & $37$ \\ 
58503.11 & $1.36\pm0.07$ & $-10.37\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.578\substack{+0.008\\ -0.008}$ & $41.08$ & $75$ \\ 
58504.77 & $1.55\pm0.11$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.553\substack{+0.008\\ -0.008}$ & $53.09$ & $224$ \\ 
58505.03 & $1.70\pm0.07$ & $-10.30\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.551\substack{+0.008\\ -0.008}$ & $40.56$ & $43$ \\ 
58506.95 & $1.32\pm0.08$ & $-10.40\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.563\substack{+0.008\\ -0.008}$ & $50.78$ & $165$ \\ 
58507.81 & $1.33\pm0.07$ & $-10.37\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.553\substack{+0.008\\ -0.008}$ & $38.45$ & $42$ \\ 
58508.34 & $1.34\pm0.08$ & $-10.38\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.553\substack{+0.008\\ -0.008}$ & $37.28$ & $40$ \\ 
58509.28 & $1.36\pm0.09$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.569\substack{+0.008\\ -0.008}$ & $35.37$ & $36$ \\ 
58510.27 & $1.46\pm0.08$ & $-10.34\substack{+0.02\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.547\substack{+0.008\\ -0.008}$ & $48.76$ & $45$ \\ 
58511.20 & $1.20\pm0.07$ & $-10.41\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.538\substack{+0.008\\ -0.008}$ & $31.43$ & $40$ \\ 
58512.20 & $1.29\pm0.07$ & $-10.42\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.519\substack{+0.008\\ -0.008}$ & $42.91$ & $42$ \\ 
58513.93 & $1.41\pm0.08$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.494\substack{+0.008\\ -0.008}$ & $28.19$ & $40$ \\ 
58514.99 & $1.42\pm0.10$ & $-10.38\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.502\substack{+0.008\\ -0.008}$ & $32.89$ & $44$ \\ 
58515.39 & $1.22\pm0.07$ & $-10.43\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.485\substack{+0.008\\ -0.008}$ & $41.02$ & $74$ \\ 
58516.59 & $1.34\pm0.09$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.455\substack{+0.008\\ -0.008}$ & $26.49$ & $38$ \\ 
58517.52 & $1.50\pm0.08$ & $-10.35\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.442\substack{+0.008\\ -0.008}$ & $25.29$ & $42$ \\ 
58519.45 & $1.28\pm0.07$ & $-10.39\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.448\substack{+0.008\\ -0.008}$ & $38.99$ & $82$ \\ 
58520.65 & $1.26\pm0.06$ & $-10.44\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.400\substack{+0.008\\ -0.008}$ & $44.27$ & $45$ \\ 
58521.57 & $1.52\pm0.08$ & $-10.35\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.392\substack{+0.008\\ -0.008}$ & $38.80$ & $91$ \\ 
58522.51 & $1.89\pm0.10$ & $-10.21\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.351\substack{+0.008\\ -0.008}$ & $41.61$ & $41$ \\ 
58523.51 & $1.52\pm0.08$ & $-10.33\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.340\substack{+0.008\\ -0.008}$ & $28.08$ & $40$ \\ 
58524.96 & $1.79\pm0.10$ & $-10.26\substack{+0.02\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.327\substack{+0.008\\ -0.008}$ & $51.13$ & $62$ \\ 
58525.62 & $1.76\pm0.10$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.325\substack{+0.008\\ -0.008}$ & $30.65$ & $39$ \\ 
58527.75 & $1.90\pm0.13$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.341\substack{+0.008\\ -0.008}$ & $26.40$ & $35$ \\ 
58528.28 & $1.71\pm0.11$ & $-10.24\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.345\substack{+0.008\\ -0.008}$ & $38.44$ & $36$ \\ 
58529.15 & $1.48\pm0.10$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.333\substack{+0.008\\ -0.008}$ & $42.26$ & $175$ \\ 
58530.34 & $1.58\pm0.10$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.309\substack{+0.008\\ -0.008}$ & $39.71$ & $60$ \\ 
58531.47 & $1.79\pm0.13$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.331\substack{+0.008\\ -0.008}$ & $41.12$ & $192$ \\ 
58532.33 & $1.75\pm0.09$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.337\substack{+0.008\\ -0.008}$ & $28.05$ & $40$ \\ 
58533.06 & $1.61\pm0.09$ & $-10.28\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.341\substack{+0.008\\ -0.008}$ & $39.53$ & $79$ \\ 
58534.66 & $2.04\pm0.16$ & $-10.19\substack{+0.04\\ -0.04}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.346\substack{+0.008\\ -0.008}$ & $32.54$ & $101$ \\ 
58535.46 & $1.77\pm0.10$ & $-10.25\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.366\substack{+0.008\\ -0.008}$ & $53.92$ & $42$ \\ 
58536.32 & $2.48\pm0.11$ & $-10.09\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.336\substack{+0.008\\ -0.008}$ & $32.08$ & $44$ \\ 
58537.37 & $2.27\pm0.14$ & $-10.16\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.346\substack{+0.008\\ -0.008}$ & $33.41$ & $37$ \\ 
58538.45 & $1.88\pm0.10$ & $-10.25\substack{+0.02\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.354\substack{+0.008\\ -0.008}$ & $29.75$ & $43$ \\ 
58539.57 & $1.95\pm0.10$ & $-10.21\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.362\substack{+0.008\\ -0.008}$ & $40.92$ & $40$ \\ 
58540.24 & $2.05\pm0.11$ & $-10.20\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.366\substack{+0.008\\ -0.008}$ & $55.14$ & $131$ \\ 
58541.42 & $1.65\pm0.09$ & $-10.31\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.367\substack{+0.008\\ -0.008}$ & $49.75$ & $41$ \\ 
58542.43 & $2.04\pm0.09$ & $-10.19\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.366\substack{+0.008\\ -0.008}$ & $44.01$ & $42$ \\ 
58543.69 & $1.99\pm0.11$ & $-10.18\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.365\substack{+0.008\\ -0.008}$ & $50.26$ & $40$ \\ 
58544.02 & $1.87\pm0.09$ & $-10.22\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.364\substack{+0.008\\ -0.008}$ & $40.20$ & $43$ \\ 
58545.94 & $2.14\pm0.11$ & $-10.18\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.362\substack{+0.008\\ -0.008}$ & $38.32$ & $39$ \\ 
58546.93 & $1.99\pm0.10$ & $-10.23\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.361\substack{+0.008\\ -0.008}$ & $41.22$ & $42$ \\ 
58547.86 & $2.08\pm0.10$ & $-10.19\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.355\substack{+0.008\\ -0.008}$ & $33.93$ & $43$ \\ 
58548.25 & $2.29\pm0.15$ & $-10.14\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.352\substack{+0.008\\ -0.008}$ & $34.22$ & $100$ \\ 
58549.85 & $2.08\pm0.10$ & $-10.18\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.346\substack{+0.008\\ -0.008}$ & $41.05$ & $42$ \\ 
58550.52 & $1.95\pm0.10$ & $-10.20\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.353\substack{+0.008\\ -0.008}$ & $48.40$ & $106$ \\ 
58551.52 & $1.66\pm0.09$ & $-10.26\substack{+0.02\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.370\substack{+0.008\\ -0.008}$ & $43.90$ & $42$ \\ 
58552.51 & $1.61\pm0.09$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.370\substack{+0.008\\ -0.008}$ & $33.88$ & $38$ \\ 
58553.44 & $2.13\pm0.12$ & $-10.17\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.379\substack{+0.008\\ -0.008}$ & $34.41$ & $41$ \\ 
58554.89 & $1.83\pm0.09$ & $-10.23\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.390\substack{+0.008\\ -0.008}$ & $56.03$ & $40$ \\ 
58555.75 & $2.03\pm0.13$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.385\substack{+0.008\\ -0.008}$ & $46.13$ & $102$ \\ 
58556.10 & $2.27\pm0.13$ & $-10.12\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.383\substack{+0.008\\ -0.008}$ & $37.00$ & $41$ \\ 
58557.96 & $1.95\pm0.11$ & $-10.19\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.378\substack{+0.008\\ -0.008}$ & $36.47$ & $40$ \\ 
58559.74 & $1.47\pm0.09$ & $-10.32\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.377\substack{+0.008\\ -0.008}$ & $39.94$ & $45$ \\ 
58560.73 & $1.73\pm0.08$ & $-10.30\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.376\substack{+0.008\\ -0.008}$ & $32.83$ & $43$ \\ 
58561.61 & $1.55\pm0.08$ & $-10.27\substack{+0.02\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.376\substack{+0.008\\ -0.008}$ & $43.43$ & $152$ \\ 
58562.79 & $1.44\pm0.08$ & $-10.34\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.360\substack{+0.008\\ -0.008}$ & $44.03$ & $43$ \\ 
58563.13 & $1.69\pm0.11$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.357\substack{+0.008\\ -0.008}$ & $34.75$ & $64$ \\ 
58570.92 & $2.07\pm0.13$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.296\substack{+0.008\\ -0.008}$ & $43.37$ & $38$ \\ 
58571.91 & $2.09\pm0.12$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.287\substack{+0.008\\ -0.008}$ & $47.87$ & $135$ \\ 
58572.84 & $1.94\pm0.13$ & $-10.21\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.292\substack{+0.008\\ -0.008}$ & $26.01$ & $35$ \\ 
58573.58 & $1.89\pm0.11$ & $-10.23\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.288\substack{+0.008\\ -0.008}$ & $42.63$ & $39$ \\ 
58574.64 & $1.76\pm0.11$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.288\substack{+0.008\\ -0.008}$ & $34.88$ & $207$ \\ 
58575.23 & $2.26\pm0.13$ & $-10.16\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.285\substack{+0.008\\ -0.008}$ & $34.04$ & $96$ \\ 
58576.50 & $2.09\pm0.11$ & $-10.21\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.264\substack{+0.008\\ -0.008}$ & $38.71$ & $192$ \\ 
58577.42 & $2.18\pm0.12$ & $-10.17\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.259\substack{+0.008\\ -0.008}$ & $43.11$ & $42$ \\ 
58578.41 & $2.21\pm0.15$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.254\substack{+0.008\\ -0.008}$ & $38.11$ & $89$ \\ 
58579.29 & $2.33\pm0.14$ & $-10.17\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.250\substack{+0.008\\ -0.008}$ & $46.54$ & $38$ \\ 
58580.47 & $2.00\pm0.10$ & $-10.22\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.252\substack{+0.008\\ -0.008}$ & $42.58$ & $41$ \\ 
58581.22 & $2.05\pm0.09$ & $-10.20\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.264\substack{+0.008\\ -0.008}$ & $48.85$ & $41$ \\ 
58582.14 & $2.38\pm0.12$ & $-10.14\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.267\substack{+0.008\\ -0.008}$ & $47.34$ & $42$ \\ 
58583.33 & $2.20\pm0.12$ & $-10.14\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.270\substack{+0.008\\ -0.008}$ & $50.79$ & $92$ \\ 
58584.40 & $2.27\pm0.10$ & $-10.15\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.272\substack{+0.008\\ -0.008}$ & $38.66$ & $44$ \\ 
58585.33 & $2.66\pm0.13$ & $-10.08\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.266\substack{+0.008\\ -0.008}$ & $38.05$ & $41$ \\ 
58586.39 & $1.96\pm0.10$ & $-10.21\substack{+0.02\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.261\substack{+0.008\\ -0.008}$ & $40.12$ & $50$ \\ 
58587.45 & $1.78\pm0.09$ & $-10.26\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.273\substack{+0.008\\ -0.008}$ & $38.61$ & $44$ \\ 
58588.24 & $2.27\pm0.12$ & $-10.15\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.277\substack{+0.008\\ -0.008}$ & $29.01$ & $40$ \\ 
58589.03 & $2.15\pm0.18$ & $-10.15\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.279\substack{+0.008\\ -0.008}$ & $39.43$ & $134$ \\ 
58590.31 & $2.45\pm0.17$ & $-10.13\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.281\substack{+0.008\\ -0.008}$ & $39.91$ & $36$ \\ 
58591.02 & $2.28\pm0.12$ & $-10.18\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.283\substack{+0.008\\ -0.008}$ & $34.60$ & $113$ \\ 
58592.28 & $2.09\pm0.11$ & $-10.20\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.286\substack{+0.008\\ -0.008}$ & $38.40$ & $82$ \\ 
58593.75 & $1.96\pm0.12$ & $-10.21\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.285\substack{+0.008\\ -0.008}$ & $57.73$ & $88$ \\ 
58594.21 & $2.01\pm0.11$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.286\substack{+0.008\\ -0.008}$ & $42.11$ & $131$ \\ 
58595.27 & $1.87\pm0.10$ & $-10.19\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.311\substack{+0.008\\ -0.008}$ & $41.37$ & $40$ \\ 
58596.01 & $1.85\pm0.11$ & $-10.25\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.306\substack{+0.008\\ -0.008}$ & $38.42$ & $41$ \\ 
58597.13 & $1.91\pm0.11$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.300\substack{+0.008\\ -0.008}$ & $17.73$ & $41$ \\ 
58601.79 & $1.70\pm0.09$ & $-10.27\substack{+0.02\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.281\substack{+0.008\\ -0.008}$ & $43.34$ & $42$ \\ 
58602.78 & $1.98\pm0.11$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.278\substack{+0.008\\ -0.008}$ & $37.29$ & $47$ \\ 
58603.25 & $1.97\pm0.15$ & $-10.17\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.281\substack{+0.008\\ -0.008}$ & $40.98$ & $35$ \\ 
58605.64 & $2.50\pm0.15$ & $-10.12\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.303\substack{+0.008\\ -0.008}$ & $38.18$ & $37$ \\ 
58606.69 & $2.01\pm0.12$ & $-10.17\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.316\substack{+0.008\\ -0.008}$ & $39.09$ & $87$ \\ 
58607.68 & $2.05\pm0.13$ & $-10.20\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.327\substack{+0.008\\ -0.008}$ & $39.00$ & $55$ \\ 
58608.55 & $1.49\pm0.09$ & $-10.32\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.335\substack{+0.008\\ -0.008}$ & $55.45$ & $40$ \\ 
58609.81 & $2.07\pm0.09$ & $-10.17\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.352\substack{+0.008\\ -0.008}$ & $37.03$ & $44$ \\ 
58610.02 & $2.33\pm0.12$ & $-10.15\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.354\substack{+0.008\\ -0.008}$ & $43.06$ & $112$ \\ 
58611.55 & $1.80\pm0.11$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.375\substack{+0.008\\ -0.008}$ & $31.60$ & $110$ \\ 
58612.86 & $1.94\pm0.12$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.393\substack{+0.008\\ -0.008}$ & $55.82$ & $74$ \\ 
58613.79 & $1.92\pm0.24$ & $-10.24\substack{+0.06\\ -0.06}$ & $2.1\substack{+0.2\\ -0.2}$ & $-11.409\substack{+0.008\\ -0.008}$ & $26.67$ & $154$ \\ 
58614.66 & $1.55\pm0.09$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.420\substack{+0.008\\ -0.008}$ & $56.78$ & $135$ \\ 
58615.59 & $1.73\pm0.10$ & $-10.26\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.393\substack{+0.008\\ -0.008}$ & $48.56$ & $184$ \\ 
58616.65 & $1.61\pm0.09$ & $-10.26\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.385\substack{+0.008\\ -0.008}$ & $34.67$ & $40$ \\ 
58617.39 & $1.49\pm0.10$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.405\substack{+0.008\\ -0.008}$ & $32.69$ & $39$ \\ 
58618.08 & $1.54\pm0.08$ & $-10.32\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.406\substack{+0.008\\ -0.008}$ & $56.64$ & $111$ \\ 
58623.71 & $1.87\pm0.15$ & $-10.24\substack{+0.04\\ -0.04}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.415\substack{+0.008\\ -0.008}$ & $32.08$ & $131$ \\ 
58624.50 & $1.56\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.418\substack{+0.008\\ -0.008}$ & $50.17$ & $100$ \\ 
58625.03 & $1.69\pm0.08$ & $-10.26\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.424\substack{+0.008\\ -0.008}$ & $57.43$ & $44$ \\ 
58626.83 & $1.57\pm0.06$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.446\substack{+0.008\\ -0.008}$ & $42.55$ & $47$ \\ 
58627.50 & $1.46\pm0.09$ & $-10.33\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.445\substack{+0.008\\ -0.008}$ & $38.42$ & $40$ \\ 
58628.75 & $1.97\pm0.10$ & $-10.22\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.476\substack{+0.008\\ -0.008}$ & $61.31$ & $44$ \\ 
58629.84 & $1.72\pm0.06$ & $-10.26\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.464\substack{+0.008\\ -0.008}$ & $51.61$ & $47$ \\ 
58630.02 & $1.80\pm0.09$ & $-10.23\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.465\substack{+0.008\\ -0.008}$ & $55.39$ & $43$ \\ 
58631.01 & $1.47\pm0.09$ & $-10.31\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.469\substack{+0.008\\ -0.008}$ & $57.52$ & $89$ \\ 
58632.07 & $1.50\pm0.06$ & $-10.33\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.488\substack{+0.008\\ -0.008}$ & $64.20$ & $45$ \\ 
58633.26 & $1.30\pm0.07$ & $-10.40\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.453\substack{+0.008\\ -0.008}$ & $34.94$ & $40$ \\ 
58634.13 & $1.66\pm0.08$ & $-10.25\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.447\substack{+0.008\\ -0.008}$ & $45.88$ & $87$ \\ 
58635.79 & $1.52\pm0.07$ & $-10.33\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.444\substack{+0.008\\ -0.008}$ & $43.19$ & $100$ \\ 
58636.58 & $1.75\pm0.10$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.446\substack{+0.008\\ -0.008}$ & $27.60$ & $105$ \\ 
58637.04 & $2.09\pm0.12$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.447\substack{+0.008\\ -0.008}$ & $42.39$ & $40$ \\ 
58638.04 & $1.69\pm0.09$ & $-10.28\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.463\substack{+0.008\\ -0.008}$ & $43.62$ & $43$ \\ 
58639.90 & $1.71\pm0.09$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.407\substack{+0.008\\ -0.008}$ & $41.85$ & $44$ \\ 
58640.69 & $1.77\pm0.09$ & $-10.27\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.413\substack{+0.008\\ -0.008}$ & $55.38$ & $39$ \\ 
58641.69 & $1.73\pm0.07$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.411\substack{+0.008\\ -0.008}$ & $38.17$ & $46$ \\ 
58642.89 & $2.06\pm0.08$ & $-10.18\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.374\substack{+0.008\\ -0.008}$ & $48.33$ & $45$ \\ 
58643.15 & $1.82\pm0.08$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.371\substack{+0.008\\ -0.008}$ & $45.30$ & $45$ \\ 
58644.15 & $2.03\pm0.09$ & $-10.20\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.364\substack{+0.008\\ -0.008}$ & $34.85$ & $46$ \\ 
58646.29 & $2.09\pm0.12$ & $-10.18\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.366\substack{+0.008\\ -0.008}$ & $49.36$ & $41$ \\ 
58647.93 & $1.81\pm0.14$ & $-10.28\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.377\substack{+0.008\\ -0.008}$ & $29.20$ & $185$ \\ 
58648.06 & $1.75\pm0.07$ & $-10.21\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.378\substack{+0.008\\ -0.008}$ & $57.61$ & $47$ \\ 
58649.67 & $1.50\pm0.08$ & $-10.33\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.393\substack{+0.008\\ -0.008}$ & $34.39$ & $65$ \\ 
58650.98 & $1.42\pm0.08$ & $-10.37\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.372\substack{+0.008\\ -0.008}$ & $35.77$ & $41$ \\ 
58651.78 & $1.87\pm0.14$ & $-10.21\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.366\substack{+0.008\\ -0.008}$ & $41.74$ & $92$ \\ 
58652.71 & $1.67\pm0.10$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.342\substack{+0.008\\ -0.008}$ & $44.32$ & $38$ \\ 
58653.77 & $1.71\pm0.11$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.327\substack{+0.008\\ -0.008}$ & $31.64$ & $38$ \\ 
58654.11 & $1.54\pm0.07$ & $-10.33\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.320\substack{+0.008\\ -0.008}$ & $46.01$ & $44$ \\ 
58655.56 & $1.45\pm0.06$ & $-10.35\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.309\substack{+0.008\\ -0.008}$ & $42.18$ & $42$ \\ 
58656.89 & $1.73\pm0.07$ & $-10.28\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.313\substack{+0.008\\ -0.008}$ & $57.66$ & $64$ \\ 
58657.49 & $1.93\pm0.10$ & $-10.24\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.313\substack{+0.008\\ -0.008}$ & $42.88$ & $40$ \\ 
58658.49 & $1.99\pm0.11$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.305\substack{+0.008\\ -0.008}$ & $44.47$ & $42$ \\ 
58659.48 & $1.84\pm0.12$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.325\substack{+0.008\\ -0.008}$ & $44.10$ & $43$ \\ 
58660.48 & $1.81\pm0.07$ & $-10.25\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.318\substack{+0.008\\ -0.008}$ & $45.64$ & $101$ \\ 
58661.42 & $1.60\pm0.08$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.310\substack{+0.008\\ -0.008}$ & $41.68$ & $81$ \\ 
58662.90 & $1.29\pm0.05$ & $-10.38\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.291\substack{+0.008\\ -0.008}$ & $53.19$ & $45$ \\ 
58664.73 & $1.56\pm0.08$ & $-10.35\substack{+0.02\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.287\substack{+0.008\\ -0.008}$ & $30.63$ & $38$ \\ 
58665.66 & $1.73\pm0.15$ & $-10.28\substack{+0.04\\ -0.04}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.297\substack{+0.008\\ -0.008}$ & $27.85$ & $51$ \\ 
58666.52 & $1.74\pm0.10$ & $-10.24\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.301\substack{+0.008\\ -0.008}$ & $32.18$ & $61$ \\ 
58667.19 & $1.92\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.291\substack{+0.008\\ -0.008}$ & $37.85$ & $45$ \\ 
58668.59 & $1.84\pm0.09$ & $-10.22\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.320\substack{+0.008\\ -0.008}$ & $69.98$ & $41$ \\ 
58669.05 & $1.99\pm0.09$ & $-10.20\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.324\substack{+0.008\\ -0.008}$ & $52.19$ & $148$ \\ 
58673.70 & $1.66\pm0.08$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.359\substack{+0.008\\ -0.008}$ & $41.03$ & $43$ \\ 
58675.63 & $1.67\pm0.08$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.364\substack{+0.008\\ -0.008}$ & $49.72$ & $44$ \\ 
58676.89 & $1.55\pm0.08$ & $-10.32\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.379\substack{+0.008\\ -0.008}$ & $31.00$ & $41$ \\ 
58677.03 & $1.66\pm0.08$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.379\substack{+0.008\\ -0.008}$ & $57.75$ & $44$ \\ 
58678.88 & $1.98\pm0.08$ & $-10.22\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.390\substack{+0.008\\ -0.008}$ & $56.20$ & $63$ \\ 
58679.22 & $1.97\pm0.09$ & $-10.21\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.393\substack{+0.008\\ -0.008}$ & $52.33$ & $42$ \\ 
58680.87 & $1.72\pm0.09$ & $-10.28\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.445\substack{+0.008\\ -0.008}$ & $76.81$ & $87$ \\ 
58681.94 & $1.72\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.438\substack{+0.008\\ -0.008}$ & $60.28$ & $42$ \\ 
58682.07 & $1.55\pm0.08$ & $-10.32\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.437\substack{+0.008\\ -0.008}$ & $39.21$ & $44$ \\ 
58683.13 & $1.36\pm0.06$ & $-10.37\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.449\substack{+0.008\\ -0.008}$ & $44.54$ & $43$ \\ 
58684.13 & $1.62\pm0.08$ & $-10.30\substack{+0.02\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.459\substack{+0.008\\ -0.008}$ & $39.42$ & $41$ \\ 
58686.05 & $1.63\pm0.07$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.480\substack{+0.008\\ -0.008}$ & $37.37$ & $56$ \\ 
58687.91 & $1.54\pm0.08$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.499\substack{+0.008\\ -0.008}$ & $37.99$ & $42$ \\ 
58688.11 & $1.35\pm0.09$ & $-10.36\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.502\substack{+0.008\\ -0.008}$ & $47.80$ & $129$ \\ 
58689.18 & $1.15\pm0.06$ & $-10.40\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.534\substack{+0.008\\ -0.008}$ & $36.40$ & $98$ \\ 
58690.70 & $1.12\pm0.06$ & $-10.44\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.546\substack{+0.008\\ -0.008}$ & $31.02$ & $42$ \\ 
58691.03 & $1.44\pm0.08$ & $-10.33\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.539\substack{+0.008\\ -0.008}$ & $35.87$ & $41$ \\ 
58692.10 & $1.53\pm0.07$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.505\substack{+0.008\\ -0.008}$ & $52.32$ & $44$ \\ 
58693.68 & $1.25\pm0.06$ & $-10.39\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.487\substack{+0.008\\ -0.008}$ & $36.72$ & $145$ \\ 
58695.61 & $1.58\pm0.09$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.509\substack{+0.008\\ -0.008}$ & $30.84$ & $69$ \\ 
58696.80 & $1.67\pm0.09$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.488\substack{+0.008\\ -0.008}$ & $41.83$ & $39$ \\ 
58697.73 & $1.69\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.473\substack{+0.008\\ -0.008}$ & $52.71$ & $41$ \\ 
58698.67 & $1.84\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.480\substack{+0.008\\ -0.008}$ & $37.70$ & $45$ \\ 
58699.07 & $1.97\pm0.09$ & $-10.22\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.484\substack{+0.008\\ -0.008}$ & $48.29$ & $43$ \\ 
58700.72 & $1.90\pm0.12$ & $-10.23\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.497\substack{+0.008\\ -0.008}$ & $41.26$ & $40$ \\ 
58701.78 & $1.90\pm0.09$ & $-10.24\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.505\substack{+0.008\\ -0.008}$ & $64.75$ & $134$ \\ 
58702.78 & $1.96\pm0.08$ & $-10.20\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.519\substack{+0.008\\ -0.008}$ & $42.46$ & $47$ \\ 
58703.71 & $1.67\pm0.09$ & $-10.27\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.535\substack{+0.008\\ -0.008}$ & $43.19$ & $45$ \\ 
58704.50 & $1.33\pm0.07$ & $-10.37\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.515\substack{+0.008\\ -0.008}$ & $39.47$ & $148$ \\ 
58705.63 & $1.74\pm0.08$ & $-10.25\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.534\substack{+0.008\\ -0.008}$ & $52.68$ & $78$ \\ 
58706.56 & $1.74\pm0.08$ & $-10.27\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.553\substack{+0.008\\ -0.008}$ & $44.77$ & $43$ \\ 
58707.49 & $1.65\pm0.07$ & $-10.28\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.579\substack{+0.008\\ -0.008}$ & $33.72$ & $59$ \\ 
58708.56 & $1.34\pm0.06$ & $-10.42\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.596\substack{+0.008\\ -0.008}$ & $32.72$ & $88$ \\ 
58709.36 & $1.31\pm0.07$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.604\substack{+0.008\\ -0.008}$ & $35.63$ & $42$ \\ 
58710.59 & $1.31\pm0.07$ & $-10.61\substack{+0.02\\ -0.03}$ & $1.6\substack{+0.1\\ -0.1}$ & $-11.636\substack{+0.008\\ -0.008}$ & $47.51$ & $58$ \\ 
58712.53 & $1.34\pm0.07$ & $-10.37\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.666\substack{+0.008\\ -0.008}$ & $34.72$ & $125$ \\ 
58713.01 & $1.29\pm0.07$ & $-10.37\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.664\substack{+0.008\\ -0.008}$ & $49.03$ & $41$ \\ 
58715.93 & $1.70\pm0.07$ & $-10.25\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.658\substack{+0.008\\ -0.008}$ & $54.19$ & $49$ \\ 
58716.19 & $1.57\pm0.07$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.657\substack{+0.008\\ -0.008}$ & $44.30$ & $62$ \\ 
58718.39 & $1.44\pm0.13$ & $-10.33\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.652\substack{+0.008\\ -0.008}$ & $27.16$ & $250$ \\ 
58719.58 & $1.21\pm0.05$ & $-10.41\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.644\substack{+0.008\\ -0.008}$ & $50.91$ & $44$ \\ 
58720.12 & $1.05\pm0.31$ & $-10.41\substack{+0.06\\ -0.06}$ & $2.1\substack{+0.2\\ -0.2}$ & $-11.637\substack{+0.008\\ -0.008}$ & $30.51$ & $279$ \\ 
58724.83 & $2.14\pm0.25$ & $-10.18\substack{+0.05\\ -0.05}$ & $2.2\substack{+0.2\\ -0.2}$ & $-11.585\substack{+0.008\\ -0.008}$ & $27.43$ & $207$ \\ 
58725.96 & $1.68\pm0.09$ & $-10.24\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.574\substack{+0.008\\ -0.008}$ & $41.03$ & $40$ \\ 
58727.62 & $1.82\pm0.07$ & $-10.27\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.555\substack{+0.008\\ -0.008}$ & $48.22$ & $45$ \\ 
58728.62 & $1.90\pm0.08$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.516\substack{+0.008\\ -0.008}$ & $40.51$ & $41$ \\ 
58729.95 & $2.09\pm0.11$ & $-10.20\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.507\substack{+0.008\\ -0.008}$ & $39.14$ & $40$ \\ 
58730.68 & $1.96\pm0.08$ & $-10.21\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.519\substack{+0.008\\ -0.008}$ & $54.04$ & $67$ \\ 
58731.15 & $2.09\pm0.11$ & $-10.15\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.530\substack{+0.008\\ -0.008}$ & $44.11$ & $114$ \\ 
58732.93 & $1.90\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.548\substack{+0.008\\ -0.008}$ & $34.60$ & $45$ \\ 
58733.80 & $1.68\pm0.08$ & $-10.27\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.562\substack{+0.008\\ -0.008}$ & $35.10$ & $42$ \\ 
58734.66 & $1.40\pm0.08$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.552\substack{+0.008\\ -0.008}$ & $39.99$ & $40$ \\ 
58735.65 & $1.58\pm0.06$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.541\substack{+0.008\\ -0.008}$ & $63.54$ & $47$ \\ 
58737.91 & $1.93\pm0.09$ & $-10.21\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.509\substack{+0.008\\ -0.008}$ & $31.99$ & $68$ \\ 
58738.84 & $1.80\pm0.09$ & $-10.23\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.512\substack{+0.008\\ -0.008}$ & $36.27$ & $42$ \\ 
58739.75 & $1.78\pm0.08$ & $-10.25\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.491\substack{+0.008\\ -0.008}$ & $38.06$ & $42$ \\ 
58740.63 & $1.58\pm0.07$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.471\substack{+0.008\\ -0.008}$ & $47.83$ & $82$ \\ 
58741.04 & $1.74\pm0.09$ & $-10.23\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.462\substack{+0.008\\ -0.008}$ & $46.17$ & $43$ \\ 
58742.75 & $1.56\pm0.07$ & $-10.30\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.446\substack{+0.008\\ -0.008}$ & $51.49$ & $74$ \\ 
58743.95 & $1.96\pm0.09$ & $-10.22\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.448\substack{+0.008\\ -0.008}$ & $50.48$ & $42$ \\ 
58744.72 & $1.78\pm0.06$ & $-10.25\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.461\substack{+0.008\\ -0.008}$ & $52.40$ & $46$ \\ 
58745.61 & $1.58\pm0.12$ & $-10.31\substack{+0.03\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.427\substack{+0.008\\ -0.008}$ & $34.87$ & $126$ \\ 
58746.54 & $1.65\pm0.08$ & $-10.28\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.448\substack{+0.008\\ -0.008}$ & $40.18$ & $111$ \\ 
58747.88 & $1.39\pm0.07$ & $-10.35\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.466\substack{+0.008\\ -0.008}$ & $44.23$ & $125$ \\ 
58748.86 & $1.38\pm0.08$ & $-10.38\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.462\substack{+0.008\\ -0.008}$ & $53.02$ & $38$ \\ 
58749.01 & $1.33\pm0.10$ & $-10.39\substack{+0.03\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.462\substack{+0.008\\ -0.008}$ & $40.30$ & $38$ \\ 
58750.40 & $1.47\pm0.07$ & $-10.32\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.462\substack{+0.008\\ -0.008}$ & $61.48$ & $116$ \\ 
58751.85 & $1.47\pm0.06$ & $-10.33\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.462\substack{+0.008\\ -0.008}$ & $55.72$ & $44$ \\ 
58752.64 & $1.43\pm0.07$ & $-10.34\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.459\substack{+0.008\\ -0.008}$ & $51.31$ & $40$ \\ 
58753.58 & $1.49\pm0.06$ & $-10.35\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.444\substack{+0.008\\ -0.008}$ & $32.51$ & $45$ \\ 
58754.77 & $1.40\pm0.08$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.423\substack{+0.008\\ -0.008}$ & $55.63$ & $210$ \\ 
58755.64 & $1.51\pm0.07$ & $-10.32\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.408\substack{+0.008\\ -0.008}$ & $37.23$ & $42$ \\ 
58756.57 & $1.43\pm0.06$ & $-10.38\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.423\substack{+0.008\\ -0.008}$ & $50.82$ & $46$ \\ 
58758.70 & $1.53\pm0.07$ & $-10.32\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.432\substack{+0.008\\ -0.008}$ & $37.73$ & $42$ \\ 
58759.49 & $1.36\pm0.07$ & $-10.37\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.427\substack{+0.008\\ -0.008}$ & $50.01$ & $43$ \\ 
58760.42 & $1.48\pm0.08$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.421\substack{+0.008\\ -0.008}$ & $41.13$ & $175$ \\ 
58762.88 & $1.87\pm0.10$ & $-10.23\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.426\substack{+0.008\\ -0.008}$ & $34.04$ & $41$ \\ 
58763.61 & $1.71\pm0.07$ & $-10.27\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.427\substack{+0.008\\ -0.008}$ & $49.88$ & $48$ \\ 
58764.80 & $1.78\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.444\substack{+0.008\\ -0.008}$ & $33.24$ & $54$ \\ 
58765.87 & $1.67\pm0.08$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.436\substack{+0.008\\ -0.008}$ & $31.38$ & $43$ \\ 
58766.67 & $1.62\pm0.10$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.454\substack{+0.008\\ -0.008}$ & $41.13$ & $41$ \\ 
58767.59 & $1.96\pm0.08$ & $-10.22\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.475\substack{+0.008\\ -0.008}$ & $39.65$ & $45$ \\ 
58768.65 & $1.91\pm0.10$ & $-10.20\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.488\substack{+0.008\\ -0.008}$ & $61.08$ & $82$ \\ 
58769.38 & $1.64\pm0.08$ & $-10.25\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.487\substack{+0.008\\ -0.008}$ & $33.68$ & $43$ \\ 
58770.31 & $1.39\pm0.06$ & $-10.34\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.499\substack{+0.008\\ -0.008}$ & $50.74$ & $43$ \\ 
58771.51 & $1.55\pm0.07$ & $-10.34\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.486\substack{+0.008\\ -0.008}$ & $40.20$ & $44$ \\ 
58772.04 & $1.61\pm0.08$ & $-10.28\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.486\substack{+0.008\\ -0.008}$ & $41.49$ & $44$ \\ 
58775.97 & $1.97\pm0.20$ & $-10.21\substack{+0.05\\ -0.05}$ & $1.9\substack{+0.2\\ -0.2}$ & $-11.481\substack{+0.008\\ -0.008}$ & $39.34$ & $130$ \\ 
58776.96 & $1.84\pm0.08$ & $-10.20\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.485\substack{+0.008\\ -0.008}$ & $34.18$ & $45$ \\ 
58777.42 & $1.65\pm0.07$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.493\substack{+0.008\\ -0.008}$ & $41.96$ & $44$ \\ 
58778.95 & $1.67\pm0.07$ & $-10.26\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.486\substack{+0.008\\ -0.008}$ & $54.07$ & $46$ \\ 
58779.35 & $1.61\pm0.07$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.481\substack{+0.008\\ -0.008}$ & $39.02$ & $44$ \\ 
58780.94 & $1.55\pm0.08$ & $-10.30\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.465\substack{+0.008\\ -0.008}$ & $47.47$ & $43$ \\ 
58781.68 & $1.97\pm0.16$ & $-10.19\substack{+0.04\\ -0.04}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.476\substack{+0.008\\ -0.008}$ & $42.96$ & $103$ \\ 
58782.60 & $1.69\pm0.08$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.485\substack{+0.008\\ -0.008}$ & $51.52$ & $42$ \\ 
58783.67 & $1.33\pm0.05$ & $-10.37\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.489\substack{+0.008\\ -0.008}$ & $33.87$ & $45$ \\ 
58784.67 & $1.24\pm0.08$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.6\substack{+0.1\\ -0.1}$ & $-11.493\substack{+0.008\\ -0.008}$ & $60.27$ & $37$ \\ 
58786.53 & $1.51\pm0.07$ & $-10.29\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.533\substack{+0.008\\ -0.008}$ & $41.15$ & $42$ \\ 
58787.78 & $1.58\pm0.08$ & $-10.30\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.546\substack{+0.008\\ -0.008}$ & $35.40$ & $42$ \\ 
58788.44 & $1.53\pm0.08$ & $-10.28\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.550\substack{+0.008\\ -0.008}$ & $54.57$ & $42$ \\ 
58789.64 & $1.31\pm0.06$ & $-10.34\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.556\substack{+0.008\\ -0.008}$ & $34.95$ & $40$ \\ 
58790.56 & $1.45\pm0.07$ & $-10.34\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.567\substack{+0.008\\ -0.008}$ & $43.71$ & $44$ \\ 
58791.90 & $1.60\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.559\substack{+0.008\\ -0.008}$ & $45.31$ & $47$ \\ 
58792.77 & $1.19\pm0.05$ & $-10.39\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.557\substack{+0.008\\ -0.008}$ & $44.68$ & $46$ \\ 
58793.43 & $1.52\pm0.08$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.556\substack{+0.008\\ -0.008}$ & $31.09$ & $73$ \\ 
58794.82 & $1.66\pm0.07$ & $-10.28\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.571\substack{+0.008\\ -0.008}$ & $37.96$ & $47$ \\ 
58796.67 & $1.59\pm0.06$ & $-10.30\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.559\substack{+0.008\\ -0.008}$ & $64.84$ & $45$ \\ 
58797.48 & $1.43\pm0.06$ & $-10.32\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.556\substack{+0.008\\ -0.008}$ & $59.04$ & $121$ \\ 
58799.67 & $1.75\pm0.11$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.553\substack{+0.008\\ -0.008}$ & $57.28$ & $41$ \\ 
58800.45 & $1.80\pm0.07$ & $-10.23\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.560\substack{+0.008\\ -0.008}$ & $49.01$ & $67$ \\ 
58801.19 & $1.75\pm0.08$ & $-10.28\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.568\substack{+0.008\\ -0.008}$ & $30.01$ & $44$ \\ 
58802.59 & $1.70\pm0.07$ & $-10.25\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.546\substack{+0.008\\ -0.008}$ & $47.30$ & $54$ \\ 
58803.58 & $1.77\pm0.08$ & $-10.25\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.555\substack{+0.008\\ -0.008}$ & $38.25$ & $73$ \\ 
58804.32 & $1.73\pm0.07$ & $-10.24\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.542\substack{+0.008\\ -0.008}$ & $47.23$ & $46$ \\ 
58805.63 & $1.79\pm0.10$ & $-10.25\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.548\substack{+0.008\\ -0.008}$ & $59.00$ & $41$ \\ 
58806.51 & $1.77\pm0.09$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.528\substack{+0.008\\ -0.008}$ & $27.26$ & $41$ \\ 
58807.56 & $2.12\pm0.09$ & $-10.18\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.513\substack{+0.008\\ -0.008}$ & $43.78$ & $88$ \\ 
58808.35 & $1.69\pm0.09$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.497\substack{+0.008\\ -0.008}$ & $37.05$ & $141$ \\ 
58809.56 & $1.36\pm0.06$ & $-10.35\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.531\substack{+0.008\\ -0.008}$ & $58.45$ & $67$ \\ 
58810.15 & $1.55\pm0.08$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.534\substack{+0.008\\ -0.008}$ & $56.40$ & $41$ \\ 
58814.27 & $1.52\pm0.06$ & $-10.32\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.544\substack{+0.008\\ -0.008}$ & $46.00$ & $45$ \\ 
58815.27 & $1.34\pm0.07$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.552\substack{+0.008\\ -0.008}$ & $29.90$ & $91$ \\ 
58816.19 & $1.43\pm0.07$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.540\substack{+0.008\\ -0.008}$ & $38.82$ & $43$ \\ 
58817.25 & $1.55\pm0.08$ & $-10.31\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.519\substack{+0.008\\ -0.008}$ & $52.54$ & $42$ \\ 
58818.25 & $1.36\pm0.09$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.525\substack{+0.008\\ -0.008}$ & $36.60$ & $39$ \\ 
58819.25 & $1.60\pm0.07$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.525\substack{+0.008\\ -0.008}$ & $42.89$ & $45$ \\ 
58820.44 & $1.70\pm0.10$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.529\substack{+0.008\\ -0.008}$ & $53.14$ & $38$ \\ 
58821.17 & $1.61\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.534\substack{+0.008\\ -0.008}$ & $53.71$ & $77$ \\ 
58822.17 & $1.73\pm0.08$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.523\substack{+0.008\\ -0.008}$ & $52.70$ & $44$ \\ 
58823.10 & $1.56\pm0.07$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.541\substack{+0.008\\ -0.008}$ & $50.34$ & $44$ \\ 
58824.63 & $1.56\pm0.10$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.554\substack{+0.008\\ -0.008}$ & $39.92$ & $117$ \\ 
58827.96 & $1.57\pm0.07$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.567\substack{+0.008\\ -0.008}$ & $54.47$ & $58$ \\ 
58828.96 & $1.54\pm0.10$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.533\substack{+0.008\\ -0.008}$ & $33.56$ & $38$ \\ 
58829.48 & $1.75\pm0.09$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.525\substack{+0.008\\ -0.008}$ & $42.45$ & $41$ \\ 
58830.81 & $1.57\pm0.07$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.513\substack{+0.008\\ -0.008}$ & $43.68$ & $44$ \\ 
58831.34 & $1.72\pm0.09$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.516\substack{+0.008\\ -0.008}$ & $39.28$ & $93$ \\ 
58832.68 & $1.69\pm0.08$ & $-10.22\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.518\substack{+0.008\\ -0.008}$ & $32.17$ & $45$ \\ 
58833.33 & $1.99\pm0.11$ & $-10.18\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.527\substack{+0.008\\ -0.008}$ & $50.77$ & $41$ \\ 
58834.33 & $1.52\pm0.18$ & $-10.37\substack{+0.05\\ -0.05}$ & $1.9\substack{+0.2\\ -0.2}$ & $-11.508\substack{+0.008\\ -0.008}$ & $24.16$ & $187$ \\ 
58835.72 & $1.93\pm0.13$ & $-10.20\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.495\substack{+0.008\\ -0.008}$ & $39.84$ & $37$ \\ 
58836.65 & $2.19\pm0.09$ & $-10.14\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.471\substack{+0.008\\ -0.008}$ & $60.95$ & $134$ \\ 
58837.59 & $1.72\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.450\substack{+0.008\\ -0.008}$ & $47.99$ & $47$ \\ 
58838.38 & $1.59\pm0.07$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.450\substack{+0.008\\ -0.008}$ & $45.40$ & $46$ \\ 
58839.84 & $1.83\pm0.08$ & $-10.25\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.439\substack{+0.008\\ -0.008}$ & $54.18$ & $44$ \\ 
58840.23 & $2.20\pm0.12$ & $-10.15\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.433\substack{+0.008\\ -0.008}$ & $62.88$ & $56$ \\ 
58841.49 & $1.63\pm0.12$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.417\substack{+0.008\\ -0.008}$ & $31.40$ & $169$ \\ 
58842.37 & $1.70\pm0.08$ & $-10.28\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.412\substack{+0.008\\ -0.008}$ & $36.42$ & $41$ \\ 
58843.69 & $2.00\pm0.12$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.431\substack{+0.008\\ -0.008}$ & $35.90$ & $39$ \\ 
58844.42 & $1.97\pm0.09$ & $-10.20\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.428\substack{+0.008\\ -0.008}$ & $44.80$ & $129$ \\ 
58845.68 & $1.93\pm0.09$ & $-10.23\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.448\substack{+0.008\\ -0.008}$ & $29.07$ & $43$ \\ 
58846.29 & $1.96\pm0.11$ & $-10.20\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.461\substack{+0.008\\ -0.008}$ & $53.46$ & $128$ \\ 
58847.60 & $1.66\pm0.07$ & $-10.27\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.461\substack{+0.008\\ -0.008}$ & $31.01$ & $46$ \\ 
58848.41 & $1.87\pm0.08$ & $-10.23\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.492\substack{+0.008\\ -0.008}$ & $41.99$ & $44$ \\ 
58849.47 & $1.72\pm0.07$ & $-10.25\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.473\substack{+0.008\\ -0.008}$ & $42.10$ & $44$ \\ 
58850.33 & $1.46\pm0.07$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.490\substack{+0.008\\ -0.008}$ & $56.84$ & $45$ \\ 
58851.39 & $1.79\pm0.10$ & $-10.25\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.492\substack{+0.008\\ -0.008}$ & $62.12$ & $60$ \\ 
58852.39 & $1.45\pm0.06$ & $-10.34\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.514\substack{+0.008\\ -0.008}$ & $41.26$ & $45$ \\ 
58853.52 & $1.68\pm0.11$ & $-10.26\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.500\substack{+0.008\\ -0.008}$ & $38.93$ & $39$ \\ 
58854.52 & $1.70\pm0.07$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.503\substack{+0.008\\ -0.008}$ & $38.39$ & $45$ \\ 
58855.04 & $1.77\pm0.08$ & $-10.25\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.506\substack{+0.008\\ -0.008}$ & $35.01$ & $44$ \\ 
58856.11 & $1.70\pm0.08$ & $-10.26\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.511\substack{+0.008\\ -0.008}$ & $36.83$ & $89$ \\ 
58857.43 & $1.63\pm0.07$ & $-10.26\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.527\substack{+0.008\\ -0.008}$ & $44.89$ & $44$ \\ 
58858.35 & $1.48\pm0.06$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.533\substack{+0.008\\ -0.008}$ & $55.58$ & $55$ \\ 
58859.36 & $1.69\pm0.07$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.542\substack{+0.008\\ -0.008}$ & $48.58$ & $45$ \\ 
58860.22 & $1.55\pm0.06$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.534\substack{+0.008\\ -0.008}$ & $38.13$ & $46$ \\ 
58861.01 & $1.48\pm0.08$ & $-10.31\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.527\substack{+0.008\\ -0.008}$ & $39.19$ & $37$ \\ 
58869.84 & $1.93\pm0.08$ & $-10.21\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.466\substack{+0.008\\ -0.008}$ & $33.97$ & $44$ \\ 
58872.04 & $1.51\pm0.06$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.475\substack{+0.008\\ -0.008}$ & $67.64$ & $57$ \\ 
58878.88 & $1.56\pm0.09$ & $-10.30\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.516\substack{+0.008\\ -0.008}$ & $37.26$ & $40$ \\ 
58879.88 & $1.59\pm0.10$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.517\substack{+0.008\\ -0.008}$ & $48.94$ & $131$ \\ 
58883.46 & $1.49\pm0.06$ & $-10.32\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.523\substack{+0.008\\ -0.008}$ & $48.14$ & $89$ \\ 
58884.46 & $1.18\pm0.07$ & $-10.38\substack{+0.03\\ -0.03}$ & $1.6\substack{+0.1\\ -0.1}$ & $-11.538\substack{+0.008\\ -0.008}$ & $58.30$ & $115$ \\ 
58885.58 & $1.00\pm0.21$ & $-10.26\substack{+0.11\\ -0.11}$ & $0.9\substack{+0.3\\ -0.3}$ & $-11.538\substack{+0.008\\ -0.008}$ & $8.02$ & $229$ \\ 
58886.05 & $1.36\pm0.07$ & $-10.36\substack{+0.02\\ -0.02}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.533\substack{+0.008\\ -0.008}$ & $52.69$ & $46$ \\ 
58887.38 & $1.66\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.503\substack{+0.008\\ -0.008}$ & $38.84$ & $44$ \\ 
58888.45 & $1.73\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.489\substack{+0.008\\ -0.008}$ & $40.68$ & $43$ \\ 
58889.04 & $1.78\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.484\substack{+0.008\\ -0.008}$ & $57.73$ & $42$ \\ 
58890.36 & $1.78\pm0.08$ & $-10.28\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.469\substack{+0.008\\ -0.008}$ & $43.49$ & $86$ \\ 
58891.57 & $2.10\pm0.10$ & $-10.18\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.453\substack{+0.008\\ -0.008}$ & $36.30$ & $53$ \\ 
58893.49 & $1.94\pm0.11$ & $-10.22\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.432\substack{+0.008\\ -0.008}$ & $45.77$ & $42$ \\ 
58894.36 & $1.81\pm0.07$ & $-10.23\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.422\substack{+0.008\\ -0.008}$ & $52.15$ & $45$ \\ 
58895.55 & $1.16\pm0.05$ & $-10.45\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.421\substack{+0.008\\ -0.008}$ & $50.18$ & $97$ \\ 
58896.41 & $1.41\pm0.07$ & $-10.36\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.433\substack{+0.008\\ -0.008}$ & $47.69$ & $45$ \\ 
58897.93 & $1.30\pm0.06$ & $-10.43\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.426\substack{+0.008\\ -0.008}$ & $59.78$ & $41$ \\ 
58898.13 & $1.38\pm0.06$ & $-10.38\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.423\substack{+0.008\\ -0.008}$ & $53.24$ & $42$ \\ 
58899.33 & $1.52\pm0.07$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.414\substack{+0.008\\ -0.008}$ & $53.59$ & $44$ \\ 
58900.20 & $1.71\pm0.07$ & $-10.28\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.416\substack{+0.008\\ -0.008}$ & $41.75$ & $45$ \\ 
58907.96 & $2.09\pm0.09$ & $-10.15\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.454\substack{+0.008\\ -0.008}$ & $47.80$ & $100$ \\ 
58911.48 & $1.97\pm0.11$ & $-10.17\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.521\substack{+0.008\\ -0.008}$ & $48.05$ & $44$ \\ 
58915.26 & $1.40\pm0.06$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.536\substack{+0.008\\ -0.008}$ & $67.76$ & $47$ \\ 
58919.25 & $1.83\pm0.09$ & $-10.20\substack{+0.02\\ -0.03}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.575\substack{+0.008\\ -0.008}$ & $26.95$ & $43$ \\ 
58920.44 & $1.81\pm0.08$ & $-10.20\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.580\substack{+0.008\\ -0.008}$ & $49.86$ & $44$ \\ 
58931.74 & $1.70\pm0.08$ & $-10.22\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.627\substack{+0.008\\ -0.008}$ & $33.33$ & $108$ \\ 
58935.99 & $2.07\pm0.12$ & $-10.17\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.649\substack{+0.008\\ -0.008}$ & $37.81$ & $40$ \\ 
58939.83 & $1.69\pm0.08$ & $-10.25\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.664\substack{+0.008\\ -0.008}$ & $34.50$ & $102$ \\ 
58943.15 & $2.04\pm0.09$ & $-10.19\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.648\substack{+0.008\\ -0.008}$ & $36.75$ & $46$ \\ 
58947.33 & $1.98\pm0.09$ & $-10.16\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.598\substack{+0.008\\ -0.008}$ & $38.79$ & $44$ \\ 
58955.10 & $2.64\pm0.12$ & $-10.09\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.485\substack{+0.008\\ -0.008}$ & $47.59$ & $41$ \\ 
58959.35 & $2.14\pm0.08$ & $-10.15\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.464\substack{+0.008\\ -0.008}$ & $41.39$ & $45$ \\ 
58963.13 & $2.51\pm0.09$ & $-10.11\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.460\substack{+0.008\\ -0.008}$ & $41.87$ & $45$ \\ 
58967.38 & $2.25\pm0.09$ & $-10.14\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.413\substack{+0.008\\ -0.008}$ & $38.55$ & $50$ \\ 
58975.08 & $2.19\pm0.08$ & $-10.17\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.351\substack{+0.008\\ -0.008}$ & $46.63$ & $45$ \\ 
58986.38 & $1.88\pm0.08$ & $-10.21\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.265\substack{+0.008\\ -0.008}$ & $33.04$ & $45$ \\ 
58991.95 & $2.10\pm0.09$ & $-10.18\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.268\substack{+0.008\\ -0.008}$ & $58.57$ & $222$ \\ 
58994.20 & $1.85\pm0.09$ & $-10.25\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.267\substack{+0.008\\ -0.008}$ & $38.43$ & $109$ \\ 
58999.98 & $1.91\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.249\substack{+0.008\\ -0.008}$ & $55.52$ & $44$ \\ 
59003.23 & $1.71\pm0.08$ & $-10.28\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.253\substack{+0.008\\ -0.008}$ & $36.51$ & $44$ \\ 
59007.01 & $1.60\pm0.09$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.254\substack{+0.008\\ -0.008}$ & $46.11$ & $48$ \\ 
59015.49 & $1.69\pm0.06$ & $-10.34\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.245\substack{+0.008\\ -0.008}$ & $29.17$ & $48$ \\ 
59020.03 & $1.64\pm0.07$ & $-10.29\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.221\substack{+0.008\\ -0.008}$ & $58.49$ & $45$ \\ 
59024.47 & $1.39\pm0.06$ & $-10.41\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.235\substack{+0.008\\ -0.008}$ & $60.20$ & $163$ \\ 
59027.59 & $2.00\pm0.11$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.261\substack{+0.008\\ -0.008}$ & $36.10$ & $87$ \\ 
59035.84 & $1.83\pm0.08$ & $-10.21\substack{+0.02\\ -0.02}$ & $1.7\substack{+0.1\\ -0.1}$ & $-11.286\substack{+0.008\\ -0.008}$ & $43.16$ & $44$ \\ 
59039.02 & $1.98\pm0.09$ & $-10.20\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.279\substack{+0.008\\ -0.008}$ & $28.45$ & $45$ \\ 
59043.87 & $1.97\pm0.09$ & $-10.26\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.270\substack{+0.008\\ -0.008}$ & $45.28$ & $42$ \\ 
59051.64 & $1.80\pm0.08$ & $-10.25\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.256\substack{+0.008\\ -0.008}$ & $50.56$ & $62$ \\ 
59055.01 & $2.07\pm0.13$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.240\substack{+0.008\\ -0.008}$ & $29.97$ & $75$ \\ 
59059.60 & $2.20\pm0.09$ & $-10.17\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.240\substack{+0.008\\ -0.008}$ & $42.39$ & $82$ \\ 
59063.84 & $2.11\pm0.09$ & $-10.19\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.271\substack{+0.008\\ -0.008}$ & $41.31$ & $42$ \\ 
59067.89 & $2.94\pm0.14$ & $-10.03\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.293\substack{+0.008\\ -0.008}$ & $31.78$ & $68$ \\ 
59071.74 & $2.33\pm0.09$ & $-10.14\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.327\substack{+0.008\\ -0.008}$ & $26.59$ & $45$ \\ 
59085.57 & $1.46\pm0.06$ & $-10.33\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.404\substack{+0.008\\ -0.008}$ & $42.87$ & $167$ \\ 
59087.82 & $1.24\pm0.06$ & $-10.41\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.417\substack{+0.008\\ -0.008}$ & $49.97$ & $42$ \\ 
59092.21 & $1.24\pm0.07$ & $-10.38\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.444\substack{+0.008\\ -0.008}$ & $42.42$ & $41$ \\ 
59095.66 & $1.57\pm0.07$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.431\substack{+0.008\\ -0.008}$ & $32.55$ & $169$ \\ 
59099.05 & $1.77\pm0.08$ & $-10.24\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.422\substack{+0.008\\ -0.008}$ & $46.97$ & $44$ \\ 
59103.61 & $2.44\pm0.10$ & $-10.13\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.455\substack{+0.008\\ -0.008}$ & $42.17$ & $43$ \\ 
59108.79 & $1.53\pm0.06$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.513\substack{+0.008\\ -0.008}$ & $59.26$ & $45$ \\ 
59110.79 & $1.56\pm0.07$ & $-10.33\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.545\substack{+0.008\\ -0.008}$ & $47.21$ & $64$ \\ 
59115.76 & $1.40\pm0.07$ & $-10.33\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.591\substack{+0.008\\ -0.008}$ & $39.27$ & $43$ \\ 
59119.55 & $1.36\pm0.06$ & $-10.35\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.615\substack{+0.008\\ -0.008}$ & $45.71$ & $44$ \\ 
59123.80 & $1.56\pm0.08$ & $-10.27\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.605\substack{+0.008\\ -0.008}$ & $35.72$ & $42$ \\ 
59128.71 & $1.53\pm0.07$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.594\substack{+0.008\\ -0.008}$ & $40.93$ & $89$ \\ 
59135.36 & $2.00\pm0.12$ & $-10.19\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.579\substack{+0.008\\ -0.008}$ & $52.85$ & $166$ \\ 
59139.54 & $1.99\pm0.13$ & $-10.18\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.560\substack{+0.008\\ -0.008}$ & $34.43$ & $38$ \\ 
59147.05 & $1.38\pm0.07$ & $-10.38\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.489\substack{+0.008\\ -0.008}$ & $50.50$ & $42$ \\ 
59152.69 & $1.54\pm0.08$ & $-10.33\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.462\substack{+0.008\\ -0.008}$ & $39.82$ & $45$ \\ 
59155.94 & $1.47\pm0.07$ & $-10.35\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.432\substack{+0.008\\ -0.008}$ & $34.59$ & $115$ \\ 
59159.46 & $1.41\pm0.08$ & $-10.36\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.414\substack{+0.008\\ -0.008}$ & $37.96$ & $51$ \\ 
59164.43 & $1.64\pm0.10$ & $-10.28\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.424\substack{+0.008\\ -0.008}$ & $42.71$ & $100$ \\ 
59167.48 & $2.00\pm0.11$ & $-10.22\substack{+0.02\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.415\substack{+0.008\\ -0.008}$ & $37.76$ & $39$ \\ 
59171.06 & $1.65\pm0.08$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.415\substack{+0.008\\ -0.008}$ & $46.84$ & $40$ \\ 
59175.17 & $1.95\pm0.09$ & $-10.21\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.423\substack{+0.008\\ -0.008}$ & $27.82$ & $66$ \\ 
59179.16 & $1.54\pm0.08$ & $-10.29\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.438\substack{+0.008\\ -0.008}$ & $40.44$ & $73$ \\ 
59183.42 & $1.41\pm0.08$ & $-10.36\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.478\substack{+0.008\\ -0.008}$ & $30.84$ & $58$ \\ 
59188.80 & $1.60\pm0.09$ & $-10.30\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.476\substack{+0.008\\ -0.008}$ & $35.25$ & $41$ \\ 
59191.05 & $1.33\pm0.12$ & $-10.46\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.463\substack{+0.008\\ -0.008}$ & $36.66$ & $79$ \\ 
59195.07 & $2.10\pm0.10$ & $-10.20\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.473\substack{+0.008\\ -0.008}$ & $52.13$ & $190$ \\ 
59199.68 & $1.59\pm0.09$ & $-10.30\substack{+0.02\\ -0.02}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.466\substack{+0.008\\ -0.008}$ & $38.98$ & $41$ \\ 
59203.84 & $1.55\pm0.08$ & $-10.31\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.463\substack{+0.008\\ -0.008}$ & $42.23$ & $44$ \\ 
59207.12 & $1.51\pm0.09$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.470\substack{+0.008\\ -0.008}$ & $24.88$ & $38$ \\ 
59211.10 & $1.67\pm0.09$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.497\substack{+0.008\\ -0.008}$ & $34.47$ & $103$ \\ 
59215.22 & $2.13\pm0.13$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.488\substack{+0.008\\ -0.008}$ & $29.90$ & $38$ \\ 
59219.80 & $1.41\pm0.09$ & $-10.36\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.476\substack{+0.008\\ -0.008}$ & $44.91$ & $142$ \\ 
59223.12 & $1.38\pm0.10$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.509\substack{+0.008\\ -0.008}$ & $38.28$ & $36$ \\ 
59227.30 & $1.10\pm0.06$ & $-10.46\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.511\substack{+0.008\\ -0.008}$ & $50.18$ & $189$ \\ 
59231.02 & $1.25\pm0.07$ & $-10.43\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.461\substack{+0.008\\ -0.008}$ & $52.30$ & $119$ \\ 
59235.80 & $0.76\pm0.08$ & $-10.68\substack{+0.05\\ -0.05}$ & $2.0\substack{+0.2\\ -0.2}$ & $-11.459\substack{+0.008\\ -0.008}$ & $24.43$ & $137$ \\ 
59239.65 & $1.17\pm0.06$ & $-10.46\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.395\substack{+0.008\\ -0.008}$ & $38.44$ & $40$ \\ 
59243.31 & $1.26\pm0.10$ & $-10.45\substack{+0.04\\ -0.04}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.340\substack{+0.008\\ -0.008}$ & $31.14$ & $68$ \\ 
59248.35 & $1.45\pm0.09$ & $-10.35\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.321\substack{+0.008\\ -0.008}$ & $31.91$ & $61$ \\ 
59251.39 & $1.21\pm0.06$ & $-10.46\substack{+0.02\\ -0.02}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.313\substack{+0.008\\ -0.008}$ & $40.14$ & $42$ \\ 
59255.32 & $1.56\pm0.10$ & $-10.32\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.296\substack{+0.008\\ -0.008}$ & $45.76$ & $100$ \\ 
59259.10 & $1.50\pm0.07$ & $-10.31\substack{+0.02\\ -0.02}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.316\substack{+0.008\\ -0.008}$ & $46.22$ & $82$ \\ 


==> Table8.tex <==
58256.95 & $33.40\pm0.17$ & $-10.243\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.739\substack{+0.008\\ -0.008}$ & $94.85$ & $98$ \\ 
58257.00 & $32.31\pm0.23$ & $-10.258\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.739\substack{+0.008\\ -0.008}$ & $102.87$ & $95$ \\ 
58272.38 & $38.23\pm0.20$ & $-10.225\substack{+0.003\\ -0.003}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.619\substack{+0.008\\ -0.008}$ & $91.36$ & $102$ \\ 
58293.62 & $32.83\pm0.21$ & $-10.290\substack{+0.003\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.738\substack{+0.008\\ -0.008}$ & $79.71$ & $102$ \\ 
58294.65 & $32.66\pm0.19$ & $-10.283\substack{+0.003\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.760\substack{+0.008\\ -0.008}$ & $119.48$ & $98$ \\ 
58302.65 & $32.52\pm0.23$ & $-10.290\substack{+0.004\\ -0.004}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.798\substack{+0.008\\ -0.008}$ & $80.84$ & $101$ \\ 
58304.43 & $41.17\pm0.25$ & $-10.180\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.781\substack{+0.008\\ -0.008}$ & $71.08$ & $103$ \\ 
58310.32 & $19.56\pm0.16$ & $-10.464\substack{+0.005\\ -0.005}$ & $1.99\substack{+0.01\\ -0.01}$ & $-11.999\substack{+0.008\\ -0.008}$ & $64.11$ & $90$ \\ 
58311.22 & $18.58\pm0.13$ & $-10.490\substack{+0.004\\ -0.004}$ & $2.01\substack{+0.01\\ -0.01}$ & $-12.049\substack{+0.008\\ -0.008}$ & $83.82$ & $95$ \\ 
58312.21 & $22.57\pm0.17$ & $-10.405\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-12.095\substack{+0.008\\ -0.008}$ & $108.33$ & $93$ \\ 
58313.57 & $27.45\pm0.16$ & $-10.330\substack{+0.003\\ -0.003}$ & $2.07\substack{+0.01\\ -0.01}$ & $-12.052\substack{+0.008\\ -0.008}$ & $111.43$ & $98$ \\ 
58314.52 & $29.26\pm0.16$ & $-10.308\substack{+0.003\\ -0.003}$ & $2.07\substack{+0.01\\ -0.01}$ & $-12.082\substack{+0.008\\ -0.008}$ & $76.22$ & $99$ \\ 
58315.30 & $26.39\pm0.15$ & $-10.349\substack{+0.003\\ -0.003}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.098\substack{+0.008\\ -0.008}$ & $89.84$ & $99$ \\ 
58317.30 & $30.20\pm0.15$ & $-10.306\substack{+0.003\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.096\substack{+0.008\\ -0.008}$ & $97.80$ & $104$ \\ 
58318.58 & $31.25\pm0.22$ & $-10.291\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.114\substack{+0.008\\ -0.008}$ & $83.50$ & $93$ \\ 
58325.65 & $26.83\pm0.19$ & $-10.345\substack{+0.004\\ -0.004}$ & $2.08\substack{+0.01\\ -0.01}$ & $-12.281\substack{+0.008\\ -0.008}$ & $92.42$ & $93$ \\ 
58327.16 & $29.54\pm0.18$ & $-10.291\substack{+0.003\\ -0.003}$ & $2.03\substack{+0.01\\ -0.01}$ & $-12.213\substack{+0.008\\ -0.008}$ & $102.68$ & $98$ \\ 
58329.19 & $27.66\pm0.21$ & $-10.329\substack{+0.004\\ -0.004}$ & $2.06\substack{+0.01\\ -0.01}$ & $-12.166\substack{+0.008\\ -0.008}$ & $86.75$ & $92$ \\ 
58331.12 & $25.09\pm0.21$ & $-10.380\substack{+0.005\\ -0.005}$ & $2.10\substack{+0.01\\ -0.01}$ & $-12.128\substack{+0.008\\ -0.008}$ & $110.33$ & $92$ \\ 
58333.50 & $31.51\pm0.15$ & $-10.294\substack{+0.002\\ -0.002}$ & $2.16\substack{+0.01\\ -0.01}$ & $-12.076\substack{+0.008\\ -0.008}$ & $147.55$ & $100$ \\ 
58336.46 & $36.81\pm0.22$ & $-10.219\substack{+0.003\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.048\substack{+0.008\\ -0.008}$ & $86.33$ & $96$ \\ 
58338.59 & $31.99\pm0.20$ & $-10.285\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-12.027\substack{+0.008\\ -0.008}$ & $91.35$ & $96$ \\ 
58340.52 & $35.74\pm0.22$ & $-10.222\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-12.083\substack{+0.008\\ -0.008}$ & $144.50$ & $97$ \\ 
58342.64 & $34.60\pm0.21$ & $-10.224\substack{+0.003\\ -0.003}$ & $2.03\substack{+0.01\\ -0.01}$ & $-12.109\substack{+0.008\\ -0.008}$ & $88.90$ & $97$ \\ 
58343.60 & $29.93\pm0.19$ & $-10.292\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.122\substack{+0.008\\ -0.008}$ & $79.28$ & $97$ \\ 
58345.21 & $29.88\pm0.21$ & $-10.309\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.130\substack{+0.008\\ -0.008}$ & $116.15$ & $102$ \\ 
58348.86 & $30.38\pm0.21$ & $-10.298\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-12.168\substack{+0.008\\ -0.008}$ & $116.54$ & $95$ \\ 
58350.96 & $29.98\pm0.19$ & $-10.312\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-12.220\substack{+0.008\\ -0.008}$ & $91.60$ & $96$ \\ 
58352.82 & $30.00\pm0.19$ & $-10.305\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-12.257\substack{+0.008\\ -0.008}$ & $103.14$ & $96$ \\ 
58354.82 & $30.46\pm0.19$ & $-10.298\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-12.230\substack{+0.008\\ -0.008}$ & $102.94$ & $96$ \\ 
58358.86 & $25.46\pm0.22$ & $-10.367\substack{+0.005\\ -0.005}$ & $2.09\substack{+0.01\\ -0.01}$ & $-12.399\substack{+0.008\\ -0.008}$ & $105.55$ & $102$ \\ 
58360.85 & $21.11\pm0.28$ & $-10.446\substack{+0.008\\ -0.008}$ & $2.10\substack{+0.02\\ -0.02}$ & $-12.495\substack{+0.008\\ -0.008}$ & $89.57$ & $95$ \\ 
58362.85 & $20.57\pm0.30$ & $-10.454\substack{+0.009\\ -0.009}$ & $2.09\substack{+0.02\\ -0.02}$ & $-12.449\substack{+0.008\\ -0.008}$ & $83.23$ & $97$ \\ 
58364.71 & $28.50\pm0.19$ & $-10.313\substack{+0.004\\ -0.004}$ & $2.07\substack{+0.01\\ -0.01}$ & $-12.365\substack{+0.008\\ -0.008}$ & $123.29$ & $103$ \\ 
58367.94 & $32.54\pm0.31$ & $-10.283\substack{+0.005\\ -0.005}$ & $2.20\substack{+0.02\\ -0.02}$ & $-12.337\substack{+0.008\\ -0.008}$ & $96.48$ & $88$ \\ 
58369.77 & $25.35\pm0.16$ & $-10.374\substack{+0.003\\ -0.003}$ & $2.10\substack{+0.01\\ -0.01}$ & $-12.212\substack{+0.008\\ -0.008}$ & $96.46$ & $97$ \\ 
58375.54 & $25.47\pm0.19$ & $-10.357\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.586\substack{+0.008\\ -0.008}$ & $94.23$ & $99$ \\ 
58377.89 & $20.43\pm0.15$ & $-10.438\substack{+0.004\\ -0.004}$ & $2.06\substack{+0.01\\ -0.01}$ & $-12.632\substack{+0.008\\ -0.008}$ & $104.17$ & $96$ \\ 
58379.95 & $21.24\pm0.14$ & $-10.414\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-12.689\substack{+0.008\\ -0.008}$ & $116.67$ & $99$ \\ 
58382.85 & $22.23\pm0.19$ & $-10.391\substack{+0.005\\ -0.005}$ & $2.04\substack{+0.01\\ -0.01}$ & $-13.385\substack{+0.008\\ -0.008}$ & $71.32$ & $93$ \\ 
58388.42 & $24.17\pm0.18$ & $-10.383\substack{+0.004\\ -0.004}$ & $2.07\substack{+0.01\\ -0.01}$ & $-12.812\substack{+0.008\\ -0.008}$ & $112.82$ & $93$ \\ 
58390.48 & $27.78\pm0.19$ & $-10.325\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-14.106\substack{+0.008\\ -0.008}$ & $100.36$ & $94$ \\ 
58392.70 & $28.28\pm0.14$ & $-10.315\substack{+0.002\\ -0.003}$ & $2.07\substack{+0.01\\ -0.01}$ & $-12.801\substack{+0.008\\ -0.008}$ & $99.79$ & $100$ \\ 
58394.92 & $20.05\pm0.13$ & $-10.444\substack{+0.003\\ -0.003}$ & $1.99\substack{+0.01\\ -0.01}$ & $-12.860\substack{+0.008\\ -0.008}$ & $96.95$ & $99$ \\ 
58396.59 & $21.53\pm0.15$ & $-10.430\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.651\substack{+0.008\\ -0.008}$ & $103.22$ & $94$ \\ 
58398.59 & $27.33\pm0.19$ & $-10.317\substack{+0.004\\ -0.004}$ & $2.01\substack{+0.01\\ -0.01}$ & $-12.573\substack{+0.008\\ -0.008}$ & $105.19$ & $101$ \\ 
58400.69 & $26.73\pm0.16$ & $-10.353\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-12.364\substack{+0.008\\ -0.008}$ & $113.07$ & $101$ \\ 
58402.59 & $26.86\pm0.19$ & $-10.352\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.485\substack{+0.008\\ -0.008}$ & $75.37$ & $95$ \\ 
58403.93 & $23.80\pm0.19$ & $-10.396\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-12.546\substack{+0.008\\ -0.008}$ & $95.67$ & $92$ \\ 
58405.89 & $24.63\pm0.27$ & $-10.397\substack{+0.005\\ -0.005}$ & $2.17\substack{+0.01\\ -0.01}$ & $-12.565\substack{+0.008\\ -0.008}$ & $83.93$ & $85$ \\ 
58407.31 & $29.23\pm0.21$ & $-10.320\substack{+0.004\\ -0.004}$ & $2.15\substack{+0.01\\ -0.01}$ & $-12.406\substack{+0.008\\ -0.008}$ & $82.26$ & $92$ \\ 
58409.69 & $31.32\pm0.18$ & $-10.291\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-12.360\substack{+0.008\\ -0.008}$ & $86.47$ & $97$ \\ 
58412.07 & $23.63\pm0.17$ & $-10.433\substack{+0.004\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-12.256\substack{+0.008\\ -0.008}$ & $101.93$ & $93$ \\ 
58414.51 & $27.64\pm0.16$ & $-10.361\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-12.174\substack{+0.008\\ -0.008}$ & $107.89$ & $101$ \\ 
58416.70 & $29.80\pm0.20$ & $-10.343\substack{+0.004\\ -0.004}$ & $2.29\substack{+0.01\\ -0.01}$ & $-12.138\substack{+0.008\\ -0.008}$ & $67.02$ & $96$ \\ 
58418.70 & $28.83\pm0.21$ & $-10.349\substack{+0.004\\ -0.004}$ & $2.25\substack{+0.01\\ -0.01}$ & $-12.174\substack{+0.008\\ -0.008}$ & $91.68$ & $95$ \\ 
58420.63 & $28.88\pm0.21$ & $-10.321\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-12.209\substack{+0.008\\ -0.008}$ & $116.71$ & $97$ \\ 
58421.24 & $30.99\pm0.23$ & $-10.291\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-12.209\substack{+0.008\\ -0.008}$ & $108.96$ & $93$ \\ 
58422.67 & $28.48\pm0.21$ & $-10.309\substack{+0.004\\ -0.004}$ & $2.04\substack{+0.01\\ -0.01}$ & $-12.258\substack{+0.008\\ -0.008}$ & $104.21$ & $94$ \\ 
58423.96 & $26.91\pm0.19$ & $-10.336\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.252\substack{+0.008\\ -0.008}$ & $98.94$ & $93$ \\ 
58426.46 & $29.16\pm0.18$ & $-10.310\substack{+0.003\\ -0.003}$ & $2.08\substack{+0.01\\ -0.01}$ & $-12.187\substack{+0.008\\ -0.008}$ & $86.61$ & $96$ \\ 
58428.20 & $34.67\pm0.19$ & $-10.248\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-12.128\substack{+0.008\\ -0.008}$ & $81.80$ & $100$ \\ 
58429.17 & $38.70\pm0.21$ & $-10.206\substack{+0.003\\ -0.003}$ & $2.18\substack{+0.01\\ -0.01}$ & $-12.080\substack{+0.008\\ -0.008}$ & $90.25$ & $99$ \\ 
58430.07 & $39.51\pm0.30$ & $-10.195\substack{+0.004\\ -0.004}$ & $2.16\substack{+0.01\\ -0.01}$ & $-12.020\substack{+0.008\\ -0.008}$ & $78.22$ & $91$ \\ 
58431.16 & $36.65\pm0.21$ & $-10.225\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.994\substack{+0.008\\ -0.008}$ & $117.50$ & $96$ \\ 
58432.97 & $43.52\pm0.34$ & $-10.146\substack{+0.004\\ -0.004}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.969\substack{+0.008\\ -0.008}$ & $79.84$ & $92$ \\ 
58433.06 & $42.37\pm0.26$ & $-10.159\substack{+0.003\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.966\substack{+0.008\\ -0.008}$ & $95.23$ & $96$ \\ 
58437.51 & $34.67\pm0.26$ & $-10.239\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.902\substack{+0.008\\ -0.008}$ & $111.77$ & $99$ \\ 
58438.42 & $33.05\pm0.34$ & $-10.271\substack{+0.006\\ -0.006}$ & $2.21\substack{+0.02\\ -0.02}$ & $-11.880\substack{+0.008\\ -0.008}$ & $93.19$ & $86$ \\ 
58439.64 & $34.47\pm0.36$ & $-10.253\substack{+0.006\\ -0.006}$ & $2.22\substack{+0.02\\ -0.02}$ & $-11.907\substack{+0.008\\ -0.008}$ & $70.12$ & $86$ \\ 
58449.22 & $34.65\pm0.24$ & $-10.224\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.911\substack{+0.008\\ -0.008}$ & $96.00$ & $96$ \\ 
58453.60 & $28.60\pm0.17$ & $-10.320\substack{+0.003\\ -0.003}$ & $2.06\substack{+0.01\\ -0.01}$ & $-11.956\substack{+0.008\\ -0.008}$ & $100.27$ & $98$ \\ 
58455.11 & $24.66\pm0.19$ & $-10.379\substack{+0.004\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.083\substack{+0.008\\ -0.008}$ & $94.08$ & $92$ \\ 
58456.98 & $22.70\pm0.17$ & $-10.428\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-12.075\substack{+0.008\\ -0.008}$ & $76.00$ & $93$ \\ 
58458.91 & $23.37\pm0.16$ & $-10.414\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-12.140\substack{+0.008\\ -0.008}$ & $84.85$ & $94$ \\ 
58460.91 & $26.84\pm0.17$ & $-10.342\substack{+0.003\\ -0.004}$ & $2.05\substack{+0.01\\ -0.01}$ & $-12.074\substack{+0.008\\ -0.008}$ & $86.06$ & $97$ \\ 
58462.90 & $23.61\pm0.17$ & $-10.387\substack{+0.004\\ -0.004}$ & $2.00\substack{+0.01\\ -0.01}$ & $-12.106\substack{+0.008\\ -0.008}$ & $88.80$ & $98$ \\ 
58464.58 & $22.86\pm0.16$ & $-10.408\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-12.115\substack{+0.008\\ -0.008}$ & $95.84$ & $95$ \\ 
58466.18 & $23.96\pm0.19$ & $-10.407\substack{+0.004\\ -0.004}$ & $2.12\substack{+0.01\\ -0.01}$ & $-12.147\substack{+0.008\\ -0.008}$ & $113.84$ & $98$ \\ 
58469.02 & $20.92\pm0.17$ & $-10.445\substack{+0.005\\ -0.005}$ & $2.06\substack{+0.01\\ -0.01}$ & $-12.130\substack{+0.008\\ -0.008}$ & $84.94$ & $94$ \\ 
58470.68 & $22.06\pm0.16$ & $-10.408\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-12.067\substack{+0.008\\ -0.008}$ & $111.55$ & $94$ \\ 
58471.77 & $28.52\pm0.25$ & $-10.327\substack{+0.005\\ -0.005}$ & $2.10\substack{+0.01\\ -0.01}$ & $-12.032\substack{+0.008\\ -0.008}$ & $80.59$ & $91$ \\ 
58473.91 & $29.54\pm0.19$ & $-10.289\substack{+0.004\\ -0.004}$ & $2.08\substack{+0.01\\ -0.01}$ & $-12.015\substack{+0.008\\ -0.008}$ & $109.48$ & $99$ \\ 
58476.07 & $34.02\pm0.32$ & $-10.259\substack{+0.005\\ -0.005}$ & $2.14\substack{+0.02\\ -0.02}$ & $-11.900\substack{+0.008\\ -0.008}$ & $90.85$ & $89$ \\ 
58479.11 & $31.86\pm0.21$ & $-10.271\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.847\substack{+0.008\\ -0.008}$ & $80.06$ & $94$ \\ 
58481.24 & $26.79\pm0.23$ & $-10.362\substack{+0.005\\ -0.005}$ & $2.18\substack{+0.02\\ -0.02}$ & $-11.859\substack{+0.008\\ -0.008}$ & $77.90$ & $98$ \\ 
58487.79 & $36.02\pm0.32$ & $-10.226\substack{+0.005\\ -0.005}$ & $2.21\substack{+0.02\\ -0.02}$ & $-11.771\substack{+0.008\\ -0.008}$ & $100.30$ & $88$ \\ 
58489.79 & $24.78\pm0.21$ & $-10.372\substack{+0.005\\ -0.005}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.747\substack{+0.008\\ -0.008}$ & $71.19$ & $90$ \\ 
58491.53 & $23.03\pm0.25$ & $-10.401\substack{+0.006\\ -0.006}$ & $2.07\substack{+0.02\\ -0.02}$ & $-11.755\substack{+0.008\\ -0.008}$ & $79.48$ & $86$ \\ 
58493.71 & $23.80\pm0.27$ & $-10.427\substack{+0.007\\ -0.007}$ & $2.26\substack{+0.02\\ -0.02}$ & $-11.758\substack{+0.008\\ -0.008}$ & $82.95$ & $88$ \\ 
58497.64 & $24.88\pm0.20$ & $-10.379\substack{+0.004\\ -0.005}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.692\substack{+0.008\\ -0.008}$ & $110.60$ & $90$ \\ 
58499.38 & $28.04\pm0.16$ & $-10.358\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.638\substack{+0.008\\ -0.008}$ & $100.46$ & $97$ \\ 
58500.48 & $28.26\pm0.17$ & $-10.371\substack{+0.003\\ -0.003}$ & $2.30\substack{+0.01\\ -0.01}$ & $-11.610\substack{+0.008\\ -0.008}$ & $75.91$ & $97$ \\ 
58501.89 & $29.41\pm0.17$ & $-10.338\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.592\substack{+0.008\\ -0.008}$ & $102.98$ & $93$ \\ 
58503.24 & $27.33\pm0.15$ & $-10.387\substack{+0.003\\ -0.003}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.588\substack{+0.008\\ -0.008}$ & $82.38$ & $97$ \\ 
58504.98 & $36.19\pm0.18$ & $-10.266\substack{+0.002\\ -0.002}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.561\substack{+0.008\\ -0.008}$ & $88.93$ & $96$ \\ 
58505.95 & $38.21\pm0.19$ & $-10.235\substack{+0.002\\ -0.002}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.560\substack{+0.008\\ -0.008}$ & $94.59$ & $97$ \\ 
58506.33 & $35.81\pm0.17$ & $-10.265\substack{+0.002\\ -0.002}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.570\substack{+0.008\\ -0.008}$ & $118.24$ & $101$ \\ 
58507.62 & $32.51\pm0.18$ & $-10.306\substack{+0.003\\ -0.003}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.565\substack{+0.008\\ -0.008}$ & $74.51$ & $94$ \\ 
58511.87 & $28.02\pm0.19$ & $-10.376\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.534\substack{+0.008\\ -0.008}$ & $87.68$ & $88$ \\ 
58513.28 & $28.94\pm0.16$ & $-10.353\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.509\substack{+0.008\\ -0.008}$ & $53.76$ & $94$ \\ 
58514.73 & $29.32\pm0.16$ & $-10.358\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.520\substack{+0.008\\ -0.008}$ & $100.34$ & $95$ \\ 
58515.86 & $33.28\pm0.22$ & $-10.307\substack{+0.003\\ -0.004}$ & $2.31\substack{+0.01\\ -0.01}$ & $-11.479\substack{+0.008\\ -0.008}$ & $106.73$ & $91$ \\ 
58517.18 & $34.06\pm0.23$ & $-10.281\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $96.08$ & $87$ \\ 
58521.53 & $38.31\pm0.23$ & $-10.265\substack{+0.003\\ -0.003}$ & $2.29\substack{+0.01\\ -0.01}$ & $-11.400\substack{+0.008\\ -0.008}$ & $93.69$ & $94$ \\ 
58523.50 & $36.85\pm0.20$ & $-10.271\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.349\substack{+0.008\\ -0.008}$ & $111.06$ & $101$ \\ 
58527.09 & $39.71\pm0.26$ & $-10.260\substack{+0.003\\ -0.003}$ & $2.32\substack{+0.01\\ -0.01}$ & $-11.340\substack{+0.008\\ -0.008}$ & $73.05$ & $92$ \\ 
58528.06 & $35.89\pm0.32$ & $-10.276\substack{+0.005\\ -0.005}$ & $2.31\substack{+0.02\\ -0.02}$ & $-11.357\substack{+0.008\\ -0.008}$ & $100.02$ & $84$ \\ 
58529.87 & $33.82\pm0.26$ & $-10.304\substack{+0.004\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.327\substack{+0.008\\ -0.008}$ & $137.05$ & $90$ \\ 
58541.28 & $35.01\pm0.19$ & $-10.244\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.378\substack{+0.008\\ -0.008}$ & $85.63$ & $91$ \\ 
58544.08 & $40.89\pm0.23$ & $-10.169\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.375\substack{+0.008\\ -0.008}$ & $83.89$ & $91$ \\ 
58545.93 & $41.68\pm0.36$ & $-10.180\substack{+0.005\\ -0.005}$ & $2.22\substack{+0.02\\ -0.02}$ & $-11.373\substack{+0.008\\ -0.008}$ & $61.39$ & $84$ \\ 
58548.20 & $45.07\pm0.26$ & $-10.137\substack{+0.003\\ -0.003}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.362\substack{+0.008\\ -0.008}$ & $78.43$ & $89$ \\ 
58550.32 & $41.08\pm0.22$ & $-10.168\substack{+0.003\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.361\substack{+0.008\\ -0.008}$ & $75.20$ & $91$ \\ 
58553.35 & $37.76\pm0.23$ & $-10.207\substack{+0.003\\ -0.003}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.390\substack{+0.008\\ -0.008}$ & $121.76$ & $89$ \\ 
58556.06 & $41.40\pm0.25$ & $-10.172\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.393\substack{+0.008\\ -0.008}$ & $95.09$ & $89$ \\ 
58559.95 & $31.03\pm0.26$ & $-10.299\substack{+0.005\\ -0.005}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.387\substack{+0.008\\ -0.008}$ & $68.49$ & $85$ \\ 
58561.50 & $30.52\pm0.16$ & $-10.322\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.386\substack{+0.008\\ -0.008}$ & $104.98$ & $94$ \\ 
58562.94 & $32.26\pm0.24$ & $-10.306\substack{+0.004\\ -0.004}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.368\substack{+0.008\\ -0.008}$ & $83.60$ & $86$ \\ 
58564.04 & $43.19\pm0.28$ & $-10.175\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.359\substack{+0.008\\ -0.008}$ & $95.56$ & $89$ \\ 
58565.78 & $41.30\pm0.25$ & $-10.201\substack{+0.003\\ -0.003}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.345\substack{+0.008\\ -0.008}$ & $87.32$ & $89$ \\ 
58567.20 & $33.05\pm0.25$ & $-10.318\substack{+0.004\\ -0.004}$ & $2.32\substack{+0.01\\ -0.01}$ & $-11.334\substack{+0.008\\ -0.008}$ & $111.00$ & $93$ \\ 
58568.80 & $36.58\pm0.22$ & $-10.264\substack{+0.003\\ -0.003}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.322\substack{+0.008\\ -0.008}$ & $90.81$ & $89$ \\ 
58570.87 & $40.49\pm0.17$ & $-10.186\substack{+0.002\\ -0.002}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.306\substack{+0.008\\ -0.008}$ & $113.95$ & $100$ \\ 
58573.06 & $39.72\pm0.19$ & $-10.227\substack{+0.002\\ -0.002}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.300\substack{+0.008\\ -0.008}$ & $89.87$ & $101$ \\ 
58575.51 & $42.77\pm0.23$ & $-10.183\substack{+0.003\\ -0.003}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.290\substack{+0.008\\ -0.008}$ & $75.32$ & $93$ \\ 
58577.45 & $44.48\pm0.27$ & $-10.170\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.269\substack{+0.008\\ -0.008}$ & $99.68$ & $89$ \\ 
58579.38 & $51.48\pm0.30$ & $-10.111\substack{+0.003\\ -0.003}$ & $2.30\substack{+0.01\\ -0.01}$ & $-11.259\substack{+0.008\\ -0.008}$ & $78.74$ & $90$ \\ 
58581.35 & $42.39\pm0.28$ & $-10.174\substack{+0.003\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.275\substack{+0.008\\ -0.008}$ & $105.65$ & $88$ \\ 
58586.70 & $41.93\pm0.31$ & $-10.224\substack{+0.004\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.277\substack{+0.008\\ -0.008}$ & $98.79$ & $104$ \\ 
58588.63 & $50.92\pm0.30$ & $-10.120\substack{+0.003\\ -0.003}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.289\substack{+0.008\\ -0.008}$ & $96.92$ & $105$ \\ 
58591.05 & $43.72\pm0.26$ & $-10.200\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.294\substack{+0.008\\ -0.008}$ & $94.87$ & $102$ \\ 
58592.65 & $47.30\pm0.24$ & $-10.113\substack{+0.003\\ -0.003}$ & $1.99\substack{+0.01\\ -0.01}$ & $-11.297\substack{+0.008\\ -0.008}$ & $102.32$ & $104$ \\ 
58594.91 & $43.32\pm0.26$ & $-10.196\substack{+0.003\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.323\substack{+0.008\\ -0.008}$ & $104.08$ & $102$ \\ 
58596.84 & $44.76\pm0.27$ & $-10.158\substack{+0.004\\ -0.004}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.311\substack{+0.008\\ -0.008}$ & $101.32$ & $112$ \\ 
58603.42 & $39.37\pm0.28$ & $-10.222\substack{+0.004\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.294\substack{+0.008\\ -0.008}$ & $79.85$ & $88$ \\ 
58605.35 & $46.82\pm0.26$ & $-10.133\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.311\substack{+0.008\\ -0.008}$ & $85.81$ & $93$ \\ 
58607.22 & $36.06\pm0.21$ & $-10.247\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.334\substack{+0.008\\ -0.008}$ & $83.84$ & $94$ \\ 
58609.28 & $39.69\pm0.21$ & $-10.198\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.357\substack{+0.008\\ -0.008}$ & $100.75$ & $96$ \\ 
58611.34 & $37.47\pm0.20$ & $-10.198\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.384\substack{+0.008\\ -0.008}$ & $126.64$ & $95$ \\ 
58612.95 & $33.59\pm0.18$ & $-10.266\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.407\substack{+0.008\\ -0.008}$ & $126.10$ & $96$ \\ 
58614.95 & $37.98\pm0.19$ & $-10.221\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.419\substack{+0.008\\ -0.008}$ & $100.90$ & $99$ \\ 
58617.01 & $34.15\pm0.21$ & $-10.270\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.415\substack{+0.008\\ -0.008}$ & $69.88$ & $94$ \\ 
58619.00 & $34.68\pm0.22$ & $-10.265\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.419\substack{+0.008\\ -0.008}$ & $60.19$ & $93$ \\ 
58621.13 & $38.41\pm0.33$ & $-10.229\substack{+0.005\\ -0.005}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.423\substack{+0.008\\ -0.008}$ & $88.91$ & $88$ \\ 
58623.22 & $34.16\pm0.19$ & $-10.271\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.431\substack{+0.008\\ -0.008}$ & $104.03$ & $98$ \\ 
58626.73 & $33.49\pm0.23$ & $-10.265\substack{+0.004\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $109.39$ & $92$ \\ 
58632.66 & $28.95\pm0.21$ & $-10.349\substack{+0.004\\ -0.004}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.476\substack{+0.008\\ -0.008}$ & $115.07$ & $94$ \\ 
58635.56 & $37.60\pm0.22$ & $-10.254\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.452\substack{+0.008\\ -0.008}$ & $92.72$ & $97$ \\ 
58637.62 & $39.99\pm0.23$ & $-10.221\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.469\substack{+0.008\\ -0.008}$ & $98.91$ & $96$ \\ 
58643.87 & $48.40\pm0.30$ & $-10.143\substack{+0.003\\ -0.003}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.376\substack{+0.008\\ -0.008}$ & $108.36$ & $101$ \\ 
58646.07 & $40.51\pm0.33$ & $-10.234\substack{+0.005\\ -0.005}$ & $2.25\substack{+0.02\\ -0.02}$ & $-11.376\substack{+0.008\\ -0.008}$ & $78.54$ & $102$ \\ 
58651.93 & $36.44\pm0.22$ & $-10.265\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.370\substack{+0.008\\ -0.008}$ & $107.25$ & $101$ \\ 
58653.93 & $32.53\pm0.21$ & $-10.339\substack{+0.004\\ -0.004}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.332\substack{+0.008\\ -0.008}$ & $90.40$ & $95$ \\ 
58655.93 & $36.37\pm0.22$ & $-10.289\substack{+0.003\\ -0.003}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.320\substack{+0.008\\ -0.008}$ & $102.36$ & $96$ \\ 
58657.96 & $42.14\pm0.26$ & $-10.219\substack{+0.003\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.317\substack{+0.008\\ -0.008}$ & $87.05$ & $96$ \\ 
58660.24 & $39.81\pm0.25$ & $-10.231\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.329\substack{+0.008\\ -0.008}$ & $122.84$ & $104$ \\ 
58662.04 & $33.55\pm0.26$ & $-10.323\substack{+0.005\\ -0.005}$ & $2.19\substack{+0.02\\ -0.02}$ & $-11.310\substack{+0.008\\ -0.008}$ & $105.27$ & $100$ \\ 
58664.24 & $38.72\pm0.25$ & $-10.254\substack{+0.004\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.296\substack{+0.008\\ -0.008}$ & $119.39$ & $101$ \\ 
58665.88 & $37.90\pm0.30$ & $-10.285\substack{+0.005\\ -0.005}$ & $2.33\substack{+0.02\\ -0.02}$ & $-11.316\substack{+0.008\\ -0.008}$ & $130.29$ & $101$ \\ 
58673.24 & $31.21\pm0.21$ & $-10.255\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.368\substack{+0.008\\ -0.008}$ & $83.94$ & $93$ \\ 
58675.30 & $30.84\pm0.18$ & $-10.256\substack{+0.003\\ -0.003}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.375\substack{+0.008\\ -0.008}$ & $87.55$ & $96$ \\ 
58677.17 & $27.85\pm0.15$ & $-10.317\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.391\substack{+0.008\\ -0.008}$ & $121.27$ & $100$ \\ 
58679.04 & $36.63\pm0.20$ & $-10.178\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.403\substack{+0.008\\ -0.008}$ & $94.91$ & $98$ \\ 
58680.40 & $32.92\pm0.21$ & $-10.239\substack{+0.004\\ -0.004}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.440\substack{+0.008\\ -0.008}$ & $110.31$ & $98$ \\ 
58683.23 & $28.39\pm0.15$ & $-10.300\substack{+0.003\\ -0.003}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.462\substack{+0.008\\ -0.008}$ & $112.99$ & $100$ \\ 
58685.11 & $31.46\pm0.20$ & $-10.249\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.482\substack{+0.008\\ -0.008}$ & $90.24$ & $97$ \\ 
58687.54 & $30.79\pm0.23$ & $-10.248\substack{+0.004\\ -0.004}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.507\substack{+0.008\\ -0.008}$ & $75.74$ & $92$ \\ 
58690.12 & $21.12\pm0.18$ & $-10.479\substack{+0.005\\ -0.005}$ & $2.02\substack{+0.02\\ -0.02}$ & $-11.566\substack{+0.008\\ -0.008}$ & $125.23$ & $91$ \\ 
58691.79 & $29.50\pm0.19$ & $-10.337\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.522\substack{+0.008\\ -0.008}$ & $100.66$ & $95$ \\ 
58694.70 & $33.85\pm0.20$ & $-10.307\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.501\substack{+0.008\\ -0.008}$ & $103.53$ & $95$ \\ 
58699.98 & $40.29\pm0.26$ & $-10.224\substack{+0.003\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.502\substack{+0.008\\ -0.008}$ & $70.32$ & $94$ \\ 
58702.27 & $39.39\pm0.26$ & $-10.248\substack{+0.004\\ -0.004}$ & $2.32\substack{+0.01\\ -0.01}$ & $-11.521\substack{+0.008\\ -0.008}$ & $93.20$ & $102$ \\ 
58704.59 & $33.01\pm0.20$ & $-10.308\substack{+0.003\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.528\substack{+0.008\\ -0.008}$ & $111.80$ & $101$ \\ 
58706.46 & $36.65\pm0.22$ & $-10.246\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.564\substack{+0.008\\ -0.008}$ & $104.06$ & $98$ \\ 
58711.99 & $25.50\pm0.22$ & $-10.400\substack{+0.005\\ -0.005}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.678\substack{+0.008\\ -0.008}$ & $96.93$ & $89$ \\ 
58712.05 & $26.95\pm0.23$ & $-10.376\substack{+0.005\\ -0.005}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.678\substack{+0.008\\ -0.008}$ & $93.68$ & $90$ \\ 
58713.92 & $29.76\pm0.19$ & $-10.309\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-11.671\substack{+0.008\\ -0.008}$ & $112.14$ & $96$ \\ 
58715.57 & $33.04\pm0.19$ & $-10.278\substack{+0.003\\ -0.003}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.669\substack{+0.008\\ -0.008}$ & $89.01$ & $96$ \\ 
58717.44 & $30.73\pm0.21$ & $-10.307\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.665\substack{+0.008\\ -0.008}$ & $103.23$ & $93$ \\ 
58719.05 & $28.63\pm0.17$ & $-10.340\substack{+0.003\\ -0.003}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.659\substack{+0.008\\ -0.008}$ & $91.12$ & $96$ \\ 
58721.15 & $22.69\pm0.18$ & $-10.453\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.635\substack{+0.008\\ -0.008}$ & $81.30$ & $91$ \\ 
58723.06 & $29.15\pm0.24$ & $-10.365\substack{+0.005\\ -0.005}$ & $2.23\substack{+0.02\\ -0.02}$ & $-11.613\substack{+0.008\\ -0.008}$ & $80.80$ & $102$ \\ 
58729.84 & $41.17\pm0.32$ & $-10.216\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.518\substack{+0.008\\ -0.008}$ & $113.65$ & $93$ \\ 
58737.40 & $37.53\pm0.38$ & $-10.222\substack{+0.006\\ -0.006}$ & $2.21\substack{+0.02\\ -0.02}$ & $-11.525\substack{+0.008\\ -0.008}$ & $80.47$ & $91$ \\ 
58739.36 & $35.93\pm0.28$ & $-10.252\substack{+0.004\\ -0.004}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.508\substack{+0.008\\ -0.008}$ & $107.56$ & $101$ \\ 
58740.65 & $35.51\pm0.29$ & $-10.261\substack{+0.005\\ -0.005}$ & $2.26\substack{+0.02\\ -0.02}$ & $-11.479\substack{+0.008\\ -0.008}$ & $97.12$ & $93$ \\ 
58742.97 & $37.81\pm0.29$ & $-10.239\substack{+0.004\\ -0.004}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $98.15$ & $92$ \\ 
58743.04 & $37.53\pm0.29$ & $-10.245\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $121.08$ & $99$ \\ 
58744.91 & $34.84\pm0.23$ & $-10.255\substack{+0.004\\ -0.004}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.456\substack{+0.008\\ -0.008}$ & $101.96$ & $96$ \\ 
58751.71 & $28.76\pm0.19$ & $-10.345\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.472\substack{+0.008\\ -0.008}$ & $101.77$ & $96$ \\ 
58753.15 & $31.04\pm0.22$ & $-10.332\substack{+0.004\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.460\substack{+0.008\\ -0.008}$ & $91.90$ & $93$ \\ 
58755.02 & $31.95\pm0.20$ & $-10.330\substack{+0.003\\ -0.003}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.425\substack{+0.008\\ -0.008}$ & $106.73$ & $96$ \\ 
58756.57 & $31.29\pm0.18$ & $-10.357\substack{+0.003\\ -0.003}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.435\substack{+0.008\\ -0.008}$ & $89.43$ & $97$ \\ 
58758.38 & $29.68\pm0.19$ & $-10.383\substack{+0.003\\ -0.003}$ & $2.29\substack{+0.01\\ -0.01}$ & $-11.444\substack{+0.008\\ -0.008}$ & $103.56$ & $101$ \\ 
58761.66 & $36.79\pm0.22$ & $-10.264\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.423\substack{+0.008\\ -0.008}$ & $93.93$ & $96$ \\ 
58765.31 & $39.32\pm0.19$ & $-10.233\substack{+0.002\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.443\substack{+0.008\\ -0.008}$ & $104.47$ & $100$ \\ 
58767.60 & $41.91\pm0.22$ & $-10.192\substack{+0.003\\ -0.003}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.488\substack{+0.008\\ -0.008}$ & $81.31$ & $100$ \\ 
58777.69 & $38.01\pm0.19$ & $-10.232\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.510\substack{+0.008\\ -0.008}$ & $79.18$ & $100$ \\ 
58779.17 & $36.84\pm0.18$ & $-10.244\substack{+0.002\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.493\substack{+0.008\\ -0.008}$ & $77.13$ & $100$ \\ 
58781.20 & $33.06\pm0.22$ & $-10.321\substack{+0.004\\ -0.004}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.481\substack{+0.008\\ -0.008}$ & $132.54$ & $101$ \\ 
58783.30 & $34.53\pm0.22$ & $-10.266\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.499\substack{+0.008\\ -0.008}$ & $106.66$ & $101$ \\ 
58785.09 & $36.54\pm0.26$ & $-10.270\substack{+0.004\\ -0.004}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.506\substack{+0.008\\ -0.008}$ & $78.25$ & $93$ \\ 
58786.96 & $37.57\pm0.24$ & $-10.238\substack{+0.003\\ -0.003}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.552\substack{+0.008\\ -0.008}$ & $100.76$ & $97$ \\ 
58789.28 & $27.66\pm0.16$ & $-10.360\substack{+0.003\\ -0.003}$ & $2.07\substack{+0.01\\ -0.01}$ & $-11.564\substack{+0.008\\ -0.008}$ & $109.04$ & $98$ \\ 
58791.61 & $31.21\pm0.20$ & $-10.302\substack{+0.004\\ -0.004}$ & $2.07\substack{+0.01\\ -0.01}$ & $-11.570\substack{+0.008\\ -0.008}$ & $85.87$ & $95$ \\ 
58793.60 & $30.96\pm0.21$ & $-10.313\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.566\substack{+0.008\\ -0.008}$ & $112.84$ & $93$ \\ 
58794.80 & $35.14\pm0.25$ & $-10.272\substack{+0.004\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.582\substack{+0.008\\ -0.008}$ & $82.94$ & $92$ \\ 
58800.52 & $36.49\pm0.25$ & $-10.227\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.573\substack{+0.008\\ -0.008}$ & $88.69$ & $100$ \\ 
58801.97 & $39.04\pm0.24$ & $-10.191\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.565\substack{+0.008\\ -0.008}$ & $65.91$ & $96$ \\ 
58805.13 & $35.05\pm0.20$ & $-10.249\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.561\substack{+0.008\\ -0.008}$ & $80.16$ & $100$ \\ 
58807.45 & $40.30\pm0.24$ & $-10.200\substack{+0.003\\ -0.003}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.524\substack{+0.008\\ -0.008}$ & $118.79$ & $101$ \\ 
58808.87 & $32.50\pm0.23$ & $-10.302\substack{+0.004\\ -0.004}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.535\substack{+0.008\\ -0.008}$ & $91.83$ & $98$ \\ 
58810.94 & $30.83\pm0.25$ & $-10.316\substack{+0.005\\ -0.005}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.548\substack{+0.008\\ -0.008}$ & $80.14$ & $91$ \\ 
58811.00 & $31.05\pm0.27$ & $-10.301\substack{+0.005\\ -0.005}$ & $2.13\substack{+0.02\\ -0.02}$ & $-11.548\substack{+0.008\\ -0.008}$ & $83.59$ & $90$ \\ 
58812.59 & $31.51\pm0.23$ & $-10.323\substack{+0.004\\ -0.004}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.555\substack{+0.008\\ -0.008}$ & $105.22$ & $91$ \\ 
58815.65 & $26.92\pm0.17$ & $-10.364\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-11.556\substack{+0.008\\ -0.008}$ & $107.45$ & $95$ \\ 
58817.45 & $31.76\pm0.18$ & $-10.295\substack{+0.003\\ -0.003}$ & $2.06\substack{+0.01\\ -0.01}$ & $-11.531\substack{+0.008\\ -0.008}$ & $68.72$ & $97$ \\ 
58819.36 & $35.29\pm0.22$ & $-10.281\substack{+0.003\\ -0.003}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.535\substack{+0.008\\ -0.008}$ & $88.02$ & $94$ \\ 
58821.49 & $32.37\pm0.19$ & $-10.307\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.537\substack{+0.008\\ -0.008}$ & $89.12$ & $97$ \\ 
58823.49 & $36.80\pm0.21$ & $-10.244\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.561\substack{+0.008\\ -0.008}$ & $92.59$ & $97$ \\ 
58825.62 & $31.75\pm0.19$ & $-10.309\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.567\substack{+0.008\\ -0.008}$ & $102.47$ & $96$ \\ 
58827.62 & $29.95\pm0.18$ & $-10.334\substack{+0.003\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.582\substack{+0.008\\ -0.008}$ & $97.19$ & $97$ \\ 
58829.88 & $30.32\pm0.20$ & $-10.324\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.526\substack{+0.008\\ -0.008}$ & $96.30$ & $95$ \\ 
58832.01 & $31.93\pm0.26$ & $-10.277\substack{+0.005\\ -0.005}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.521\substack{+0.008\\ -0.008}$ & $100.93$ & $93$ \\ 
58833.86 & $39.73\pm0.36$ & $-10.184\substack{+0.004\\ -0.005}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.525\substack{+0.008\\ -0.008}$ & $78.46$ & $87$ \\ 
58835.88 & $38.11\pm0.28$ & $-10.186\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.499\substack{+0.008\\ -0.008}$ & $104.57$ & $95$ \\ 
58836.01 & $38.22\pm0.30$ & $-10.197\substack{+0.004\\ -0.005}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.496\substack{+0.008\\ -0.008}$ & $92.62$ & $93$ \\ 
58844.21 & $39.61\pm0.25$ & $-10.212\substack{+0.003\\ -0.003}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.439\substack{+0.008\\ -0.008}$ & $89.25$ & $92$ \\ 
58847.69 & $39.45\pm0.21$ & $-10.189\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.479\substack{+0.008\\ -0.008}$ & $111.19$ & $96$ \\ 
58849.83 & $33.11\pm0.20$ & $-10.241\substack{+0.003\\ -0.003}$ & $2.06\substack{+0.01\\ -0.01}$ & $-11.493\substack{+0.008\\ -0.008}$ & $87.27$ & $93$ \\ 
58851.80 & $32.09\pm0.24$ & $-10.269\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.513\substack{+0.008\\ -0.008}$ & $97.43$ & $94$ \\ 
58853.64 & $32.49\pm0.28$ & $-10.251\substack{+0.005\\ -0.005}$ & $2.07\substack{+0.02\\ -0.02}$ & $-11.510\substack{+0.008\\ -0.008}$ & $73.55$ & $90$ \\ 
58855.80 & $35.74\pm0.23$ & $-10.216\substack{+0.004\\ -0.004}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.521\substack{+0.008\\ -0.008}$ & $105.81$ & $92$ \\ 
58857.80 & $33.86\pm0.22$ & $-10.237\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.540\substack{+0.008\\ -0.008}$ & $96.13$ & $93$ \\ 
58859.80 & $31.38\pm0.26$ & $-10.253\substack{+0.005\\ -0.005}$ & $2.00\substack{+0.01\\ -0.01}$ & $-11.547\substack{+0.008\\ -0.008}$ & $100.03$ & $85$ \\ 
58861.80 & $31.41\pm0.20$ & $-10.254\substack{+0.004\\ -0.004}$ & $1.98\substack{+0.01\\ -0.01}$ & $-11.530\substack{+0.008\\ -0.008}$ & $109.69$ & $91$ \\ 
58863.61 & $26.11\pm0.16$ & $-10.352\substack{+0.003\\ -0.003}$ & $2.03\substack{+0.01\\ -0.01}$ & $-11.514\substack{+0.008\\ -0.008}$ & $88.76$ & $93$ \\ 
58865.22 & $31.05\pm0.19$ & $-10.298\substack{+0.003\\ -0.003}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.501\substack{+0.008\\ -0.008}$ & $98.02$ & $93$ \\ 
58866.71 & $34.96\pm0.19$ & $-10.241\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.489\substack{+0.008\\ -0.008}$ & $89.66$ & $94$ \\ 
58868.85 & $33.20\pm0.25$ & $-10.284\substack{+0.004\\ -0.004}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.475\substack{+0.008\\ -0.008}$ & $89.63$ & $86$ \\ 
58870.84 & $37.58\pm0.18$ & $-10.202\substack{+0.002\\ -0.002}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.478\substack{+0.008\\ -0.008}$ & $99.58$ & $97$ \\ 
58871.67 & $34.37\pm0.31$ & $-10.244\substack{+0.005\\ -0.005}$ & $2.13\substack{+0.02\\ -0.02}$ & $-11.484\substack{+0.008\\ -0.008}$ & $89.51$ & $85$ \\ 
58873.22 & $35.52\pm0.18$ & $-10.247\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.495\substack{+0.008\\ -0.008}$ & $101.74$ & $95$ \\ 
58875.16 & $31.60\pm0.17$ & $-10.287\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.509\substack{+0.008\\ -0.008}$ & $91.32$ & $93$ \\ 
58876.97 & $28.02\pm0.16$ & $-10.347\substack{+0.003\\ -0.003}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.522\substack{+0.008\\ -0.008}$ & $86.15$ & $93$ \\ 
58877.68 & $31.72\pm0.23$ & $-10.306\substack{+0.004\\ -0.004}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.527\substack{+0.008\\ -0.008}$ & $113.73$ & $88$ \\ 
58879.49 & $29.27\pm0.29$ & $-10.299\substack{+0.006\\ -0.006}$ & $2.05\substack{+0.02\\ -0.02}$ & $-11.527\substack{+0.008\\ -0.008}$ & $95.12$ & $81$ \\ 
58884.72 & $28.81\pm0.20$ & $-10.329\substack{+0.004\\ -0.004}$ & $2.01\substack{+0.01\\ -0.01}$ & $-11.554\substack{+0.008\\ -0.008}$ & $112.93$ & $95$ \\ 
58887.53 & $36.60\pm0.23$ & $-10.239\substack{+0.003\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.510\substack{+0.008\\ -0.008}$ & $127.62$ & $97$ \\ 
58889.57 & $33.50\pm0.18$ & $-10.255\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.505\substack{+0.008\\ -0.008}$ & $99.37$ & $99$ \\ 
58891.63 & $41.70\pm0.23$ & $-10.200\substack{+0.003\\ -0.003}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.461\substack{+0.008\\ -0.008}$ & $121.90$ & $98$ \\ 
58893.40 & $37.66\pm0.24$ & $-10.228\substack{+0.003\\ -0.003}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.442\substack{+0.008\\ -0.008}$ & $100.15$ & $91$ \\ 
58902.65 & $32.65\pm0.24$ & $-10.317\substack{+0.004\\ -0.004}$ & $2.34\substack{+0.01\\ -0.01}$ & $-11.430\substack{+0.008\\ -0.008}$ & $102.75$ & $83$ \\ 
58903.97 & $34.78\pm0.25$ & $-10.276\substack{+0.004\\ -0.004}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.432\substack{+0.008\\ -0.008}$ & $92.01$ & $84$ \\ 
58905.59 & $45.07\pm0.29$ & $-10.151\substack{+0.003\\ -0.003}$ & $2.31\substack{+0.01\\ -0.01}$ & $-11.435\substack{+0.008\\ -0.008}$ & $97.97$ & $85$ \\ 
58909.60 & $33.97\pm0.21$ & $-10.258\substack{+0.003\\ -0.003}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.510\substack{+0.008\\ -0.008}$ & $67.00$ & $92$ \\ 
58910.86 & $35.82\pm0.29$ & $-10.210\substack{+0.005\\ -0.005}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.531\substack{+0.008\\ -0.008}$ & $56.44$ & $84$ \\ 
58911.31 & $35.47\pm0.27$ & $-10.203\substack{+0.004\\ -0.004}$ & $2.06\substack{+0.01\\ -0.01}$ & $-11.531\substack{+0.008\\ -0.008}$ & $92.87$ & $86$ \\ 
58915.75 & $26.76\pm0.21$ & $-10.353\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.552\substack{+0.008\\ -0.008}$ & $89.76$ & $86$ \\ 
58917.39 & $25.68\pm0.27$ & $-10.334\substack{+0.006\\ -0.006}$ & $1.96\substack{+0.02\\ -0.02}$ & $-11.568\substack{+0.008\\ -0.008}$ & $75.39$ & $80$ \\ 
58919.20 & $33.34\pm0.22$ & $-10.234\substack{+0.004\\ -0.004}$ & $2.04\substack{+0.01\\ -0.01}$ & $-11.586\substack{+0.008\\ -0.008}$ & $83.98$ & $88$ \\ 
58921.27 & $35.40\pm0.23$ & $-10.217\substack{+0.003\\ -0.003}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.594\substack{+0.008\\ -0.008}$ & $104.40$ & $89$ \\ 
58923.07 & $34.72\pm0.22$ & $-10.242\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.601\substack{+0.008\\ -0.008}$ & $85.08$ & $89$ \\ 
58929.79 & $35.73\pm0.23$ & $-10.216\substack{+0.003\\ -0.003}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.629\substack{+0.008\\ -0.008}$ & $85.64$ & $89$ \\ 
58931.55 & $36.21\pm0.25$ & $-10.213\substack{+0.004\\ -0.004}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.637\substack{+0.008\\ -0.008}$ & $66.33$ & $87$ \\ 
58933.41 & $34.95\pm0.21$ & $-10.212\substack{+0.003\\ -0.003}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.646\substack{+0.008\\ -0.008}$ & $95.09$ & $89$ \\ 
58935.42 & $34.32\pm0.21$ & $-10.216\substack{+0.003\\ -0.003}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.657\substack{+0.008\\ -0.008}$ & $119.13$ & $89$ \\ 
58937.60 & $29.67\pm0.23$ & $-10.283\substack{+0.004\\ -0.004}$ & $2.07\substack{+0.01\\ -0.01}$ & $-11.670\substack{+0.008\\ -0.008}$ & $73.56$ & $86$ \\ 
58939.87 & $33.50\pm0.17$ & $-10.246\substack{+0.003\\ -0.003}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.674\substack{+0.008\\ -0.008}$ & $109.71$ & $95$ \\ 
58941.71 & $31.85\pm0.24$ & $-10.250\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-11.671\substack{+0.008\\ -0.008}$ & $113.73$ & $86$ \\ 
58943.49 & $34.86\pm0.25$ & $-10.220\substack{+0.004\\ -0.004}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.655\substack{+0.008\\ -0.008}$ & $80.52$ & $86$ \\ 
58945.04 & $38.40\pm0.37$ & $-10.165\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.639\substack{+0.008\\ -0.008}$ & $81.50$ & $81$ \\ 
58953.41 & $42.22\pm0.26$ & $-10.201\substack{+0.003\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.511\substack{+0.008\\ -0.008}$ & $78.33$ & $101$ \\ 
58955.66 & $50.81\pm0.31$ & $-10.130\substack{+0.003\\ -0.003}$ & $2.31\substack{+0.01\\ -0.01}$ & $-11.490\substack{+0.008\\ -0.008}$ & $85.11$ & $95$ \\ 
58957.37 & $52.15\pm0.27$ & $-10.122\substack{+0.003\\ -0.003}$ & $2.33\substack{+0.01\\ -0.01}$ & $-11.477\substack{+0.008\\ -0.008}$ & $101.05$ & $103$ \\ 
58963.86 & $45.85\pm0.29$ & $-10.149\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.460\substack{+0.008\\ -0.008}$ & $90.16$ & $103$ \\ 
58969.26 & $48.63\pm0.30$ & $-10.104\substack{+0.003\\ -0.003}$ & $2.29\substack{+0.01\\ -0.01}$ & $-11.407\substack{+0.008\\ -0.008}$ & $74.38$ & $90$ \\ 
58971.20 & $43.16\pm0.28$ & $-10.152\substack{+0.003\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.392\substack{+0.008\\ -0.008}$ & $83.21$ & $91$ \\ 
58973.33 & $42.46\pm0.22$ & $-10.164\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.376\substack{+0.008\\ -0.008}$ & $70.89$ & $95$ \\ 
58975.26 & $43.28\pm0.23$ & $-10.185\substack{+0.003\\ -0.003}$ & $2.37\substack{+0.01\\ -0.01}$ & $-11.359\substack{+0.008\\ -0.008}$ & $101.82$ & $101$ \\ 
58977.26 & $45.61\pm0.21$ & $-10.137\substack{+0.002\\ -0.002}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.341\substack{+0.008\\ -0.008}$ & $109.25$ & $98$ \\ 
58979.50 & $50.17\pm0.34$ & $-10.103\substack{+0.004\\ -0.004}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.321\substack{+0.008\\ -0.008}$ & $104.69$ & $90$ \\ 
58981.42 & $38.88\pm0.22$ & $-10.239\substack{+0.003\\ -0.003}$ & $2.29\substack{+0.01\\ -0.01}$ & $-11.305\substack{+0.008\\ -0.008}$ & $92.83$ & $94$ \\ 
58983.35 & $39.14\pm0.23$ & $-10.245\substack{+0.003\\ -0.003}$ & $2.33\substack{+0.01\\ -0.01}$ & $-11.290\substack{+0.008\\ -0.008}$ & $89.58$ & $93$ \\ 
58985.26 & $42.68\pm0.25$ & $-10.197\substack{+0.003\\ -0.003}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.276\substack{+0.008\\ -0.008}$ & $90.40$ & $95$ \\ 
58987.26 & $40.26\pm0.37$ & $-10.210\substack{+0.005\\ -0.005}$ & $2.21\substack{+0.02\\ -0.02}$ & $-11.275\substack{+0.008\\ -0.008}$ & $95.74$ & $87$ \\ 
58994.55 & $43.26\pm0.24$ & $-10.201\substack{+0.003\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.276\substack{+0.008\\ -0.008}$ & $108.63$ & $99$ \\ 
59008.58 & $38.80\pm0.20$ & $-10.215\substack{+0.003\\ -0.003}$ & $2.00\substack{+0.01\\ -0.01}$ & $-11.264\substack{+0.008\\ -0.008}$ & $84.09$ & $99$ \\ 
59014.56 & $39.10\pm0.24$ & $-10.264\substack{+0.003\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.262\substack{+0.008\\ -0.008}$ & $100.11$ & $96$ \\ 
59022.87 & $35.44\pm0.34$ & $-10.340\substack{+0.006\\ -0.006}$ & $2.35\substack{+0.02\\ -0.02}$ & $-11.234\substack{+0.008\\ -0.008}$ & $107.57$ & $99$ \\ 
59025.00 & $42.03\pm0.38$ & $-10.248\substack{+0.005\\ -0.005}$ & $2.35\substack{+0.02\\ -0.02}$ & $-11.252\substack{+0.008\\ -0.008}$ & $84.08$ & $93$ \\ 
59027.00 & $49.80\pm0.40$ & $-10.144\substack{+0.005\\ -0.005}$ & $2.25\substack{+0.02\\ -0.02}$ & $-11.269\substack{+0.008\\ -0.008}$ & $101.41$ & $98$ \\ 
59028.72 & $45.76\pm0.24$ & $-10.163\substack{+0.003\\ -0.003}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.276\substack{+0.008\\ -0.008}$ & $116.39$ & $100$ \\ 
59029.88 & $39.77\pm0.33$ & $-10.231\substack{+0.005\\ -0.005}$ & $2.13\substack{+0.02\\ -0.01}$ & $-11.280\substack{+0.008\\ -0.008}$ & $84.35$ & $89$ \\ 
59034.31 & $38.93\pm0.28$ & $-10.214\substack{+0.004\\ -0.004}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.298\substack{+0.008\\ -0.008}$ & $84.00$ & $90$ \\ 
59036.63 & $39.59\pm0.31$ & $-10.216\substack{+0.004\\ -0.004}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.295\substack{+0.008\\ -0.008}$ & $68.35$ & $88$ \\ 
59038.89 & $45.19\pm0.24$ & $-10.182\substack{+0.003\\ -0.003}$ & $2.31\substack{+0.01\\ -0.01}$ & $-11.290\substack{+0.008\\ -0.008}$ & $126.64$ & $98$ \\ 
59042.55 & $44.17\pm0.31$ & $-10.205\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.282\substack{+0.008\\ -0.008}$ & $104.56$ & $94$ \\ 
59043.95 & $37.81\pm0.29$ & $-10.271\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.281\substack{+0.008\\ -0.008}$ & $75.09$ & $89$ \\ 
59044.01 & $36.95\pm0.26$ & $-10.284\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.01\\ -0.01}$ & $-11.280\substack{+0.008\\ -0.008}$ & $116.60$ & $91$ \\ 
59053.90 & $42.40\pm0.22$ & $-10.193\substack{+0.003\\ -0.003}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.254\substack{+0.008\\ -0.008}$ & $97.71$ & $98$ \\ 
59056.47 & $37.76\pm0.23$ & $-10.281\substack{+0.003\\ -0.003}$ & $2.29\substack{+0.01\\ -0.01}$ & $-11.246\substack{+0.008\\ -0.008}$ & $116.79$ & $95$ \\ 
59060.66 & $43.35\pm0.23$ & $-10.201\substack{+0.003\\ -0.003}$ & $2.23\substack{+0.01\\ -0.01}$ & $-11.260\substack{+0.008\\ -0.008}$ & $94.79$ & $97$ \\ 
59062.59 & $48.40\pm0.28$ & $-10.145\substack{+0.003\\ -0.003}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.278\substack{+0.008\\ -0.008}$ & $103.38$ & $95$ \\ 
59064.59 & $44.18\pm0.25$ & $-10.172\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.285\substack{+0.008\\ -0.008}$ & $98.72$ & $98$ \\ 
59066.56 & $46.09\pm0.26$ & $-10.165\substack{+0.003\\ -0.003}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.292\substack{+0.008\\ -0.008}$ & $110.90$ & $97$ \\ 
59070.92 & $44.46\pm0.28$ & $-10.174\substack{+0.003\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.334\substack{+0.008\\ -0.008}$ & $92.60$ & $96$ \\ 
59072.73 & $46.47\pm0.30$ & $-10.146\substack{+0.004\\ -0.004}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.343\substack{+0.008\\ -0.008}$ & $95.43$ & $99$ \\ 
59074.96 & $47.04\pm0.28$ & $-10.161\substack{+0.003\\ -0.003}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.356\substack{+0.008\\ -0.008}$ & $94.51$ & $101$ \\ 
59076.91 & $41.70\pm0.22$ & $-10.212\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.366\substack{+0.008\\ -0.008}$ & $134.90$ & $98$ \\ 
59077.97 & $39.65\pm0.23$ & $-10.226\substack{+0.003\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.373\substack{+0.008\\ -0.008}$ & $97.89$ & $96$ \\ 
59080.91 & $38.62\pm0.22$ & $-10.230\substack{+0.003\\ -0.003}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.390\substack{+0.008\\ -0.008}$ & $96.18$ & $96$ \\ 
59082.88 & $41.21\pm0.32$ & $-10.207\substack{+0.004\\ -0.004}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.402\substack{+0.008\\ -0.008}$ & $86.32$ & $90$ \\ 
59083.01 & $42.84\pm0.27$ & $-10.190\substack{+0.003\\ -0.003}$ & $2.22\substack{+0.01\\ -0.01}$ & $-11.402\substack{+0.008\\ -0.008}$ & $71.58$ & $93$ \\ 
59084.93 & $31.84\pm0.25$ & $-10.318\substack{+0.005\\ -0.005}$ & $2.15\substack{+0.02\\ -0.01}$ & $-11.413\substack{+0.008\\ -0.008}$ & $88.65$ & $100$ \\ 
59088.99 & $35.53\pm0.28$ & $-10.275\substack{+0.005\\ -0.005}$ & $2.21\substack{+0.01\\ -0.01}$ & $-11.438\substack{+0.008\\ -0.008}$ & $114.45$ & $99$ \\ 
59093.97 & $24.18\pm0.29$ & $-10.401\substack{+0.008\\ -0.008}$ & $1.92\substack{+0.02\\ -0.02}$ & $-11.451\substack{+0.008\\ -0.008}$ & $85.60$ & $84$ \\ 
59095.94 & $38.63\pm0.25$ & $-10.233\substack{+0.003\\ -0.003}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.439\substack{+0.008\\ -0.008}$ & $83.65$ & $92$ \\ 
59101.27 & $43.67\pm0.26$ & $-10.147\substack{+0.003\\ -0.003}$ & $2.27\substack{+0.01\\ -0.01}$ & $-11.449\substack{+0.008\\ -0.008}$ & $75.83$ & $96$ \\ 
59103.86 & $50.50\pm0.28$ & $-10.077\substack{+0.003\\ -0.003}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.468\substack{+0.008\\ -0.008}$ & $107.14$ & $99$ \\ 
59105.31 & $42.48\pm0.30$ & $-10.144\substack{+0.004\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.479\substack{+0.008\\ -0.008}$ & $123.31$ & $99$ \\ 
59107.95 & $40.50\pm0.27$ & $-10.150\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.506\substack{+0.008\\ -0.008}$ & $101.27$ & $95$ \\ 
59109.31 & $31.90\pm0.25$ & $-10.259\substack{+0.005\\ -0.005}$ & $2.13\substack{+0.01\\ -0.01}$ & $-11.539\substack{+0.008\\ -0.008}$ & $101.01$ & $93$ \\ 
59116.29 & $27.44\pm0.19$ & $-10.344\substack{+0.004\\ -0.004}$ & $2.04\substack{+0.01\\ -0.01}$ & $-11.608\substack{+0.008\\ -0.008}$ & $85.72$ & $95$ \\ 
59118.43 & $27.68\pm0.14$ & $-10.325\substack{+0.003\\ -0.003}$ & $1.99\substack{+0.01\\ -0.01}$ & $-11.628\substack{+0.008\\ -0.008}$ & $97.22$ & $101$ \\ 
59120.59 & $28.64\pm0.18$ & $-10.317\substack{+0.004\\ -0.004}$ & $2.02\substack{+0.01\\ -0.01}$ & $-11.623\substack{+0.008\\ -0.008}$ & $83.14$ & $98$ \\ 
59122.53 & $36.04\pm0.19$ & $-10.228\substack{+0.003\\ -0.003}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.618\substack{+0.008\\ -0.008}$ & $98.96$ & $99$ \\ 
59124.47 & $28.00\pm0.18$ & $-10.346\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.614\substack{+0.008\\ -0.008}$ & $94.02$ & $97$ \\ 
59126.20 & $31.30\pm0.29$ & $-10.300\substack{+0.004\\ -0.004}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.610\substack{+0.008\\ -0.008}$ & $105.04$ & $87$ \\ 
59128.12 & $30.62\pm0.21$ & $-10.299\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.605\substack{+0.008\\ -0.008}$ & $63.69$ & $97$ \\ 
59129.56 & $33.45\pm0.22$ & $-10.268\substack{+0.004\\ -0.004}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.602\substack{+0.008\\ -0.008}$ & $71.94$ & $94$ \\ 
59130.75 & $36.64\pm0.25$ & $-10.221\substack{+0.004\\ -0.004}$ & $2.08\substack{+0.01\\ -0.01}$ & $-11.599\substack{+0.008\\ -0.008}$ & $111.99$ & $94$ \\ 
59136.81 & $36.36\pm0.29$ & $-10.230\substack{+0.005\\ -0.005}$ & $2.11\substack{+0.01\\ -0.01}$ & $-11.586\substack{+0.008\\ -0.008}$ & $98.63$ & $90$ \\ 
59138.33 & $36.38\pm0.23$ & $-10.237\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.583\substack{+0.008\\ -0.008}$ & $83.45$ & $95$ \\ 
59141.04 & $33.05\pm0.22$ & $-10.287\substack{+0.004\\ -0.004}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.553\substack{+0.008\\ -0.008}$ & $103.29$ & $98$ \\ 
59142.79 & $30.68\pm0.34$ & $-10.320\substack{+0.006\\ -0.006}$ & $2.14\substack{+0.02\\ -0.02}$ & $-11.534\substack{+0.008\\ -0.008}$ & $80.66$ & $86$ \\ 
59144.40 & $32.40\pm0.21$ & $-10.298\substack{+0.004\\ -0.004}$ & $2.16\substack{+0.01\\ -0.01}$ & $-11.518\substack{+0.008\\ -0.008}$ & $103.43$ & $94$ \\ 
59148.93 & $34.20\pm0.24$ & $-10.271\substack{+0.004\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.493\substack{+0.008\\ -0.008}$ & $78.66$ & $94$ \\ 
59150.52 & $29.12\pm0.20$ & $-10.349\substack{+0.004\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.487\substack{+0.008\\ -0.008}$ & $110.83$ & $93$ \\ 
59151.84 & $32.89\pm0.20$ & $-10.302\substack{+0.003\\ -0.003}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.480\substack{+0.008\\ -0.008}$ & $100.35$ & $95$ \\ 
59153.87 & $28.73\pm0.19$ & $-10.365\substack{+0.003\\ -0.004}$ & $2.18\substack{+0.01\\ -0.01}$ & $-11.461\substack{+0.008\\ -0.008}$ & $80.44$ & $93$ \\ 
59155.71 & $28.29\pm0.24$ & $-10.369\substack{+0.005\\ -0.005}$ & $2.15\substack{+0.02\\ -0.02}$ & $-11.443\substack{+0.008\\ -0.008}$ & $67.67$ & $89$ \\ 
59157.68 & $31.11\pm0.21$ & $-10.352\substack{+0.004\\ -0.004}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.426\substack{+0.008\\ -0.008}$ & $91.46$ & $92$ \\ 
59165.69 & $39.17\pm0.34$ & $-10.204\substack{+0.005\\ -0.005}$ & $2.24\substack{+0.02\\ -0.02}$ & $-11.429\substack{+0.008\\ -0.008}$ & $62.32$ & $88$ \\ 
59166.40 & $35.07\pm0.24$ & $-10.258\substack{+0.004\\ -0.004}$ & $2.24\substack{+0.01\\ -0.01}$ & $-11.427\substack{+0.008\\ -0.008}$ & $93.91$ & $98$ \\ 
59170.40 & $33.50\pm0.21$ & $-10.289\substack{+0.003\\ -0.003}$ & $2.30\substack{+0.01\\ -0.01}$ & $-11.424\substack{+0.008\\ -0.008}$ & $82.41$ & $100$ \\ 
59172.72 & $39.57\pm0.31$ & $-10.192\substack{+0.004\\ -0.004}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.430\substack{+0.008\\ -0.008}$ & $103.42$ & $89$ \\ 
59179.54 & $38.85\pm0.23$ & $-10.216\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.454\substack{+0.008\\ -0.008}$ & $100.56$ & $96$ \\ 
59181.25 & $33.12\pm0.23$ & $-10.290\substack{+0.004\\ -0.004}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.475\substack{+0.008\\ -0.008}$ & $105.38$ & $92$ \\ 
59183.48 & $27.89\pm0.20$ & $-10.360\substack{+0.004\\ -0.004}$ & $2.09\substack{+0.01\\ -0.01}$ & $-11.489\substack{+0.008\\ -0.008}$ & $78.44$ & $92$ \\ 
59185.35 & $29.33\pm0.19$ & $-10.338\substack{+0.004\\ -0.004}$ & $2.10\substack{+0.01\\ -0.01}$ & $-11.492\substack{+0.008\\ -0.008}$ & $90.85$ & $94$ \\ 
59187.36 & $29.89\pm0.29$ & $-10.331\substack{+0.006\\ -0.006}$ & $2.12\substack{+0.02\\ -0.02}$ & $-11.495\substack{+0.008\\ -0.008}$ & $120.79$ & $86$ \\ 
59189.60 & $26.50\pm0.26$ & $-10.391\substack{+0.005\\ -0.005}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.479\substack{+0.008\\ -0.008}$ & $98.52$ & $85$ \\ 
59191.30 & $27.42\pm0.23$ & $-10.372\substack{+0.005\\ -0.005}$ & $2.19\substack{+0.02\\ -0.02}$ & $-11.472\substack{+0.008\\ -0.008}$ & $115.97$ & $97$ \\ 
59192.98 & $34.23\pm0.28$ & $-10.268\substack{+0.005\\ -0.005}$ & $2.15\substack{+0.02\\ -0.02}$ & $-11.465\substack{+0.008\\ -0.008}$ & $90.06$ & $97$ \\ 
59193.11 & $34.69\pm0.29$ & $-10.251\substack{+0.005\\ -0.005}$ & $2.16\substack{+0.02\\ -0.02}$ & $-11.465\substack{+0.008\\ -0.008}$ & $114.88$ & $98$ \\ 
59195.20 & $37.17\pm0.39$ & $-10.225\substack{+0.006\\ -0.006}$ & $2.24\substack{+0.02\\ -0.02}$ & $-11.483\substack{+0.008\\ -0.008}$ & $75.11$ & $91$ \\ 
59213.22 & $29.82\pm0.19$ & $-10.266\substack{+0.004\\ -0.004}$ & $2.03\substack{+0.01\\ -0.01}$ & $-11.507\substack{+0.008\\ -0.008}$ & $95.92$ & $93$ \\ 
59215.07 & $38.84\pm0.19$ & $-10.191\substack{+0.002\\ -0.002}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.499\substack{+0.008\\ -0.008}$ & $75.58$ & $96$ \\ 
59217.36 & $40.38\pm0.22$ & $-10.170\substack{+0.003\\ -0.003}$ & $2.17\substack{+0.01\\ -0.01}$ & $-11.483\substack{+0.008\\ -0.008}$ & $92.84$ & $96$ \\ 
59219.49 & $29.67\pm0.17$ & $-10.310\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.484\substack{+0.008\\ -0.008}$ & $86.25$ & $97$ \\ 
59223.62 & $25.88\pm0.29$ & $-10.352\substack{+0.007\\ -0.007}$ & $2.09\substack{+0.02\\ -0.02}$ & $-11.525\substack{+0.008\\ -0.008}$ & $115.27$ & $84$ \\ 
59225.17 & $21.84\pm0.18$ & $-10.411\substack{+0.005\\ -0.005}$ & $2.03\substack{+0.01\\ -0.01}$ & $-11.539\substack{+0.008\\ -0.008}$ & $81.20$ & $86$ \\ 
59226.98 & $19.78\pm0.18$ & $-10.459\substack{+0.006\\ -0.006}$ & $2.02\substack{+0.02\\ -0.02}$ & $-11.527\substack{+0.008\\ -0.008}$ & $87.29$ & $84$ \\ 
59227.05 & $20.78\pm0.25$ & $-10.425\substack{+0.007\\ -0.007}$ & $1.98\substack{+0.02\\ -0.02}$ & $-11.525\substack{+0.008\\ -0.008}$ & $59.60$ & $79$ \\ 
59228.97 & $24.57\pm0.16$ & $-10.386\substack{+0.004\\ -0.004}$ & $2.12\substack{+0.01\\ -0.01}$ & $-11.483\substack{+0.008\\ -0.008}$ & $114.07$ & $91$ \\ 
59230.99 & $24.93\pm0.18$ & $-10.393\substack{+0.004\\ -0.004}$ & $2.19\substack{+0.01\\ -0.01}$ & $-11.471\substack{+0.008\\ -0.008}$ & $55.26$ & $86$ \\ 
59231.63 & $24.92\pm0.20$ & $-10.404\substack{+0.004\\ -0.005}$ & $2.25\substack{+0.01\\ -0.01}$ & $-11.474\substack{+0.008\\ -0.008}$ & $70.91$ & $82$ \\ 
59232.50 & $20.26\pm0.13$ & $-10.409\substack{+0.003\\ -0.003}$ & $2.15\substack{+0.01\\ -0.01}$ & $-11.478\substack{+0.008\\ -0.008}$ & $76.48$ & $88$ \\ 
59233.39 & $20.39\pm0.15$ & $-10.423\substack{+0.004\\ -0.004}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.482\substack{+0.008\\ -0.008}$ & $68.72$ & $86$ \\ 
59234.98 & $14.55\pm0.11$ & $-10.567\substack{+0.005\\ -0.005}$ & $2.07\substack{+0.01\\ -0.01}$ & $-11.481\substack{+0.008\\ -0.008}$ & $89.53$ & $85$ \\ 
59236.98 & $19.60\pm0.12$ & $-10.501\substack{+0.003\\ -0.003}$ & $2.14\substack{+0.01\\ -0.01}$ & $-11.450\substack{+0.008\\ -0.008}$ & $79.97$ & $89$ \\ 
59239.46 & $19.46\pm0.11$ & $-10.450\substack{+0.003\\ -0.003}$ & $2.28\substack{+0.01\\ -0.01}$ & $-11.407\substack{+0.008\\ -0.008}$ & $110.41$ & $102$ \\ 
59240.26 & $24.67\pm0.23$ & $-10.416\substack{+0.005\\ -0.006}$ & $2.27\substack{+0.02\\ -0.02}$ & $-11.391\substack{+0.008\\ -0.008}$ & $73.55$ & $92$ \\ 
59241.17 & $22.12\pm0.18$ & $-10.463\substack{+0.005\\ -0.005}$ & $2.17\substack{+0.02\\ -0.02}$ & $-11.374\substack{+0.008\\ -0.008}$ & $79.13$ & $97$ \\ 
59243.24 & $20.27\pm0.18$ & $-10.517\substack{+0.005\\ -0.005}$ & $2.24\substack{+0.02\\ -0.02}$ & $-11.350\substack{+0.008\\ -0.008}$ & $72.64$ & $83$ \\ 
59245.18 & $25.44\pm0.27$ & $-10.408\substack{+0.006\\ -0.006}$ & $2.31\substack{+0.02\\ -0.02}$ & $-11.340\substack{+0.008\\ -0.008}$ & $61.55$ & $78$ \\ 
59248.93 & $36.20\pm0.23$ & $-10.284\substack{+0.003\\ -0.004}$ & $2.20\substack{+0.01\\ -0.01}$ & $-11.332\substack{+0.008\\ -0.008}$ & $118.43$ & $98$ \\ 
59253.49 & $33.96\pm0.22$ & $-10.282\substack{+0.003\\ -0.003}$ & $2.33\substack{+0.01\\ -0.01}$ & $-11.304\substack{+0.008\\ -0.008}$ & $90.10$ & $96$ \\ 
59255.41 & $34.95\pm0.25$ & $-10.278\substack{+0.004\\ -0.004}$ & $2.34\substack{+0.01\\ -0.01}$ & $-11.308\substack{+0.008\\ -0.008}$ & $75.80$ & $87$ \\ 
59257.23 & $40.96\pm0.28$ & $-10.220\substack{+0.004\\ -0.004}$ & $2.34\substack{+0.01\\ -0.01}$ & $-11.321\substack{+0.008\\ -0.008}$ & $96.40$ & $98$ \\ 
59258.56 & $38.32\pm0.29$ & $-10.268\substack{+0.004\\ -0.004}$ & $2.26\substack{+0.02\\ -0.01}$ & $-11.326\substack{+0.008\\ -0.008}$ & $96.16$ & $100$ \\ 


==> Table9.tex <==
58256.95 & $0.55\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.739\substack{+0.008\\ -0.008}$ & $31.66$ & $37$ \\ 
58257.00 & $0.53\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.739\substack{+0.008\\ -0.008}$ & $22.60$ & $150$ \\ 
58272.38 & $0.59\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.619\substack{+0.008\\ -0.008}$ & $30.23$ & $210$ \\ 
58293.62 & $0.50\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.738\substack{+0.008\\ -0.008}$ & $29.98$ & $94$ \\ 
58294.65 & $0.52\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.760\substack{+0.008\\ -0.008}$ & $42.25$ & $242$ \\ 
58302.65 & $0.55\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.798\substack{+0.008\\ -0.008}$ & $38.96$ & $32$ \\ 
58304.43 & $0.66\pm0.04$ & $-10.18\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.781\substack{+0.008\\ -0.008}$ & $41.35$ & $105$ \\ 
58310.32 & $0.34\pm0.03$ & $-10.45\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.999\substack{+0.008\\ -0.008}$ & $22.70$ & $126$ \\ 
58311.22 & $0.36\pm0.03$ & $-10.42\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.049\substack{+0.008\\ -0.008}$ & $39.44$ & $246$ \\ 
58312.21 & $0.37\pm0.03$ & $-10.42\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.095\substack{+0.008\\ -0.008}$ & $25.29$ & $35$ \\ 
58313.57 & $0.48\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.052\substack{+0.008\\ -0.008}$ & $30.41$ & $32$ \\ 
58314.52 & $0.52\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.082\substack{+0.008\\ -0.008}$ & $21.50$ & $69$ \\ 
58315.30 & $0.43\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.098\substack{+0.008\\ -0.008}$ & $37.11$ & $111$ \\ 
58317.30 & $0.47\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.096\substack{+0.008\\ -0.008}$ & $38.75$ & $36$ \\ 
58318.58 & $0.50\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.114\substack{+0.008\\ -0.008}$ & $26.06$ & $245$ \\ 
58325.65 & $0.48\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.281\substack{+0.008\\ -0.008}$ & $60.47$ & $112$ \\ 
58327.16 & $0.57\pm0.03$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.213\substack{+0.008\\ -0.008}$ & $41.71$ & $68$ \\ 
58329.19 & $0.46\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.166\substack{+0.008\\ -0.008}$ & $33.51$ & $89$ \\ 
58331.12 & $0.42\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.128\substack{+0.008\\ -0.008}$ & $30.33$ & $35$ \\ 
58333.50 & $0.52\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.076\substack{+0.008\\ -0.008}$ & $21.69$ & $204$ \\ 
58336.46 & $0.60\pm0.03$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.048\substack{+0.008\\ -0.008}$ & $31.43$ & $142$ \\ 
58338.59 & $0.52\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.027\substack{+0.008\\ -0.008}$ & $48.07$ & $227$ \\ 
58340.52 & $0.62\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.083\substack{+0.008\\ -0.008}$ & $35.17$ & $35$ \\ 
58342.64 & $0.62\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.109\substack{+0.008\\ -0.008}$ & $50.67$ & $271$ \\ 
58343.60 & $0.50\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.122\substack{+0.008\\ -0.008}$ & $49.19$ & $86$ \\ 
58345.21 & $0.49\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.130\substack{+0.008\\ -0.008}$ & $30.06$ & $131$ \\ 
58348.86 & $0.55\pm0.03$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.168\substack{+0.008\\ -0.008}$ & $28.88$ & $152$ \\ 
58350.96 & $0.50\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.220\substack{+0.008\\ -0.008}$ & $29.39$ & $36$ \\ 
58352.82 & $0.49\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.257\substack{+0.008\\ -0.008}$ & $23.83$ & $34$ \\ 
58354.82 & $0.52\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.230\substack{+0.008\\ -0.008}$ & $33.43$ & $77$ \\ 
58358.86 & $0.36\pm0.03$ & $-10.45\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.399\substack{+0.008\\ -0.008}$ & $29.08$ & $88$ \\ 
58360.85 & $0.39\pm0.03$ & $-10.40\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.495\substack{+0.008\\ -0.008}$ & $37.20$ & $92$ \\ 
58362.85 & $0.35\pm0.03$ & $-10.44\substack{+0.03\\ -0.04}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.449\substack{+0.008\\ -0.008}$ & $15.45$ & $135$ \\ 
58364.71 & $0.49\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.365\substack{+0.008\\ -0.008}$ & $47.58$ & $335$ \\ 
58367.94 & $0.53\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.337\substack{+0.008\\ -0.008}$ & $45.10$ & $94$ \\ 
58369.77 & $0.43\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.212\substack{+0.008\\ -0.008}$ & $36.70$ & $64$ \\ 
58375.54 & $0.42\pm0.03$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.586\substack{+0.008\\ -0.008}$ & $29.94$ & $162$ \\ 
58377.89 & $0.36\pm0.03$ & $-10.45\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.632\substack{+0.008\\ -0.008}$ & $25.00$ & $144$ \\ 
58379.95 & $0.34\pm0.03$ & $-10.45\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.689\substack{+0.008\\ -0.008}$ & $21.90$ & $105$ \\ 
58382.85 & $0.39\pm0.03$ & $-10.42\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-13.385\substack{+0.008\\ -0.008}$ & $44.49$ & $65$ \\ 
58388.42 & $0.37\pm0.03$ & $-10.43\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.812\substack{+0.008\\ -0.008}$ & $26.20$ & $65$ \\ 
58390.48 & $0.47\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-14.106\substack{+0.008\\ -0.008}$ & $42.58$ & $93$ \\ 
58392.70 & $0.44\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.801\substack{+0.008\\ -0.008}$ & $33.12$ & $220$ \\ 
58394.92 & $0.35\pm0.03$ & $-10.45\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.860\substack{+0.008\\ -0.008}$ & $27.16$ & $32$ \\ 
58396.59 & $0.36\pm0.03$ & $-10.45\substack{+0.03\\ -0.04}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.651\substack{+0.008\\ -0.008}$ & $17.23$ & $106$ \\ 
58398.59 & $0.45\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.573\substack{+0.008\\ -0.008}$ & $34.28$ & $33$ \\ 
58400.69 & $0.45\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.364\substack{+0.008\\ -0.008}$ & $25.19$ & $53$ \\ 
58402.59 & $0.42\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.485\substack{+0.008\\ -0.008}$ & $42.97$ & $36$ \\ 
58403.93 & $0.40\pm0.03$ & $-10.40\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.546\substack{+0.008\\ -0.008}$ & $38.71$ & $103$ \\ 
58405.89 & $0.43\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.565\substack{+0.008\\ -0.008}$ & $33.18$ & $31$ \\ 
58407.31 & $0.51\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-12.406\substack{+0.008\\ -0.008}$ & $35.29$ & $66$ \\ 
58409.69 & $0.47\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.360\substack{+0.008\\ -0.008}$ & $16.84$ & $32$ \\ 
58412.07 & $0.38\pm0.03$ & $-10.42\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.256\substack{+0.008\\ -0.008}$ & $26.37$ & $33$ \\ 
58414.51 & $0.47\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.174\substack{+0.008\\ -0.008}$ & $36.14$ & $165$ \\ 
58416.70 & $0.46\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-12.138\substack{+0.008\\ -0.008}$ & $21.85$ & $75$ \\ 
58418.70 & $0.42\pm0.03$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-12.174\substack{+0.008\\ -0.008}$ & $30.09$ & $202$ \\ 
58420.63 & $0.47\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.209\substack{+0.008\\ -0.008}$ & $29.44$ & $204$ \\ 
58421.24 & $0.51\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.209\substack{+0.008\\ -0.008}$ & $33.61$ & $38$ \\ 
58422.67 & $0.48\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.258\substack{+0.008\\ -0.008}$ & $32.15$ & $36$ \\ 
58423.96 & $0.47\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.252\substack{+0.008\\ -0.008}$ & $22.53$ & $33$ \\ 
58426.46 & $0.54\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.187\substack{+0.008\\ -0.008}$ & $61.37$ & $103$ \\ 
58428.20 & $0.58\pm0.03$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.128\substack{+0.008\\ -0.008}$ & $38.40$ & $39$ \\ 
58429.17 & $0.62\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.080\substack{+0.008\\ -0.008}$ & $27.20$ & $36$ \\ 
58430.07 & $0.63\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-12.020\substack{+0.008\\ -0.008}$ & $31.97$ & $33$ \\ 
58431.16 & $0.61\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.994\substack{+0.008\\ -0.008}$ & $24.26$ & $36$ \\ 
58432.97 & $0.67\pm0.04$ & $-10.17\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.969\substack{+0.008\\ -0.008}$ & $35.56$ & $102$ \\ 
58433.06 & $0.70\pm0.04$ & $-10.16\substack{+0.02\\ -0.02}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.966\substack{+0.008\\ -0.008}$ & $40.51$ & $333$ \\ 
58437.51 & $0.62\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.902\substack{+0.008\\ -0.008}$ & $40.67$ & $229$ \\ 
58438.42 & $0.58\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.880\substack{+0.008\\ -0.008}$ & $33.84$ & $50$ \\ 
58439.64 & $0.51\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.907\substack{+0.008\\ -0.008}$ & $44.18$ & $224$ \\ 
58449.22 & $0.55\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.911\substack{+0.008\\ -0.008}$ & $35.30$ & $98$ \\ 
58453.60 & $0.49\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.956\substack{+0.008\\ -0.008}$ & $40.73$ & $181$ \\ 
58455.11 & $0.37\pm0.03$ & $-10.43\substack{+0.03\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.083\substack{+0.008\\ -0.008}$ & $26.73$ & $110$ \\ 
58456.98 & $0.34\pm0.03$ & $-10.48\substack{+0.03\\ -0.04}$ & $2.4\substack{+0.1\\ -0.1}$ & $-12.075\substack{+0.008\\ -0.008}$ & $21.91$ & $27$ \\ 
58458.91 & $0.35\pm0.03$ & $-10.44\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.140\substack{+0.008\\ -0.008}$ & $21.06$ & $31$ \\ 
58460.91 & $0.41\pm0.03$ & $-10.38\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-12.074\substack{+0.008\\ -0.008}$ & $20.52$ & $33$ \\ 
58462.90 & $0.44\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-12.106\substack{+0.008\\ -0.008}$ & $34.52$ & $37$ \\ 
58464.58 & $0.39\pm0.03$ & $-10.40\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.115\substack{+0.008\\ -0.008}$ & $24.86$ & $176$ \\ 
58466.18 & $0.39\pm0.03$ & $-10.42\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.147\substack{+0.008\\ -0.008}$ & $35.17$ & $34$ \\ 
58469.02 & $0.34\pm0.03$ & $-10.45\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-12.130\substack{+0.008\\ -0.008}$ & $33.15$ & $116$ \\ 
58470.68 & $0.42\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.067\substack{+0.008\\ -0.008}$ & $15.67$ & $156$ \\ 
58471.77 & $0.47\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-12.032\substack{+0.008\\ -0.008}$ & $47.41$ & $34$ \\ 
58473.91 & $0.56\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-12.015\substack{+0.008\\ -0.008}$ & $40.11$ & $32$ \\ 
58476.07 & $0.54\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.900\substack{+0.008\\ -0.008}$ & $36.70$ & $61$ \\ 
58479.11 & $0.56\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.847\substack{+0.008\\ -0.008}$ & $46.43$ & $111$ \\ 
58481.24 & $0.41\pm0.03$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.859\substack{+0.008\\ -0.008}$ & $26.22$ & $31$ \\ 
58487.79 & $0.61\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.771\substack{+0.008\\ -0.008}$ & $43.88$ & $157$ \\ 
58489.79 & $0.40\pm0.03$ & $-10.43\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.747\substack{+0.008\\ -0.008}$ & $33.71$ & $33$ \\ 
58491.53 & $0.40\pm0.03$ & $-10.40\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.755\substack{+0.008\\ -0.008}$ & $24.79$ & $227$ \\ 
58493.71 & $0.40\pm0.03$ & $-10.41\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.758\substack{+0.008\\ -0.008}$ & $31.08$ & $333$ \\ 
58497.64 & $0.44\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.692\substack{+0.008\\ -0.008}$ & $40.69$ & $98$ \\ 
58499.38 & $0.40\pm0.03$ & $-10.42\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.638\substack{+0.008\\ -0.008}$ & $25.84$ & $52$ \\ 
58500.48 & $0.51\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.610\substack{+0.008\\ -0.008}$ & $19.80$ & $300$ \\ 
58501.89 & $0.48\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.592\substack{+0.008\\ -0.008}$ & $32.33$ & $107$ \\ 
58503.24 & $0.43\pm0.03$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.588\substack{+0.008\\ -0.008}$ & $18.74$ & $31$ \\ 
58504.98 & $0.60\pm0.04$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.561\substack{+0.008\\ -0.008}$ & $16.96$ & $34$ \\ 
58505.95 & $0.60\pm0.04$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.560\substack{+0.008\\ -0.008}$ & $22.54$ & $33$ \\ 
58506.33 & $0.57\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.570\substack{+0.008\\ -0.008}$ & $28.73$ & $157$ \\ 
58507.62 & $0.50\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.565\substack{+0.008\\ -0.008}$ & $23.15$ & $142$ \\ 
58511.87 & $0.43\pm0.03$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.534\substack{+0.008\\ -0.008}$ & $33.85$ & $32$ \\ 
58513.28 & $0.47\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.509\substack{+0.008\\ -0.008}$ & $32.09$ & $27$ \\ 
58514.73 & $0.46\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.5\substack{+0.1\\ -0.1}$ & $-11.520\substack{+0.008\\ -0.008}$ & $27.83$ & $199$ \\ 
58515.86 & $0.52\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.479\substack{+0.008\\ -0.008}$ & $25.32$ & $128$ \\ 
58517.18 & $0.54\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.456\substack{+0.008\\ -0.008}$ & $27.41$ & $248$ \\ 
58521.53 & $0.58\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.400\substack{+0.008\\ -0.008}$ & $19.20$ & $35$ \\ 
58523.50 & $0.55\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.349\substack{+0.008\\ -0.008}$ & $29.69$ & $35$ \\ 
58527.09 & $0.63\pm0.04$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.5\substack{+0.1\\ -0.1}$ & $-11.340\substack{+0.008\\ -0.008}$ & $25.17$ & $228$ \\ 
58528.06 & $0.57\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.357\substack{+0.008\\ -0.008}$ & $41.84$ & $94$ \\ 
58529.87 & $0.53\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.327\substack{+0.008\\ -0.008}$ & $17.96$ & $154$ \\ 
58541.28 & $0.62\pm0.04$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.378\substack{+0.008\\ -0.008}$ & $27.84$ & $186$ \\ 
58544.08 & $0.70\pm0.04$ & $-10.16\substack{+0.02\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.375\substack{+0.008\\ -0.008}$ & $52.34$ & $56$ \\ 
58545.93 & $0.68\pm0.04$ & $-10.17\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.373\substack{+0.008\\ -0.008}$ & $32.01$ & $39$ \\ 
58548.20 & $0.71\pm0.04$ & $-10.17\substack{+0.02\\ -0.02}$ & $2.6\substack{+0.1\\ -0.1}$ & $-11.362\substack{+0.008\\ -0.008}$ & $33.71$ & $65$ \\ 
58550.32 & $0.77\pm0.04$ & $-10.13\substack{+0.02\\ -0.02}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.361\substack{+0.008\\ -0.008}$ & $27.66$ & $37$ \\ 
58553.35 & $0.67\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.390\substack{+0.008\\ -0.008}$ & $33.50$ & $47$ \\ 
58556.06 & $0.71\pm0.04$ & $-10.16\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.393\substack{+0.008\\ -0.008}$ & $27.19$ & $85$ \\ 
58559.95 & $0.53\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.387\substack{+0.008\\ -0.008}$ & $38.13$ & $193$ \\ 
58561.50 & $0.46\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.386\substack{+0.008\\ -0.008}$ & $36.89$ & $123$ \\ 
58562.94 & $0.50\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.368\substack{+0.008\\ -0.008}$ & $23.19$ & $34$ \\ 
58564.04 & $0.73\pm0.04$ & $-10.15\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.359\substack{+0.008\\ -0.008}$ & $28.16$ & $37$ \\ 
58565.78 & $0.62\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.345\substack{+0.008\\ -0.008}$ & $38.31$ & $35$ \\ 
58567.20 & $0.55\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.334\substack{+0.008\\ -0.008}$ & $22.67$ & $96$ \\ 
58568.80 & $0.56\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.322\substack{+0.008\\ -0.008}$ & $36.41$ & $188$ \\ 
58570.87 & $0.73\pm0.04$ & $-10.16\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.306\substack{+0.008\\ -0.008}$ & $37.00$ & $68$ \\ 
58573.06 & $0.66\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.300\substack{+0.008\\ -0.008}$ & $34.84$ & $35$ \\ 
58575.51 & $0.68\pm0.04$ & $-10.18\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.290\substack{+0.008\\ -0.008}$ & $31.31$ & $34$ \\ 
58577.45 & $0.78\pm0.04$ & $-10.14\substack{+0.02\\ -0.02}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.269\substack{+0.008\\ -0.008}$ & $42.99$ & $243$ \\ 
58579.38 & $0.80\pm0.04$ & $-10.12\substack{+0.02\\ -0.02}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.259\substack{+0.008\\ -0.008}$ & $35.97$ & $35$ \\ 
58581.35 & $0.68\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.275\substack{+0.008\\ -0.008}$ & $44.67$ & $110$ \\ 
58586.70 & $0.65\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.277\substack{+0.008\\ -0.008}$ & $28.61$ & $109$ \\ 
58588.63 & $0.77\pm0.04$ & $-10.13\substack{+0.02\\ -0.02}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.289\substack{+0.008\\ -0.008}$ & $46.41$ & $155$ \\ 
58591.05 & $0.64\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.294\substack{+0.008\\ -0.008}$ & $45.41$ & $105$ \\ 
58592.65 & $0.72\pm0.04$ & $-10.14\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.297\substack{+0.008\\ -0.008}$ & $47.86$ & $36$ \\ 
58594.91 & $0.74\pm0.04$ & $-10.16\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.323\substack{+0.008\\ -0.008}$ & $35.56$ & $113$ \\ 
58596.84 & $0.72\pm0.04$ & $-10.15\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.311\substack{+0.008\\ -0.008}$ & $30.36$ & $55$ \\ 
58603.42 & $0.62\pm0.04$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.294\substack{+0.008\\ -0.008}$ & $31.05$ & $163$ \\ 
58605.35 & $0.77\pm0.04$ & $-10.13\substack{+0.02\\ -0.02}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.311\substack{+0.008\\ -0.008}$ & $34.46$ & $37$ \\ 
58607.22 & $0.56\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.334\substack{+0.008\\ -0.008}$ & $25.80$ & $33$ \\ 
58609.28 & $0.64\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.357\substack{+0.008\\ -0.008}$ & $25.43$ & $130$ \\ 
58611.34 & $0.70\pm0.04$ & $-10.16\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.384\substack{+0.008\\ -0.008}$ & $26.55$ & $39$ \\ 
58612.95 & $0.61\pm0.04$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.407\substack{+0.008\\ -0.008}$ & $37.25$ & $221$ \\ 
58614.95 & $0.61\pm0.04$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.419\substack{+0.008\\ -0.008}$ & $34.48$ & $129$ \\ 
58617.01 & $0.60\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.415\substack{+0.008\\ -0.008}$ & $413.93$ & $767$ \\ 
58619.00 & $0.56\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.419\substack{+0.008\\ -0.008}$ & $35.03$ & $53$ \\ 
58621.13 & $0.67\pm0.04$ & $-10.18\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.423\substack{+0.008\\ -0.008}$ & $34.68$ & $43$ \\ 
58623.22 & $0.56\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.431\substack{+0.008\\ -0.008}$ & $31.13$ & $84$ \\ 
58626.73 & $0.58\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.456\substack{+0.008\\ -0.008}$ & $30.69$ & $35$ \\ 
58632.66 & $0.48\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.476\substack{+0.008\\ -0.008}$ & $33.49$ & $31$ \\ 
58635.56 & $0.62\pm0.04$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.452\substack{+0.008\\ -0.008}$ & $32.61$ & $44$ \\ 
58637.62 & $0.62\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.469\substack{+0.008\\ -0.008}$ & $38.27$ & $52$ \\ 
58643.87 & $0.79\pm0.04$ & $-10.12\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.376\substack{+0.008\\ -0.008}$ & $43.07$ & $66$ \\ 
58646.07 & $0.64\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.376\substack{+0.008\\ -0.008}$ & $30.37$ & $32$ \\ 
58651.93 & $0.57\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.370\substack{+0.008\\ -0.008}$ & $27.05$ & $34$ \\ 
58653.93 & $0.47\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.332\substack{+0.008\\ -0.008}$ & $26.36$ & $122$ \\ 
58655.93 & $0.48\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.320\substack{+0.008\\ -0.008}$ & $30.07$ & $33$ \\ 
58657.96 & $0.62\pm0.04$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.317\substack{+0.008\\ -0.008}$ & $35.02$ & $86$ \\ 
58660.24 & $0.60\pm0.04$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.329\substack{+0.008\\ -0.008}$ & $33.52$ & $188$ \\ 
58662.04 & $0.55\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.310\substack{+0.008\\ -0.008}$ & $43.59$ & $84$ \\ 
58664.24 & $0.55\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.296\substack{+0.008\\ -0.008}$ & $22.76$ & $85$ \\ 
58665.88 & $0.56\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.316\substack{+0.008\\ -0.008}$ & $35.74$ & $194$ \\ 
58673.24 & $0.55\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.368\substack{+0.008\\ -0.008}$ & $368.55$ & $767$ \\ 
58675.30 & $0.57\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.375\substack{+0.008\\ -0.008}$ & $32.51$ & $179$ \\ 
58677.17 & $0.50\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.391\substack{+0.008\\ -0.008}$ & $30.04$ & $35$ \\ 
58679.04 & $0.66\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.403\substack{+0.008\\ -0.008}$ & $27.45$ & $34$ \\ 
58680.40 & $0.54\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.440\substack{+0.008\\ -0.008}$ & $31.00$ & $35$ \\ 
58683.23 & $0.50\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.462\substack{+0.008\\ -0.008}$ & $23.34$ & $190$ \\ 
58685.11 & $0.57\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.482\substack{+0.008\\ -0.008}$ & $32.21$ & $38$ \\ 
58687.54 & $0.53\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.507\substack{+0.008\\ -0.008}$ & $31.07$ & $82$ \\ 
58690.12 & $0.31\pm0.03$ & $-10.51\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.566\substack{+0.008\\ -0.008}$ & $42.55$ & $31$ \\ 
58691.79 & $0.52\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.522\substack{+0.008\\ -0.008}$ & $28.47$ & $117$ \\ 
58694.70 & $0.54\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.501\substack{+0.008\\ -0.008}$ & $24.74$ & $38$ \\ 
58699.98 & $0.59\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.502\substack{+0.008\\ -0.008}$ & $34.19$ & $58$ \\ 
58702.27 & $0.56\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.521\substack{+0.008\\ -0.008}$ & $34.61$ & $78$ \\ 
58704.59 & $0.47\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.528\substack{+0.008\\ -0.008}$ & $31.63$ & $107$ \\ 
58706.46 & $0.56\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.564\substack{+0.008\\ -0.008}$ & $36.26$ & $38$ \\ 
58711.99 & $0.41\pm0.03$ & $-10.40\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.678\substack{+0.008\\ -0.008}$ & $44.71$ & $353$ \\ 
58712.05 & $0.47\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.678\substack{+0.008\\ -0.008}$ & $27.51$ & $136$ \\ 
58713.92 & $0.46\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.671\substack{+0.008\\ -0.008}$ & $38.18$ & $116$ \\ 
58715.57 & $0.50\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.669\substack{+0.008\\ -0.008}$ & $33.22$ & $235$ \\ 
58717.44 & $0.50\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.665\substack{+0.008\\ -0.008}$ & $27.89$ & $50$ \\ 
58719.05 & $0.51\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.659\substack{+0.008\\ -0.008}$ & $15.61$ & $51$ \\ 
58721.15 & $0.32\pm0.03$ & $-10.49\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.635\substack{+0.008\\ -0.008}$ & $31.96$ & $192$ \\ 
58723.06 & $0.49\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.5\substack{+0.1\\ -0.1}$ & $-11.613\substack{+0.008\\ -0.008}$ & $28.78$ & $83$ \\ 
58729.84 & $0.63\pm0.04$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.518\substack{+0.008\\ -0.008}$ & $39.56$ & $208$ \\ 
58737.40 & $0.61\pm0.04$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.525\substack{+0.008\\ -0.008}$ & $17.86$ & $34$ \\ 
58739.36 & $0.62\pm0.04$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.508\substack{+0.008\\ -0.008}$ & $32.64$ & $36$ \\ 
58740.65 & $0.58\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.479\substack{+0.008\\ -0.008}$ & $26.04$ & $201$ \\ 
58742.97 & $0.66\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.456\substack{+0.008\\ -0.008}$ & $36.13$ & $35$ \\ 
58743.04 & $0.62\pm0.04$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.456\substack{+0.008\\ -0.008}$ & $40.46$ & $161$ \\ 
58744.91 & $0.62\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.456\substack{+0.008\\ -0.008}$ & $35.80$ & $203$ \\ 
58751.71 & $0.48\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.472\substack{+0.008\\ -0.008}$ & $27.07$ & $34$ \\ 
58753.15 & $0.47\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.460\substack{+0.008\\ -0.008}$ & $26.63$ & $34$ \\ 
58755.02 & $0.44\pm0.03$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.425\substack{+0.008\\ -0.008}$ & $23.88$ & $133$ \\ 
58756.57 & $0.45\pm0.03$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.435\substack{+0.008\\ -0.008}$ & $32.13$ & $146$ \\ 
58758.38 & $0.42\pm0.03$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.444\substack{+0.008\\ -0.008}$ & $36.47$ & $275$ \\ 
58761.66 & $0.56\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.423\substack{+0.008\\ -0.008}$ & $35.14$ & $34$ \\ 
58765.31 & $0.67\pm0.04$ & $-10.18\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.443\substack{+0.008\\ -0.008}$ & $38.42$ & $37$ \\ 
58767.60 & $0.66\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.488\substack{+0.008\\ -0.008}$ & $35.21$ & $133$ \\ 
58777.69 & $0.52\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.510\substack{+0.008\\ -0.008}$ & $31.78$ & $251$ \\ 
58779.17 & $0.52\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.493\substack{+0.008\\ -0.008}$ & $28.66$ & $152$ \\ 
58781.20 & $0.55\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.481\substack{+0.008\\ -0.008}$ & $31.85$ & $84$ \\ 
58783.30 & $0.50\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.499\substack{+0.008\\ -0.008}$ & $23.56$ & $62$ \\ 
58785.09 & $0.51\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.506\substack{+0.008\\ -0.008}$ & $27.11$ & $107$ \\ 
58786.96 & $0.61\pm0.04$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.552\substack{+0.008\\ -0.008}$ & $39.61$ & $145$ \\ 
58789.28 & $0.45\pm0.03$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.564\substack{+0.008\\ -0.008}$ & $28.61$ & $173$ \\ 
58791.61 & $0.50\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.570\substack{+0.008\\ -0.008}$ & $37.10$ & $34$ \\ 
58793.60 & $0.47\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.566\substack{+0.008\\ -0.008}$ & $27.07$ & $33$ \\ 
58794.80 & $0.53\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.582\substack{+0.008\\ -0.008}$ & $28.99$ & $148$ \\ 
58800.52 & $0.64\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.573\substack{+0.008\\ -0.008}$ & $32.16$ & $196$ \\ 
58801.97 & $0.65\pm0.04$ & $-10.17\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.565\substack{+0.008\\ -0.008}$ & $25.18$ & $38$ \\ 
58805.13 & $0.62\pm0.04$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.561\substack{+0.008\\ -0.008}$ & $30.44$ & $92$ \\ 
58807.45 & $0.70\pm0.04$ & $-10.17\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.524\substack{+0.008\\ -0.008}$ & $35.59$ & $174$ \\ 
58808.87 & $0.52\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.535\substack{+0.008\\ -0.008}$ & $37.12$ & $125$ \\ 
58810.94 & $0.50\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.548\substack{+0.008\\ -0.008}$ & $34.74$ & $167$ \\ 
58811.00 & $0.48\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.548\substack{+0.008\\ -0.008}$ & $14.48$ & $35$ \\ 
58812.59 & $0.50\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.555\substack{+0.008\\ -0.008}$ & $29.39$ & $167$ \\ 
58815.65 & $0.42\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $1.8\substack{+0.1\\ -0.1}$ & $-11.556\substack{+0.008\\ -0.008}$ & $28.92$ & $177$ \\ 
58817.45 & $0.53\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.531\substack{+0.008\\ -0.008}$ & $33.73$ & $190$ \\ 
58819.36 & $0.60\pm0.03$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.535\substack{+0.008\\ -0.008}$ & $29.25$ & $32$ \\ 
58821.49 & $0.50\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.537\substack{+0.008\\ -0.008}$ & $43.59$ & $155$ \\ 
58823.49 & $0.57\pm0.03$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.561\substack{+0.008\\ -0.008}$ & $37.12$ & $192$ \\ 
58825.62 & $0.50\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.567\substack{+0.008\\ -0.008}$ & $28.53$ & $221$ \\ 
58827.62 & $0.50\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.582\substack{+0.008\\ -0.008}$ & $35.29$ & $42$ \\ 
58829.88 & $0.44\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.526\substack{+0.008\\ -0.008}$ & $34.76$ & $157$ \\ 
58832.01 & $0.55\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.521\substack{+0.008\\ -0.008}$ & $40.98$ & $208$ \\ 
58833.86 & $0.58\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.525\substack{+0.008\\ -0.008}$ & $35.15$ & $131$ \\ 
58835.88 & $0.66\pm0.04$ & $-10.18\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.499\substack{+0.008\\ -0.008}$ & $32.44$ & $35$ \\ 
58836.01 & $0.60\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.496\substack{+0.008\\ -0.008}$ & $36.73$ & $37$ \\ 
58844.21 & $0.63\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.439\substack{+0.008\\ -0.008}$ & $21.17$ & $252$ \\ 
58847.69 & $0.67\pm0.04$ & $-10.17\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.479\substack{+0.008\\ -0.008}$ & $49.44$ & $36$ \\ 
58849.83 & $0.62\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.493\substack{+0.008\\ -0.008}$ & $30.89$ & $169$ \\ 
58851.80 & $0.55\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.513\substack{+0.008\\ -0.008}$ & $33.42$ & $92$ \\ 
58853.64 & $0.52\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.510\substack{+0.008\\ -0.008}$ & $33.97$ & $166$ \\ 
58855.80 & $0.64\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.521\substack{+0.008\\ -0.008}$ & $40.77$ & $119$ \\ 
58857.80 & $0.65\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.540\substack{+0.008\\ -0.008}$ & $33.91$ & $114$ \\ 
58859.80 & $0.60\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.547\substack{+0.008\\ -0.008}$ & $33.34$ & $92$ \\ 
58861.80 & $0.59\pm0.03$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.530\substack{+0.008\\ -0.008}$ & $37.51$ & $46$ \\ 
58863.61 & $0.47\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.514\substack{+0.008\\ -0.008}$ & $48.64$ & $137$ \\ 
58865.22 & $0.50\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.501\substack{+0.008\\ -0.008}$ & $47.71$ & $113$ \\ 
58866.71 & $0.62\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.489\substack{+0.008\\ -0.008}$ & $24.63$ & $175$ \\ 
58868.85 & $0.49\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.475\substack{+0.008\\ -0.008}$ & $46.77$ & $95$ \\ 
58870.84 & $0.66\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.478\substack{+0.008\\ -0.008}$ & $29.16$ & $176$ \\ 
58871.67 & $0.53\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.484\substack{+0.008\\ -0.008}$ & $41.49$ & $36$ \\ 
58873.22 & $0.62\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.495\substack{+0.008\\ -0.008}$ & $39.56$ & $35$ \\ 
58875.16 & $0.50\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.509\substack{+0.008\\ -0.008}$ & $40.87$ & $84$ \\ 
58876.97 & $0.45\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.522\substack{+0.008\\ -0.008}$ & $31.86$ & $98$ \\ 
58877.68 & $0.52\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.527\substack{+0.008\\ -0.008}$ & $33.41$ & $37$ \\ 
58879.49 & $0.45\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.527\substack{+0.008\\ -0.008}$ & $36.11$ & $98$ \\ 
58884.72 & $0.52\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.554\substack{+0.008\\ -0.008}$ & $34.22$ & $36$ \\ 
58887.53 & $0.56\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.510\substack{+0.008\\ -0.008}$ & $34.81$ & $60$ \\ 
58889.57 & $0.60\pm0.04$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.505\substack{+0.008\\ -0.008}$ & $13.02$ & $34$ \\ 
58891.63 & $0.66\pm0.04$ & $-10.18\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.461\substack{+0.008\\ -0.008}$ & $37.67$ & $54$ \\ 
58893.40 & $0.58\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.442\substack{+0.008\\ -0.008}$ & $32.58$ & $107$ \\ 
58902.65 & $0.47\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.430\substack{+0.008\\ -0.008}$ & $23.46$ & $72$ \\ 
58903.97 & $0.55\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.432\substack{+0.008\\ -0.008}$ & $15.72$ & $32$ \\ 
58905.59 & $0.73\pm0.04$ & $-10.15\substack{+0.02\\ -0.02}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.435\substack{+0.008\\ -0.008}$ & $44.71$ & $113$ \\ 
58909.60 & $0.59\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.510\substack{+0.008\\ -0.008}$ & $25.85$ & $169$ \\ 
58910.86 & $0.50\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.531\substack{+0.008\\ -0.008}$ & $26.49$ & $152$ \\ 
58911.31 & $0.60\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.531\substack{+0.008\\ -0.008}$ & $42.75$ & $133$ \\ 
58915.75 & $0.41\pm0.03$ & $-10.38\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.552\substack{+0.008\\ -0.008}$ & $28.59$ & $157$ \\ 
58917.39 & $0.43\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.568\substack{+0.008\\ -0.008}$ & $25.93$ & $34$ \\ 
58919.20 & $0.58\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.586\substack{+0.008\\ -0.008}$ & $32.29$ & $39$ \\ 
58921.27 & $0.64\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.594\substack{+0.008\\ -0.008}$ & $24.48$ & $139$ \\ 
58923.07 & $0.58\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.601\substack{+0.008\\ -0.008}$ & $40.36$ & $143$ \\ 
58929.79 & $0.60\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.629\substack{+0.008\\ -0.008}$ & $32.12$ & $218$ \\ 
58931.55 & $0.61\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.637\substack{+0.008\\ -0.008}$ & $43.67$ & $113$ \\ 
58933.41 & $0.61\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.646\substack{+0.008\\ -0.008}$ & $30.12$ & $120$ \\ 
58935.42 & $0.63\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.657\substack{+0.008\\ -0.008}$ & $38.42$ & $172$ \\ 
58937.60 & $0.55\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.670\substack{+0.008\\ -0.008}$ & $32.36$ & $114$ \\ 
58939.87 & $0.60\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.674\substack{+0.008\\ -0.008}$ & $33.62$ & $41$ \\ 
58941.71 & $0.70\pm0.04$ & $-10.17\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.671\substack{+0.008\\ -0.008}$ & $27.74$ & $37$ \\ 
58943.49 & $0.61\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.655\substack{+0.008\\ -0.008}$ & $29.19$ & $35$ \\ 
58945.04 & $0.73\pm0.04$ & $-10.13\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.639\substack{+0.008\\ -0.008}$ & $39.91$ & $37$ \\ 
58953.41 & $0.69\pm0.04$ & $-10.16\substack{+0.02\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.511\substack{+0.008\\ -0.008}$ & $46.61$ & $160$ \\ 
58955.66 & $0.81\pm0.04$ & $-10.10\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.490\substack{+0.008\\ -0.008}$ & $44.89$ & $36$ \\ 
58957.37 & $0.79\pm0.04$ & $-10.14\substack{+0.02\\ -0.02}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.477\substack{+0.008\\ -0.008}$ & $47.23$ & $135$ \\ 
58963.86 & $0.77\pm0.04$ & $-10.14\substack{+0.02\\ -0.02}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.460\substack{+0.008\\ -0.008}$ & $30.08$ & $193$ \\ 
58969.26 & $0.81\pm0.04$ & $-10.10\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.407\substack{+0.008\\ -0.008}$ & $49.80$ & $268$ \\ 
58971.20 & $0.78\pm0.04$ & $-10.12\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.392\substack{+0.008\\ -0.008}$ & $30.87$ & $94$ \\ 
58973.33 & $0.70\pm0.04$ & $-10.19\substack{+0.02\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.376\substack{+0.008\\ -0.008}$ & $25.14$ & $37$ \\ 
58975.26 & $0.65\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.359\substack{+0.008\\ -0.008}$ & $26.36$ & $199$ \\ 
58977.26 & $0.69\pm0.04$ & $-10.18\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.341\substack{+0.008\\ -0.008}$ & $40.18$ & $65$ \\ 
58979.50 & $0.82\pm0.04$ & $-10.10\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.321\substack{+0.008\\ -0.008}$ & $30.18$ & $134$ \\ 
58981.42 & $0.60\pm0.04$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.305\substack{+0.008\\ -0.008}$ & $43.01$ & $100$ \\ 
58983.35 & $0.63\pm0.04$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.290\substack{+0.008\\ -0.008}$ & $25.55$ & $144$ \\ 
58985.26 & $0.73\pm0.04$ & $-10.16\substack{+0.02\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.276\substack{+0.008\\ -0.008}$ & $33.01$ & $81$ \\ 
58987.26 & $0.67\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.275\substack{+0.008\\ -0.008}$ & $38.02$ & $37$ \\ 
58994.55 & $0.68\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.276\substack{+0.008\\ -0.008}$ & $36.95$ & $88$ \\ 
59008.58 & $0.56\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.264\substack{+0.008\\ -0.008}$ & $36.19$ & $204$ \\ 
59014.56 & $0.60\pm0.04$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.262\substack{+0.008\\ -0.008}$ & $35.86$ & $68$ \\ 
59022.87 & $0.47\pm0.03$ & $-10.38\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.234\substack{+0.008\\ -0.008}$ & $22.69$ & $249$ \\ 
59025.00 & $0.61\pm0.04$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.252\substack{+0.008\\ -0.008}$ & $21.07$ & $207$ \\ 
59027.00 & $0.71\pm0.04$ & $-10.17\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.269\substack{+0.008\\ -0.008}$ & $45.63$ & $144$ \\ 
59028.72 & $0.75\pm0.04$ & $-10.13\substack{+0.02\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.276\substack{+0.008\\ -0.008}$ & $35.12$ & $36$ \\ 
59029.88 & $0.68\pm0.04$ & $-10.16\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.280\substack{+0.008\\ -0.008}$ & $28.40$ & $158$ \\ 
59034.31 & $0.65\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.298\substack{+0.008\\ -0.008}$ & $25.81$ & $36$ \\ 
59036.63 & $0.60\pm0.03$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.295\substack{+0.008\\ -0.008}$ & $33.75$ & $185$ \\ 
59038.89 & $0.70\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.290\substack{+0.008\\ -0.008}$ & $41.72$ & $42$ \\ 
59042.55 & $0.64\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.282\substack{+0.008\\ -0.008}$ & $30.27$ & $61$ \\ 
59043.95 & $0.53\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.281\substack{+0.008\\ -0.008}$ & $25.56$ & $226$ \\ 
59044.01 & $0.49\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.280\substack{+0.008\\ -0.008}$ & $22.94$ & $34$ \\ 
59053.90 & $0.70\pm0.04$ & $-10.18\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.254\substack{+0.008\\ -0.008}$ & $44.29$ & $82$ \\ 
59056.47 & $0.52\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.246\substack{+0.008\\ -0.008}$ & $26.51$ & $35$ \\ 
59060.66 & $0.61\pm0.04$ & $-10.25\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.260\substack{+0.008\\ -0.008}$ & $34.42$ & $195$ \\ 
59062.59 & $0.79\pm0.04$ & $-10.11\substack{+0.02\\ -0.02}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.278\substack{+0.008\\ -0.008}$ & $19.34$ & $39$ \\ 
59064.59 & $0.72\pm0.04$ & $-10.17\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.285\substack{+0.008\\ -0.008}$ & $28.83$ & $41$ \\ 
59066.56 & $0.65\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.292\substack{+0.008\\ -0.008}$ & $29.48$ & $34$ \\ 
59070.92 & $0.76\pm0.04$ & $-10.13\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.334\substack{+0.008\\ -0.008}$ & $43.98$ & $35$ \\ 
59072.73 & $0.74\pm0.04$ & $-10.12\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.343\substack{+0.008\\ -0.008}$ & $22.51$ & $41$ \\ 
59074.96 & $0.63\pm0.04$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.356\substack{+0.008\\ -0.008}$ & $34.44$ & $182$ \\ 
59076.91 & $0.65\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.366\substack{+0.008\\ -0.008}$ & $25.76$ & $80$ \\ 
59077.97 & $0.60\pm0.04$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.373\substack{+0.008\\ -0.008}$ & $38.22$ & $160$ \\ 
59080.91 & $0.64\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.390\substack{+0.008\\ -0.008}$ & $32.53$ & $37$ \\ 
59082.88 & $0.69\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.402\substack{+0.008\\ -0.008}$ & $38.36$ & $114$ \\ 
59083.01 & $0.65\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.402\substack{+0.008\\ -0.008}$ & $48.76$ & $142$ \\ 
59084.93 & $0.50\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.413\substack{+0.008\\ -0.008}$ & $46.43$ & $219$ \\ 
59088.99 & $0.56\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.438\substack{+0.008\\ -0.008}$ & $28.14$ & $193$ \\ 
59093.97 & $0.39\pm0.03$ & $-10.43\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.451\substack{+0.008\\ -0.008}$ & $41.12$ & $83$ \\ 
59095.94 & $0.65\pm0.04$ & $-10.21\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.439\substack{+0.008\\ -0.008}$ & $30.62$ & $176$ \\ 
59101.27 & $0.74\pm0.04$ & $-10.16\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.449\substack{+0.008\\ -0.008}$ & $29.80$ & $123$ \\ 
59103.86 & $0.86\pm0.04$ & $-10.09\substack{+0.02\\ -0.02}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.468\substack{+0.008\\ -0.008}$ & $34.87$ & $209$ \\ 
59105.31 & $0.80\pm0.04$ & $-10.11\substack{+0.02\\ -0.02}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.479\substack{+0.008\\ -0.008}$ & $50.13$ & $49$ \\ 
59107.95 & $0.70\pm0.04$ & $-10.16\substack{+0.02\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.506\substack{+0.008\\ -0.008}$ & $24.28$ & $106$ \\ 
59109.31 & $0.59\pm0.03$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.539\substack{+0.008\\ -0.008}$ & $41.87$ & $30$ \\ 
59116.29 & $0.42\pm0.03$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.608\substack{+0.008\\ -0.008}$ & $25.21$ & $90$ \\ 
59118.43 & $0.42\pm0.03$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.628\substack{+0.008\\ -0.008}$ & $31.47$ & $34$ \\ 
59120.59 & $0.49\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.623\substack{+0.008\\ -0.008}$ & $37.27$ & $35$ \\ 
59122.53 & $0.59\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.618\substack{+0.008\\ -0.008}$ & $39.67$ & $35$ \\ 
59124.47 & $0.48\pm0.03$ & $-10.33\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.614\substack{+0.008\\ -0.008}$ & $23.00$ & $105$ \\ 
59126.20 & $0.55\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.610\substack{+0.008\\ -0.008}$ & $37.05$ & $73$ \\ 
59128.12 & $0.50\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.605\substack{+0.008\\ -0.008}$ & $35.57$ & $158$ \\ 
59129.56 & $0.54\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.602\substack{+0.008\\ -0.008}$ & $31.00$ & $36$ \\ 
59130.75 & $0.57\pm0.03$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.599\substack{+0.008\\ -0.008}$ & $43.13$ & $155$ \\ 
59136.81 & $0.60\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.586\substack{+0.008\\ -0.008}$ & $31.92$ & $121$ \\ 
59138.33 & $0.54\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.583\substack{+0.008\\ -0.008}$ & $41.75$ & $31$ \\ 
59141.04 & $0.60\pm0.04$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.553\substack{+0.008\\ -0.008}$ & $33.15$ & $133$ \\ 
59142.79 & $0.49\pm0.03$ & $-10.32\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.534\substack{+0.008\\ -0.008}$ & $45.55$ & $201$ \\ 
59144.40 & $0.49\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.518\substack{+0.008\\ -0.008}$ & $32.67$ & $159$ \\ 
59148.93 & $0.54\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.493\substack{+0.008\\ -0.008}$ & $21.95$ & $86$ \\ 
59150.52 & $0.48\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.487\substack{+0.008\\ -0.008}$ & $35.96$ & $139$ \\ 
59151.84 & $0.51\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.480\substack{+0.008\\ -0.008}$ & $26.35$ & $31$ \\ 
59153.87 & $0.41\pm0.03$ & $-10.41\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.461\substack{+0.008\\ -0.008}$ & $24.13$ & $207$ \\ 
59155.71 & $0.42\pm0.03$ & $-10.41\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.443\substack{+0.008\\ -0.008}$ & $36.91$ & $169$ \\ 
59157.68 & $0.50\pm0.03$ & $-10.34\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.426\substack{+0.008\\ -0.008}$ & $36.85$ & $308$ \\ 
59165.69 & $0.61\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.429\substack{+0.008\\ -0.008}$ & $26.99$ & $34$ \\ 
59166.40 & $0.53\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.427\substack{+0.008\\ -0.008}$ & $36.91$ & $64$ \\ 
59170.40 & $0.53\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.424\substack{+0.008\\ -0.008}$ & $34.04$ & $86$ \\ 
59172.72 & $0.70\pm0.04$ & $-10.16\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.430\substack{+0.008\\ -0.008}$ & $33.58$ & $128$ \\ 
59179.54 & $0.69\pm0.04$ & $-10.17\substack{+0.02\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.454\substack{+0.008\\ -0.008}$ & $41.26$ & $87$ \\ 
59181.25 & $0.60\pm0.03$ & $-10.23\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.475\substack{+0.008\\ -0.008}$ & $23.01$ & $38$ \\ 
59183.48 & $0.49\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.489\substack{+0.008\\ -0.008}$ & $37.10$ & $33$ \\ 
59185.35 & $0.52\pm0.03$ & $-10.30\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.492\substack{+0.008\\ -0.008}$ & $48.49$ & $85$ \\ 
59187.36 & $0.47\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.495\substack{+0.008\\ -0.008}$ & $23.50$ & $62$ \\ 
59189.60 & $0.45\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.479\substack{+0.008\\ -0.008}$ & $50.39$ & $183$ \\ 
59191.30 & $0.44\pm0.03$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.472\substack{+0.008\\ -0.008}$ & $31.76$ & $100$ \\ 
59192.98 & $0.54\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.465\substack{+0.008\\ -0.008}$ & $44.87$ & $258$ \\ 
59193.11 & $0.55\pm0.03$ & $-10.29\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.465\substack{+0.008\\ -0.008}$ & $31.57$ & $94$ \\ 
59195.20 & $0.59\pm0.03$ & $-10.24\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.483\substack{+0.008\\ -0.008}$ & $21.47$ & $36$ \\ 
59213.22 & $0.54\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.507\substack{+0.008\\ -0.008}$ & $36.94$ & $115$ \\ 
59215.07 & $0.66\pm0.04$ & $-10.19\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.499\substack{+0.008\\ -0.008}$ & $39.85$ & $55$ \\ 
59217.36 & $0.63\pm0.04$ & $-10.22\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.483\substack{+0.008\\ -0.008}$ & $35.45$ & $221$ \\ 
59219.49 & $0.50\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.484\substack{+0.008\\ -0.008}$ & $32.73$ & $107$ \\ 
59223.62 & $0.43\pm0.03$ & $-10.37\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.525\substack{+0.008\\ -0.008}$ & $24.75$ & $100$ \\ 
59225.17 & $0.38\pm0.03$ & $-10.44\substack{+0.04\\ -0.04}$ & $1.9\substack{+0.1\\ -0.1}$ & $-11.539\substack{+0.008\\ -0.008}$ & $25.16$ & $130$ \\ 
59226.98 & $0.41\pm0.03$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.527\substack{+0.008\\ -0.008}$ & $37.63$ & $31$ \\ 
59227.05 & $0.39\pm0.03$ & $-10.42\substack{+0.03\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.525\substack{+0.008\\ -0.008}$ & $33.73$ & $93$ \\ 
59228.97 & $0.48\pm0.03$ & $-10.35\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.483\substack{+0.008\\ -0.008}$ & $24.55$ & $135$ \\ 
59230.99 & $0.43\pm0.03$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.471\substack{+0.008\\ -0.008}$ & $43.97$ & $158$ \\ 
59231.63 & $0.43\pm0.03$ & $-10.39\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.474\substack{+0.008\\ -0.008}$ & $30.09$ & $196$ \\ 
59232.50 & $0.41\pm0.03$ & $-10.42\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.478\substack{+0.008\\ -0.008}$ & $49.58$ & $29$ \\ 
59233.39 & $0.41\pm0.03$ & $-10.40\substack{+0.03\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.482\substack{+0.008\\ -0.008}$ & $29.49$ & $53$ \\ 
59234.98 & $0.28\pm0.02$ & $-10.54\substack{+0.04\\ -0.04}$ & $1.7\substack{+0.1\\ -1.7}$ & $-11.481\substack{+0.008\\ -0.008}$ & $30.00$ & $32$ \\ 
59236.98 & $0.37\pm0.03$ & $-10.45\substack{+0.04\\ -0.04}$ & $2.0\substack{+0.1\\ -0.1}$ & $-11.450\substack{+0.008\\ -0.008}$ & $45.38$ & $46$ \\ 
59239.46 & $0.44\pm0.03$ & $-10.41\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.407\substack{+0.008\\ -0.008}$ & $43.80$ & $283$ \\ 
59240.26 & $0.48\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.391\substack{+0.008\\ -0.008}$ & $23.31$ & $34$ \\ 
59241.17 & $0.40\pm0.03$ & $-10.44\substack{+0.04\\ -0.04}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.374\substack{+0.008\\ -0.008}$ & $36.53$ & $32$ \\ 
59243.24 & $0.34\pm0.03$ & $-10.51\substack{+0.04\\ -0.04}$ & $2.3\substack{+0.1\\ -0.1}$ & $-11.350\substack{+0.008\\ -0.008}$ & $25.86$ & $27$ \\ 
59245.18 & $0.46\pm0.03$ & $-10.36\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.340\substack{+0.008\\ -0.008}$ & $23.56$ & $72$ \\ 
59248.93 & $0.51\pm0.03$ & $-10.31\substack{+0.03\\ -0.03}$ & $2.1\substack{+0.1\\ -0.1}$ & $-11.332\substack{+0.008\\ -0.008}$ & $41.20$ & $103$ \\ 
59253.49 & $0.61\pm0.04$ & $-10.26\substack{+0.03\\ -0.03}$ & $2.4\substack{+0.1\\ -0.1}$ & $-11.304\substack{+0.008\\ -0.008}$ & $40.34$ & $253$ \\ 
59255.41 & $0.58\pm0.03$ & $-10.27\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.308\substack{+0.008\\ -0.008}$ & $29.64$ & $189$ \\ 
59257.23 & $0.66\pm0.04$ & $-10.20\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.321\substack{+0.008\\ -0.008}$ & $27.71$ & $32$ \\ 
59258.56 & $0.57\pm0.03$ & $-10.28\substack{+0.03\\ -0.03}$ & $2.2\substack{+0.1\\ -0.1}$ & $-11.326\substack{+0.008\\ -0.008}$ & $354.02$ & $767$ \\ 

